Look-Ahead and Look-Back Flows: Training-Free Image Generation with Trajectory Smoothing

Recent advances have reformulated diffusion models as deterministic ordinary differential equations (ODEs) through the framework of flow matching, providing a unified formulation for the noise-to-data generative process. Various training-free flow matching approaches have been developed to improve image generation through flow velocity field adjustment, eliminating the need for costly retraining. However, Modifying the velocity field $v$ introduces errors that propagate through the full generation path, whereas adjustments to the latent trajectory $z$ are naturally corrected by the pretrained velocity network, reducing error accumulation. In this paper, we propose two complementary training-free latent-trajectory adjustment approaches based on future and past velocity $v$ and latent trajectory $z$ information that refine the generative path directly in latent space. We propose two training-free trajectory smoothing schemes: \emph{Look-Ahead}, which averages the current and next-step latents using a curvature-gated weight, and \emph{Look-Back}, which smoothes latents using an exponential moving average with decay. We demonstrate through extensive experiments and comprehensive evaluation metrics that the proposed training-free trajectory smoothing models substantially outperform various state-of-the-art models across multiple datasets including COCO17, CUB-200, and Flickr30K.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

\usepackage{bm}
%\usepackage{subfig}
\usepackage{capt-of}
\usepackage{mathtools}
\usepackage{siunitx}
% \usepackage[figurename=Figure]{caption}
%\usepackage{stfloats}
\usepackage{amsfonts}
\usepackage{scrextend}
\usepackage{xspace}
\usepackage{xcolor}
\usepackage{multirow}
% \usepackage{floatrow}
% \usepackage{wrapfig}
\usepackage{amsthm}
\usepackage{thmtools}
\usepackage{algorithm,algpseudocode}
% \usepackage{mathbbol}
%\floatsetup[table]{capposition=top}
%\usepackage{algorithm}      % algorithm
%\usepackage[noend]{algpseudocode} % algorithm
%\usepackage[title]{appendix}
\usepackage[export]{adjustbox}
\usepackage{url}
%\usepackage{subfig}
%\usepackage{natbib}
%\usepackage[sort&compress]{natbib}
\usepackage{lineno}
% \usepackage{xr}
\usepackage{pifont}
\usepackage{booktabs}
% \usepackage{subfig}
% \usepackage{subcaption}
\usepackage{soul}
\usepackage{tikz}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{decorations.pathmorphing}
% \usepackage{subfig}
\usepackage{subcaption}
\usepackage{algorithm}
\usepackage{algpseudocode}
% \usepackage{amsmath}
% \usepackage[ruled,vlined]{algorithm2e}
\usepackage{adjustbox}
\usepackage{graphicx}
\usepackage{array}
% \usepackage{xr}

\usepackage{pgfplots}
\usepackage{tikz-3dplot}
\pgfplotsset{compat=1.18}
\usepgfplotslibrary{colormaps, external}
\usetikzlibrary{arrows.meta, 3d, decorations.pathmorphing, calc, backgrounds, positioning}

\colorlet{manifoldcolor}{gray!20}
\colorlet{p0color}{blue!80}
\colorlet{p1color}{red!80}
\colorlet{geodesiccolor}{black}
\colorlet{targetvectorcolor}{green!60!black}
\colorlet{predictedvectorcolor}{orange!90!black}
\colorlet{tangentplanecolor}{gray}


\newcounter{algsubstate}
\renewcommand{\thealgsubstate}{\alph{algsubstate}}
\newenvironment{algsubstates}
{\setcounter{algsubstate}{0}%
	\renewcommand{\State}{%
		\stepcounter{algsubstate}%
		\Statex {\footnotesize\thealgsubstate:}\space}}
{}

\DeclareMathOperator{\vectolower}{vec\_to\_lower}

\newcommand{\imgpath}{fig/generated_images}
\newcommand{\imgw}{0.13\textwidth} % tweak if needed

%\makeatletter
%\let\OldStatex\Statex
%\renewcommand{\Statex}[1][3]{%
%	\setlength\@tempdima{\algorithmicindent}%
%	\OldStatex\hskip\dimexpr#1\@tempdima\relax}
%\makeatother

% \newfloatcommand{capbtabbox}{table}[][\FBwidth]
% \floatsetup{heightadjust=object}

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\minimize}{minimize}

% Include other packages here, before hyperref.

% If you comment hyperref and then uncomment it, you should delete
% egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% run, let it finish, and you should be clear).

\def\TODO#1{\textcolor{red}{{\bf [TODO:}~#1{\bf ]}}}
\def\NOTE#1{\textcolor{blue}{{\bf [NOTE:}~#1{\bf ]}}}
\def\POINT#1{\textcolor[RGB]{146,38,143}{{\bf [POINT:}~#1{\bf ]}}}
% \def\REVISION#1{\textcolor[RGB]{0,0,0}{#1}}
\def\REVISION#1{\textcolor[RGB]{0,0,255}{#1}}
\def\WCOLOR#1{\textcolor[RGB]{0,0,255}{#1}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{theorem*}{Theorem}
\newtheorem{problem}{Problem}

\newenvironment{proofof}[1]{\begin{proof}[of {#1}]}{\end{proof}}

% \newcommand{\secref}[1]{\mbox{Section~\ref{#1}}}
\newcommand{\appref}[1]{\mbox{Appendix~\ref{#1}}}
\newcommand{\thref}[1]{\mbox{Theorem~\ref{#1}}}
\newcommand{\defref}[1]{\mbox{Definition~\ref{#1}}}
\newcommand{\corref}[1]{\mbox{Corollary~\ref{#1}}}
\newcommand{\lemref}[1]{\mbox{Lemma~\ref{#1}}}
\newcommand{\clref}[1]{\mbox{Claim~\ref{#1}}}
\newcommand{\propref}[1]{\mbox{Proposition~\ref{#1}}}
\newcommand{\factref}[1]{\mbox{Fact~\ref{#1}}}
\newcommand{\remref}[1]{\mbox{Remark~\ref{#1}}}
% \newcommand{\figref}[1]{\mbox{Fig.~\ref{#1}}}
% \renewcommand{\algref}[1]{\mbox{Algorithm~\ref{#1}}}
% \newcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
% Have to use \renewcommand because exists already in amsmath
\renewcommand{\eqref}[1]{\mbox{Eq.~(\ref{#1})}}
\newcommand{\consref}[1]{\mbox{Construction~\ref{#1}}}
\newcommand{\tabref}[1]{\mbox{Table~\ref{#1}}}


\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot}
\def\ie{\emph{i.e}\onedot}
\def\cf{\emph{c.f}\onedot}
\def\etc{\emph{etc}\onedot}
\def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}

\newcommand{\mengyu}[1]{{\color{blue}[Mengyu]: #1}}
\newcommand{\yu}[1]{{\color{cyan}[Yu]: #1}}
\newcommand{\yan}[1]{{\color{Red}[Yan]: #1}}
\newcommand{\shi}[1]{{\color{purple}[Min]: #1}}
\newcommand{\Osama}[1]{{\color{Red}[Osama]: #1}}

\newcommand{\Hao}[1]{{\color{orange}[Hao]: #1}}


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand{\M}{\mathcal{M}}
\newcommand{\T}{\mathrm{T}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\inner}[1]{\langle#1\rangle}
\DeclareMathOperator{\Log}{Log}   % <---  \Log
\DeclareMathOperator{\Exp}{Exp}   %        \Exp
\DeclareMathOperator{\Id}{Id}     %        \Id
\DeclareMathOperator{\dist}{dist} %        \dist
\newcommand{\I}{\mathbb{I}}

\newcommand{\expmap}{\exp}
\newcommand{\logmap}{\log}
\newcommand{\proj}{\text{proj}}

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

==> sec/data_bk.tex <==
\begin{table*}[t]
\centering
% \captionsetup{width=.8\linewidth}
\scriptsize
\caption{Performance of generated images produced by various loss reweighting methods on the test set (5K samples) of MS COCO-17. The first captions are used for training, while the captions with the highest CLIPScores are used for testing.
}
% \vspace{-2ex}
\label{tab:perf_caption_coco17}
\adjustbox{width=1\textwidth}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Method} & \textbf{FID} {$\downarrow$} & \textbf{IS} {$\uparrow$} & \textbf{CLIPScore} {$\uparrow$} & \textbf{BLEU-4} {$\uparrow$}  & \textbf{METEOR} {$\uparrow$} & \textbf{ROUGE-L} {$\uparrow$} & \textbf{CLAIR} {$\uparrow$}   \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} 
% Rectified Diffusion & 28.36  & 18.73 & 12.18 & 7.80 & 28.97 & 37.59 & 13.89 & 33.75 & 56.79 \\
% Rectified Diffusion & 20.17 & 33.80 & 31.91 & 7.44 & 28.41 & 33.16 \\
% SDv3.5 (pretrained, CFG=1, Steps=30) &   \\
% SDv3.5 (pretrained, CFG=2, Steps=30) &   \\
% SDv3.5 (pretrained, CFG=3, Steps=30) &   \\
% SDv3.5 (pretrained, CFG=4, Steps=25) &  \\
% SDv3.5 (pretrained, CFG=4, Steps=30) &  \\
% SDv3.5 (pretrained, CFG=4, Steps=35) &   \\
% SDv3.5 (pretrained, CFG=4, Steps=15) &   \\
SDv3.5 (pretrained, CFG=7, Steps=25) & 28.46 & 33.64 & 32.84 & 7.99 & 29.17 & 35.11 & 71.45 \\
SDv3.5 w/ A-Euler & 27.64 & 34.63 & 32.84 & 7.96 & 29.09 & 35.17 & 71.23 \\
SDv3.5 w/ Self-Guidance &  40.98 & 28.54 & 31.21 & 6.52 & 26.18 & 31.59 & 62.26 \\
SDv3.5 w/ Momentum & 29.36 & 33.27 & 33.29 & 8.26 & 29.43 & 35.27 &  71.41 \\
% SDv3.5 (pretrained) w/ FAO &  \\
% SDv3.5 w/ FAO Moment ($\beta$=0.001) &  \\
% SDv3.5 w/ FAO Moment ($\beta$=0.01) &  \\
% SDv3.5 w/ FAO Moment ($\beta$=0.1) &  \\
% SDv3.5 w/ FAO Moment ($\beta$=0.2) &  \\
% SDv3.5 w/ FAO Moment ($\beta$=0.4) &  \\
% SDv3.5 w/ FAO Moment ($\beta$=0.6) &  \\
% SDv3.5 w/ FAO Moment ($\beta$=0.8) &  \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.8) & 27.95 & 34.10 & 32.86 & 8.12 & 29.45 & 35.28 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.9, $\tau_{curv}$=1) & 26.46 & 35.32 & 32.89 & 8.48 & 30.12 & 35.63 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.9, $\tau_{curv}$=10, Yan) & 26.34 & 35.49 & 32.94 & 8.55 & 30.29 & 35.68 \\
SDv3.5 w/ Look-Ahead ($\gamma$=0.9, $\tau_{curv}$=10, Henry) & 26.17 & 34.60 & 32.96 & 8.82 & 30.45 & 36.15 & 72.99 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.9, $\tau_{curv}$=20, Henry) & 26.45 & 33.82 & 32.92 & 8.46 & 29.65 & 35.60 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.95) & 26.30 & 35.40 & 32.93 & 8.52 & 30.20 & 35.85 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.99) & 27.60 & 34.80 & 32.88 & 8.20 & 29.85 & 35.40 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.1, mid=0, Yan) & 26.15 & 35.58 & 32.93 & 8.64 & 30.23 & 35.61 \\
SDv3.5 w/ Look-Back ($\lambda$=0.1, mid=0, Henry) & 26.27 & 34.81 & 32.94 & 8.76 & 30.53 & 36.17 & 72.77 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.2) & 26.90 & 34.95 & 32.89 & 8.35 & 29.95 & 35.60 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.4) & 28.10 & 34.10 & 32.82 & 8.05 & 29.40 & 35.05 \\
% FLUX.1 (pretrained, CFG=7, Steps=25) & 34.33 & 34.56 & 32.26 & 8.83 & 30.87 & 35.81  \\
% FLUX.1 w/ Look-Ahead &  \REVISION{Todd} \\
% FLUX.1 w/ Look-Back &  \REVISION{Todd} \\
\bottomrule
\end{tabular}}
\end{table*}

\begin{table*}[t]
\centering
% \captionsetup{width=.8\linewidth}
\scriptsize
\caption{Performance of generated images produced by various loss reweighting methods on the test set (9K samples) of LAION-Aesthetics. The first captions are used for training, while the captions with the highest CLIPScores are used for testing.
}
% \vspace{-2ex}
\label{tab:perf_caption_coco17}
\adjustbox{width=1\textwidth}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Method} & \textbf{FID} {$\downarrow$} & \textbf{IS} {$\uparrow$} & \textbf{CLIPScore} {$\uparrow$} & \textbf{BLEU-4} {$\uparrow$}  & \textbf{METEOR} {$\uparrow$} & \textbf{ROUGE-L} {$\uparrow$} & \textbf{CLAIR} {$\uparrow$}   \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} 
% Rectified Diffusion & 28.36  & 18.73 & 12.18 & 7.80 & 28.97 & 37.59 & 13.89 & 33.75 & 56.79 \\
% Rectified Diffusion & 15.43 & 17.08 & 31.96 & 0.44 & 7.39 & 5.86 \\
SDv3.5 (pretrained, CFG=7, Steps=25) & 24.83 & 18.89 & 31.32 & 0.32 & 5.92 & 4.95 & 49.72 \\
SDv3.5 w/ A-Euler & 23.59 & 19.17 & 31.35 & 0.34 & 6.00 & 5.07 & 49.98 \\
SDv3.5 w/ Self-Guidance & 50.32 & 14.90 & 27.24 & 0.29 & 4.67 & 4.44 & 40.42 \\
SDv3.5 w/ Momentum &  28.99 & 18.87 & 31.25 & 0.34 & 5.88 & 5.00 & 49.00 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.8) & \REVISION{Henry: inference\_sd35\_lookahead\_laion.sh} \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.9, $\tau_{curv}$=10) & 22.11 & 19.02 & 31.83 & 0.45 & 7.06 & 5.61  \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.9, $\tau_{curv}$=20) & 22.19 & 18.95 & 31.83 & 0.46 & 7.20 & 5.68  \\
SDv3.5 w/ Look-Ahead ($\gamma$=0.95, $\tau_{curv}$=20) & 21.48 & 19.53 & 31.67 & 0.37 & 6.46 & 5.25 & 51.55 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.05) & 21.65 & 19.55 & 31.61 & 0.39 & 6.47 & 5.30  \\
% SDv3.5 w/ Look-Back ($\lambda$=0.1) & 21.64 & 19.34 & 31.78 & 0.42 & 7.08 & 5.56  \\
SDv3.5 w/ Look-Back ($\lambda$=0.1, mid=0) & 21.64 & 19.33 & 31.78 & 0.42 & 7.08 & 5.56 & 52.89 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.2) &  \\
% SDv3.5 w/ Look-Back ($\lambda$=0.4) &  \\
% FLUX.1 (pretrained, CFG=7, Steps=25) & 30.99 & 18.87 & 29.73 & 0.50 & 7.63 & 5.77  \\
% FLUX.1 w/ Look-Ahead ($\gamma$ = 0.95) & 30.87 & 18.91 & 29.74 & 0.51 & 7.55 & 5.71  \\
% FLUX.1 w/ Look-Ahead ($\gamma$ = 0.9) & 30.87 & 18.96 & 29.74 & 0.51 & 7.55 & 5.71  \\
% FLUX.1 w/ Look-Back ($\lambda$ = 0.1) & 30.85 & 19.03 & 29.73 & 0.49 & 7.50 & 5.71  \\
% FLUX.1 w/ Look-Back ($\lambda$ = 0.05) & 30.87 & 18.95 & 29.74 & 0.51 & 7.55 & 5.71  \\
\bottomrule
\end{tabular}}
\end{table*}

\begin{table*}[t]
\centering
% \captionsetup{width=.8\linewidth}
\scriptsize
\caption{Performance of generated images produced by various loss reweighting methods on the test set (1K samples) of Flickr30K. The first captions are used for training, while the captions with the highest CLIPScores are used for testing.
}
% \vspace{-2ex}
\label{tab:perf_caption_coco17}
\adjustbox{width=1\textwidth}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Method} & \textbf{FID} {$\downarrow$} & \textbf{IS} {$\uparrow$} & \textbf{CLIPScore} {$\uparrow$} & \textbf{BLEU-4} {$\uparrow$}  & \textbf{METEOR} {$\uparrow$} & \textbf{ROUGE-L} {$\uparrow$} & \textbf{CLAIR} {$\uparrow$}   \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} 
% Rectified Diffusion & 28.36  & 18.73 & 12.18 & 7.80 & 28.97 & 37.59 & 13.89 & 33.75 & 56.79 \\
% Rectified Diffusion & 70.00 & 18.62 & 32.63 & 4.34 & 22.96 & 27.71 \\
% SDv3.5 (pretrained, CFG=1, Steps=30) & 132.54 & 7.67 & 27.96  \\
% SDv3.5 (pretrained, CFG=2, Steps=30) & 75.56 & 16.21 & 33.02  \\
% SDv3.5 (pretrained, CFG=3, Steps=30) & 75.10 & 17.89 & 33.37  \\
% SDv3.5 (pretrained, CFG=4, Steps=25) & 74.83 & 17.81 & 33.51  \\
% SDv3.5 (pretrained, CFG=4, Steps=30) & 74.83 & 17.81 & 33.51  \\
% SDv3.5 (pretrained, CFG=4, Steps=35) & 74.83 & 17.81 & 33.51  \\
% SDv3.5 (pretrained, CFG=4, Steps=15) & 77.93 & 18.18 & 33.81 & 4.40 & 24.76 & 29.88  \\
% SDv3.5 (pretrained, CFG=7, Steps=30) & 79.43 & 18.03 & 33.81 & 4.21 & 23.68 & 29.07  \\
% SDv3.5 (pretrained, CFG=3, Steps=25) & 76.07 & 18.72 & 33.72 & 4.70 & 24.33 & 29.72 \\ \midrule
SDv3.5 (pretrained, CFG=7, Steps=25) & 79.58 & 17.95 & 33.79 & 4.12 & 23.88 & 29.30 & 68.03 \\
SDv3.5 w/ A-Euler &  78.57 & 17.83 & 33.71 & 3.91 & 22.99 & 29.00 & 67.56 \\
SDv3.5 w/ Self-Guidance & 93.07 & 14.44 & 31.60 & 3.35 & 20.80 & 26.27 & 57.35 \\
SDv3.5 w/ Momentum &  79.05 & 17.56 & 34.20 & 4.18 & 24.27 & 29.32 & 67.20 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.95, $\tau_{curv}$=1) & 77.14 & 18.17 & 33.81 & 4.49 & 24.04 & 29.37 \\
SDv3.5 w/ Look-Ahead ($\gamma$=0.9, $\tau_{curv}$=1) & 75.88 & 18.12 & 33.88 & 4.97 & 25.32 & 30.58 & 70.16 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.9, $\tau_{curv}$=15) & 76.79 & 18.17 & 33.83 & 4.68 & 24.80 & 30.04 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.9, $\tau_{curv}$=20) & 77.55 & 18.41 & 33.85 & 4.44 & 24.44 & 29.81 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.9, $\tau_{curv}$=25) & 77.81 & 18.21 & 33.87 & 4.49 & 24.41 & 29.71 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.95, $\tau_{curv}$=15) & 78.15 & 17.97 & 33.84 & 4.47 & 24.06 & 29.31 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.95, $\tau_{curv}$=20) & 78.87 & 18.02 & 33.83 & 4.39 & 24.11 & 29.25 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.95, $\tau_{curv}$=25) & 79.13 & 17.89 & 33.84 & 4.34 & 24.15 & 29.32 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.2, mid=0) & 81.36 & 16.65 & 34.06 & 4.69 & 25.60 & 30.26 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.1, mid=0) & 75.23 & 18.02 & 33.78 & 4.82 & 25.39 & 30.29 \\
SDv3.5 w/ Look-Back ($\lambda$=0.1, mid=0.25) & 75.62 & 18.30 & 33.86 & 4.73 & 25.26 & 30.07 & 69.43 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.1, mid=0.5) & 75.62 & 18.50 & 33.86 & 4.73 & 25.26 & 30.07 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.05, mid=0) & 76.61 & 17.87 & 33.79 & 4.47 & 24.69 & 30.02 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.08, mid=0) & 75.08 & 17.99 & 33.84 & 4.62 & 25.04 & 30.01 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.01, mid=0.01) & 78.69 & 18.45 & 33.85 & 4.39 & 24.31 & 29.59 \\ 
% FLUX.1.Schnell (CFG=1, Steps=4) & 77.96 & 18.37 & 33.71 & 5.54 & 26.87 & 31.35 \\
% FLUX.1.Schnell w/ ($\gamma$=0.9) & 78.67 & 19.21 & 33.78 & 5.61 & 27.30 & 31.90 \\
% FLUX.1.Schnell w/ Look-Back ($\lambda$=0.1, mid=0) & 78.65 & 19.17 & 33.78 & 5.56 & 27.08 & 31.71 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.95, cfg=3) & 74.57 & 18.31 & 33.71 & 4.52 & 24.75 & 29.65 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.925, cfg=3) & 76.14 & 17.56 & 33.69 & 4.71 & 24.75 & 29.80 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.9, cfg=3) & 80.00 & 16.11 & 33.67 & 4.75 & 24.91 & 29.90 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.05, cfg=3) & 74.81 & 18.58 & 33.71 & 4.66 & 24.84 & 29.68 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.1, cfg=3) & 78.31 & 17.43 & 33.68 & 4.86 & 25.11 & 30.11 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.15, cfg=3) & 87.03 & 14.92 & 33.57 & 4.59 & 24.84 & 29.49 \\ \midrule
% SDv3.5 (pretrained, CFG=7, Steps=30) & 79.43 & 18.03 & 33.81 & 4.21 & 23.68 & 29.07  \\
% SDv3.5 (pretrained) w/ FAO & 80.12 & 17.24 & 33.83 & 4.02 & 23.54 & 28.85 \\
% SDv3.5 w/ FAO Moment ($\beta$=0.001) & 79.37 & 18.20 & 33.81 & 4.39 & 23.74 & 29.32 \\
% SDv3.5 w/ FAO Moment ($\beta$=0.01) & 79.51 & 17.63 & 33.78 & 4.25 & 23.75 & 29.41 \\
% SDv3.5 w/ FAO Moment ($\beta$=0.1) & 92.74 & 14.24 & 31.10 & 3.67 & 21.59 & 26.71 \\
% SDv3.5 w/ FAO Moment ($\beta$=0.2) & 80.31 & 18.35 & 33.77 & 4.35 & 23.92 & 29.71 \\
% SDv3.5 w/ FAO Moment ($\beta$=0.4) & 79.96 & 17.59 & 33.78 & 4.36 & 24.13 & 29.39 \\
% SDv3.5 w/ FAO Moment ($\beta$=0.6) & 79.85 & 17.80 & 33.94 & 4.29 & 23.95 & 29.47 \\
% SDv3.5 w/ FAO Moment ($\beta$=0.8) & 79.22 & 17.17 & 34.23 & 4.79 & 24.66 & 30.09 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.8) & 88.13 & 15.03 & 34.04 & 4.47 & 25.02 & 29.79 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.9) & 76.27 & 18.12 & 33.89 & 4.71 & 25.03 & 30.07 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.95) & 76.27 & 18.75 & 33.76 & 4.21 & 24.33 & 29.75 \\
% SDv3.5 w/ Look-Ahead ($\gamma$=0.99) & 78.88 & 18.47 & 33.83 & 4.51 & 24.33 & 29.95 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.1) & 76.35 & 18.07 & 33.86 & 4.80 & 25.40 & 30.22 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.2) & 82.46 & 17.02 & 34.04 & 4.65 & 25.69 & 30.18 \\
% SDv3.5 w/ Look-Back ($\lambda$=0.4) & 113.23 & 12.41 & 34.03 & 4.08 & 23.67 & 27.92 \\
% FLUX.1 (pretrained, CFG=7, Steps=25) & 84.70 & 17.39 & 32.93 & 5.03 & 25.66 & 30.22  \\
% FLUX.1 w/ Look-Ahead ($\gamma$=0.9, $\tau_{curv}$=1) &  84.62 & 19.00 & 32.90 & 4.78 & 25.65 & 29.77 \\
% FLUX.1 w/ Look-Ahead ($\gamma$=0.8) & 84.67 & 17.90 & 32.93 & 5.15 & 25.12 & 29.84  \\
% FLUX.1 w/ Look-Ahead ($\gamma$=0.7) &  85.38 & 17.16 & 32.76 & 5.17 & 25.58 & 30.50 \\
% FLUX.1 w/ Look-Ahead ($\gamma$=0.6) & 85.30 & 17.64 & 32.77 & 5.10 & 25.86 & 30.44  \\
% FLUX.1 w/ Look-Ahead ($\gamma$=0.8, $\tau_{curv}$=15) &   \\
% FLUX.1 w/ Look-Back ($\lambda$=0.1) & 84.82 & 18.93 & 32.89 & 4.83 & 25.98 & 29.98 \\
% FLUX.1 w/ Look-Back ($\lambda$=0.05) & 84.62 & 19.07 & 32.90 & 4.78 & 25.65 & 29.77 \\
% FLUX.1 w/ Look-Back ($\lambda$=0.01) & 84.62 & 18.76 & 32.90 & 4.78 & 25.65 & 29.77 \\
% FLUX.1.Dev (pretrained, CFG=3.5, Steps=50) & 83.04 & 18.13 & 32.87 & 4.97 & 25.53 & 30.16 \\
% FLUX.1 w/ Look-Ahead ($\gamma$=0.9, $\tau_{curv}$=1) &  82.78 & 18.67 & 32.91 & 5.25 & 25.95 & 30.23 \\
% FLUX.1.Schnell (pretrained, CFG=0, Steps=4) & 77.96 & 18.43 & 33.71 & 5.54 & 26.87 & 31.35 \\
\bottomrule
\end{tabular}}
\end{table*}

==> sec/method_bk.tex <==
\section{Problem Statement}
\label{sec:problem_statement}

% \section{Riemannian Rectified Flow}

% Let $(\M,g)$ be a complete, connected Riemannian manifold of dimension $d=\dim\M$ (finite, possibly large).  Denote the exponential map and logarithmic map by
% \[
% \Exp_{z}\colon\T_{z}\M\to\M,\qquad 
% \Log_{z}\colon\M\supset U_{z}\to\T_{z}\M,
% \]
% and parallel transport along the unique minimizing geodesic from $z$ to $w$ by $\Gamma_{z\to w}\colon\T_{z}\M\to\T_{w}\M$.

% \subsection{Forward interpolation}
% Given an initial distribution $p_{0}$ on $\M$ and a prior $p_{1}$ (e.g.\ the Riemannian Gaussian centered at $z_{0}$ with variance $\sigma^{2}$), draw $(x_{0},x_{1})\sim\pi$, where $\pi$ is any coupling with marginals $p_{0}$ and $p_{1}$.  Define the geodesic interpolation
% \[
% z_{t}:=\Exp_{x_{0}}\!\bigl(t\Log_{x_{0}}(x_{1})\bigr),\qquad t\in[0,1].
% \]
% The conditional velocity field along this curve is
% \[
% u_{t}(z\mid x_{0},x_{1}) := \frac{d}{dt}z_{t}\in\T_{z_{t}}\M.
% \]
% Marginalising over $\pi$ gives the \emph{target vector field}
% \[
% u_{t}(z)=\E_{\pi}\!\bigl[u_{t}(z\mid x_{0},x_{1})\mid z_{t}=z\bigr]\in\T_{z}\M.
% \]

% \subsection{Riemannian Conditional Flow Matching (RCFM)}
% Let $v_{\theta}(z,t)\in\T_{z}\M$ be a neural network output.  The loss is
% \begin{equation}
% \mathcal{L}_{\mathrm{RCFM}}(\theta)=
% \E_{t\sim\U(0,1)}\;
% \E_{(x_{0},x_{1})\sim\pi}\;
% \E_{z_{t}}\,
% \norm{v_{\theta}(z_{t},t)-u_{t}(z_{t}\mid x_{0},x_{1})}^{2}_{g_{z_{t}}}
% \end{equation}
% Because $u_{t}(z_{t}\mid x_{0},x_{1})=\tfrac{1}{t}\Log_{z_{t}}(x_{1})$, the loss can be written in noise-prediction form
% \[
% \mathcal{L}_{\mathrm{RCFM}}(\theta)=
% \E_{t,x_{0},x_{1}}\,
% \norm{v_{\theta}(z_{t},t)-\tfrac{1}{t}\Log_{z_{t}}(x_{1})}^{2}_{g_{z_{t}}}.
% \]

% \subsection{Sampling}
% Once trained, generate samples by integrating the ODE
% \[
% \frac{dz_{t}}{dt}=v_{\theta}(z_{t},t),\qquad z_{0}\sim p_{1},
% \]
% using any Riemannian ODE solver.

% \subsection{Euclidean special case}
% The above formulas reduce to the standard rectified–flow objective iff
% \begin{enumerate}
%   \item $\M=\mathbb{R}^{d}$;
%   \item $g_{z}=I_{d}$ (constant Euclidean metric);
%   \item $\Exp_{z}(v)=z+v$ and $\Log_{z}(w)=w-z$;
%   \item $\Gamma_{z\to w}=\mathrm{Id}$.
% \end{enumerate}
% Under these conditions
% \[
% u_{t}(z\mid x_{0},x_{1})=\frac{x_{1}-x_{0}}{t},\qquad
% \mathcal{L}_{\mathrm{RCFM}}(\theta)=
% \E_{t,x_{0},x_{1}}\norm{v_{\theta}(z_{t},t)-\frac{x_{1}-x_{0}}{t}}^{2}.
% \]


% % --------------
% Let $(\M, g)$ be a complete, connected $d$-dimensional Riemannian manifold equipped with metric tensor $g$. Denote by $\Exp_z : \T_z\M \to \M$ the exponential map and $\Log_z : U_z \subseteq \M \to \T_z\M$ the logarithmic map defined on a neighborhood $U_z$ of $z$, where geodesics are unique and minimizing. Let $\Gamma_{z \to w} : \T_z\M \to \T_w\M$ denote parallel transport along the unique minimizing geodesic from $z$ to $w$.

% We consider the problem of learning a generative model that maps a prior distribution $p_1$ on $\M$ to a target distribution $p_0$ via a flow of diffeomorphisms induced by a time-dependent vector field. To this end, we propose the following computationally tractable algorithm based on Riemannian Conditional Flow Matching (RCFM).

% \section{Riemannian Rectified Flow via Conditional Flow Matching (RRF-CFM)}

% \subsection{Forward Interpolation}
% Given samples $(x_0, x_1) \sim \pi$, where $\pi$ is any coupling between $p_0$ and $p_1$, define the geodesic interpolation:
% \[
% z_t := \Exp_{x_0}\left( t \cdot \Log_{x_0}(x_1) \right), \quad t \in [0,1].
% \]
% The conditional velocity field along this path is given by:
% \[
% u_t(z \mid x_0, x_1) = \frac{d}{dt} z_t \Big|_{z_t = z} \in \T_{z_t}\M.
% \]
% Using the identity $u_t(z_t \mid x_0, x_1) = \frac{1}{t} \Log_{z_t}(x_1)$ for $t > 0$, the marginal target vector field is:
% \[
% u_t(z) := \mathbb{E}_{\pi}\left[ u_t(z \mid x_0, x_1) \,\middle|\, z_t = z \right] \in \T_z\M.
% \]

% \subsection{Neural Parametrization and Loss Function}
% Let $v_\theta : \M \times [0,1] \to \T\M$ be a smooth vector field parametrized by a neural network, with $v_\theta(z,t) \in \T_z\M$. We train $v_\theta$ using the following loss functional:
% \[
% \mathcal{L}_{\mathrm{RRF-CFM}}(\theta) := 
% \mathbb{E}_{t \sim \mathcal{U}(0,1)}\;
% \mathbb{E}_{(x_0,x_1) \sim \pi}\;
% \mathbb{E}_{z_t \sim p_t \mid x_0,x_1}\,
% \left\| v_\theta(z_t, t) - \frac{1}{t} \Log_{z_t}(x_1) \right\|_{g_{z_t}}^2,
% \]
% where $p_t \mid x_0,x_1$ denotes the conditional distribution of $z_t$ under the geodesic interpolation from $x_0$ to $x_1$.

% \subsection{Computational Tractability via Sampling and Approximation}
% To render the expectation computationally feasible, we employ Monte Carlo estimation:

% \begin{enumerate}
%   \item Sample $t_i \sim \mathcal{U}(0,1)$ independently.
%   \item Sample $(x_0^{(i)}, x_1^{(i)}) \sim \pi$ independently.
%   \item Compute $z_{t_i}^{(i)} = \Exp_{x_0^{(i)}}\left( t_i \cdot \Log_{x_0^{(i)}}(x_1^{(i)}) \right)$.
%   \item Evaluate the loss at each batch element:
%     \[
%     \ell_i = \left\| v_\theta(z_{t_i}^{(i)}, t_i) - \frac{1}{t_i} \Log_{z_{t_i}^{(i)}}(x_1^{(i)}) \right\|_{g_{z_{t_i}^{(i)}}}^2.
%     \]
% \end{enumerate}

% The empirical loss is then:
% \[
% \hat{\mathcal{L}}_{\mathrm{RRF-CFM}}(\theta) = \frac{1}{N} \sum_{i=1}^N \ell_i.
% \]

% This formulation avoids explicit integration over the full density $p_t$ and instead relies on implicit sampling through geodesic interpolation, making it scalable even for high-dimensional or complex manifolds.

% \subsection{Training Algorithm}
% \begin{algorithm}[H]
% \caption{Riemannian Rectified Flow via Conditional Flow Matching (RRF-CFM)}
% \label{alg:rrf_cfm}
% \begin{algorithmic}[1]
% \State \textbf{Input:} Data samples $\{x_0^{(i)}\}_{i=1}^N \sim p_0$, prior samples $\{x_1^{(i)}\}_{i=1}^N \sim p_1$, coupling $\pi$, neural network $v_\theta$, learning rate $\eta$, number of iterations $T$.
% \State Initialize parameters $\theta$ of $v_\theta$.
% \For{$k = 1$ to $T$}
%   \State Sample $t_i \sim \mathcal{U}(0,1)$ for $i = 1,\dots,N$.
%   \State Sample $(x_0^{(i)}, x_1^{(i)}) \sim \pi$ (e.g., independent draws).
%   \State For each $i$, compute:
%   \[
%   z_{t_i}^{(i)} = \Exp_{x_0^{(i)}}\left( t_i \cdot \Log_{x_0^{(i)}}(x_1^{(i)}) \right)
%   \]
%   \State Compute gradients:
%   \[
%   \nabla_\theta \hat{\mathcal{L}}_{\mathrm{RRF-CFM}}(\theta) = \frac{1}{N} \sum_{i=1}^N \nabla_\theta \left\| v_\theta(z_{t_i}^{(i)}, t_i) - \frac{1}{t_i} \Log_{z_{t_i}^{(i)}}(x_1^{(i)}) \right\|_{g_{z_{t_i}^{(i)}}}^2
%   \]
%   \State Update: $\theta \leftarrow \theta - \eta \cdot \nabla_\theta \hat{\mathcal{L}}_{\mathrm{RRF-CFM}}(\theta)$
% \EndFor
% \State \textbf{Output:} Trained vector field $v_\theta$
% \end{algorithmic}
% \end{algorithm}

% \subsection{Sampling Procedure}
% Once trained, generate samples from $p_0$ by integrating the Riemannian ODE:
% \[
% \frac{dz_t}{dt} = v_\theta(z_t, t), \quad z_0 \sim p_1,
% \]
% using a numerically stable Riemannian ODE solver (e.g., Runge-Kutta methods adapted to manifolds such as \cite{li2021riemannian} or \cite{mishra2023riemannian}).

% Let $\Phi_{0 \to 1}^\theta : \M \to \M$ denote the flow generated by $v_\theta$. Then, the pushforward $\Phi_{0 \to 1}^\theta \# p_1$ approximates $p_0$.

% % \subsection{Complexity and Scalability}
% % \begin{itemize}
% % \item The computational cost per step is dominated by evaluating $\Exp$ and $\Log$ operations and their derivatives (via automatic differentiation).
% %   \item On manifolds with closed-form $\Exp$ and $\Log$ (e.g., spheres, hyperbolic spaces, Stiefel manifolds), this method is highly efficient.
% %   \item For manifolds without closed forms (e.g., general submanifolds), numerical solvers for geodesics can be used, with error controlled via adaptive integration.
% %   \item The use of Monte Carlo sampling ensures scalability to large datasets and high dimensions.
% % \end{itemize}

% \subsection{Complexity and Scalability}
% \label{subsec:complexity_scalability}

% The computational efficiency of Riemannian Rectified Flow (RRF-CFM) hinges on the tractability of geodesic operations ($\Exp$ and $\Log$). The overall complexity per training step is dominated by these operations and their derivatives, which are typically computed via automatic differentiation. Below, we compare the practical feasibility of different approaches for implementing RRF-CFM on various manifolds.

% \begin{table*}[!t]
% \centering
% \caption{Comparison of Computational Complexity and Feasibility for Riemannian Rectified Flow}
% \label{tab:complexity_comparison}
% \begin{tabular}{|l|c|c|c|}
% \hline
% \textbf{Manifold/Method} & \textbf{Geodesic Ops Complexity} & \textbf{Memory Requirements} & \textbf{Implementation Difficulty} \\
% \hline
% \hline
% Euclidean space $\mathbb{R}^d$ & $\mathcal{O}(d)$ & Low & Very Low \\
% \hline
% Sphere $\mathbb{S}^d$ & $\mathcal{O}(d)$ & Low & Low \\
% \hline
% Hyperbolic space $\mathbb{H}^d$ & $\mathcal{O}(d)$ & Low & Low \\
% \hline
% Stiefel manifold $\mathrm{St}(n,k)$ & $\mathcal{O}(nk^2)$ & Medium & Medium \\
% \hline
% General submanifold (e.g., embedded in $\mathbb{R}^D$) & $\mathcal{O}(D^3)$ & High & High \\
% \hline
% Numerical geodesic solver (generic manifold) & $\mathcal{O}(N_{\text{steps}} \cdot D^3)$ & High & High \\
% \hline
% \end{tabular}
% \end{table*}

% The table above summarizes key aspects of each approach:
% \begin{itemize}
%     \item \textbf{Euclidean space}: The simplest case where $\Exp_z(v) = z + v$ and $\Log_z(w) = w - z$. This reduces RRF-CFM to standard rectified flow, with minimal overhead.
%   \item \textbf{Spheres, Hyperbolic spaces, Stiefel manifolds}: These have closed-form expressions for $\Exp$ and $\Log$, enabling efficient computation at $\mathcal{O}(d)$ or $\mathcal{O}(nk^2)$ complexity. This makes them highly suitable for RRF-CFM.
%   \item \textbf{General submanifolds}: When no closed-form exists, numerical solvers (e.g., Runge-Kutta on the geodesic equation) must be used. The cost scales with the ambient dimension $D$ and the number of integration steps $N_{\text{steps}}$, leading to high memory usage and computational expense.
%   \item \textbf{Numerical geodesic solver}: For arbitrary manifolds without analytical formulas, this is the most general but computationally intensive option. Adaptive integration can control error but increases cost.
% \end{itemize}

% Despite these challenges, RRF-CFM remains scalable due to its reliance on Monte Carlo sampling. By drawing independent samples $(t_i, x_0^{(i)}, x_1^{(i)})$ and computing $z_{t_i}^{(i)}$ only for these points, the method avoids explicit density integration over $p_t$. This enables efficient training on large datasets and high-dimensional manifolds, provided that the underlying geodesic operations are computable.


% \subsection{Complexity and Scalability}

% Table~\ref{tab:complexity} summarizes the computational cost of each major component in RRF-CFM for the most common Riemannian manifolds encountered in practice.  
% We split the analysis into (1) \emph{closed-form} settings, where closed-form expressions for $\Exp$, $\Log$ and parallel transport are available, and (2) \emph{numerical} settings, where these operators require iterative solvers.  
% The dominant cost at every training step is the evaluation of the loss $\ell_i$ for each sample in the mini-batch.  

% \begin{table}[h!]
% \centering
% \renewcommand{\arraystretch}{1.15}
% \caption{Per-sample computational complexity of RRF-CFM.  
% $d$ denotes the manifold dimension, $T_{\text{geo}}$ the number of iterations of a generic geodesic solver (usually $\mathcal{O}(1)$–$\mathcal{O}(10)$), and $T_{\text{int}}$ the number of sub-steps of the ODE solver used at sampling time.}
% \label{tab:complexity}
% \begin{tabular}{@{}llll@{}}
% \toprule
% \textbf{Manifold} & \textbf{Operator} & \textbf{Closed-form cost} & \textbf{Numerical cost} \\
% \midrule
% \multirow{3}{*}{$\mathbb{R}^{d}$} & $\Exp,\Log,\Gamma$ & $\mathcal{O}(d)$ & — \\
% & Loss $\ell_i$ & $\mathcal{O}(d)$ & — \\
% & Sampling (RK4) & $\mathcal{O}(d\,T_{\text{int}})$ & — \\
% \midrule
% \multirow{3}{*}{Sphere $\mathbb{S}^{d}$} & $\Exp,\Log$ & $\mathcal{O}(d)$ & $\mathcal{O}(d\,T_{\text{geo}})$ \\
% & $\Gamma$ (parallel transport) & $\mathcal{O}(d)$ & $\mathcal{O}(d\,T_{\text{geo}})$ \\
% & Sampling & $\mathcal{O}(d\,T_{\text{int}})$ & $\mathcal{O}(d\,T_{\text{geo}}\,T_{\text{int}})$ \\
% \midrule
% \multirow{3}{*}{Hyperboloid $\mathbb{H}^{d}$} & $\Exp,\Log$ & $\mathcal{O}(d)$ & $\mathcal{O}(d\,T_{\text{geo}})$ \\
% & $\Gamma$ & $\mathcal{O}(d)$ & $\mathcal{O}(d\,T_{\text{geo}})$ \\
% & Sampling & $\mathcal{O}(d\,T_{\text{int}})$ & $\mathcal{O}(d\,T_{\text{geo}}\,T_{\text{int}})$ \\
% \midrule
% \multirow{3}{*}{Stiefel $\mathrm{St}(n,p)$} & $\Exp,\Log$ & $\mathcal{O}(np^{2})$ & $\mathcal{O}(np^{2}+T_{\text{geo}}F)$ \\
% & $\Gamma$ & $\mathcal{O}(np^{2})$ & $\mathcal{O}(np^{2}+T_{\text{geo}}F)$ \\
% & Sampling & $\mathcal{O}(np^{2}\,T_{\text{int}})$ & $\mathcal{O}(np^{2}+T_{\text{geo}}F\,T_{\text{int}})$ \\
% \midrule
% \multirow{3}{*}{SPD $\mathcal{S}_{++}^{d}$} & $\Exp,\Log$ & $\mathcal{O}(d^{3})$ & $\mathcal{O}(d^{3}+T_{\text{geo}}F)$ \\
% & $\Gamma$ & $\mathcal{O}(d^{3})$ & $\mathcal{O}(d^{3}+T_{\text{geo}}F)$ \\
% & Sampling & $\mathcal{O}(d^{3}\,T_{\text{int}})$ & $\mathcal{O}(d^{3}+T_{\text{geo}}F\,T_{\text{int}})$ \\
% \bottomrule
% \end{tabular}
% \end{table}

% \textbf{Remarks.}  
% \begin{itemize}
%   \item $F$ denotes the cost of one geodesic solver iteration (dominated by a matrix exponential or SVD for Stiefel/SPD).  
%   \item In practice, closed-form expressions exist for spheres, hyperboloids, and low-rank Stiefel manifolds, yielding the favorable $\mathcal{O}(d)$ or $\mathcal{O}(np^{2})$ entries.  
%   \item Monte-Carlo sampling keeps the memory footprint at $\mathcal{O}(N d)$, where $N$ is the mini-batch size, enabling scaling to large datasets.  
%   \item For high-dimensional general manifolds without closed-form geodesics, adaptive solvers (e.g.\ implicit Runge–Kutta) can be used; the cost becomes $\mathcal{O}(d\,T_{\text{geo}}\,T_{\text{int}})$ per sample.  
% \end{itemize}

% \subsection{Special Case: Euclidean Manifold (Will be merged)}
% When $\M = \mathbb{R}^d$, $g = I_d$, $\Exp_z(v) = z + v$, $\Log_z(w) = w - z$, and $\Gamma_{z\to w} = \mathrm{Id}$, the above reduces to standard rectified flow:
% \[
% \mathcal{L}_{\mathrm{RRF-CFM}}(\theta) = \mathbb{E}_{t,x_0,x_1} \left\| v_\theta(z_t,t) - \frac{x_1 - x_0}{t} \right\|^2,
% \]
% with $z_t = x_0 + t(x_1 - x_0)$.

% Thus, RRF-CFM generalizes rectified flow to arbitrary Riemannian manifolds while preserving computational efficiency and interpretability.


% -------------
\section{Rectified Flow in Euclidean Space (Recap)}

In its original formulation, Rectified Flow operates within a Euclidean space $\R^n$. The model establishes a straight-line path, denoted by $z_t$, between a data point $x_0 \sim p_0$ and a noise sample $\epsilon \sim p_1$:
\begin{equation}
    z_t = (1-t)x_0 + t\epsilon
\end{equation}
This path is generated by a constant velocity vector field, which serves as the learning target for the neural network:
\begin{equation}
    u_t(z_t|\epsilon) = \frac{d z_t}{dt} = \epsilon - x_0
\end{equation}
The training objective is to learn a vector field $v_\Theta(z, t)$ that accurately matches this target velocity field.

\section{Rectified Flow on a Riemannian Manifold}

Let $(\M, g)$ be an $n$-dimensional Riemannian manifold, where $g$ is the metric tensor. We generalize the straight-line path to a \textbf{geodesic}, the shortest path between two points on $\M$.

\subsection{Geodesic Path Formulation}
The geodesic path $\gamma(t): [0, 1] \to \M$ connecting a data point $x_0 \in \M$ to a noise point $\epsilon \in \M$ is defined using the \textbf{exponential map} ($\expmap$) and the \textbf{logarithmic map} ($\logmap$).

\begin{enumerate}
    \item First, we determine the initial velocity vector $v \in T_{x_0}\M$ (the tangent space at $x_0$) that defines the geodesic from $x_0$ to $\epsilon$. This is given by the logarithmic map:
    \begin{equation}
        v = \logmap_{x_0}(\epsilon)
    \end{equation}

    \item The geodesic path $z_t$ is then constructed by traversing along this initial velocity vector for a time $t$ using the exponential map:
    \begin{equation}
        z_t = \expmap_{x_0}(t \cdot v) = \expmap_{x_0}(t \cdot \logmap_{x_0}(\epsilon))
    \end{equation}
    This equation serves as the Riemannian equivalent of linear interpolation.
\end{enumerate}

\subsection{Velocity Vector Field}
The velocity vector of the geodesic path at time $t$, denoted $u_t(z_t|\epsilon) \in T_{z_t}\M$, is given by the \textbf{parallel transport} of the initial velocity vector $v$ along the geodesic $\gamma$. Let $P^\gamma_{t \leftarrow 0}: T_{x_0}\M \to T_{z_t}\M$ represent the parallel transport operator. The velocity field is:
\begin{equation}
    u_t(z_t|\epsilon) = \frac{d z_t}{dt} = P^\gamma_{t \leftarrow 0}(v) = P^\gamma_{t \leftarrow 0}(\logmap_{x_0}(\epsilon))
\end{equation}

\subsection{Flow Matching Objective on $\M$}
The objective is to train a neural network that parameterizes a vector field $v_\Theta(z, t)$ on the manifold to match the geodesic velocity field $u_t$. The Conditional Flow Matching loss on the manifold is defined as:
\begin{equation}
    \mathcal{L}_{CFM} = \E_{t, x_0, \epsilon} \left[ \norm{ v_\Theta(z_t, t) - u_t(z_t|\epsilon) }_{g(z_t)}^2 \right]
\end{equation}
where $\norm{ \cdot }_{g(z_t)}$ is the norm induced by the metric $g$ at the point $z_t$. Substituting the expressions for $z_t$ and $u_t$, we get the full objective function:
\begin{equation}
    \mathcal{L}_{CFM} = \E_{t \sim \mathcal{U}[0,1], x_0 \sim p_0, \epsilon \sim p_1} \left[ \norm{ v_\Theta(\expmap_{x_0}(t \cdot \logmap_{x_0}(\epsilon)), t) - P^\gamma_{t \leftarrow 0}(\logmap_{x_0}(\epsilon)) }_{g(\expmap_{x_0}(t \cdot \logmap_{x_0}(\epsilon)))}^2 \right]
\end{equation}
This formulation is general and holds for manifolds of any dimension.

\section{Condition for Euclidean Space as a Special Case}

The Euclidean space $\R^n$ is a special instance of a Riemannian manifold where the \textbf{Riemann curvature tensor is identically zero}. Such a manifold is referred to as \textbf{flat}.

Under the condition of zero curvature, the geometric operators on the manifold simplify considerably:
\begin{itemize}
    \item \textbf{Metric Tensor}: The metric $g_p$ at any point $p$ corresponds to the standard Euclidean dot product. The norm becomes the Euclidean $L_2$ norm: $\norm{v}_{g(p)}^2 = \norm{v}_2^2$.
    \item \textbf{Exponential Map}: The exponential map simplifies to vector addition:
    \[
        \expmap_p(v) = p + v
    \]
    \item \textbf{Logarithmic Map}: The logarithmic map simplifies to vector subtraction:
    \[
        \logmap_p(q) = q - p
    \]
    \item \textbf{Parallel Transport}: In a flat space, vectors do not change direction when transported. Consequently, parallel transport is the identity operation:
    \[
        P^\gamma_{t \leftarrow 0}(v) = v
    \]
\end{itemize}

Applying these simplifications to our Riemannian formulation demonstrates the reduction to the Euclidean case:

\begin{enumerate}
    \item \textbf{The Path $z_t$}:
    \[
        z_t = \expmap_{x_0}(t \cdot \logmap_{x_0}(\epsilon)) = x_0 + t \cdot (\epsilon - x_0) = (1-t)x_0 + t\epsilon
    \]
    This recovers the exact straight-line path from the original paper.

    \item \textbf{The Velocity Field $u_t$}:
    \[
        u_t(z_t|\epsilon) = P^\gamma_{t \leftarrow 0}(\logmap_{x_0}(\epsilon)) = \logmap_{x_0}(\epsilon) = \epsilon - x_0
    \]
    This recovers the constant velocity vector field.
\end{enumerate}
Therefore, when the curvature of the manifold is zero, the generalized Rectified Flow on a Riemannian manifold reduces precisely to the original formulation in Euclidean space.

\section{Computational Tractability}

The tractability of the geodesic-based Rectified Flow hinges on the computational cost of three fundamental geometric operations for a given manifold $(\M, g)$:

\begin{itemize}
    \item \textbf{Logarithmic Map ($\log_{x_0}(\epsilon)$):} Computing the initial velocity of the geodesic connecting two points.
    \item \textbf{Exponential Map ($\expmap_{x_0}(v)$):} Computing the point reached by following a geodesic from an initial point with a given velocity.
    \item \textbf{Parallel Transport ($P^\gamma_{t \leftarrow 0}(v)$):} Transporting a vector along a geodesic without altering its length or direction relative to the curved path.
\end{itemize}

For a general, arbitrary manifold, these operations lack \textbf{closed-form solutions}. They typically require solving complex systems of ordinary differential equations (ODEs), which is computationally prohibitive to perform within the training loop of a deep learning model.

However, the method becomes highly tractable for specific, well-studied manifolds where these operations possess efficient, analytical formulas. These are the manifolds most commonly employed in geometric deep learning, such as the sphere $\mathbb{S}^{n-1}$, where all necessary operations have efficient solutions derived from basic trigonometry and linear algebra.

\section{Tractable Approximation}

For many manifolds of practical interest (e.g., spheres, tori), a simpler and more computationally efficient formulation is possible. The central idea is to use linear interpolation in a surrounding \textbf{ambient Euclidean space} and then \textbf{project} the resulting path back onto the manifold. This approach circumvents the need to compute geodesics, logarithmic maps, or parallel transport directly.

\subsection{Formulation via Ambient Space Projection}

Assume our $n$-dimensional manifold $\M$ is embedded in a higher-dimensional Euclidean space $\R^D$ (for example, the 2-sphere $\mathbb{S}^2$ embedded in $\R^3$). Let $\proj_{\M}: \R^D \to \M$ be the projection operator.

\begin{enumerate}
    \item \textbf{Linear Interpolation in Ambient Space:} We first define a simple straight-line path $z'_t$ in the ambient space $\R^D$ between points $x_0, \epsilon \in \M \subset \R^D$:
    \[
        z'_t = (1-t)x_0 + t\epsilon
    \]

    \item \textbf{Projection onto Manifold:} The path $z_t$ on the manifold $\M$ is obtained by projecting $z'_t$ at each time step:
    \[
        z_t = \proj_{\M}(z'_t)
    \]

    \item \textbf{Deriving the Velocity Field:} The target velocity field $u_t(z_t|\epsilon)$ is the time derivative of $z_t$. Using the chain rule, this is equivalent to projecting the simple Euclidean velocity $(\epsilon - x_0)$ onto the tangent space $T_{z_t}\M$. This is computed via the Jacobian of the projection operator, $J_{\proj_{\M}}(z'_t)$:
    \[
        u_t(z_t|\epsilon) = \frac{d}{dt} \proj_{\M}(z'_t) = J_{\proj_{\M}}(z'_t) \cdot (\epsilon - x_0)
    \]

    \item \textbf{Improved Loss Function:} The new training objective is to match this more easily computed velocity field:
    \begin{equation}
        \mathcal{L}_{\text{proj}} = \E_{t, x_0, \epsilon} \left[ \norm{ v_\Theta(z_t, t) - J_{\proj_{\M}}(z'_t) \cdot (\epsilon - x_0) }_{g(z_t)}^2 \right]
    \end{equation}
    where $z'_t = (1-t)x_0 + t\epsilon$ and $z_t = \proj_{\M}(z'_t)$.
\end{enumerate}


\section*{Algorithm for Training Riemannian Rectified Flow via Ambient Space Projection}

The following algorithm details the training procedure for a generative model on a Riemannian manifold $\M$ embedded in a Euclidean space $\R^D$. This method avoids direct computation of geodesics by using linear interpolation in the ambient space and projecting onto the manifold.

\begin{algorithm}[H]
\caption{Training Riemannian Rectified Flow via Projection}
\label{alg:riemannian_rf}
\begin{algorithmic}[1]
\Statex \textbf{Require:}
\Statex \quad $v_\Theta$: Neural network with parameters $\Theta$ that outputs a vector in the tangent space.
\Statex \quad $p_0(\mathbf{x})$: Data distribution on the manifold $\M$.
\Statex \quad $p_1(\mathbf{x})$: Noise distribution on the manifold $\M$.
\Statex \quad $\M$: The Riemannian manifold, embedded in $\R^D$.
\Statex \quad $\proj_{\M}(\cdot)$: Operator that projects a point from $\R^D$ to $\M$.
\Statex \quad $J_{\proj_{\M}}(\cdot)$: Jacobian of the projection operator.
\Statex \quad $\alpha$: Learning rate.
\Statex \quad $N_{steps}$: Total number of training steps.
\Statex
\State Initialize network parameters $\Theta$.
\For{step = 1 to $N_{steps}$}
    \State Sample a data point $x_0 \sim p_0(\mathbf{x})$.
    \State Sample a noise point $\epsilon \sim p_1(\mathbf{x})$.
    \State Sample a time step $t \sim \mathcal{U}(0, 1)$.
    \Statex
    \State \Comment{1. Interpolate in the ambient Euclidean space $\R^D$.}
    \State $z'_t \gets (1-t)x_0 + t\epsilon$
    \Statex
    \State \Comment{2. Project the interpolated point onto the manifold $\M$.}
    \State $z_t \gets \proj_{\M}(z'_t)$
    \Statex
    \State \Comment{3. Calculate the target velocity on the tangent space $T_{z_t}\M$.}
    \State \Comment{This is the projection of the ambient velocity $(\epsilon-x_0)$.}
    \State $u_t \gets J_{\proj_{\M}}(z'_t) \cdot (\epsilon - x_0)$
    \Statex
    \State \Comment{4. Get the model's predicted velocity from the current point on the manifold.}
    \State $v_{pred} \gets v_\Theta(z_t, t)$
    \Statex
    \State \Comment{5. Compute the loss using the manifold's metric $g$ at point $z_t$.}
    \State $\mathcal{L} \gets \norm{ v_{pred} - u_t }_{g(z_t)}^2$
    \Statex
    \State \Comment{6. Update model parameters using the gradient of the loss.}
    \State $\Theta \gets \Theta - \alpha \nabla_\Theta \mathcal{L}$
\EndFor
\State
\State \Return Trained parameters $\Theta$.
\end{algorithmic}
\end{algorithm}

% ---------------------------------
\section{Rectified Flow in Euclidean Space (Recap)}

In its original formulation, Rectified Flow operates within a Euclidean space $\R^n$. The model establishes a straight-line path, denoted by $z_t$, between a data point $x_0 \sim p_0$ and a noise sample $\epsilon \sim p_1$:
\begin{equation}
    z_t = (1-t)x_0 + t\epsilon
\end{equation}
This path is generated by a constant velocity vector field, which serves as the learning target for the neural network:
\begin{equation}
    u_t(z_t|\epsilon) = \frac{d z_t}{dt} = \epsilon - x_0
\end{equation}
The training objective is to learn a vector field $v_\Theta(z, t)$ that accurately matches this target velocity field.

\section{Generalizing Rectified Flow to Riemannian Manifolds}

Let $(\M, g)$ be an $n$-dimensional Riemannian manifold, where $g$ is the metric tensor. We generalize the straight-line path to a \textbf{geodesic}, the shortest path between two points on $\M$.

\subsection{Geodesic Path Formulation}
The geodesic path $\gamma(t): [0, 1] \to \M$ connecting a data point $x_0 \in \M$ to a noise point $\epsilon \in \M$ is defined using the \textbf{exponential map} ($\expmap$) and the \textbf{logarithmic map} ($\logmap$).

\begin{enumerate}
    \item First, we determine the initial velocity vector $v \in T_{x_0}\M$ (the tangent space at $x_0$) that defines the geodesic from $x_0$ to $\epsilon$. This is given by the logarithmic map:
    \begin{equation}
        v = \logmap_{x_0}(\epsilon)
    \end{equation}

    \item The geodesic path $z_t$ is then constructed by traversing along this initial velocity vector for a time $t$ using the exponential map:
    \begin{equation}
        z_t = \expmap_{x_0}(t \cdot v) = \expmap_{x_0}(t \cdot \logmap_{x_0}(\epsilon))
    \end{equation}
    This equation serves as the Riemannian equivalent of linear interpolation.
\end{enumerate}

\subsection{Velocity Vector Field on the Manifold}
The velocity vector of the geodesic path at time $t$, denoted $u_t(z_t|\epsilon) \in T_{z_t}\M$, is given by the \textbf{parallel transport} of the initial velocity vector $v$ along the geodesic $\gamma$. Let $P^\gamma_{t \leftarrow 0}: T_{x_0}\M \to T_{z_t}\M$ represent the parallel transport operator. The velocity field is:
\begin{equation}
    u_t(z_t|\epsilon) = \frac{d z_t}{dt} = P^\gamma_{t \leftarrow 0}(v) = P^\gamma_{t \leftarrow 0}(\logmap_{x_0}(\epsilon))
\end{equation}

\subsection{Flow Matching Objective on $\M$}
The objective is to train a neural network that parameterizes a vector field $v_\Theta(z, t)$ on the manifold to match the geodesic velocity field $u_t$. The Conditional Flow Matching loss on the manifold is defined as:
\begin{equation}
    \mathcal{L}_{CFM} = \E_{t, x_0, \epsilon} \left[ \norm{ v_\Theta(z_t, t) - u_t(z_t|\epsilon) }_{g(z_t)}^2 \right]
\end{equation}
where $\norm{ \cdot }_{g(z_t)}$ is the norm induced by the metric $g$ at the point $z_t$. Substituting the expressions for $z_t$ and $u_t$, we get the full objective function:
\begin{equation}
    \mathcal{L}_{CFM} = \E_{t \sim \mathcal{U}[0,1], x_0 \sim p_0, \epsilon \sim p_1} \left[ \norm{ v_\Theta(\expmap_{x_0}(t \cdot \logmap_{x_0}(\epsilon)), t) - P^\gamma_{t \leftarrow 0}(\logmap_{x_0}(\epsilon)) }_{g(\expmap_{x_0}(t \cdot \logmap_{x_0}(\epsilon)))}^2 \right]
\end{equation}
This formulation is general and holds for any Riemannian manifold.

\section{Special Case: Reduction to Euclidean Space}

The Euclidean space $\R^n$ is a special instance of a Riemannian manifold where the \textbf{Riemann curvature tensor is identically zero}. Such a manifold is referred to as \textbf{flat}. Under this condition, the geometric operators simplify considerably:
\begin{itemize}
    \item \textbf{Metric Tensor}: $g_p$ is the standard dot product, so $\norm{v}_{g(p)}^2 = \norm{v}_2^2$.
    \item \textbf{Exponential Map}: $\expmap_p(v) = p + v$.
    \item \textbf{Logarithmic Map}: $\logmap_p(q) = q - p$.
    \item \textbf{Parallel Transport}: $P^\gamma_{t \leftarrow 0}(v) = v$.
\end{itemize}
Applying these simplifications, the path $z_t$ and velocity $u_t$ reduce to their Euclidean forms:
\begin{enumerate}
    \item \textbf{The Path $z_t$}:
    \[
        z_t = \expmap_{x_0}(t \cdot \logmap_{x_0}(\epsilon)) = x_0 + t \cdot (\epsilon - x_0) = (1-t)x_0 + t\epsilon
    \]
    \item \textbf{The Velocity Field $u_t$}:
    \[
        u_t(z_t|\epsilon) = P^\gamma_{t \leftarrow 0}(\logmap_{x_0}(\epsilon)) = \logmap_{x_0}(\epsilon) = \epsilon - x_0
    \]
\end{enumerate}
Thus, the generalized framework naturally recovers the original formulation when the manifold is flat.

\section{Tractability and Specific Manifolds}

\subsection{The Challenge of General Manifolds}
The tractability of the geodesic-based flow hinges on the computational cost of the logarithmic map, exponential map, and parallel transport. For a general, arbitrary manifold, these operations lack \textbf{closed-form solutions} and require solving computationally expensive ODEs, making them unsuitable for deep learning training loops.

\subsection{Example: The Sphere ($\mathbb{S}^{n-1}$)}
The method becomes highly tractable for specific, well-studied manifolds where these operations have efficient, analytical formulas. The sphere $\mathbb{S}^{n-1} = \{x \in \R^n \mid \norm{x}_2 = 1\}$ is a prime example.
\begin{itemize}
    \item \textbf{Logarithmic Map:} The log map finds the tangent vector $v \in T_{x_0}\mathbb{S}^{n-1}$ that points towards $\epsilon$.
    \[ \logmap_{x_0}(\epsilon) = \frac{\theta}{\sin(\theta)}(\epsilon - \cos(\theta) x_0), \quad \text{where } \theta = \arccos(x_0^T \epsilon) \]
    \item \textbf{Exponential Map:} The exp map traverses a great circle (the geodesic) from $x_0$ with initial velocity $v$.
    \[ \expmap_{x_0}(v) = \cos(\norm{v}_2) x_0 + \sin(\norm{v}_2) \frac{v}{\norm{v}_2} \]
    \item \textbf{Parallel Transport:} Transporting $w \in T_{x_0}\mathbb{S}^{n-1}$ along the geodesic to $z_t = \expmap_{x_0}(tv)$ is given by:
    \[ P_{t \leftarrow 0}(w) = -\sin(t\norm{v}_2)\norm{v}_2 x_0 + \cos(t\norm{v}_2)\frac{v}{\norm{v}_2} + \left(w - \frac{v^T w}{\norm{v}_2^2} v\right) \]
\end{itemize}
Other tractable manifolds include hyperbolic spaces (Poincar\'e ball) and tori.

\section{A Tractable Approximation: Projection from Ambient Space}

For many manifolds, an even simpler formulation is to perform linear interpolation in a surrounding \textbf{ambient Euclidean space} and then \textbf{project} the path back onto the manifold. This approach circumvents the need for geodesics, log/exp maps, and parallel transport.

\subsection{General Formulation via Projection}
Assume our $n$-dimensional manifold $\M$ is embedded in a higher-dimensional Euclidean space $\R^D$. Let $\proj_{\M}: \R^D \to \M$ be the projection operator.
\begin{enumerate}
    \item \textbf{Linear Interpolation in Ambient Space:} Define a straight line $z'_t$ in $\R^D$:
    \[
        z'_t = (1-t)x_0 + t\epsilon
    \]
    \item \textbf{Projection onto Manifold:} The path $z_t$ on $\M$ is obtained by projecting $z'_t$:
    \[
        z_t = \proj_{\M}(z'_t)
    \]
    \item \textbf{Deriving the Velocity Field:} The target velocity $u_t$ is the time derivative of $z_t$. Using the chain rule, this is the projection of the ambient velocity $(\epsilon - x_0)$ onto the tangent space $T_{z_t}\M$, computed via the Jacobian of the projection, $J_{\proj_{\M}}(z'_t)$:
    \[
        u_t(z_t|\epsilon) = \frac{d}{dt} \proj_{\M}(z'_t) = J_{\proj_{\M}}(z'_t) \cdot (\epsilon - x_0)
    \]
    \item \textbf{Simplified Loss Function:} The new training objective is:
    \begin{equation}
        \mathcal{L}_{\text{proj}} = \E_{t, x_0, \epsilon} \left[ \norm{ v_\Theta(z_t, t) - J_{\proj_{\M}}(z'_t) \cdot (\epsilon - x_0) }_{g(z_t)}^2 \right]
    \end{equation}
\end{enumerate}

\subsection{Application to the Sphere ($\mathbb{S}^{n-1}$)}
For the sphere $\mathbb{S}^{n-1}$ embedded in $\R^n$, the projection operations are very simple:
\begin{itemize}
    \item \textbf{Projection Operator:} Normalization to unit length.
    \[ \proj_{\mathbb{S}^{n-1}}(x) = \frac{x}{\norm{x}_2} \]
    \item \textbf{Velocity Field:} The Jacobian projects the ambient velocity onto the tangent space at $z_t$. The tangent space $T_{z_t}\mathbb{S}^{n-1}$ is the set of vectors orthogonal to $z_t$. The projection of a vector $v$ onto this space is:
    \[ J_{\proj_{\mathbb{S}^{n-1}}}(z'_t) \cdot v \approx \proj_{T_{z_t}}(v) = v - (v^T z_t) z_t \]
    Applying this to the ambient velocity $v = (\epsilon - x_0)$:
    \[ u_t = (\epsilon - x_0) - ((\epsilon - x_0)^T z_t) z_t, \quad \text{where } z_t = \frac{(1-t)x_0 + t\epsilon}{\norm{(1-t)x_0 + t\epsilon}_2} \]
\end{itemize}
This provides a highly efficient and purely algebraic way to compute the training target.

\section*{Algorithm for Training Riemannian Rectified Flow via Ambient Space Projection}

The following algorithm details the training procedure using the efficient projection-based method.

\begin{algorithm}[H]
\caption{Training Riemannian Rectified Flow via Projection}
\label{alg:riemannian_rf}
\begin{algorithmic}[1]
\Statex \textbf{Require:}
\Statex \quad $v_\Theta$: Neural network with parameters $\Theta$ that outputs a vector in the tangent space.
\Statex \quad $p_0(\mathbf{x})$: Data distribution on the manifold $\M$.
\Statex \quad $p_1(\mathbf{x})$: Noise distribution on the manifold $\M$.
\Statex \quad $\M$: The Riemannian manifold, embedded in $\R^D$.
\Statex \quad $\proj_{\M}(\cdot)$: Operator that projects a point from $\R^D$ to $\M$.
\Statex \quad $J_{\proj_{\M}}(\cdot)$: Jacobian of the projection operator (or equivalent tangent space projection).
\Statex
\State Initialize network parameters $\Theta$.
\For{each training step}
    \State Sample a data point $x_0 \sim p_0(\mathbf{x})$.
    \State Sample a noise point $\epsilon \sim p_1(\mathbf{x})$.
    \State Sample a time step $t \sim \mathcal{U}(0, 1)$.
    \Statex
    \State \Comment{1. Interpolate in the ambient Euclidean space $\R^D$.}
    \State $z'_t \gets (1-t)x_0 + t\epsilon$
    \Statex
    \State \Comment{2. Project the interpolated point onto the manifold $\M$.}
    \State $z_t \gets \proj_{\M}(z'_t)$
    \Statex
    \State \Comment{3. Calculate the target velocity on the tangent space $T_{z_t}\M$.}
    \State \Comment{This is the projection of the ambient velocity $(\epsilon-x_0)$.}
    \State $u_t \gets J_{\proj_{\M}}(z'_t) \cdot (\epsilon - x_0)$
    \Statex
    \State \Comment{4. Get the model's predicted velocity at the current point on the manifold.}
    \State $v_{pred} \gets v_\Theta(z_t, t)$
    \Statex
    \State \Comment{5. Compute the loss using the manifold's metric $g$ at point $z_t$.}
    \State $\mathcal{L} \gets \norm{ v_{pred} - u_t }_{g(z_t)}^2$
    \Statex
    \State \Comment{6. Update model parameters via gradient descent on $\mathcal{L}$.}
    \State $\Theta \gets \Theta - \alpha \nabla_\Theta \mathcal{L}$
\EndFor
\State
\State \Return Trained parameters $\Theta$.
\end{algorithmic}
\end{algorithm}

% -----------------------------
\section{Rectified Flow in Euclidean Space (Recap)}

In its original formulation, Rectified Flow operates within a Euclidean space $\R^n$. The model establishes a straight-line path, denoted by $z_t$, between a data point $x_0 \sim p_0$ and a noise sample $\epsilon \sim p_1$:
\begin{equation}
    z_t = (1-t)x_0 + t\epsilon
\end{equation}
This path is generated by a constant velocity vector field, which serves as the learning target for the neural network:
\begin{equation}
    u_t(z_t|\epsilon) = \frac{d z_t}{dt} = \epsilon - x_0
\end{equation}
The training objective is to learn a vector field $v_\Theta(z, t)$ that accurately matches this target velocity field.

\section{Generalizing Rectified Flow to Riemannian Manifolds}

Let $(\M, g)$ be an $n$-dimensional Riemannian manifold, where $g$ is the metric tensor. We generalize the straight-line path to a \textbf{geodesic}, the shortest path between two points on $\M$.

\subsection{Geodesic Path Formulation}
The geodesic path $\gamma(t): [0, 1] \to \M$ connecting a data point $x_0 \in \M$ to a noise point $\epsilon \in \M$ is defined using the \textbf{exponential map} ($\expmap$) and the \textbf{logarithmic map} ($\logmap$).

\begin{enumerate}
    \item First, we determine the initial velocity vector $v \in T_{x_0}\M$ (the tangent space at $x_0$) that defines the geodesic from $x_0$ to $\epsilon$. This is given by the logarithmic map:
    \begin{equation}
        v = \logmap_{x_0}(\epsilon)
    \end{equation}

    \item The geodesic path $z_t$ is then constructed by traversing along this initial velocity vector for a time $t$ using the exponential map:
    \begin{equation}
        z_t = \expmap_{x_0}(t \cdot v) = \expmap_{x_0}(t \cdot \logmap_{x_0}(\epsilon))
    \end{equation}
    This equation serves as the Riemannian equivalent of linear interpolation.
\end{enumerate}

\subsection{Velocity Vector Field on the Manifold}
The velocity vector of the geodesic path at time $t$, denoted $u_t(z_t|\epsilon) \in T_{z_t}\M$, is given by the \textbf{parallel transport} of the initial velocity vector $v$ along the geodesic $\gamma$. Let $P^\gamma_{t \leftarrow 0}: T_{x_0}\M \to T_{z_t}\M$ represent the parallel transport operator. The velocity field is:
\begin{equation}
    u_t(z_t|\epsilon) = \frac{d z_t}{dt} = P^\gamma_{t \leftarrow 0}(v) = P^\gamma_{t \leftarrow 0}(\logmap_{x_0}(\epsilon))
\end{equation}

\subsection{Flow Matching Objective on $\M$}
The objective is to train a neural network that parameterizes a vector field $v_\Theta(z, t)$ on the manifold to match the geodesic velocity field $u_t$. The Conditional Flow Matching loss on the manifold is defined as:
\begin{equation}
    \mathcal{L}_{CFM} = \E_{t, x_0, \epsilon} \left[ \norm{ v_\Theta(z_t, t) - u_t(z_t|\epsilon) }_{g(z_t)}^2 \right]
\end{equation}
where $\norm{ \cdot }_{g(z_t)}$ is the norm induced by the metric $g$ at the point $z_t$. Substituting the expressions for $z_t$ and $u_t$, we get the full objective function:
\begin{equation}
    \mathcal{L}_{CFM} = \E_{t \sim \mathcal{U}[0,1], x_0 \sim p_0, \epsilon \sim p_1} \left[ \norm{ v_\Theta(\expmap_{x_0}(t \cdot \logmap_{x_0}(\epsilon)), t) - P^\gamma_{t \leftarrow 0}(\logmap_{x_0}(\epsilon)) }_{g(\expmap_{x_0}(t \cdot \logmap_{x_0}(\epsilon)))}^2 \right]
\end{equation}
This formulation is general and holds for any Riemannian manifold.

\section{Special Case: Reduction to Euclidean Space}

The Euclidean space $\R^n$ is a special instance of a Riemannian manifold where the \textbf{Riemann curvature tensor is identically zero}. Such a manifold is referred to as \textbf{flat}. Under this condition, the geometric operators simplify considerably:
\begin{itemize}
    \item \textbf{Metric Tensor}: $g_p$ is the standard dot product, so $\norm{v}_{g(p)}^2 = \norm{v}_2^2$.
    \item \textbf{Exponential Map}: $\expmap_p(v) = p + v$.
    \item \textbf{Logarithmic Map}: $\logmap_p(q) = q - p$.
    \item \textbf{Parallel Transport}: $P^\gamma_{t \leftarrow 0}(v) = v$.
\end{itemize}
Applying these simplifications, the path $z_t$ and velocity $u_t$ reduce to their Euclidean forms:
\begin{enumerate}
    \item \textbf{The Path $z_t$}:
    \[
        z_t = \expmap_{x_0}(t \cdot \logmap_{x_0}(\epsilon)) = x_0 + t \cdot (\epsilon - x_0) = (1-t)x_0 + t\epsilon
    \]
    \item \textbf{The Velocity Field $u_t$}:
    \[
        u_t(z_t|\epsilon) = P^\gamma_{t \leftarrow 0}(\logmap_{x_0}(\epsilon)) = \logmap_{x_0}(\epsilon) = \epsilon - x_0
    \]
\end{enumerate}
Thus, the generalized framework naturally recovers the original formulation when the manifold is flat.

\section{Tractability and Specific Manifolds}

\subsection{The Challenge of General Manifolds}
The tractability of the geodesic-based flow hinges on the computational cost of the logarithmic map, exponential map, and parallel transport. For a general, arbitrary manifold, these operations lack \textbf{closed-form solutions} and require solving computationally expensive ODEs, making them unsuitable for deep learning training loops.

\subsection{Example: The Sphere ($\mathbb{S}^{n-1}$)}
The method becomes highly tractable for specific, well-studied manifolds where these operations have efficient, analytical formulas. The sphere $\mathbb{S}^{n-1} = \{x \in \R^n \mid \norm{x}_2 = 1\}$ is a prime example.
\begin{itemize}
    \item \textbf{Logarithmic Map:} The log map finds the tangent vector $v \in T_{x_0}\mathbb{S}^{n-1}$ that points towards $\epsilon$.
    \[ \logmap_{x_0}(\epsilon) = \frac{\theta}{\sin(\theta)}(\epsilon - \cos(\theta) x_0), \quad \text{where } \theta = \arccos(x_0^T \epsilon) \]
    \item \textbf{Exponential Map:} The exp map traverses a great circle (the geodesic) from $x_0$ with initial velocity $v$.
    \[ \expmap_{x_0}(v) = \cos(\norm{v}_2) x_0 + \sin(\norm{v}_2) \frac{v}{\norm{v}_2} \]
    \item \textbf{Parallel Transport:} Transporting $w \in T_{x_0}\mathbb{S}^{n-1}$ along the geodesic to $z_t = \expmap_{x_0}(tv)$ is given by:
    \[ P_{t \leftarrow 0}(w) = -\sin(t\norm{v}_2)\norm{v}_2 x_0 + \cos(t\norm{v}_2)\frac{v}{\norm{v}_2} + \left(w - \frac{v^T w}{\norm{v}_2^2} v\right) \]
\end{itemize}
Other tractable manifolds include hyperbolic spaces (Poincar\'e ball) and tori.

\section{A Tractable Approximation: Projection from Ambient Space}

For many manifolds, an even simpler formulation is to perform linear interpolation in a surrounding \textbf{ambient Euclidean space} and then \textbf{project} the path back onto the manifold. This approach circumvents the need for geodesics, log/exp maps, and parallel transport.

\subsection{General Formulation via Projection}
Assume our $n$-dimensional manifold $\M$ is embedded in a higher-dimensional Euclidean space $\R^D$. Let $\proj_{\M}: \R^D \to \M$ be the projection operator.
\begin{enumerate}
    \item \textbf{Linear Interpolation in Ambient Space:} Define a straight line $z'_t$ in $\R^D$:
    \[
        z'_t = (1-t)x_0 + t\epsilon
    \]
    \item \textbf{Projection onto Manifold:} The path $z_t$ on $\M$ is obtained by projecting $z'_t$:
    \[
        z_t = \proj_{\M}(z'_t)
    \]
    \item \textbf{Deriving the Velocity Field:} The target velocity $u_t$ is the time derivative of $z_t$. Using the chain rule, this is the projection of the ambient velocity $(\epsilon - x_0)$ onto the tangent space $T_{z_t}\M$, computed via the Jacobian of the projection, $J_{\proj_{\M}}(z'_t)$:
    \[
        u_t(z_t|\epsilon) = \frac{d}{dt} \proj_{\M}(z'_t) = J_{\proj_{\M}}(z'_t) \cdot (\epsilon - x_0)
    \]
    \item \textbf{Simplified Loss Function:} The new training objective is:
    \begin{equation}
        \mathcal{L}_{\text{proj}} = \E_{t, x_0, \epsilon} \left[ \norm{ v_\Theta(z_t, t) - J_{\proj_{\M}}(z'_t) \cdot (\epsilon - x_0) }_{g(z_t)}^2 \right]
    \end{equation}
\end{enumerate}

\subsection{Application to the Sphere ($\mathbb{S}^{n-1}$)}
For the sphere $\mathbb{S}^{n-1}$ embedded in $\R^n$, the projection operations are very simple:
\begin{itemize}
    \item \textbf{Projection Operator:} Normalization to unit length.
    \[ \proj_{\mathbb{S}^{n-1}}(x) = \frac{x}{\norm{x}_2} \]
    \item \textbf{Velocity Field:} The Jacobian projects the ambient velocity onto the tangent space at $z_t$. The tangent space $T_{z_t}\mathbb{S}^{n-1}$ is the set of vectors orthogonal to $z_t$. The projection of a vector $v$ onto this space is:
    \[ J_{\proj_{\mathbb{S}^{n-1}}}(z'_t) \cdot v \approx \proj_{T_{z_t}}(v) = v - (v^T z_t) z_t \]
    Applying this to the ambient velocity $v = (\epsilon - x_0)$:
    \[ u_t = (\epsilon - x_0) - ((\epsilon - x_0)^T z_t) z_t, \quad \text{where } z_t = \frac{(1-t)x_0 + t\epsilon}{\norm{(1-t)x_0 + t\epsilon}_2} \]
\end{itemize}
This provides a highly efficient and purely algebraic way to compute the training target.

\section*{Algorithm for Training Riemannian Rectified Flow via Ambient Space Projection}

The following algorithm details the training procedure using the efficient projection-based method.

\begin{algorithm}[H]
\caption{Training Riemannian Rectified Flow via Projection}
\label{alg:riemannian_rf}
\begin{algorithmic}[1]
\Statex \textbf{Require:}
\Statex \quad \textit{Model:}
\Statex \quad\quad $v_\Theta$: Neural network with parameters $\Theta$.
\Statex \quad \textit{Data:}
\Statex \quad\quad $p_0(\mathbf{x})$: Data distribution on the manifold $\M$.
\Statex \quad\quad $p_1(\mathbf{x})$: Noise distribution on the manifold $\M$.
\Statex \quad \textit{Manifold specifics:}
\Statex \quad\quad $\M$: The Riemannian manifold, embedded in $\R^D$.
\Statex \quad\quad $\proj_{\M}(\cdot)$: Projection operator from $\R^D$ to $\M$.
\Statex \quad\quad $J_{\proj_{\M}}(\cdot)$: Jacobian of the projection operator.
\Statex \quad \textit{Hyperparameters:}
\Statex \quad\quad $B$: Batch size.
\Statex \quad\quad $N_{steps}$: Total number of training steps.
\Statex \quad\quad $\alpha$: Learning rate.
\Statex \quad\quad Optimizer: e.g., AdamW with parameters $(\beta_1, \beta_2, \text{weight\_decay})$.
\Statex
\State Initialize network parameters $\Theta$ and Optimizer.
\For{step = 1 to $N_{steps}$}
    \State Sample a batch of data points $\{x_0^{(i)}\}_{i=1}^B \sim p_0(\mathbf{x})$.
    \State Sample a batch of noise points $\{\epsilon^{(i)}\}_{i=1}^B \sim p_1(\mathbf{x})$.
    \State Sample a batch of time steps $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0, 1)$.
    \Statex
    \State \Comment{1. Interpolate in ambient space for the batch.}
    \State $\{z'^{(i)}_t\}_{i=1}^B \gets \{(1-t^{(i)})x_0^{(i)} + t^{(i)}\epsilon^{(i)}\}_{i=1}^B$
    \Statex
    \State \Comment{2. Project the interpolated points onto the manifold $\M$.}
    \State $\{z^{(i)}_t\}_{i=1}^B \gets \{\proj_{\M}(z'^{(i)}_t)\}_{i=1}^B$
    \Statex
    \State \Comment{3. Calculate the target velocities on the tangent spaces.}
    \State $\{u^{(i)}_t\}_{i=1}^B \gets \{J_{\proj_{\M}}(z'^{(i)}_t) \cdot (\epsilon^{(i)} - x_0^{(i)})\}_{i=1}^B$
    \Statex
    \State \Comment{4. Get the model's predicted velocities.}
    \State $\{v^{(i)}_{pred}\}_{i=1}^B \gets \{v_\Theta(z^{(i)}_t, t^{(i)})\}_{i=1}^B$
    \Statex
    \State \Comment{5. Compute the mean loss over the batch.}
    \State $\mathcal{L} \gets \frac{1}{B} \sum_{i=1}^B \norm{ v^{(i)}_{pred} - u^{(i)}_t }_{g(z^{(i)}_t)}^2$
    \Statex
    \State \Comment{6. Update model parameters using the gradient of the batch loss.}
    \State $\Theta \gets \text{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$
\EndFor
\State
\State \Return Trained parameters $\Theta$.
\end{algorithmic}
\end{algorithm}

% ----------------------
\section{Adaptive Geodesic-Projection Rectified Flow (AGP-Flow) Sep 13}

Let $(\M, g)$ be a Riemannian manifold embedded in $\R^D$. We assume access to the following operators:
\begin{itemize}
    \item A \textbf{projection operator} $\proj_{\M}: \R^D \to \M$ (possibly set-valued or undefined at singularities).
    \item A \textbf{geodesic operator} $\text{Geo}(x_0, \epsilon, t) = \expmap_{x_0}(t \cdot \logmap_{x_0}(\epsilon))$, available for certain $(x_0, \epsilon)$ pairs or manifolds.
    \item A \textbf{geodesic velocity} $u^{\text{geo}}_t = P^\gamma_{t \leftarrow 0}(\logmap_{x_0}(\epsilon))$, where $P^\gamma$ is parallel transport along the geodesic.
    \item A \textbf{projection-based velocity} $u^{\text{proj}}_t = J_{\proj_{\M}}(z'_t) \cdot (\epsilon - x_0)$, where $z'_t = (1-t)x_0 + t\epsilon$ and $J_{\proj_{\M}}$ is the Jacobian of projection.
    \item A \textbf{metric-compatible norm} $\norm{\cdot}_{g(z)}$ induced by the Riemannian metric at $z \in \M$.
\end{itemize}

\subsection{Adaptive Path Selection}

To balance computational efficiency with geometric fidelity, we define a switching criterion based on:
\begin{itemize}
    \item \textbf{Tractability flag} $\mathcal{T}(x_0, \epsilon)$: Boolean indicating whether $\logmap_{x_0}(\epsilon)$ and $\expmap$ are computable in closed-form or within computational budget.
    \item \textbf{Distance threshold} $\delta > 0$: If the geodesic distance $d_{\M}(x_0, \epsilon) > \delta$, prefer geodesic interpolation (projection may be inaccurate over long curved paths).
    \item \textbf{Singularity detector} $\mathcal{S}(z'_t)$: Returns \texttt{True} if projection is ill-defined (e.g., $z'_t = 0$ on the sphere $\mathbb{S}^{n-1}$).
\end{itemize}

The interpolated point $z_t$ and target velocity $u_t$ are selected adaptively:

\begin{equation}
    z_t =
    \begin{cases}
        \expmap_{x_0}(t \cdot \logmap_{x_0}(\epsilon)) & \text{if } \mathcal{T}(x_0, \epsilon) \land d_{\M}(x_0, \epsilon) > \delta \\
        \proj_{\M}((1-t)x_0 + t\epsilon) & \text{if } \neg \mathcal{S}((1-t)x_0 + t\epsilon) \\
        \proj_{\M}((1-t)x_0 + t\epsilon + \eta_t) & \text{otherwise (add noise $\eta_t \sim \mathcal{N}(0, \sigma^2 I)$)}
    \end{cases}
\end{equation}

\begin{equation}
    u_t =
    \begin{cases}
        P^\gamma_{t \leftarrow 0}(\logmap_{x_0}(\epsilon)) & \text{if using geodesic path} \\
        \Pi_{T_{z_t}\M} \left( J_{\proj_{\M}}(z'_t) \cdot (\epsilon - x_0) \right) & \text{if using projected path}
    \end{cases}
\end{equation}

Here, $\Pi_{T_{z_t}\M}(\cdot)$ denotes explicit orthogonal projection onto the tangent space $T_{z_t}\M$, ensuring $u_t$ is a valid tangent vector even if the Jacobian computation is approximate or extrinsic.

\subsection{Metric-Aligned Loss with Geodesic Regularization}

To ensure the learned vector field respects the intrinsic geometry of $\M$ and remains close to the optimal geodesic transport, we introduce a regularized training objective:

\begin{equation}
    \mathcal{L}_{\text{AGP}} = \E_{t, x_0, \epsilon} \left[ \norm{ v_\Theta(z_t, t) - u_t }_{g(z_t)}^2 + \lambda \cdot \I_{\mathcal{T}(x_0,\epsilon)} \cdot d_{\M}^2\left( z_t, \text{Geo}(x_0, \epsilon, t) \right) \right]
\end{equation}

where:
\begin{itemize}
    \item $\lambda \geq 0$ is a tunable regularization weight.
    \item $\I_{\mathcal{T}(x_0,\epsilon)}$ is the indicator function (1 if geodesic is tractable, 0 otherwise).
    \item $d_{\M}(\cdot, \cdot)$ is the geodesic distance on $\M$.
\end{itemize}

This regularizer encourages the projected path to remain geometrically close to the true geodesic when computable, improving consistency without requiring full geodesic computation at every step.

\subsection{Robust Sampling with Projection Correction}

During sampling, we integrate the learned vector field with a projection correction step to ensure trajectories remain on $\M$:

\begin{algorithm}[H]
\caption{Sampling via AGP-Flow with Projection Correction}
\label{alg:sampling}
\begin{algorithmic}[1]
\Require Trained model $v_\Theta$, noise sample $\epsilon \sim p_1$, ODE solver step size $\Delta t$, projection $\proj_{\M}$.
\State $z_1 \gets \epsilon$
\For{$t = 1$ \textbf{to} $0$ by $-\Delta t$}
    \State $\dot{z} \gets v_\Theta(z_t, t)$ \Comment{Predict velocity in ambient or tangent space}
    \State $z_{t - \Delta t}^{\text{temp}} \gets z_t - \dot{z} \cdot \Delta t$ \Comment{Euler step (or use higher-order solver)}
    \State $z_{t - \Delta t} \gets \proj_{\M}(z_{t - \Delta t}^{\text{temp}})$ \Comment{Project back to manifold}
\EndFor
\Return $z_0$
\end{algorithmic}
\end{algorithm}

\noindent \textbf{Note:} For higher-order ODE solvers (e.g., Dormand-Prince), apply projection after \textit{each} intermediate step to prevent numerical drift off the manifold.

\subsection{Manifold-Specific Implementation Notes}

\begin{itemize}
    \item \textbf{Sphere $\mathbb{S}^{n-1}$}: Use geodesic interpolation when angular distance $\theta = \arccos(x_0^\T \epsilon) > 0.8\pi$ (near-antipodal points). Add noise $\eta_t$ if $\|z'_t\|_2 < \varepsilon$.
    
    \item \textbf{Hyperbolic space $\mathbb{H}^n$ (Poincaré ball)}: Prefer geodesic (Möbius operations are closed-form and cheap). Avoid projection — it is non-isometric and distorts geometry.
    
    \item \textbf{SPD matrices $\mathcal{S}_{++}^n$}: Use geodesic under affine-invariant or log-Euclidean metric. Projection via eigenvalue clipping is approximate and metric-inconsistent — use only as fallback.
    
    \item \textbf{General embedded $\M$}: Precompute or cache $\logmap/\expmap$ for common point pairs; fall back to projection with regularization when intractable.
\end{itemize}

\section*{Algorithm: Training Adaptive Geodesic-Projection Rectified Flow}

\begin{algorithm}[H]
\caption{Training AGP-Flow}
\label{alg:agp_flow}
\begin{algorithmic}[1]
\Require
\begin{itemize}
    \item \textit{Model:} Neural network $v_\Theta$ with parameters $\Theta$.
    \item \textit{Data:} Distributions $p_0$ (data), $p_1$ (noise) on $\M$.
    \item \textit{Manifold Ops:} $\proj_{\M}, J_{\proj_{\M}}, \expmap, \logmap, P^\gamma, d_{\M}$ (partial availability acceptable).
    \item \textit{Hyperparameters:} Batch size $B$, steps $N_{\text{steps}}$, learning rate $\alpha$, regularization $\lambda$, distance threshold $\delta$, noise scale $\sigma$, singularity threshold $\varepsilon$.
\end{itemize}
\State Initialize $\Theta$ and optimizer (e.g., AdamW).
\For{step = 1 to $N_{\text{steps}}$}
    \State Sample $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{\epsilon^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
    \For{$i = 1$ to $B$}
        \State $z'^{(i)}_t \gets (1-t^{(i)})x_0^{(i)} + t^{(i)}\epsilon^{(i)}$
        \If{$\mathcal{T}(x_0^{(i)}, \epsilon^{(i)})$ and $d_{\M}(x_0^{(i)}, \epsilon^{(i)}) > \delta$}
            \State $z^{(i)}_t \gets \expmap_{x_0^{(i)}}(t^{(i)} \cdot \logmap_{x_0^{(i)}}(\epsilon^{(i)}))$
            \State $u^{(i)}_t \gets P^\gamma_{t^{(i)} \leftarrow 0}(\logmap_{x_0^{(i)}}(\epsilon^{(i)}))$
            \State $z^{\text{geo}} \gets z^{(i)}_t$ \Comment{Store for regularization}
        \Else
            \If{$\mathcal{S}(z'^{(i)}_t)$ or $\|z'^{(i)}_t\| < \varepsilon$}
                \State $z'^{(i)}_t \gets z'^{(i)}_t + \eta^{(i)}_t, \quad \eta^{(i)}_t \sim \mathcal{N}(0, \sigma^2 I_D)$
            \EndIf
            \State $z^{(i)}_t \gets \proj_{\M}(z'^{(i)}_t)$
            \State $u^{(i)}_t \gets \Pi_{T_{z^{(i)}_t}\M} \left( J_{\proj_{\M}}(z'^{(i)}_t) \cdot (\epsilon^{(i)} - x_0^{(i)}) \right)$
            \If{$\mathcal{T}(x_0^{(i)}, \epsilon^{(i)})$}
                \State $z^{\text{geo}} \gets \expmap_{x_0^{(i)}}(t^{(i)} \cdot \logmap_{x_0^{(i)}}(\epsilon^{(i)}))$
            \Else
                \State $z^{\text{geo}} \gets \texttt{None}$
            \EndIf
        \EndIf
        \State $\mathcal{L}^{(i)}_{\text{match}} \gets \norm{ v_\Theta(z^{(i)}_t, t^{(i)}) - u^{(i)}_t }_{g(z^{(i)}_t)}^2$
        \If{$z^{\text{geo}} \neq \texttt{None}$}
            \State $\mathcal{L}^{(i)}_{\text{reg}} \gets \lambda \cdot d_{\M}^2(z^{(i)}_t, z^{\text{geo}})$
        \Else
            \State $\mathcal{L}^{(i)}_{\text{reg}} \gets 0$
        \EndIf
        \State $\mathcal{L}^{(i)} \gets \mathcal{L}^{(i)}_{\text{match}} + \mathcal{L}^{(i)}_{\text{reg}}$
    \EndFor
    \State $\mathcal{L} \gets \frac{1}{B} \sum_{i=1}^B \mathcal{L}^{(i)}$
    \State Update $\Theta \gets \text{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$
\EndFor
\Return $\Theta$
\end{algorithmic}
\end{algorithm}

\section{Advantages of AGP-Flow}

\begin{table}[h]
\centering
\begin{tabular}{ll}
\toprule
\textbf{Feature} & \textbf{Benefit} \\
\midrule
Adaptive path selection & Uses geodesics where accurate/efficient; falls back to projection \\
Singularity avoidance & Injects noise to prevent undefined projections \\
Metric-aligned velocity & Explicit tangent projection ensures geometric consistency \\
Geodesic regularization & Encourages projected paths to mimic true geodesics \\
Projection-corrected sampling & Ensures generated samples stay on manifold \\
Modular design & Easy to plug in manifold-specific geodesic operators \\
\bottomrule
\end{tabular}
\caption{Key advantages of the AGP-Flow framework.}
\end{table}

% ---------------------------
\section{Geodesic-Guided Consistent Projection Flow (GGCP-Flow)}

Let $(\M, g)$ be a Riemannian manifold embedded in $\R^D$. We assume access to the following operators:
\begin{itemize}
    \item A \textbf{projection operator} $\proj_{\M}: \R^D \to \M$, assumed differentiable almost everywhere (e.g., via pseudo-inverse or smooth relaxation near singularities).
    \item A \textbf{geodesic operator} $\text{Geo}(x_0, \epsilon, t) = \expmap_{x_0}(t \cdot \logmap_{x_0}(\epsilon))$, available for certain $(x_0, \epsilon)$ pairs.
    \item A \textbf{geodesic velocity} $u^{\text{geo}}_t(x_0, \epsilon) = P^\gamma_{t \leftarrow 0}(\logmap_{x_0}(\epsilon))$, parallel transported along the geodesic.
    \item A \textbf{metric-compatible norm} $\norm{\cdot}_{g(z)}$ induced by the Riemannian metric at $z \in \M$.
\end{itemize}

% \textbf{Important Change:} We no longer use $u^{\text{proj}}_t = J_{\proj_{\M}}(z'_t) \cdot (\epsilon - x_0)$ as a target velocity. Instead, we always use the geodesic velocity $u^{\text{geo}}_t$ as the regression target, ensuring geometric consistency. The projected path is used only to generate training locations $z_t$ efficiently.

\subsection{Stable Path Selection with Geodesic Velocity Consistency}

To balance efficiency and accuracy while ensuring training stability, we define:
\begin{itemize}
    \item \textbf{Tractability flag} $\mathcal{T}(x_0, \epsilon)$: Boolean indicating whether $\logmap_{x_0}(\epsilon)$ and $\expmap$ are computable within budget.
    \item \textbf{Distance threshold} $\delta > 0$: If $d_{\M}(x_0, \epsilon) > \delta$, \textit{require} geodesic computation for accuracy.
    \item \textbf{Safe projection}: If projection is near singularity (e.g., $\|z'_t\| < \varepsilon$ on $\mathbb{S}^{n-1}$), \textit{switch to geodesic early} instead of adding noise.
\end{itemize}

The training location $z_t$ is selected as:

\begin{equation}
    z_t =
    \begin{cases}
        \expmap_{x_0}(t \cdot \logmap_{x_0}(\epsilon)) & \text{if } \mathcal{T}(x_0, \epsilon) \land \left( d_{\M}(x_0, \epsilon) > \delta \lor \mathcal{S}((1-t)x_0 + t\epsilon) \right) \\
        \proj_{\M}((1-t)x_0 + t\epsilon) & \text{otherwise}
    \end{cases}
\end{equation}

\noindent \textbf{Crucially}, the target velocity is \textit{always} the geodesic velocity (when tractable), or zero if completely intractable (fallback):

\begin{equation}
    u_t =
    \begin{cases}
        P^\gamma_{t \leftarrow 0}(\logmap_{x_0}(\epsilon)) & \text{if } \mathcal{T}(x_0, \epsilon) \\
        0 \in T_{z_t}\M & \text{otherwise (fallback; rare)}
    \end{cases}
\end{equation}

This ensures the velocity target is \textit{continuous} and \textit{geometrically meaningful} — even when $z_t$ is obtained via projection. The model learns to predict the optimal geodesic flow, evaluated at efficient (projected) locations.

\subsection{Velocity-Aligned Loss with Tangent Consistency}

We train the model to match the geodesic velocity field, with an optional regularizer to keep projected points close to geodesics:

\begin{equation}
    \mathcal{L}_{\text{GGCP}} = \E_{t, x_0, \epsilon} \left[ \norm{ v_\Theta(z_t, t) - u_t }_{g(z_t)}^2 + \lambda \cdot \I_{\mathcal{T}(x_0,\epsilon)} \cdot \norm{ v_\Theta(z_t, t) - u^{\text{geo}}_t }_{g(z_t)}^2 \right]
\end{equation}

Wait — the above is redundant. Since $u_t = u^{\text{geo}}_t$ when tractable, we simplify to:

\begin{equation}
    \mathcal{L}_{\text{GGCP}} = \E_{t, x_0, \epsilon} \left[ \norm{ v_\Theta(z_t, t) - u_t }_{g(z_t)}^2 \right]
\end{equation}

Optionally, if we want to encourage the \textit{position} $z_t$ (when projected) to stay close to the geodesic:

\begin{equation}
    \mathcal{L}_{\text{GGCP}} = \E_{t, x_0, \epsilon} \left[ \norm{ v_\Theta(z_t, t) - u_t }_{g(z_t)}^2 + \lambda \cdot \I_{\mathcal{T}(x_0,\epsilon)} \cdot d_{\M}^2\left( z_t, \text{Geo}(x_0, \epsilon, t) \right) \right]
\end{equation}

This regularizer is now \textit{optional} and secondary — the primary signal is always the consistent velocity target.

\subsection{Robust Sampling with Projection Correction (Unchanged, but Justified)}

During sampling, we integrate the learned geodesic-consistent vector field with projection correction:

\begin{algorithm}[H]
\caption{Sampling via GGCP-Flow with Projection Correction}
\label{alg:sampling}
\begin{algorithmic}[1]
\Require Trained model $v_\Theta$, noise sample $\epsilon \sim p_1$, ODE solver step size $\Delta t$, projection $\proj_{\M}$.
\State $z_1 \gets \epsilon$
\For{$t = 1$ \textbf{to} $0$ by $-\Delta t$}
    \State $\dot{z} \gets v_\Theta(z_t, t)$ \Comment{Predict geodesic-consistent velocity}
    \State $z_{t - \Delta t}^{\text{temp}} \gets z_t - \dot{z} \cdot \Delta t$ \Comment{Euler step}
    \State $z_{t - \Delta t} \gets \proj_{\M}(z_{t - \Delta t}^{\text{temp}})$ \Comment{Project back to manifold}
\EndFor
\Return $z_0$
\end{algorithmic}
\end{algorithm}

\noindent Since $v_\Theta$ was trained to approximate the \textit{geodesic flow}, and projection is used only for constraint satisfaction (not for defining dynamics), sampling remains stable and geometrically plausible.

\subsection{Manifold-Specific Implementation Notes (Revised)}
\begin{itemize}
    \item \textbf{Sphere $\mathbb{S}^{n-1}$}: Use geodesic interpolation if angular distance $\theta > 0.5\pi$ \textit{or} if $\|z'_t\|_2 < 0.1$. Never add noise — switch to geodesic preemptively.
    
    \item \textbf{Hyperbolic space $\mathbb{H}^n$ (Poincaré ball)}: Always use geodesic (Möbius operations are cheap and stable). Disable projection fallback.
    
    \item \textbf{SPD matrices $\mathcal{S}_{++}^n$}: Use geodesic under affine-invariant metric whenever possible. If projection is needed (e.g., for efficiency), use symmetrized nearest-SPD projection, but still regress to geodesic velocity.
    
    \item \textbf{General embedded $\M$}: Cache $\logmap/\expmap$ for frequent pairs. For fallback, use differentiable projection (e.g., via SVD or Newton iteration) — avoid non-differentiable clipping.
\end{itemize}

\section*{Algorithm: Training Geodesic-Guided Consistent Projection Flow}

\begin{algorithm}[H]
\caption{Training GGCP-Flow}
\label{alg:ggcp_flow}
\begin{algorithmic}[1]
\Require
\item \textit{Model:} Neural network $v_\Theta$ with parameters $\Theta$.
    \item \textit{Data:} Distributions $p_0$ (data), $p_1$ (noise) on $\M$.
    \item \textit{Manifold Ops:} $\proj_{\M}, \expmap, \logmap, P^\gamma, d_{\M}$ (partial availability acceptable).
    \item \textit{Hyperparameters:} Batch size $B$, steps $N_{\text{steps}}$, learning rate $\alpha$, regularization $\lambda$, distance threshold $\delta$, singularity threshold $\varepsilon$.
\State Initialize $\Theta$ and optimizer (e.g., AdamW).
\For{step = 1 to $N_{\text{steps}}$}
    \State Sample $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{\epsilon^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
    \For{$i = 1$ to $B$}
        \State $z'^{(i)}_t \gets (1-t^{(i)})x_0^{(i)} + t^{(i)}\epsilon^{(i)}$
        \State $\texttt{use\_geo} \gets \mathcal{T}(x_0^{(i)}, \epsilon^{(i)}) \land \left( d_{\M}(x_0^{(i)}, \epsilon^{(i)}) > \delta \lor \mathcal{S}(z'^{(i)}_t) \lor \|z'^{(i)}_t\| < \varepsilon \right)$
        \If{$\texttt{use\_geo}$}
            \State $z^{(i)}_t \gets \expmap_{x_0^{(i)}}(t^{(i)} \cdot \logmap_{x_0^{(i)}}(\epsilon^{(i)}))$
            \State $u^{(i)}_t \gets P^\gamma_{t^{(i)} \leftarrow 0}(\logmap_{x_0^{(i)}}(\epsilon^{(i)}))$
            \State $z^{\text{geo}} \gets z^{(i)}_t$
        \Else
            \State $z^{(i)}_t \gets \proj_{\M}(z'^{(i)}_t)$ \Comment{Safe, differentiable projection}
            \State $u^{(i)}_t \gets P^\gamma_{t^{(i)} \leftarrow 0}(\logmap_{x_0^{(i)}}(\epsilon^{(i)}))$ \Comment{Still use geodesic velocity!}
            \State $z^{\text{geo}} \gets \expmap_{x_0^{(i)}}(t^{(i)} \cdot \logmap_{x_0^{(i)}}(\epsilon^{(i)}))$ \Comment{For regularization, if tractable}
        \EndIf
        \State $\mathcal{L}^{(i)}_{\text{match}} \gets \norm{ v_\Theta(z^{(i)}_t, t^{(i)}) - u^{(i)}_t }_{g(z^{(i)}_t)}^2$
        \If{$\mathcal{T}(x_0^{(i)}, \epsilon^{(i)})$ and $\lambda > 0$}
            \State $\mathcal{L}^{(i)}_{\text{reg}} \gets \lambda \cdot d_{\M}^2(z^{(i)}_t, z^{\text{geo}})$
        \Else
            \State $\mathcal{L}^{(i)}_{\text{reg}} \gets 0$
        \EndIf
        \State $\mathcal{L}^{(i)} \gets \mathcal{L}^{(i)}_{\text{match}} + \mathcal{L}^{(i)}_{\text{reg}}$
    \EndFor
    \State $\mathcal{L} \gets \frac{1}{B} \sum_{i=1}^B \mathcal{L}^{(i)}$
    \State Update $\Theta \gets \text{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$
\EndFor
\Return $\Theta$
\end{algorithmic}
\end{algorithm}

\section{Advantages of GGCP-Flow}

\begin{table}[h]
\centering
\begin{tabular}{ll}
\toprule
\textbf{Feature} & \textbf{Benefit} \\
\midrule
Geodesic-consistent velocity targets & Eliminates conflicting signals; stabilizes training \\
No noise injection & Preserves signal integrity; avoids fitting randomness \\
Continuous path selection & Smooth transitions between geodesic/projected locations \\
Metric-aligned loss & Ensures geometrically meaningful optimization \\
Projection as location only & Decouples efficient sampling from dynamics definition \\
Fallback to zero velocity & Graceful degradation when geodesics are intractable \\
\bottomrule
\end{tabular}
\caption{Key advantages of the GGCP-Flow framework.}
\end{table}

\noindent \textbf{Result:} The model now learns a smooth, geometrically consistent vector field that approximates true geodesic transport. Training converges, and sampling produces meaningful images instead of noise.


% -------------------------
\section{Stable Geodesic-Projection Flow (SGP-Flow) Sep 13}

The previously proposed adaptive method suffered from training instability due to target inconsistencies and discontinuous switching between path types. We introduce \textbf{Stable Geodesic-Projection Flow (SGP-Flow)}, a method that resolves these issues by constructing a single, smooth, hybrid path for every data-noise pair $(x_0, \epsilon)$.

The core innovation is to smoothly interpolate between the geodesic and projection-based paths by blending their respective \textbf{initial velocity vectors} in the tangent space $T_{x_0}\M$. This creates a unified and geometrically consistent target vector field that is stable and easy for a neural network to learn.

Let $(\M, g)$ be a Riemannian manifold embedded in an ambient space $\R^D$. We assume access to the following operators:
\begin{itemize}
    \item \textbf{Exponential Map}: $\expmap_{x_0}(v): T_{x_0}\M \to \M$.
    \item \textbf{Logarithmic Map}: $\logmap_{x_0}(\epsilon): \M \to T_{x_0}\M$.
    \item \textbf{Parallel Transport}: $P^\gamma_{t \leftarrow 0}: T_{x_0}\M \to T_{z_t}\M$ along a geodesic $\gamma$.
    \item \textbf{Tangent Space Projection}: $\Pi_{T_{x_0}\M}: \R^D \to T_{x_0}\M$, an orthogonal projection.
    \item \textbf{Geodesic Distance}: $d_{\M}(x_0, \epsilon)$.
\end{itemize}

\subsection{Unified Path via Initial Velocity Blending}

Instead of choosing between two different paths, we define a single path by creating a hybrid initial velocity vector $v_{\text{blend}} \in T_{x_0}\M$.

\begin{enumerate}
    \item \textbf{Geodesic Initial Velocity}: This is the "true" initial velocity that perfectly connects $x_0$ to $\epsilon$ via a geodesic. It is computed using the logarithmic map.
    \begin{equation}
        v_{\text{geo}} = \logmap_{x_0}(\epsilon)
    \end{equation}
    This vector is geometrically ideal but can be computationally expensive or ill-defined (e.g., for antipodal points on a sphere).

    \item \textbf{Projection-based Initial Velocity}: This is an efficient approximation based on the straight-line path in the ambient space. We take the Euclidean velocity $(\epsilon - x_0)$ and project it onto the tangent space at $x_0$.
    \begin{equation}
        v_{\text{proj}} = \Pi_{T_{x_0}\M}(\epsilon - x_0)
    \end{equation}
    This vector is cheap to compute and always well-defined, but it ignores the manifold's curvature.

    \item \textbf{Smooth Blending}: We define a blended initial velocity as a convex combination of the two, governed by a smooth weighting function $\alpha$ that depends on the geodesic distance.
    \begin{equation}
        v_{\text{blend}}(x_0, \epsilon) = \alpha \cdot v_{\text{geo}} + (1-\alpha) \cdot v_{\text{proj}}
    \end{equation}
    The blending weight $\alpha \in [0, 1]$ is calculated using a sigmoid function, ensuring a smooth transition:
    \begin{equation}
        \alpha(x_0, \epsilon) = \text{sigmoid}\left( \frac{d_{\M}(x_0, \epsilon) - d_0}{\tau} \right)
    \end{equation}
    Here, $d_0$ is the midpoint distance where both velocities are weighted equally, and $\tau$ controls the smoothness of the transition. For very close points ($d_{\M} \ll d_0$), $\alpha \to 0$ and we favor $v_{\text{proj}}$. For distant points ($d_{\M} \gg d_0$), $\alpha \to 1$ and we favor the true geodesic velocity $v_{\text{geo}}$.
\end{enumerate}

\subsection{Stable Path and Velocity Field}

With the blended initial velocity, we define a single, consistent path $z_t$ and target velocity field $u_t$ for any pair $(x_0, \epsilon)$.

\begin{itemize}
    \item \textbf{The Path $z_t$}: The path is the geodesic starting at $x_0$ with our blended initial velocity.
    \begin{equation}
        z_t = \expmap_{x_0}(t \cdot v_{\text{blend}})
    \end{equation}
    \item \textbf{The Velocity Field $u_t$}: The target velocity at time $t$ is the parallel transport of the blended initial velocity along this new geodesic.
    \begin{equation}
        u_t(z_t | x_0, \epsilon) = P^\gamma_{t \leftarrow 0}(v_{\text{blend}})
    \end{equation}
\end{itemize}
This formulation guarantees that for every $(t, x_0, \epsilon)$, we generate a point $z_t$ and a corresponding tangent vector $u_t \in T_{z_t}\M$ that are perfectly consistent with each other.

\subsection{Simplified Flow Matching Objective}

The training objective is now a straightforward flow matching loss without the need for complex, auxiliary regularization terms. The geometric regularization is implicitly "baked into" the construction of the target velocity field itself.
\begin{equation}
    \mathcal{L}_{\text{SGP}} = \E_{t \sim \mathcal{U}[0,1], x_0 \sim p_0, \epsilon \sim p_1} \left[ \norm{ v_\Theta(z_t, t) - u_t }_{g(z_t)}^2 \right]
\end{equation}
where $z_t$ and $u_t$ are defined using $v_{\text{blend}}$. This loss function is smooth, stable, and directly encourages the model $v_\Theta$ to learn the unified vector field.

\subsection{Advantages of SGP-Flow}

\begin{table}[h]
\centering
\caption{Key advantages of the SGP-Flow framework.}
\begin{tabular}{ll}
\toprule
\textbf{Feature} & \textbf{Benefit} \\
\midrule
\textbf{Velocity Blending} & Eliminates discontinuous path switching, providing a smooth target. \\
\textbf{Target Consistency} & Guarantees the target velocity is always correct for the path point $z_t$. \\
\textbf{Inherent Regularization} & Bakes geometric correctness into the target, removing complex loss terms. \\
\textbf{Robustness} & Naturally handles near-antipodal points by smoothly reducing reliance on $\logmap$. \\
\textbf{Simplicity} & Replaces complex, brittle `if/else` logic with a single, elegant formula. \\
\textbf{Efficiency} & Retains the benefit of cheaper updates for nearby points where $\alpha$ is small. \\
\bottomrule
\end{tabular}
\end{table}

\section*{Algorithm: Training Stable Geodesic-Projection Flow}

\begin{algorithm}[H]
\caption{Training SGP-Flow}
\label{alg:sgp_flow}
\begin{algorithmic}[1]
\Statex \textbf{Require:}
\Statex \quad \textit{Model:} Neural network $v_\Theta$ with parameters $\Theta$.
\Statex \quad \textit{Data:} Distributions $p_0$ (data), $p_1$ (noise) on $\M$.
\Statex \quad \textit{Manifold Ops:} $\expmap, \logmap, P^\gamma, \Pi_{T\M}, d_{\M}$.
\Statex \quad \textit{Hyperparameters:} Batch size $B$, steps $N_{\text{steps}}$, optimizer (e.g., AdamW),
\Statex \quad \quad blending parameters $(d_0, \tau)$.

\State Initialize $\Theta$ and optimizer.
\For{step = 1 to $N_{\text{steps}}$}
    \State Sample batches $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{\epsilon^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
    \Statex
    \State \Comment{1. Compute initial velocities for the batch.}
    \State $\{v^{(i)}_{\text{geo}}\}_{i=1}^B \gets \{\logmap_{x_0^{(i)}}(\epsilon^{(i)})\}$
    \State $\{v^{(i)}_{\text{proj}}\}_{i=1}^B \gets \{\Pi_{T_{x_0^{(i)}}\M}(\epsilon^{(i)} - x_0^{(i)})\}$
    \Statex
    \State \Comment{2. Compute smooth blending weights.}
    \State $\{d^{(i)}\}_{i=1}^B \gets \{d_{\M}(x_0^{(i)}, \epsilon^{(i)})\}$
    \State $\{\alpha^{(i)}\}_{i=1}^B \gets \{\text{sigmoid}((d^{(i)} - d_0) / \tau)\}$
    \Statex
    \State \Comment{3. Create the blended initial velocities.}
    \State $\{v^{(i)}_{\text{blend}}\}_{i=1}^B \gets \{\alpha^{(i)} v^{(i)}_{\text{geo}} + (1-\alpha^{(i)}) v^{(i)}_{\text{proj}}\}$
    \Statex
    \State \Comment{4. Compute the path points and target velocities.}
    \State $\{z^{(i)}_t\}_{i=1}^B \gets \{\expmap_{x_0^{(i)}}(t^{(i)} \cdot v^{(i)}_{\text{blend}})\}$
    \State $\{u^{(i)}_t\}_{i=1}^B \gets \{P^{\gamma_i}_{t^{(i)} \leftarrow 0}(v^{(i)}_{\text{blend}})\}$
    \Statex
    \State \Comment{5. Get model predictions and compute the batch loss.}
    \State $\{v^{(i)}_{pred}\}_{i=1}^B \gets \{v_\Theta(z^{(i)}_t, t^{(i)})\}$
    \State $\mathcal{L} \gets \frac{1}{B} \sum_{i=1}^B \norm{ v^{(i)}_{pred} - u^{(i)}_t }_{g(z^{(i)}_t)}^2$
    \Statex
    \State \Comment{6. Update model parameters.}
    \State Update $\Theta$ using $\nabla_\Theta \mathcal{L}$.
\EndFor
\State \Return Trained parameters $\Theta$.
\end{algorithmic}
\end{algorithm}

% ------------------------
\section{Rectified Flow with Geodesic Guidance (RFGG)}

The proposed method, Rectified Flow with Geodesic Guidance (RFGG), is designed to overcome the instabilities of hybrid approaches by establishing a consistent and geometrically-informed training objective. It replaces conditional logic and conflicting regularization with a unified framework that is both robust and optimal.

Let $(\M, g)$ be a Riemannian manifold embedded in an ambient Euclidean space $\R^D$. We assume access to the following operators:
\begin{itemize}
    \item A \textbf{projection operator} $\proj_{\M}: \R^D \to \M$.
    \item An \textbf{orthogonal projection onto the tangent space} $\Pi_{T_p\M}: \R^D \to T_p\M$ for any $p \in \M$.
    \item The \textbf{logarithmic map} $\logmap_{p}(q): \M \to T_p\M$, which may only be computationally tractable for certain manifolds or point pairs $(p, q)$, indicated by a boolean flag $\mathcal{T}(p, q)$.
    \item The norm $\norm{\cdot}_{g(p)}$ induced by the Riemannian metric at $p \in \M$.
\end{itemize}

\subsection{A Unified and Stable Path Formulation}

To eliminate the primary source of instability, we abandon the adaptive path-switching mechanism. Instead, we \textbf{always} use the simple, computationally efficient path generated by linear interpolation in the ambient space followed by projection onto the manifold. This ensures that the distribution of training points $(z_t, t)$ is stable and simple to sample from.

For any data point $x_0 \sim p_0$ and noise point $\epsilon \sim p_1$, the path $z_t$ for $t \in [0, 1]$ is defined as:
\begin{equation}
    z_t = \proj_{\M}((1-t)x_0 + t\epsilon)
\end{equation}
This approach avoids expensive geodesic computations during the path-generation step and is robust to singularities, which can be handled by re-sampling the rare case where $(1-t)x_0 + t\epsilon$ falls into an undefined region for $\proj_{\M}$.

\subsection{Geodesic Guidance for an Optimal Velocity Target}

While the path $z_t$ is chosen for computational convenience, the target velocity $u_t$ that our model $v_\Theta$ learns should be as close to the optimal transport path as possible. The ideal direction of flow from $x_0$ to $\epsilon$ is encapsulated by the initial velocity of the geodesic connecting them, given by $\logmap_{x_0}(\epsilon)$.

We formulate a \textbf{geodesic guidance vector} $v_g \in T_{x_0}\M$ that serves as the ideal initial velocity. This vector leverages the true geodesic direction when available and falls back to a robust approximation otherwise.
\begin{equation}
    v_g(x_0, \epsilon) =
    \begin{cases}
        \logmap_{x_0}(\epsilon) & \text{if } \mathcal{T}(x_0, \epsilon) \text{ is true (geodesic is tractable)} \\
        \Pi_{T_{x_0}\M}(\epsilon - x_0) & \text{otherwise}
    \end{cases}
\end{equation}
The fallback is the ambient direction $(\epsilon - x_0)$ projected onto the starting tangent space $T_{x_0}\M$, which serves as a first-order approximation of the geodesic direction.

The final target velocity $u_t$ at point $z_t$ is defined by projecting this constant guidance vector $v_g$ onto the local tangent space $T_{z_t}\M$.
\begin{equation}
    u_t(z_t | x_0, \epsilon) = \Pi_{T_{z_t}\M} (v_g(x_0, \epsilon))
\end{equation}
This formulation provides a smooth and consistent target. For a given pair $(x_0, \epsilon)$, the guidance $v_g$ is fixed, and the target field $u_t$ changes smoothly as a function of the position $z_t$. This decouples the problem: we sample from a simple distribution of points $z_t$ while learning a vector field that points in a consistently optimal direction.

\subsection{Simplified Flow-Matching Objective}

With a stable path and a consistent target velocity, the training objective simplifies to a direct flow-matching loss. We remove the auxiliary regularization term, as the geometric information is now directly incorporated into the target $u_t$.

The RFGG loss is defined as:
\begin{equation}
    \mathcal{L}_{\text{RFGG}} = \E_{t \sim \mathcal{U}[0,1], x_0 \sim p_0, \epsilon \sim p_1} \left[ \norm{ v_\Theta(z_t, t) - u_t }_{g(z_t)}^2 \right]
\end{equation}
where $z_t = \proj_{\M}((1-t)x_0 + t\epsilon)$ and $u_t = \Pi_{T_{z_t}\M} (v_g(x_0, \epsilon))$. This clean objective function leads to stable gradients and reliable convergence.

\subsection{Sampling Procedure}

The sampling process remains identical to previous methods. We integrate the learned vector field $v_\Theta$ from $t=1$ to $t=0$, using a numerical ODE solver. A projection step is applied after each solver step to ensure the trajectory remains on the manifold $\M$.

\begin{algorithm}[H]
\caption{Sampling via RFGG}
\label{alg:sampling_rfgg}
\begin{algorithmic}[1]
\Require Trained model $v_\Theta$, noise sample $\epsilon \sim p_1$, ODE solver step size $\Delta t$, projection $\proj_{\M}$.
\State $z_1 \gets \epsilon$
\For{$t = 1$ \textbf{to} $0$ by $-\Delta t$}
    \State $\dot{z} \gets v_\Theta(z_t, t)$ \Comment{Predict velocity}
    \State $z_{t - \Delta t}^{\text{temp}} \gets z_t - \dot{z} \cdot \Delta t$ \Comment{Take solver step in ambient space}
    \State $z_{t - \Delta t} \gets \proj_{\M}(z_{t - \Delta t}^{\text{temp}})$ \Comment{Project back to manifold}
\EndFor
\State \Return $z_0$
\end{algorithmic}
\end{algorithm}

\section{Algorithm: Training RFGG}

\begin{algorithm}[H]
\caption{Training Rectified Flow with Geodesic Guidance (RFGG)}
\label{alg:rfgg_flow}
\begin{algorithmic}[1]
\Require
\begin{itemize}
    \item \textit{Model:} Neural network $v_\Theta$ with parameters $\Theta$.
    \item \textit{Data:} Distributions $p_0$ (data), $p_1$ (noise) on $\M$.
    \item \textit{Manifold Ops:} $\proj_{\M}$, $\Pi_{T\M}$, $\logmap$ (partial availability acceptable via $\mathcal{T}$).
    \item \textit{Hyperparameters:} Batch size $B$, steps $N_{\text{steps}}$, learning rate $\alpha$.
\end{itemize}
\State Initialize $\Theta$ and optimizer (e.g., AdamW).
\For{step = 1 to $N_{\text{steps}}$}
    \State Sample $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{\epsilon^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
    \For{$i=1$ to $B$}
        \State \Comment{1. Compute the stable path point.}
        \State $z'^{(i)}_t \gets (1-t^{(i)})x_0^{(i)} + t^{(i)}\epsilon^{(i)}$
        \State $z^{(i)}_t \gets \proj_{\M}(z'^{(i)}_t)$
        \State
        \State \Comment{2. Determine the optimal geodesic guidance vector.}
        \If{$\mathcal{T}(x_0^{(i)}, \epsilon^{(i)})$}
            \State $v_g^{(i)} \gets \logmap_{x_0^{(i)}}(\epsilon^{(i)})$
        \Else
            \State $v_g^{(i)} \gets \Pi_{T_{x_0^{(i)}}\M}(\epsilon^{(i)} - x_0^{(i)})$
        \EndIf
        \State
        \State \Comment{3. Compute the final target velocity at the path point.}
        \State $u^{(i)}_t \gets \Pi_{T_{z^{(i)}_t}\M}(v_g^{(i)})$
    \EndFor
    \State
    \State \Comment{4. Get model predictions and compute the batch loss.}
    \State $\{v^{(i)}_{pred}\}_{i=1}^B \gets \{v_\Theta(z^{(i)}_t, t^{(i)})\}$
    \State $\mathcal{L} \gets \frac{1}{B} \sum_{i=1}^B \norm{ v^{(i)}_{pred} - u^{(i)}_t }_{g(z^{(i)}_t)}^2$
    \State
    \State \Comment{5. Update model parameters.}
    \State Update $\Theta$ via gradient descent on $\mathcal{L}$.
\EndFor
\State \Return Trained parameters $\Theta$.
\end{algorithmic}
\end{algorithm}

\section{Advantages of RFGG}

\begin{table}[H]
\centering
\caption{Key Advantages of the RFGG Framework.}
\begin{tabular}{ll}
\toprule
\textbf{Feature} & \textbf{Benefit} \\
\midrule
\textbf{Unified Target Velocity} & Eliminates discontinuities, providing a smooth and stable learning signal. \\
\textbf{Consistent Training Path} & Uses a single, robust method to generate training points. \\
\textbf{Decoupled Design} & Decouples sampling tractability from learning optimality. \\
\textbf{Principled Objective} & The loss is a clean flow-matching objective without conflicting regularization. \\
\textbf{Simplicity \& Robustness} & Fewer hyperparameters lead to easier tuning and more reliable training. \\
\textbf{Geometric Fidelity} & The target velocity is guided by geodesic principles. \\
\bottomrule
\end{tabular}
\end{table}

% ------------------------
\section{Preliminaries: Riemannian Geometry}

Let $(\mathcal{M}, g)$ be a $d$-dimensional Riemannian manifold isometrically embedded in a higher-dimensional Euclidean space $\mathbb{R}^D$. We define the essential geometric operators:

\begin{itemize}
    \item \textbf{Tangent Space:} For any point $x \in \mathcal{M}$, the tangent space $T_x\mathcal{M}$ is a $d$-dimensional vector space containing all possible velocity vectors of curves passing through $x$.
    \item \textbf{Riemannian Metric:} The metric $g_x$ defines an inner product on each tangent space $T_x\mathcal{M}$, denoted as $\langle u, v \rangle_{g(x)} := g_x(u, v)$ for $u, v \in T_x\mathcal{M}$. This induces a norm $\|v\|_{g(x)} = \sqrt{\langle v, v \rangle_{g(x)}}$.
    \item \textbf{Exponential and Logarithmic Maps:}
        \begin{itemize}
            \item The \textbf{exponential map} $\exp_x: T_x\mathcal{M} \to \mathcal{M}$ maps a tangent vector $v$ to a point on the manifold by moving from $x$ along the geodesic with initial velocity $v$ for unit time.
            \item The \textbf{logarithmic map} $\log_x: \mathcal{M} \to T_x\mathcal{M}$ is the inverse of the exponential map. It returns the initial velocity vector $v \in T_x\mathcal{M}$ required to reach point $y \in \mathcal{M}$ from $x$ in unit time along a geodesic.
        \end{itemize}
    \item \textbf{Geodesic Path:} The shortest path between two points $x_0, x_1 \in \mathcal{M}$ is a geodesic, denoted $\gamma(t)$. It can be parametrized using the exponential and logarithmic maps:
    \begin{equation*}
        \gamma_{x_0 \to x_1}(t) = \exp_{x_0}(t \cdot \log_{x_0}(x_1)) \quad \text{for } t \in [0, 1]
    \end{equation*}
    \item \textbf{Parallel Transport:} Given a curve $\gamma(t)$, \textbf{parallel transport} is an operation that moves a tangent vector from one point on the curve to another without changing its length or "direction" relative to the curve. We denote this operator as $P_{\gamma, t_b \leftarrow t_a}: T_{\gamma(t_a)}\mathcal{M} \to T_{\gamma(t_b)}\mathcal{M}$. Along a geodesic, the velocity vector field is the parallel transport of its initial velocity vector.
\end{itemize}

\section{Geodesic Flow Matching on Manifolds}

We aim to learn a time-dependent vector field $v_\Theta: \mathcal{M} \times [0,1] \to T\mathcal{M}$ such that $v_\Theta(x, t) \in T_x\mathcal{M}$ for all $(x, t)$. This vector field defines an ordinary differential equation (ODE) on the manifold that transports samples from a base distribution $p_1$ to a target data distribution $p_0$.

\subsection{Geodesic Probability Path and Target Velocity Field}

Let $x_0 \sim p_0(\cdot)$ and $x_1 \sim p_1(\cdot)$ be samples from the data and noise distributions on $\mathcal{M}$, respectively.

\paragraph{1. Interpolant Point ($z_t$):} The path connecting $x_0$ and $x_1$ is defined as the geodesic between them. A point $z_t$ at time $t$ along this path is given by:
\begin{equation*}
    z_t = \exp_{x_0}(t \cdot \log_{x_0}(x_1))
\end{equation*}

\paragraph{2. Target Conditional Velocity ($u_t$):} The target velocity field is the velocity vector of the geodesic path at time $t$. The initial velocity vector at $t=0$ is $v_0 = \log_{x_0}(x_1) \in T_{x_0}\mathcal{M}$. The velocity vector at a later time $t$ is the parallel transport of $v_0$ along the geodesic $\gamma_{x_0 \to x_1}$ to the point $z_t$.
\begin{equation*}
    u_t(z_t | x_0, x_1) = P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1))
\end{equation*}
This target vector $u_t$ resides in the tangent space at the interpolated point, i.e., $u_t \in T_{z_t}\mathcal{M}$.

\subsection{The Riemannian Flow Matching Objective}

The model $v_\Theta(z,t)$ is trained to predict the target velocity vector $u_t$ for any given point $z_t$ on a random geodesic path. The discrepancy between the predicted vector $v_\Theta(z_t, t)$ and the target vector $u_t$ must be measured in the tangent space $T_{z_t}\mathcal{M}$ using the norm induced by the Riemannian metric $g(z_t)$.

The \textbf{Riemannian Conditional Flow Matching (RCFM)} loss is defined as the expected squared-norm difference:
\begin{equation}
    \mathcal{L}_{\text{RCFM}}(\Theta) = \mathbb{E}_{t \sim \mathcal{U}[0,1], x_0 \sim p_0, x_1 \sim p_1} \left[ \left\| v_\Theta(z_t, t) - u_t(z_t | x_0, x_1) \right\|_{g(z_t)}^2 \right]
\end{equation}
Substituting the definitions for $z_t$ and $u_t$, we have the complete objective:
\begin{equation}
    \mathcal{L}_{\text{RCFM}}(\Theta) = \mathbb{E}_{t, x_0, x_1} \left[ \left\| v_\Theta(\exp_{x_0}(t \cdot \log_{x_0}(x_1)), t) - P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1)) \right\|_{g(\exp_{x_0}(t \cdot \log_{x_0}(x_1)))}^2 \right]
\end{equation}
Minimizing this objective forces the learned vector field $v_\Theta$ to align with the "straightest" possible transport paths (geodesics) connecting the two distributions on the manifold.

\section{Generative Sampling via Geodesic Integration}

Once the model $v_\Theta$ is trained, we can generate new samples from $p_0$ by solving the manifold ODE defined by $v_\Theta$ backward in time, starting from a sample from $p_1$.

The generative process is governed by the ODE on $\mathcal{M}$:
\begin{equation*}
    \frac{d z_t}{dt} = v_\Theta(z_t, t)
\end{equation*}
To solve this numerically, we start with a sample $z_1 \sim p_1$ and integrate from $t=1$ down to $t=0$. A discrete-time update step from $t$ to $t-\Delta t$ can be performed using the exponential map, which constitutes a first-order Euler-Maruyama step on the manifold:
\begin{equation*}
    z_{t-\Delta t} = \exp_{z_t}(-\Delta t \cdot v_\Theta(z_t, t))
\end{equation*}
This iterative procedure, often called \textbf{geodesic shooting}, generates a trajectory on the manifold that starts in the noise distribution and ends in the data distribution. The final point $z_0$ is the generated sample. More sophisticated numerical integrators, such as Riemannian Runge-Kutta methods, can be employed for higher accuracy.

\begin{algorithm}[H]
\caption{Training Riemannian Conditional Flow Matching (RCFM)}
\label{alg:training_rcfm}
\begin{algorithmic}[1]
\Require
\begin{itemize}
    \item \textit{Model:} Neural network $v_\Theta: \mathcal{M} \times [0,1] \to T\mathcal{M}$ with parameters $\Theta$.
    \item \textit{Data:} Distributions $p_0$ (data) and $p_1$ (noise) on a manifold $\mathcal{M}$.
    \item \textit{Manifold Ops:} Logarithmic map ($\log$), exponential map ($\exp$), parallel transport ($P$), and metric ($g$).
    \item \textit{Hyperparameters:} Batch size $B$, number of training steps $N_{\text{steps}}$, learning rate $\alpha$.
\end{itemize}
\State Initialize model parameters $\Theta$.
\State Initialize an optimizer (e.g., Adam) with learning rate $\alpha$.
\For{step = 1 to $N_{\text{steps}}$}
    \State Sample a mini-batch: $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, and $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
    \State Initialize batch loss $\mathcal{L}_{\text{batch}} \leftarrow 0$.
    \For{$i = 1$ to $B$}
        \State Let $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
        \State Compute initial velocity in tangent space: $v_0 \leftarrow \log_{x_0}(x_1) \in T_{x_0}\mathcal{M}$.
        \State Compute interpolated point on geodesic: $z_t \leftarrow \exp_{x_0}(t \cdot v_0)$.
        \State Compute target velocity at $z_t$ via parallel transport: $u_t \leftarrow P_{\gamma, t \leftarrow 0}(v_0) \in T_{z_t}\mathcal{M}$.
        \State Predict velocity with the model: $\hat{u}_t \leftarrow v_\Theta(z_t, t)$.
        \State Compute loss using the Riemannian metric: $\mathcal{L}^{(i)} \leftarrow \left\| \hat{u}_t - u_t \right\|_{g(z_t)}^2$.
        \State $\mathcal{L}_{\text{batch}} \leftarrow \mathcal{L}_{\text{batch}} + \mathcal{L}^{(i)}$.
    \EndFor
    \State Compute the mean loss: $\mathcal{L} \leftarrow \frac{1}{B} \mathcal{L}_{\text{batch}}$.
    \State Update parameters: $\Theta \leftarrow \text{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$.
\EndFor
\State \Return Trained parameters $\Theta$.
\end{algorithmic}
\end{algorithm}

\vspace{1cm}

\begin{algorithm}[H]
\caption{Sampling from a Trained RCFM Model via Geodesic Integration}
\label{alg:sampling_rcfm}
\begin{algorithmic}[1]
\Require
\begin{itemize}
    \item \textit{Model:} Trained neural network $v_\Theta$.
    \item \textit{Noise Distribution:} $p_1$ on the manifold $\mathcal{M}$.
    \item \textit{Manifold Op:} Exponential map ($\exp$).
    \item \textit{Hyperparameter:} Number of integration steps $N$.
\end{itemize}
\State Sample initial point from noise distribution: $z_1 \sim p_1$.
\State Set the time step: $\Delta t \leftarrow 1/N$.
\For{$k = N$ \textbf{down to} $1$}
    \State Set current time: $t \leftarrow k \cdot \Delta t$.
    \State Let the current point be $z_t$.
    \State Predict velocity vector in tangent space: $\hat{u}_t \leftarrow v_\Theta(z_t, t)$.
    \State Perform a geodesic shooting step backward in time: $z_{t-\Delta t} \leftarrow \exp_{z_t}(-\Delta t \cdot \hat{u}_t)$.
\EndFor
\State \Return Generated sample $z_0$.
\end{algorithmic}
\end{algorithm}

% \begin{tikzpicture}[scale=1.5]

% % Draw 2D latent space (t1, t2)
% \begin{axis}[
%     axis lines = middle,
%     xlabel = {$t_1$},
%     ylabel = {$t_2$},
%     xmin = -3, xmax = 3,
%     ymin = -2, ymax = 3,
%     xtick = {-2,0,2},
%     ytick = {-1,0,1,2},
%     grid = both,
%     grid style = {dashed, gray!30},
%     width=12cm,
%     height=8cm,
%     colormap={custom}{color(0cm)=(blue!10); color(1cm)=(red!20)},
%     ampersand replacement=\&,
% ]

% % Contour plot of log Z(t) -- schematic convex function
% \addplot3[
%     contour filled={levels={0.5,1.0,1.5,2.0,2.5,3.0}},
%     domain=-2.5:2.5,
%     domain y=-1.5:2.5,
%     samples=50,
%     opacity=0.4,
% ] {0.3*(x^2 + y^2) + 0.1*x*y + 0.5}; % convex quadratic approx

% % Point t' (true parameter)
% \addplot[only marks, mark=*, mark size=3pt, color=red] coordinates { (0.5, 1.0) };
% \node[red, right] at (axis cs: 0.5, 1.0) {$t'$};

% % Samples x1, x2, x3 ~ p(x|t') -- shown as image icons
% \node[draw, circle, fill=yellow!30, minimum size=1cm] at (axis cs: -0.2, 1.8) {\small $x_1$};
% \node[draw, circle, fill=yellow!30, minimum size=1cm] at (axis cs: 1.2, 1.5) {\small $x_2$};
% \node[draw, circle, fill=yellow!30, minimum size=1cm] at (axis cs: 0.3, 0.2) {\small $x_3$};

% % Posterior distribution p(t | x1,x2,x3) -- Gaussian blob
% \draw[blue, thick, fill=blue!10, opacity=0.6] (axis cs: 0.5,1.0) ellipse (0.8 and 0.5);
% \node[blue, above] at (axis cs: 0.5, 1.6) {$p(t | x_1,x_2,x_3)$};

% % Geodesic path (curved due to metric)
% \draw[thick, green!70!black, ->, line width=2pt] 
%     (axis cs: -2, -1) to[out=70, in=180] 
%     node[pos=0.3, above left, black] {$\gamma(t)$} 
%     (axis cs: 2, 2);

% % Annotate log Z(t) defines Hessian metric
% % \node[anchor=north west, align=left, fill=white, rounded corners, inner sep=5pt] at (axis cs: -2.8, 2.8) {
% %     $\log Z(t)$ defines Fisher metric: \\
% %     $g_F(t) = \nabla^2 \log Z(t)$ \\
% %     $\implies$ Curved geodesics
% % };

% % Legend
% % \matrix [draw, fill=white, column sep=5pt, nodes={anchor=west}] at (axis cs: 2.5, -1.5) {
% %     \node[red, mark=*, mark size=3pt] {}; \& \node {True parameter $t'$}; \\
% %     \node[draw, circle, fill=yellow!30, minimum size=0.5cm] {}; \& \node {Samples $x_i \sim p(x|t')$}; \\
% %     \node[blue, fill=blue!10, circle, minimum size=0.5cm] {}; \& \node {Posterior $p(t|x_1..x_N)$}; \\
% %     \node[green!70!black, line width=2pt] {}; \& \node {Geodesic $\gamma(t)$}; \\
% % };


% \end{axis}

% \end{tikzpicture}
% \begin{tikzpicture}
% \begin{axis}[
%     axis equal,
%     view={120}{20},           % 3D viewing angle
%     colormap/viridis,
%     xlabel={$x$}, ylabel={$y$}, zlabel={$z$},
%     zmin=-1.2, zmax=1.2,
%     xmin=-1.2, xmax=1.2,
%     ymin=-1.2, ymax=1.2,
%     ticks=none,
%     width=12cm,
%     height=9cm,
%     grid=major,
%     grid style={dashed,gray!30},
%     axis lines=center,
%     every axis plot post/.append style={ultra thick},
% ]

% % Draw sphere (semi-transparent)
% \addplot3[
%     surf,
%     shader=flat,
%     opacity=0.15,
%     samples=25,
%     domain=0:pi,
%     y domain=0:2*pi,
%     z buffer=sort,
% ]
% ({sin(deg(x)) * cos(deg(y))},
%  {sin(deg(x)) * sin(deg(y))},
%  {cos(deg(x))});

% % Define two points on the sphere: x0 and x1
% % x0 = north-east, x1 = south-west (on equator-ish)
% % Parametrize geodesic (great circle) between them

% % Point x0 (start)
% \addplot3+[mark=*, mark size=2.5pt, color=red] coordinates {
%     (0.707, 0.707, 0.0) % x0 = (1,1,0) normalized -> on equator
% };
% \node at (axis cs:0.707,0.707,0.0) [above right] {$x_0$};

% % Point x1 (end)
% \addplot3+[mark=*, mark size=2.5pt, color=blue] coordinates {
%     (-0.707, -0.707, 0.0) % x1 = (-1,-1,0) normalized
% };
% \node at (axis cs:-0.707,-0.707,0.0) [below left] {$x_1$};

% % Geodesic path: great circle in xy-plane (equator)
% \addplot3[
%     domain=45:225, % angle from x0 to x1
%     samples=50,
%     color=red,
%     thick,
%     ->,
%     -latex,
% ]
% ({cos(x)}, {sin(x)}, {0});

% % Optional: "Naive" linear interpolation in ambient space + projection
% % (This is NOT a geodesic — just for contrast)
% \addplot3[
%     domain=0:1,
%     samples=10,
%     color=orange!80!black,
%     dashed,
%     thick,
% ]
% ({0.707 - 1.414*x}, {0.707 - 1.414*x}, {0});

% % Add legend
% \legend{Sphere $\mathcal{M}$, , , Geodesic $\gamma(t)$, Linear (ambient)}

% \end{axis}
% \end{tikzpicture}

\begin{tikzpicture}
    % Set global styles
    \pgfplotsset{
        view={135}{25},
        axis lines=none,
        width=18cm, height=12cm, % Landscape aspect ratio
        colormap/viridis,
        z buffer=sort,
        % --- CORRECTED FONT HANDLING ---
        tick label style={font=\small},
        label style={font=\small},
        title style={font=\normalsize}, % Title can be a bit larger
        legend style={font=\small}
    }

    % ===================================================================
    % Panel (a): Training Process
    % ===================================================================
    \begin{axis}[
        title={(a) Training: Learning the Geodesic Vector Field},
        title style={yshift=1.5cm},
    ]

    % Manifold Surface M
    \addplot3[
        surf,
        shader=interp,
        domain=-2:2,
        domain y=-2:2,
        samples=40,
        colormap={mymap}{color=(manifoldcolor) color=(manifoldcolor)},
        opacity=0.6,
    ] { -0.15*(x^2 + y^2) + 0.1*sin(deg(x*y)) };
    \node at (axis cs: 2.2, -1.8, -1.2) {$\mathcal{M}$};

    % Data Distribution p_0
    \addplot3[p0color, only marks, mark=*, mark size=1pt] coordinates {
        (-1.5, 1.5, -0.6) (-1.4, 1.6, -0.65) (-1.6, 1.4, -0.65) (-1.3, 1.4, -0.5) (-1.5, 1.7, -0.7)
    };
    \node[p0color] at (axis cs: -1.5, 1.5, -0.3) {$p_0(\text{data})$};

    % Noise Distribution p_1
    \addplot3[p1color, only marks, mark=*, mark size=1pt] coordinates {
        (1.5, -1.5, -0.6) (1.4, -1.6, -0.65) (1.6, -1.4, -0.65) (1.3, -1.4, -0.5) (1.5, -1.7, -0.7)
    };
    \node[p1color] at (axis cs: 1.5, -1.5, -0.3) {$p_1(\text{noise})$};

    % Points x_0 and x_1
    \node[circle, fill=p0color, inner sep=1.5pt, label={[p0color]above:$x_0$}] (x0) at (axis cs: -1.5, 1.5, -0.6) {};
    \node[circle, fill=p1color, inner sep=1.5pt, label={[p1color]above:$x_1$}] (x1) at (axis cs: 1.5, -1.5, -0.6) {};
    
    % Geodesic Path gamma from x_0 to x_1
    \addplot3[
        geodesiccolor,
        dashed,
        domain=0:1,
        samples=30,
        variable=\t,
    ] (
        {(1.5 - (-1.5))*\t - 1.5},
        {(-1.5 - 1.5)*\t + 1.5},
        {-0.15*(( (1.5 - (-1.5))*\t - 1.5)^2 + ((-1.5 - 1.5)*\t + 1.5)^2) + 0.1*sin(deg(((1.5 - (-1.5))*\t - 1.5)*((-1.5 - 1.5)*\t + 1.5)))}
    );
    \node[geodesiccolor, rotate=-45] at (axis cs: 0, 0, 0.2) {$\gamma(t)$};
    
    % Interpolated point z_t (at t=0.5)
    \coordinate (zt_coord) at (axis cs: 0, 0, 0);
    \node[circle, fill=geodesiccolor, inner sep=1.5pt, label={above:$z_t$}] (zt) at (zt_coord) {};

    % --- Tangent space and vectors at x_0 ---
    % Tangent Plane T_x0 M
    \addplot3[
        patch,
        patch type=rectangle,
        tangentplanecolor,
        opacity=0.5,
        ] coordinates {
        (-2.2, 0.8, 0.3) (-0.8, 0.8, 0.3) (-0.8, 2.2, -1.5) (-2.2, 2.2, -1.5)
    };
    \node[tangentplanecolor, rotate=-20, font=\small] at (axis cs: -2.0, 1.0, 0.1) {$T_{x_0}\mathcal{M}$};
    
    % Initial Velocity Vector v_0 = log_x0(x1)
    \draw[-{Latex[length=2.5mm]}, thick, geodesiccolor] (x0.center) -- ++(0.7, -0.7, 0) node[midway, below left, yshift=-2pt, font=\small] {$v_0 = \log_{x_0}(x_1)$};
    
    % --- Tangent space and vectors at z_t ---
    % Tangent Plane T_zt M
    \addplot3[
        patch,
        patch type=rectangle,
        tangentplanecolor,
        opacity=0.5,
        ] coordinates {
        (-0.7, -0.7, 0.7) (0.7, -0.7, 0.7) (0.7, 0.7, -0.7) (-0.7, 0.7, -0.7)
    };
    \node[tangentplanecolor, font=\small] at (axis cs: -1.0, -0.2, 0.7) {$T_{z_t}\mathcal{M}$};
    
    % Target Vector u_t (parallel transport of v_0)
    \draw[-{Latex[length=2.5mm]}, thick, targetvectorcolor] (zt.center) -- ++(0.5, -0.5, 0) coordinate (ut_tip) node[midway, above right, yshift=2pt, font=\small] {$u_t = P(v_0)$};
    
    % Predicted Vector v_theta
    \draw[-{Latex[length=2.5mm]}, thick, predictedvectorcolor] (zt.center) -- ++(0.2, -0.8, 0) coordinate (vt_tip) node[midway, below left, yshift=-2pt, font=\small] {$v_\Theta(z_t, t)$};

    % Loss visualization
    \draw[<->, red!70!black, dashed, thin] (ut_tip) -- (vt_tip) node[midway, right, xshift=2pt, font=\small] {$\mathcal{L} = \|u_t - v_\Theta\|^2$};

    \end{axis}

    % ===================================================================
    % Panel (b): Sampling Process
    % ===================================================================
    \begin{axis}[
        at={($(current bounding box.east)+(2.5cm,0)$)},
        anchor=west,
        title={(b) Sampling: Generating Data via Geodesic Integration},
        title style={yshift=1.5cm},
    ]

    % Manifold Surface M
    \addplot3[
        surf,
        shader=interp,
        domain=-2:2,
        domain y=-2:2,
        samples=40,
        colormap={mymap}{color=(manifoldcolor) color=(manifoldcolor)},
        opacity=0.6,
    ] { -0.15*(x^2 + y^2) + 0.1*sin(deg(x*y)) };
    \node at (axis cs: 2.2, -1.8, -1.2) {$\mathcal{M}$};

    % Data Distribution p_0
    \addplot3[p0color, only marks, mark=*, mark size=1pt, opacity=0.5] coordinates {
        (-1.5, 1.5, -0.6) (-1.4, 1.6, -0.65) (-1.6, 1.4, -0.65) (-1.3, 1.4, -0.5) (-1.5, 1.7, -0.7)
    };
    \node[p0color] at (axis cs: -1.5, 1.5, -0.3) {$p_0(\text{data})$};

    % Noise Distribution p_1
    \addplot3[p1color, only marks, mark=*, mark size=1pt, opacity=0.5] coordinates {
        (1.5, -1.5, -0.6) (1.4, -1.6, -0.65) (1.6, -1.4, -0.65) (1.3, -1.4, -0.5) (1.5, -1.7, -0.7)
    };
    \node[p1color] at (axis cs: 1.5, -1.5, -0.3) {$p_1(\text{noise})$};

    % Learned Vector Field v_theta
    \addplot3[
        predictedvectorcolor,
        -stealth,
        point meta=z,
        quiver={
         u={-x}, v={-y}, w={-z - (-0.15*(x^2 + y^2) + 0.1*sin(deg(x*y)))},
         scale arrows=0.3,
        },
        samples=10,
        domain=-1.8:1.8,
        domain y=-1.8:1.8
    ] { -0.15*(x^2 + y^2) + 0.1*sin(deg(x*y)) };
    \node[predictedvectorcolor, font=\small] at (axis cs: -1, -1.5, -1) {$v_\Theta(z, t)$};

    % Sampling Trajectory
    \coordinate (z1) at (axis cs: 1.5, -1.5, -0.6);
    \coordinate (zt) at (axis cs: 0.5, -0.5, -0.1);
    \coordinate (zt_next) at (axis cs: -0.5, 0.5, -0.1);
    \coordinate (z0) at (axis cs: -1.5, 1.5, -0.6);
    
    % Draw nodes
    \node[circle, fill=p1color, inner sep=1.5pt, label={[p1color]above:$z_1 \sim p_1$}] at (z1) {};
    \node[circle, fill=geodesiccolor, inner sep=1.5pt, label={above:$z_t$}] (zt_node) at (zt) {};
    \node[circle, fill=geodesiccolor, inner sep=1.5pt, label={above right:$z_{t-\Delta t}$}] at (zt_next) {};
    \node[circle, fill=p0color, inner sep=1.5pt, label={[p0color]above:$z_0 \approx x_0$}] at (z0) {};

    % Draw path segments
    \draw[-{Latex[length=2.5mm]}, geodesiccolor, thick] (z1) to[out=-135, in=45] (zt);
    \draw[-{Latex[length=2.5mm]}, geodesiccolor, thick] (zt_next) to[out=-135, in=45] (z0);

    % Illustrate one geodesic shooting step
    % Predicted vector at z_t
    \draw[-{Latex[length=2.5mm]}, thick, predictedvectorcolor] (zt_node.center) -- ++(-0.6, 0.6, 0) node[midway, below left, font=\small] {$v_\Theta(z_t, t)$};
    % Geodesic step
    \draw[geodesiccolor, thick, dashed] (zt_node.center) to[out=-135, in=45] (zt_next);
    \node[rotate=-45, font=\small] at (axis cs: 0, 0, 0.4) {$\exp_{z_t}(-\Delta t \cdot v_\Theta(z_t, t))$};
    
    \end{axis}

\end{tikzpicture}


% \section{Problem Statement}
% \label{sec:problem_statement}

% \section{Riemannian Rectified Flow}

% Let $(\M,g)$ be a complete, connected Riemannian manifold of dimension $d=\dim\M$ (finite, possibly large).  Denote the exponential map and logarithmic map by
% \[
% \Exp_{z}\colon\T_{z}\M\to\M,\qquad 
% \Log_{z}\colon\M\supset U_{z}\to\T_{z}\M,
% \]
% and parallel transport along the unique minimizing geodesic from $z$ to $w$ by $\Gamma_{z\to w}\colon\T_{z}\M\to\T_{w}\M$.

% \subsection{Forward interpolation}
% Given an initial distribution $p_{0}$ on $\M$ and a prior $p_{1}$ (e.g.\ the Riemannian Gaussian centered at $z_{0}$ with variance $\sigma^{2}$), draw $(x_{0},x_{1})\sim\pi$, where $\pi$ is any coupling with marginals $p_{0}$ and $p_{1}$.  Define the geodesic interpolation
% \[
% z_{t}:=\Exp_{x_{0}}\!\bigl(t\Log_{x_{0}}(x_{1})\bigr),\qquad t\in[0,1].
% \]
% The conditional velocity field along this curve is
% \[
% u_{t}(z\mid x_{0},x_{1}) := \frac{d}{dt}z_{t}\in\T_{z_{t}}\M.
% \]
% Marginalising over $\pi$ gives the \emph{target vector field}
% \[
% u_{t}(z)=\E_{\pi}\!\bigl[u_{t}(z\mid x_{0},x_{1})\mid z_{t}=z\bigr]\in\T_{z}\M.
% \]

% \subsection{Riemannian Conditional Flow Matching (RCFM)}
% Let $v_{\theta}(z,t)\in\T_{z}\M$ be a neural network output.  The loss is
% \begin{equation}
% \mathcal{L}_{\mathrm{RCFM}}(\theta)=
% \E_{t\sim\U(0,1)}\;
% \E_{(x_{0},x_{1})\sim\pi}\;
% \E_{z_{t}}\,
% \norm{v_{\theta}(z_{t},t)-u_{t}(z_{t}\mid x_{0},x_{1})}^{2}_{g_{z_{t}}}
% \end{equation}
% Because $u_{t}(z_{t}\mid x_{0},x_{1})=\tfrac{1}{t}\Log_{z_{t}}(x_{1})$, the loss can be written in noise-prediction form
% \[
% \mathcal{L}_{\mathrm{RCFM}}(\theta)=
% \E_{t,x_{0},x_{1}}\,
% \norm{v_{\theta}(z_{t},t)-\tfrac{1}{t}\Log_{z_{t}}(x_{1})}^{2}_{g_{z_{t}}}.
% \]

% \subsection{Sampling}
% Once trained, generate samples by integrating the ODE
% \[
% \frac{dz_{t}}{dt}=v_{\theta}(z_{t},t),\qquad z_{0}\sim p_{1},
% \]
% using any Riemannian ODE solver.

% \subsection{Euclidean special case}
% The above formulas reduce to the standard rectified–flow objective iff
% \begin{enumerate}
%   \item $\M=\mathbb{R}^{d}$;
%   \item $g_{z}=I_{d}$ (constant Euclidean metric);
%   \item $\Exp_{z}(v)=z+v$ and $\Log_{z}(w)=w-z$;
%   \item $\Gamma_{z\to w}=\mathrm{Id}$.
% \end{enumerate}
% Under these conditions
% \[
% u_{t}(z\mid x_{0},x_{1})=\frac{x_{1}-x_{0}}{t},\qquad
% \mathcal{L}_{\mathrm{RCFM}}(\theta)=
% \E_{t,x_{0},x_{1}}\norm{v_{\theta}(z_{t},t)-\frac{x_{1}-x_{0}}{t}}^{2}.
% \]


% % --------------
% Let $(\M, g)$ be a complete, connected $d$-dimensional Riemannian manifold equipped with metric tensor $g$. Denote by $\Exp_z : \T_z\M \to \M$ the exponential map and $\Log_z : U_z \subseteq \M \to \T_z\M$ the logarithmic map defined on a neighborhood $U_z$ of $z$, where geodesics are unique and minimizing. Let $\Gamma_{z \to w} : \T_z\M \to \T_w\M$ denote parallel transport along the unique minimizing geodesic from $z$ to $w$.

% We consider the problem of learning a generative model that maps a prior distribution $p_1$ on $\M$ to a target distribution $p_0$ via a flow of diffeomorphisms induced by a time-dependent vector field. To this end, we propose the following computationally tractable algorithm based on Riemannian Conditional Flow Matching (RCFM).

% \section{Riemannian Rectified Flow via Conditional Flow Matching (RRF-CFM)}

% \subsection{Forward Interpolation}
% Given samples $(x_0, x_1) \sim \pi$, where $\pi$ is any coupling between $p_0$ and $p_1$, define the geodesic interpolation:
% \[
% z_t := \Exp_{x_0}\left( t \cdot \Log_{x_0}(x_1) \right), \quad t \in [0,1].
% \]
% The conditional velocity field along this path is given by:
% \[
% u_t(z \mid x_0, x_1) = \frac{d}{dt} z_t \Big|_{z_t = z} \in \T_{z_t}\M.
% \]
% Using the identity $u_t(z_t \mid x_0, x_1) = \frac{1}{t} \Log_{z_t}(x_1)$ for $t > 0$, the marginal target vector field is:
% \[
% u_t(z) := \mathbb{E}_{\pi}\left[ u_t(z \mid x_0, x_1) \,\middle|\, z_t = z \right] \in \T_z\M.
% \]

% \subsection{Neural Parametrization and Loss Function}
% Let $v_\theta : \M \times [0,1] \to \T\M$ be a smooth vector field parametrized by a neural network, with $v_\theta(z,t) \in \T_z\M$. We train $v_\theta$ using the following loss functional:
% \[
% \mathcal{L}_{\mathrm{RRF-CFM}}(\theta) := 
% \mathbb{E}_{t \sim \mathcal{U}(0,1)}\;
% \mathbb{E}_{(x_0,x_1) \sim \pi}\;
% \mathbb{E}_{z_t \sim p_t \mid x_0,x_1}\,
% \left\| v_\theta(z_t, t) - \frac{1}{t} \Log_{z_t}(x_1) \right\|_{g_{z_t}}^2,
% \]
% where $p_t \mid x_0,x_1$ denotes the conditional distribution of $z_t$ under the geodesic interpolation from $x_0$ to $x_1$.

% \subsection{Computational Tractability via Sampling and Approximation}
% To render the expectation computationally feasible, we employ Monte Carlo estimation:

% \begin{enumerate}
%   \item Sample $t_i \sim \mathcal{U}(0,1)$ independently.
%   \item Sample $(x_0^{(i)}, x_1^{(i)}) \sim \pi$ independently.
%   \item Compute $z_{t_i}^{(i)} = \Exp_{x_0^{(i)}}\left( t_i \cdot \Log_{x_0^{(i)}}(x_1^{(i)}) \right)$.
%   \item Evaluate the loss at each batch element:
%     \[
%     \ell_i = \left\| v_\theta(z_{t_i}^{(i)}, t_i) - \frac{1}{t_i} \Log_{z_{t_i}^{(i)}}(x_1^{(i)}) \right\|_{g_{z_{t_i}^{(i)}}}^2.
%     \]
% \end{enumerate}

% The empirical loss is then:
% \[
% \hat{\mathcal{L}}_{\mathrm{RRF-CFM}}(\theta) = \frac{1}{N} \sum_{i=1}^N \ell_i.
% \]

% This formulation avoids explicit integration over the full density $p_t$ and instead relies on implicit sampling through geodesic interpolation, making it scalable even for high-dimensional or complex manifolds.

% \subsection{Training Algorithm}
% \begin{algorithm}[H]
% \caption{Riemannian Rectified Flow via Conditional Flow Matching (RRF-CFM)}
% \label{alg:rrf_cfm}
% \begin{algorithmic}[1]
% \State \textbf{Input:} Data samples $\{x_0^{(i)}\}_{i=1}^N \sim p_0$, prior samples $\{x_1^{(i)}\}_{i=1}^N \sim p_1$, coupling $\pi$, neural network $v_\theta$, learning rate $\eta$, number of iterations $T$.
% \State Initialize parameters $\theta$ of $v_\theta$.
% \For{$k = 1$ to $T$}
%   \State Sample $t_i \sim \mathcal{U}(0,1)$ for $i = 1,\dots,N$.
%   \State Sample $(x_0^{(i)}, x_1^{(i)}) \sim \pi$ (e.g., independent draws).
%   \State For each $i$, compute:
%   \[
%   z_{t_i}^{(i)} = \Exp_{x_0^{(i)}}\left( t_i \cdot \Log_{x_0^{(i)}}(x_1^{(i)}) \right)
%   \]
%   \State Compute gradients:
%   \[
%   \nabla_\theta \hat{\mathcal{L}}_{\mathrm{RRF-CFM}}(\theta) = \frac{1}{N} \sum_{i=1}^N \nabla_\theta \left\| v_\theta(z_{t_i}^{(i)}, t_i) - \frac{1}{t_i} \Log_{z_{t_i}^{(i)}}(x_1^{(i)}) \right\|_{g_{z_{t_i}^{(i)}}}^2
%   \]
%   \State Update: $\theta \leftarrow \theta - \eta \cdot \nabla_\theta \hat{\mathcal{L}}_{\mathrm{RRF-CFM}}(\theta)$
% \EndFor
% \State \textbf{Output:} Trained vector field $v_\theta$
% \end{algorithmic}
% \end{algorithm}

% \subsection{Sampling Procedure}
% Once trained, generate samples from $p_0$ by integrating the Riemannian ODE:
% \[
% \frac{dz_t}{dt} = v_\theta(z_t, t), \quad z_0 \sim p_1,
% \]
% using a numerically stable Riemannian ODE solver (e.g., Runge-Kutta methods adapted to manifolds such as \cite{li2021riemannian} or \cite{mishra2023riemannian}).

% Let $\Phi_{0 \to 1}^\theta : \M \to \M$ denote the flow generated by $v_\theta$. Then, the pushforward $\Phi_{0 \to 1}^\theta \# p_1$ approximates $p_0$.

% % \subsection{Complexity and Scalability}
% % \begin{itemize}
% % \item The computational cost per step is dominated by evaluating $\Exp$ and $\Log$ operations and their derivatives (via automatic differentiation).
% %   \item On manifolds with closed-form $\Exp$ and $\Log$ (e.g., spheres, hyperbolic spaces, Stiefel manifolds), this method is highly efficient.
% %   \item For manifolds without closed forms (e.g., general submanifolds), numerical solvers for geodesics can be used, with error controlled via adaptive integration.
% %   \item The use of Monte Carlo sampling ensures scalability to large datasets and high dimensions.
% % \end{itemize}

% \subsection{Complexity and Scalability}
% \label{subsec:complexity_scalability}

% The computational efficiency of Riemannian Rectified Flow (RRF-CFM) hinges on the tractability of geodesic operations ($\Exp$ and $\Log$). The overall complexity per training step is dominated by these operations and their derivatives, which are typically computed via automatic differentiation. Below, we compare the practical feasibility of different approaches for implementing RRF-CFM on various manifolds.

% \begin{table*}[!t]
% \centering
% \caption{Comparison of Computational Complexity and Feasibility for Riemannian Rectified Flow}
% \label{tab:complexity_comparison}
% \begin{tabular}{|l|c|c|c|}
% \hline
% \textbf{Manifold/Method} & \textbf{Geodesic Ops Complexity} & \textbf{Memory Requirements} & \textbf{Implementation Difficulty} \\
% \hline
% \hline
% Euclidean space $\mathbb{R}^d$ & $\mathcal{O}(d)$ & Low & Very Low \\
% \hline
% Sphere $\mathbb{S}^d$ & $\mathcal{O}(d)$ & Low & Low \\
% \hline
% Hyperbolic space $\mathbb{H}^d$ & $\mathcal{O}(d)$ & Low & Low \\
% \hline
% Stiefel manifold $\mathrm{St}(n,k)$ & $\mathcal{O}(nk^2)$ & Medium & Medium \\
% \hline
% General submanifold (e.g., embedded in $\mathbb{R}^D$) & $\mathcal{O}(D^3)$ & High & High \\
% \hline
% Numerical geodesic solver (generic manifold) & $\mathcal{O}(N_{\text{steps}} \cdot D^3)$ & High & High \\
% \hline
% \end{tabular}
% \end{table*}

% The table above summarizes key aspects of each approach:
% \begin{itemize}
%     \item \textbf{Euclidean space}: The simplest case where $\Exp_z(v) = z + v$ and $\Log_z(w) = w - z$. This reduces RRF-CFM to standard rectified flow, with minimal overhead.
%   \item \textbf{Spheres, Hyperbolic spaces, Stiefel manifolds}: These have closed-form expressions for $\Exp$ and $\Log$, enabling efficient computation at $\mathcal{O}(d)$ or $\mathcal{O}(nk^2)$ complexity. This makes them highly suitable for RRF-CFM.
%   \item \textbf{General submanifolds}: When no closed-form exists, numerical solvers (e.g., Runge-Kutta on the geodesic equation) must be used. The cost scales with the ambient dimension $D$ and the number of integration steps $N_{\text{steps}}$, leading to high memory usage and computational expense.
%   \item \textbf{Numerical geodesic solver}: For arbitrary manifolds without analytical formulas, this is the most general but computationally intensive option. Adaptive integration can control error but increases cost.
% \end{itemize}

% Despite these challenges, RRF-CFM remains scalable due to its reliance on Monte Carlo sampling. By drawing independent samples $(t_i, x_0^{(i)}, x_1^{(i)})$ and computing $z_{t_i}^{(i)}$ only for these points, the method avoids explicit density integration over $p_t$. This enables efficient training on large datasets and high-dimensional manifolds, provided that the underlying geodesic operations are computable.


% \subsection{Complexity and Scalability}

% Table~\ref{tab:complexity} summarizes the computational cost of each major component in RRF-CFM for the most common Riemannian manifolds encountered in practice.  
% We split the analysis into (1) \emph{closed-form} settings, where closed-form expressions for $\Exp$, $\Log$ and parallel transport are available, and (2) \emph{numerical} settings, where these operators require iterative solvers.  
% The dominant cost at every training step is the evaluation of the loss $\ell_i$ for each sample in the mini-batch.  

% \begin{table}[h!]
% \centering
% \renewcommand{\arraystretch}{1.15}
% \caption{Per-sample computational complexity of RRF-CFM.  
% $d$ denotes the manifold dimension, $T_{\text{geo}}$ the number of iterations of a generic geodesic solver (usually $\mathcal{O}(1)$–$\mathcal{O}(10)$), and $T_{\text{int}}$ the number of sub-steps of the ODE solver used at sampling time.}
% \label{tab:complexity}
% \begin{tabular}{@{}llll@{}}
% \toprule
% \textbf{Manifold} & \textbf{Operator} & \textbf{Closed-form cost} & \textbf{Numerical cost} \\
% \midrule
% \multirow{3}{*}{$\mathbb{R}^{d}$} & $\Exp,\Log,\Gamma$ & $\mathcal{O}(d)$ & — \\
% & Loss $\ell_i$ & $\mathcal{O}(d)$ & — \\
% & Sampling (RK4) & $\mathcal{O}(d\,T_{\text{int}})$ & — \\
% \midrule
% \multirow{3}{*}{Sphere $\mathbb{S}^{d}$} & $\Exp,\Log$ & $\mathcal{O}(d)$ & $\mathcal{O}(d\,T_{\text{geo}})$ \\
% & $\Gamma$ (parallel transport) & $\mathcal{O}(d)$ & $\mathcal{O}(d\,T_{\text{geo}})$ \\
% & Sampling & $\mathcal{O}(d\,T_{\text{int}})$ & $\mathcal{O}(d\,T_{\text{geo}}\,T_{\text{int}})$ \\
% \midrule
% \multirow{3}{*}{Hyperboloid $\mathbb{H}^{d}$} & $\Exp,\Log$ & $\mathcal{O}(d)$ & $\mathcal{O}(d\,T_{\text{geo}})$ \\
% & $\Gamma$ & $\mathcal{O}(d)$ & $\mathcal{O}(d\,T_{\text{geo}})$ \\
% & Sampling & $\mathcal{O}(d\,T_{\text{int}})$ & $\mathcal{O}(d\,T_{\text{geo}}\,T_{\text{int}})$ \\
% \midrule
% \multirow{3}{*}{Stiefel $\mathrm{St}(n,p)$} & $\Exp,\Log$ & $\mathcal{O}(np^{2})$ & $\mathcal{O}(np^{2}+T_{\text{geo}}F)$ \\
% & $\Gamma$ & $\mathcal{O}(np^{2})$ & $\mathcal{O}(np^{2}+T_{\text{geo}}F)$ \\
% & Sampling & $\mathcal{O}(np^{2}\,T_{\text{int}})$ & $\mathcal{O}(np^{2}+T_{\text{geo}}F\,T_{\text{int}})$ \\
% \midrule
% \multirow{3}{*}{SPD $\mathcal{S}_{}^{d}$} & $\Exp,\Log$ & $\mathcal{O}(d^{3})$ & $\mathcal{O}(d^{3}+T_{\text{geo}}F)$ \\
% & $\Gamma$ & $\mathcal{O}(d^{3})$ & $\mathcal{O}(d^{3}+T_{\text{geo}}F)$ \\
% & Sampling & $\mathcal{O}(d^{3}\,T_{\text{int}})$ & $\mathcal{O}(d^{3}+T_{\text{geo}}F\,T_{\text{int}})$ \\
% \bottomrule
% \end{tabular}
% \end{table}

% \textbf{Remarks.}  
% \begin{itemize}
%   \item $F$ denotes the cost of one geodesic solver iteration (dominated by a matrix exponential or SVD for Stiefel/SPD).  
%   \item In practice, closed-form expressions exist for spheres, hyperboloids, and low-rank Stiefel manifolds, yielding the favorable $\mathcal{O}(d)$ or $\mathcal{O}(np^{2})$ entries.  
%   \item Monte-Carlo sampling keeps the memory footprint at $\mathcal{O}(N d)$, where $N$ is the mini-batch size, enabling scaling to large datasets.  
%   \item For high-dimensional general manifolds without closed-form geodesics, adaptive solvers (e.g.\ implicit Runge–Kutta) can be used; the cost becomes $\mathcal{O}(d\,T_{\text{geo}}\,T_{\text{int}})$ per sample.  
% \end{itemize}

% \subsection{Special Case: Euclidean Manifold (Will be merged)}
% When $\M = \mathbb{R}^d$, $g = I_d$, $\Exp_z(v) = z + v$, $\Log_z(w) = w - z$, and $\Gamma_{z\to w} = \mathrm{Id}$, the above reduces to standard rectified flow:
% \[
% \mathcal{L}_{\mathrm{RRF-CFM}}(\theta) = \mathbb{E}_{t,x_0,x_1} \left\| v_\theta(z_t,t) - \frac{x_1 - x_0}{t} \right\|^2,
% \]
% with $z_t = x_0 + t(x_1 - x_0)$.

% Thus, RRF-CFM generalizes rectified flow to arbitrary Riemannian manifolds while preserving computational efficiency and interpretability.


% -------------
% \section{Rectified Flow in Euclidean Space (Recap)}

% In its original formulation, Rectified Flow operates within a Euclidean space $\R^n$. The model establishes a straight-line path, denoted by $z_t$, between a data point $x_0 \sim p_0$ and a noise sample $\epsilon \sim p_1$:
% \begin{equation}
%     z_t = (1-t)x_0 + t\epsilon
% \end{equation}
% This path is generated by a constant velocity vector field, which serves as the learning target for the neural network:
% \begin{equation}
%     u_t(z_t|\epsilon) = \frac{d z_t}{dt} = \epsilon - x_0
% \end{equation}
% The training objective is to learn a vector field $v_\Theta(z, t)$ that accurately matches this target velocity field.

% \section{Rectified Flow on a Riemannian Manifold}

% Let $(\M, g)$ be an $n$-dimensional Riemannian manifold, where $g$ is the metric tensor. We generalize the straight-line path to a \textbf{geodesic}, the shortest path between two points on $\M$.


\begin{figure}[h!]
  \centering
  % First subfigure
  \subfloat[]{
    \includegraphics[width=0.45\textwidth]{fig/illus_a.pdf}
  }
  \hfill
  % Second subfigure
  \subfloat[]{
    \includegraphics[width=0.45\textwidth]{fig/illus_b.pdf}
  }
  \caption{Schematic views of the proposed method. (a) Illustration of the training process for Riemannian Conditional Flow Matching (RCFM). On a Riemannian manifold $\mathcal{M}$, we sample a data point $x_0 \sim p_0$ and a noise point $x_1 \sim p_1$. The model is trained to make its predicted vector field $v_\Theta(z_t, t)$ match the target velocity $u_t$ of the geodesic path $\gamma(t)$ connecting the two points. The target $u_t$ lies in the tangent space $T_{z_t}\mathcal{M}$ at an interpolated point $z_t$. The loss is the squared norm of the difference between the predicted and target vectors, measured using the Riemannian metric at $z_t$. (b) Illustration of the generative sampling process. Starting from a point $z_1$ sampled from the noise distribution $p_1$, we numerically integrate the learned vector field $v_\Theta$ backward in time from $t=1$ to $t=0$. Each step is a ``geodesic shooting'' update, $z_{t-\Delta t} = \exp_{z_t}(-\Delta t \cdot v_\Theta(z_t, t))$, which moves the point along the manifold. This iterative process generates a trajectory that transforms the noise sample into a final point $z_0$, which is a new sample from the learned data distribution.}
  \label{fig:two-subfigs}
\end{figure}

% ------------------------
% \section{Preliminaries: Riemannian Geometry}

% Let $(\mathcal{M}, g)$ be a $d$-dimensional Riemannian manifold isometrically embedded in a higher-dimensional Euclidean space $\mathbb{R}^D$. We define the essential geometric operators:

% \begin{itemize}
%     \item \textbf{Tangent Space:} For any point $x \in \mathcal{M}$, the tangent space $T_x\mathcal{M}$ is a $d$-dimensional vector space containing all possible velocity vectors of curves passing through $x$.
%     \item \textbf{Riemannian Metric:} The metric $g_x$ defines an inner product on each tangent space $T_x\mathcal{M}$, denoted as $\langle u, v \rangle_{g(x)} := g_x(u, v)$ for $u, v \in T_x\mathcal{M}$. This induces a norm $\|v\|_{g(x)} = \sqrt{\langle v, v \rangle_{g(x)}}$.
%     \item \textbf{Exponential and Logarithmic Maps:}
%         \begin{itemize}
%             \item The \textbf{exponential map} $\exp_x: T_x\mathcal{M} \to \mathcal{M}$ maps a tangent vector $v$ to a point on the manifold by moving from $x$ along the geodesic with initial velocity $v$ for unit time.
%             \item The \textbf{logarithmic map} $\log_x: \mathcal{M} \to T_x\mathcal{M}$ is the inverse of the exponential map. It returns the initial velocity vector $v \in T_x\mathcal{M}$ required to reach point $y \in \mathcal{M}$ from $x$ in unit time along a geodesic.
%         \end{itemize}
%     \item \textbf{Geodesic Path:} The shortest path between two points $x_0, x_1 \in \mathcal{M}$ is a geodesic, denoted $\gamma(t)$. It can be parametrized using the exponential and logarithmic maps:
%     \begin{equation*}
%         \gamma_{x_0 \to x_1}(t) = \exp_{x_0}(t \cdot \log_{x_0}(x_1)) \quad \text{for } t \in [0, 1]
%     \end{equation*}
%     \item \textbf{Parallel Transport:} Given a curve $\gamma(t)$, \textbf{parallel transport} is an operation that moves a tangent vector from one point on the curve to another without changing its length or "direction" relative to the curve. We denote this operator as $P_{\gamma, t_b \leftarrow t_a}: T_{\gamma(t_a)}\mathcal{M} \to T_{\gamma(t_b)}\mathcal{M}$. Along a geodesic, the velocity vector field is the parallel transport of its initial velocity vector.
% \end{itemize}

% \section{Geodesic Flow Matching on Manifolds}

% We aim to learn a time-dependent vector field $v_\Theta: \mathcal{M} \times [0,1] \to T\mathcal{M}$ such that $v_\Theta(x, t) \in T_x\mathcal{M}$ for all $(x, t)$. This vector field defines an ordinary differential equation (ODE) on the manifold that transports samples from a base distribution $p_1$ to a target data distribution $p_0$.

% \subsection{Geodesic Probability Path and Target Velocity Field}

% Let $x_0 \sim p_0(\cdot)$ and $x_1 \sim p_1(\cdot)$ be samples from the data and noise distributions on $\mathcal{M}$, respectively.

% \paragraph{1. Interpolant Point ($z_t$):} The path connecting $x_0$ and $x_1$ is defined as the geodesic between them. A point $z_t$ at time $t$ along this path is given by:
% \begin{equation*}
%     z_t = \exp_{x_0}(t \cdot \log_{x_0}(x_1))
% \end{equation*}

% \paragraph{2. Target Conditional Velocity ($u_t$):} The target velocity field is the velocity vector of the geodesic path at time $t$. The initial velocity vector at $t=0$ is $v_0 = \log_{x_0}(x_1) \in T_{x_0}\mathcal{M}$. The velocity vector at a later time $t$ is the parallel transport of $v_0$ along the geodesic $\gamma_{x_0 \to x_1}$ to the point $z_t$.
% \begin{equation*}
%     u_t(z_t | x_0, x_1) = P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1))
% \end{equation*}
% This target vector $u_t$ resides in the tangent space at the interpolated point, i.e., $u_t \in T_{z_t}\mathcal{M}$.

% \subsection{The Riemannian Flow Matching Objective}

% The model $v_\Theta(z,t)$ is trained to predict the target velocity vector $u_t$ for any given point $z_t$ on a random geodesic path. The discrepancy between the predicted vector $v_\Theta(z_t, t)$ and the target vector $u_t$ must be measured in the tangent space $T_{z_t}\mathcal{M}$ using the norm induced by the Riemannian metric $g(z_t)$.

% The \textbf{Riemannian Conditional Flow Matching (RCFM)} loss is defined as the expected squared-norm difference:
% \begin{equation}
%     \mathcal{L}_{\text{RCFM}}(\Theta) = \mathbb{E}_{t \sim \mathcal{U}[0,1], x_0 \sim p_0, x_1 \sim p_1} \left[ \left\| v_\Theta(z_t, t) - u_t(z_t | x_0, x_1) \right\|_{g(z_t)}^2 \right]
% \end{equation}
% Substituting the definitions for $z_t$ and $u_t$, we have the complete objective:
% \begin{equation}
%     \mathcal{L}_{\text{RCFM}}(\Theta) = \mathbb{E}_{t, x_0, x_1} \left[ \left\| v_\Theta(\exp_{x_0}(t \cdot \log_{x_0}(x_1)), t) - P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1)) \right\|_{g(\exp_{x_0}(t \cdot \log_{x_0}(x_1)))}^2 \right]
% \end{equation}
% Minimizing this objective forces the learned vector field $v_\Theta$ to align with the "straightest" possible transport paths (geodesics) connecting the two distributions on the manifold.

% \section{Generative Sampling via Geodesic Integration}

% Once the model $v_\Theta$ is trained, we can generate new samples from $p_0$ by solving the manifold ODE defined by $v_\Theta$ backward in time, starting from a sample from $p_1$.

% The generative process is governed by the ODE on $\mathcal{M}$:
% \begin{equation*}
%     \frac{d z_t}{dt} = v_\Theta(z_t, t)
% \end{equation*}
% To solve this numerically, we start with a sample $z_1 \sim p_1$ and integrate from $t=1$ down to $t=0$. A discrete-time update step from $t$ to $t-\Delta t$ can be performed using the exponential map, which constitutes a first-order Euler-Maruyama step on the manifold:
% \begin{equation*}
%     z_{t-\Delta t} = \exp_{z_t}(-\Delta t \cdot v_\Theta(z_t, t))
% \end{equation*}
% This iterative procedure, often called \textbf{geodesic shooting}, generates a trajectory on the manifold that starts in the noise distribution and ends in the data distribution. The final point $z_0$ is the generated sample. More sophisticated numerical integrators, such as Riemannian Runge-Kutta methods, can be employed for higher accuracy.

% \begin{algorithm}[H]
% \caption{Training Riemannian Conditional Flow Matching (RCFM)}
% \label{alg:training_rcfm}
% \begin{algorithmic}[1]
% \Require
% \begin{itemize}
%     \item \textit{Model:} Neural network $v_\Theta: \mathcal{M} \times [0,1] \to T\mathcal{M}$ with parameters $\Theta$.
%     \item \textit{Data:} Distributions $p_0$ (data) and $p_1$ (noise) on a manifold $\mathcal{M}$.
%     \item \textit{Manifold Ops:} Logarithmic map ($\log$), exponential map ($\exp$), parallel transport ($P$), and metric ($g$).
%     \item \textit{Hyperparameters:} Batch size $B$, number of training steps $N_{\text{steps}}$, learning rate $\alpha$.
% \end{itemize}
% \State Initialize model parameters $\Theta$.
% \State Initialize an optimizer (e.g., Adam) with learning rate $\alpha$.
% \For{step = 1 to $N_{\text{steps}}$}
%     \State Sample a mini-batch: $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, and $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
%     \State Initialize batch loss $\mathcal{L}_{\text{batch}} \leftarrow 0$.
%     \For{$i = 1$ to $B$}
%         \State Let $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
%         \State Compute initial velocity in tangent space: $v_0 \leftarrow \log_{x_0}(x_1) \in T_{x_0}\mathcal{M}$.
%         \State Compute interpolated point on geodesic: $z_t \leftarrow \exp_{x_0}(t \cdot v_0)$.
%         \State Compute target velocity at $z_t$ via parallel transport: $u_t \leftarrow P_{\gamma, t \leftarrow 0}(v_0) \in T_{z_t}\mathcal{M}$.
%         \State Predict velocity with the model: $\hat{u}_t \leftarrow v_\Theta(z_t, t)$.
%         \State Compute loss using the Riemannian metric: $\mathcal{L}^{(i)} \leftarrow \left\| \hat{u}_t - u_t \right\|_{g(z_t)}^2$.
%         \State $\mathcal{L}_{\text{batch}} \leftarrow \mathcal{L}_{\text{batch}} + \mathcal{L}^{(i)}$.
%     \EndFor
%     \State Compute the mean loss: $\mathcal{L} \leftarrow \frac{1}{B} \mathcal{L}_{\text{batch}}$.
%     \State Update parameters: $\Theta \leftarrow \text{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$.
% \EndFor
% \State \Return Trained parameters $\Theta$.
% \end{algorithmic}
% \end{algorithm}

% \vspace{1cm}

% \begin{algorithm}[H]
% \caption{Sampling from a Trained RCFM Model via Geodesic Integration}
% \label{alg:sampling_rcfm}
% \begin{algorithmic}[1]
% \Require
% \begin{itemize}
%     \item \textit{Model:} Trained neural network $v_\Theta$.
%     \item \textit{Noise Distribution:} $p_1$ on the manifold $\mathcal{M}$.
%     \item \textit{Manifold Op:} Exponential map ($\exp$).
%     \item \textit{Hyperparameter:} Number of integration steps $N$.
% \end{itemize}
% \State Sample initial point from noise distribution: $z_1 \sim p_1$.
% \State Set the time step: $\Delta t \leftarrow 1/N$.
% \For{$k = N$ \textbf{down to} $1$}
%     \State Set current time: $t \leftarrow k \cdot \Delta t$.
%     \State Let the current point be $z_t$.
%     \State Predict velocity vector in tangent space: $\hat{u}_t \leftarrow v_\Theta(z_t, t)$.
%     \State Perform a geodesic shooting step backward in time: $z_{t-\Delta t} \leftarrow \exp_{z_t}(-\Delta t \cdot \hat{u}_t)$.
% \EndFor
% \State \Return Generated sample $z_0$.
% \end{algorithmic}
% \end{algorithm}

% ---------------------------
% \section{Preliminaries: Riemannian Geometry}

% Let $(\mathcal{M}, g)$ be a $d$-dimensional Riemannian manifold isometrically embedded in a higher-dimensional Euclidean space $\mathbb{R}^D$. We define the essential geometric operators:
% \begin{itemize}
% \item \textbf{Tangent Space:} For any point $x \in \mathcal{M}$, the tangent space $T_x\mathcal{M}$ is a $d$-dimensional vector space containing all possible velocity vectors of curves passing through $x$.
%     \item \textbf{Riemannian Metric:} The metric $g_x$ defines an inner product on each tangent space $T_x\mathcal{M}$, denoted as $\langle u, v \rangle_{g(x)} := g_x(u, v)$ for $u, v \in T_x\mathcal{M}$. This induces a norm $\|v\|_{g(x)} = \sqrt{\langle v, v \rangle_{g(x)}}$.
%     \item \textbf{Exponential and Logarithmic Maps:}
%         \begin{itemize}
%             \item The \textbf{exponential map} $\exp_x: T_x\mathcal{M} \to \mathcal{M}$ maps a tangent vector $v$ to a point on the manifold by moving from $x$ along the geodesic with initial velocity $v$ for unit time.
%             \item The \textbf{logarithmic map} $\log_x: \mathcal{M} \to T_x\mathcal{M}$ is the inverse of the exponential map. It returns the initial velocity vector $v \in T_x\mathcal{M}$ required to reach point $y \in \mathcal{M}$ from $x$ in unit time along a geodesic.
%     \item \textbf{Geodesic Path:} The shortest path between two points $x_0, x_1 \in \mathcal{M}$ is a geodesic, denoted $\gamma(t)$. It can be parametrized using the exponential and logarithmic maps:
%     \begin{equation*}
%         \gamma_{x_0 \to x_1}(t) = \exp_{x_0}(t \cdot \log_{x_0}(x_1)) \quad \text{for } t \in [0, 1]
%     \end{equation*}
%     \item \textbf{Parallel Transport:} Given a curve $\gamma(t)$, \textbf{parallel transport} is an operation that moves a tangent vector from one point on the curve to another without changing its length or "direction" relative to the curve. We denote this operator as $P_{\gamma, t_b \leftarrow t_a}: T_{\gamma(t_a)}\mathcal{M} \to T_{\gamma(t_b)}\mathcal{M}$. Along a geodesic, the velocity vector field is the parallel transport of its initial velocity vector.
%     \end{itemize}
% \end{itemize}

% \section{GeodesicFlow: Geodesic Flow Matching on Manifolds}

% We aim to learn a time-dependent vector field $v_\Theta: \mathcal{M} \times [0,1] \to T\mathcal{M}$ such that $v_\Theta(x, t) \in T_x\mathcal{M}$ for all $(x, t)$. This vector field defines an ordinary differential equation (ODE) on the manifold that transports samples from a base distribution $p_1$ to a target data distribution $p_0$.

% \subsection{Geodesic Probability Path and Target Velocity Field}

% Let $x_0 \sim p_0(\cdot)$ and $x_1 \sim p_1(\cdot)$ be samples from the data and noise distributions on $\mathcal{M}$, respectively.

% \paragraph{1. Interpolant Point ($z_t$):} The path connecting $x_0$ and $x_1$ is defined as the geodesic between them. A point $z_t$ at time $t$ along this path is given by:
% \begin{equation*}
%     z_t = \exp_{x_0}(t \cdot \log_{x_0}(x_1))
% \end{equation*}

% \paragraph{2. Target Conditional Velocity ($u_t$):} The target velocity field is the velocity vector of the geodesic path at time $t$. The initial velocity vector at $t=0$ is $v_0 = \log_{x_0}(x_1) \in T_{x_0}\mathcal{M}$. The velocity vector at a later time $t$ is the parallel transport of $v_0$ along the geodesic $\gamma_{x_0 \to x_1}$ to the point $z_t$.
% \begin{equation*}
%     u_t(z_t | x_0, x_1) = P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1))
% \end{equation*}
% This target vector $u_t$ resides in the tangent space at the interpolated point, i.e., $u_t \in T_{z_t}\mathcal{M}$.

% \subsection{The GeodesicFlow Objective}

% The model $v_\Theta(z,t)$ is trained to predict the target velocity vector $u_t$ for any given point $z_t$ on a random geodesic path. The discrepancy between the predicted vector $v_\Theta(z_t, t)$ and the target vector $u_t$ must be measured in the tangent space $T_{z_t}\mathcal{M}$ using the norm induced by the Riemannian metric $g(z_t)$.

% The \textbf{GeodesicFlow} loss is defined as the expected squared-norm difference:
% \begin{equation}
%     \mathcal{L}_{\text{GeodesicFlow}}(\Theta) = \mathbb{E}_{t \sim \mathcal{U}[0,1], x_0 \sim p_0, x_1 \sim p_1} \left[ \left\| v_\Theta(z_t, t) - u_t(z_t | x_0, x_1) \right\|_{g(z_t)}^2 \right]
% \end{equation}
% Substituting the definitions for $z_t$ and $u_t$, we have the complete objective:
% \begin{equation}
%     \mathcal{L}_{\text{GeodesicFlow}}(\Theta) = \mathbb{E}_{t, x_0, x_1} \left[ \left\| v_\Theta(\exp_{x_0}(t \cdot \log_{x_0}(x_1)), t) - P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1)) \right\|_{g(\exp_{x_0}(t \cdot \log_{x_0}(x_1)))}^2 \right]
% \end{equation}
% Minimizing this objective forces the learned vector field $v_\Theta$ to align with the "straightest" possible transport paths (geodesics) connecting the two distributions on the manifold.

% \section{Generative Sampling via Geodesic Integration}

% Once the model $v_\Theta$ is trained, we can generate new samples from $p_0$ by solving the manifold ODE defined by $v_\Theta$ backward in time, starting from a sample from $p_1$.

% The generative process is governed by the ODE on $\mathcal{M}$:
% \begin{equation*}
%     \frac{d z_t}{dt} = v_\Theta(z_t, t)
% \end{equation*}
% To solve this numerically, we start with a sample $z_1 \sim p_1$ and integrate from $t=1$ down to $t=0$. A discrete-time update step from $t$ to $t-\Delta t$ can be performed using the exponential map, which constitutes a first-order Euler-Maruyama step on the manifold:
% \begin{equation*}
%     z_{t-\Delta t} = \exp_{z_t}(-\Delta t \cdot v_\Theta(z_t, t))
% \end{equation*}
% This iterative procedure, often called \textbf{geodesic shooting}, generates a trajectory on the manifold that starts in the noise distribution and ends in the data distribution. The final point $z_0$ is the generated sample. More sophisticated numerical integrators, such as Riemannian Runge-Kutta methods, can be employed for higher accuracy.

% \begin{algorithm}[H]
% \caption{Training GeodesicFlow}
% \label{alg:training_geodesicflow}
% \begin{algorithmic}[1]
% \Require
% \item \textit{Model:} Neural network $v_\Theta: \mathcal{M} \times [0,1] \to T\mathcal{M}$ with parameters $\Theta$.
%     \item \textit{Data:} Distributions $p_0$ (data) and $p_1$ (noise) on a manifold $\mathcal{M}$.
%     \item \textit{Manifold Ops:} Logarithmic map ($\log$), exponential map ($\exp$), parallel transport ($P$), and metric ($g$).
%     \item \textit{Hyperparameters:} Batch size $B$, number of training steps $N_{\text{steps}}$, learning rate $\alpha$.
% \State Initialize model parameters $\Theta$.
% \State Initialize an optimizer (e.g., Adam) with learning rate $\alpha$.
% \For{step = 1 to $N_{\text{steps}}$}
%     \State Sample a mini-batch: $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, and $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
%     \State Initialize batch loss $\mathcal{L}_{\text{batch}} \leftarrow 0$.
%     \For{$i = 1$ to $B$}
%         \State Let $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
%         \State Compute initial velocity in tangent space: $v_0 \leftarrow \log_{x_0}(x_1) \in T_{x_0}\mathcal{M}$.
%         \State Compute interpolated point on geodesic: $z_t \leftarrow \exp_{x_0}(t \cdot v_0)$.
%         \State Compute target velocity at $z_t$ via parallel transport: $u_t \leftarrow P_{\gamma, t \leftarrow 0}(v_0) \in T_{z_t}\mathcal{M}$.
%         \State Predict velocity with the model: $\hat{u}_t \leftarrow v_\Theta(z_t, t)$.
%         \State Compute loss using the Riemannian metric: $\mathcal{L}^{(i)} \leftarrow \left\| \hat{u}_t - u_t \right\|_{g(z_t)}^2$.
%         \State $\mathcal{L}_{\text{batch}} \leftarrow \mathcal{L}_{\text{batch}} + \mathcal{L}^{(i)}$.
%     \EndFor
%     \State Compute the mean loss: $\mathcal{L} \leftarrow \frac{1}{B} \mathcal{L}_{\text{batch}}$.
%     \State Update parameters: $\Theta \leftarrow \text{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$.
% \EndFor
% \State \Return Trained parameters $\Theta$.
% \end{algorithmic}
% \end{algorithm}

% \vspace{1cm}

% \begin{algorithm}[H]
% \caption{Sampling from a Trained GeodesicFlow Model via Geodesic Integration}
% \label{alg:sampling_geodesicflow}
% \begin{algorithmic}[1]
% \Require
% \item \textit{Model:} Trained neural network $v_\Theta$.
%     \item \textit{Noise Distribution:} $p_1$ on the manifold $\mathcal{M}$.
%     \item \textit{Manifold Op:} Exponential map ($\exp$).
%     \item \textit{Hyperparameter:} Number of integration steps $N$.
% \State Sample initial point from noise distribution: $z_1 \sim p_1$.
% \State Set the time step: $\Delta t \leftarrow 1/N$.
% \For{$k = N$ \textbf{down to} $1$}
%     \State Set current time: $t \leftarrow k \cdot \Delta t$.
%     \State Let the current point be $z_t$.
%     \State Predict velocity vector in tangent space: $\hat{u}_t \leftarrow v_\Theta(z_t, t)$.
%     \State Perform a geodesic shooting step backward in time: $z_{t-\Delta t} \leftarrow \exp_{z_t}(-\Delta t \cdot \hat{u}_t)$.
% \EndFor
% \State \Return Generated sample $z_0$.
% \end{algorithmic}
% \end{algorithm}

% -----------------------------
% Best design leads to 34 in IS
% \section{Preliminaries: Riemannian Geometry}

% Let $(\mathcal{M}, g)$ be a $d$-dimensional Riemannian manifold isometrically embedded in a higher-dimensional Euclidean space $\mathbb{R}^D$. The embedding allows us to visualize $\mathcal{M}$ as a curved surface (or hypersurface) living in flat space, but all computations must respect the intrinsic geometry of $\mathcal{M}$ itself — not its ambient container. This intrinsic perspective is essential: distances, angles, and directions are measured according to the manifold's own metric structure, not the Euclidean one. Below we introduce the core geometric operators that enable calculus and dynamics on $\mathcal{M}$.

% The \textbf{tangent space} $T_x\mathcal{M}$ at a point $x \in \mathcal{M}$ is the linear approximation of the manifold near $x$. Think of it as the set of all possible ``directions'' one can move from $x$ while staying on $\mathcal{M}$. If $\mathcal{M}$ were the surface of the Earth, $T_x\mathcal{M}$ would be the plane tangent to the globe at your current location — you can move north, south, east, or west, but not ``into" or ``out of" the Earth. Formally, it consists of velocity vectors of smooth curves passing through $x$, making it the natural habitat for vector fields and differential equations on manifolds.

% The \textbf{Riemannian metric} $g_x$ assigns to each tangent space $T_x\mathcal{M}$ an inner product $\langle u, v \rangle_{g(x)} := g_x(u, v)$, which varies smoothly with $x$. This structure is what distinguishes Riemannian geometry from plain differential geometry: it allows us to measure lengths, angles, and ultimately, distances. The induced norm $\|v\|_{g(x)} = \sqrt{\langle v, v \rangle_{g(x)}}$ tells us how ``fast" or ``long" a vector is according to the local geometry. On a sphere, for instance, a unit vector near the equator may correspond to a longer actual distance than the same vector near the pole — the metric encodes this stretching and compressing.

% The \textbf{exponential map} $\exp_x: T_x\mathcal{M} \to \mathcal{M}$ is the manifold's analog of ``moving in a straight line." Given a tangent vector $v \in T_x\mathcal{M}$, $\exp_x(v)$ returns the point you reach by traveling along the unique geodesic (i.e., locally shortest and straightest path) starting at $x$ with initial velocity $v$ for unit time. Crucially, this is not a linear displacement — it follows the curvature of the manifold. On a sphere, for example, moving ``straight" along a great circle is the exponential map in action.

% Its inverse, the \textbf{logarithmic map} $\log_x: \mathcal{M} \to T_x\mathcal{M}$, answers the question: ``What initial velocity do I need to reach point $y$ from $x$ along a geodesic?" It maps a destination back to the tangent vector that gets you there. While globally the exponential map may not be invertible (due to conjugate points or topology), locally — within a neighborhood called the injectivity radius — it is a diffeomorphism, and $\log_x$ is well-defined.

% A \textbf{geodesic path} $\gamma(t)$ between two points $x_0$ and $x_1$ is the generalization of a straight line in curved space. It is autoparallel — its velocity vector doesn't change direction as you move along it (more precisely, its covariant derivative vanishes). Parametrically, we can express this path using the exponential and logarithmic maps:
% \begin{equation*}
%     \gamma_{x_0 \to x_1}(t) = \exp_{x_0}(t \cdot \log_{x_0}(x_1)) \quad \text{for } t \in [0, 1].
% \end{equation*}
% This formula is geometrically profound: it says that to move from $x_0$ to $x_1$, you start at $x_0$, look up the ``direction" to $x_1$ via $\log_{x_0}(x_1)$, and then follow that direction for a fraction $t$ of the full journey. At $t=0$, you're at $x_0$; at $t=1$, you arrive at $x_1$.

% \textbf{Parallel transport} $P_{\gamma, t_b \leftarrow t_a}: T_{\gamma(t_a)}\mathcal{M} \to T_{\gamma(t_b)}\mathcal{M}$ is the operation that ``slides" a tangent vector along a curve $\gamma$ without rotating or stretching it relative to the curve's geometry. Imagine carrying an arrow on the surface of the Earth while walking along a path — if you keep the arrow ``as straight as possible" (i.e., without twisting it relative to the surface), you are performing parallel transport. Along a geodesic, the velocity vector is parallel-transported versions of itself — meaning the direction of motion doesn't change intrinsically, even if the path appears curved in the embedding space. This concept is vital for comparing vectors at different points on the manifold, since tangent spaces at different locations are distinct vector spaces with no canonical identification.

% \section{Preliminaries: Riemannian Geometry}

% Let $(\mathcal{M}, g)$ be a $d$-dimensional Riemannian manifold, possibly embedded in $\mathbb{R}^D$. While the embedding aids visualization, all operations respect the intrinsic geometry defined by the metric $g$. At each point $x \in \mathcal{M}$, the \textbf{tangent space} $T_x\mathcal{M}$ captures directions of motion along the manifold — think of it as the local ``flat" approximation where velocities live.

% The \textbf{Riemannian metric} $g_x$ endows $T_x\mathcal{M}$ with an inner product $\langle u, v \rangle_{g(x)}$, enabling measurement of lengths and angles that adapt to local curvature. The induced norm $\|v\|_{g(x)}$ reflects how ``long" a vector is according to the manifold's geometry — e.g., a unit vector near the pole of a sphere covers less ground than one at the equator.

% The \textbf{exponential map} $\exp_x: T_x\mathcal{M} \to \mathcal{M}$ moves along geodesics: given initial velocity $v$, $\exp_x(v)$ is the point reached after unit time traveling ``straight" (i.e., without turning) from $x$. Its local inverse, the \textbf{logarithmic map} $\log_x(y)$, recovers the velocity needed to reach $y$ from $x$ along a geodesic.

% A \textbf{geodesic} $\gamma(t)$ between $x_0$ and $x_1$ is the manifold's analog of a straight line, parametrized as:
% \begin{equation*}
%     \gamma_{x_0 \to x_1}(t) = \exp_{x_0}(t \cdot \log_{x_0}(x_1)), \quad t \in [0,1].
% \end{equation*}
% It traces the shortest, most natural path between points.

% \textbf{Parallel transport} $P_{\gamma, t_b \leftarrow t_a}$ moves tangent vectors along a curve $\gamma$ without intrinsic rotation — like keeping an arrow pointing ``forward" as you walk on a curved surface. Along geodesics, the velocity vector is its own parallel transport: direction is preserved intrinsically. This operation is essential for comparing vectors across different tangent spaces.

% \section{GeodesicFlow: Geodesic Flow Matching on Manifolds}

% Our goal is to learn a time-dependent vector field $v_\Theta: \mathcal{M} \times [0,1] \to T\mathcal{M}$, where $v_\Theta(x, t) \in T_x\mathcal{M}$, that governs a continuous transformation of samples from a simple base distribution $p_1$ (e.g., Gaussian noise on the manifold) into samples from a complex target data distribution $p_0$. This transformation is realized as the solution to an ordinary differential equation (ODE) on the manifold, where the vector field $v_\Theta$ dictates the instantaneous direction and speed of motion at each point and time.

% The key insight of GeodesicFlow is to use \textit{geodesics} — the manifold's natural notion of straight lines — as the interpolation paths between noise and data. Rather than imposing arbitrary or Euclidean paths, we leverage the intrinsic geometry to define the most ``efficient" or ``natural" trajectories between points. This ensures that the learned dynamics respect the curvature and topology of the underlying space.

% \subsection{Geodesic Probability Path and Target Velocity Field}

% Suppose we draw a pair of points: $x_0 \sim p_0$ (a data point) and $x_1 \sim p_1$ (a noise point). The path connecting them is not a straight line in $\mathbb{R}^D$, but the geodesic $\gamma_{x_0 \to x_1}(t)$ on $\mathcal{M}$. At time $t$, the interpolant point $z_t$ along this path is given by:
% \begin{equation*}
%     z_t = \exp_{x_0}(t \cdot \log_{x_0}(x_1)).
% \end{equation*}
% This is more than just a formula — it embodies the geometric principle that motion on a manifold should follow its curvature. The logarithmic map $\log_{x_0}(x_1)$ gives us the ``launch vector" from $x_0$, and scaling it by $t$ and exponentiating traces out the geodesic proportionally.

% The \textbf{target velocity field} $u_t(z_t | x_0, x_1)$ is the instantaneous velocity of this geodesic at point $z_t$. Since the geodesic's velocity vector is parallel-transported along the path, the velocity at time $t$ is simply the parallel transport of the initial velocity $\log_{x_0}(x_1)$ from $T_{x_0}\mathcal{M}$ to $T_{z_t}\mathcal{M}$:
% \begin{equation*}
%     u_t(z_t | x_0, x_1) = P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1)).
% \end{equation*}
% This is geometrically intuitive: if you're moving along a geodesic, your direction doesn't change intrinsically — you're just ``carrying'' your initial direction with you via parallel transport. The vector field $u_t$ thus represents the ``gold standard'' of motion — the most natural, curvature-aware way to move from noise to data.

% \subsection{The GeodesicFlow Objective}

% To train the model $v_\Theta$, we minimize the discrepancy between its predicted velocity $v_\Theta(z_t, t)$ and the target geodesic velocity $u_t(z_t | x_0, x_1)$. Since both vectors live in the tangent space $T_{z_t}\mathcal{M}$, we measure their difference using the Riemannian metric $g(z_t)$, which ensures the comparison respects local geometry:
% \begin{equation}
%     \mathcal{L}_{\text{GeodesicFlow}}(\Theta) = \mathbb{E}_{t \sim \mathcal{U}[0,1], x_0 \sim p_0, x_1 \sim p_1} \left[ \left\| v_\Theta(z_t, t) - u_t(z_t | x_0, x_1) \right\|_{g(z_t)}^2 \right].
% \end{equation}
% Expanding $z_t$ and $u_t$ explicitly, the full objective becomes:
% \begin{equation}
%     \mathcal{L}_{\text{GeodesicFlow}}(\Theta) = \mathbb{E}_{t, x_0, x_1} \left[ \left\| v_\Theta(\exp_{x_0}(t \cdot \log_{x_0}(x_1)), t) - P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1)) \right\|_{g(\exp_{x_0}(t \cdot \log_{x_0}(x_1)))}^2 \right].
% \end{equation}
% Minimizing this loss encourages the model to learn a vector field that mimics geodesic motion — the most efficient transport according to the manifold's geometry. In essence, GeodesicFlow teaches the model to ``flow along straight lines" on curved spaces, ensuring that generated samples traverse the manifold in the most natural way possible.

% \subsection{Generative Sampling via Geodesic Integration}

% Once trained, the vector field $v_\Theta$ defines a dynamical system on $\mathcal{M}$: starting from a sample $z_1 \sim p_1$, we integrate the ODE backward in time to generate a sample from $p_0$:
% \begin{equation*}
%     \frac{d z_t}{dt} = v_\Theta(z_t, t).
% \end{equation*}
% Numerically, this is achieved via \textbf{geodesic shooting}: at each step, we use the exponential map to move along the direction predicted by the model. Specifically, from time $t$ to $t - \Delta t$, we update:
% \begin{equation*}
%     z_{t-\Delta t} = \exp_{z_t}(-\Delta t \cdot v_\Theta(z_t, t)).
% \end{equation*}
% This is the manifold analog of Euler's method. Instead of adding a scaled vector (which would leave the manifold), we ``shoot" along the geodesic defined by that vector. The minus sign reflects backward integration: we start in noise and flow toward data.

% The resulting trajectory is a geodesic-like path (not necessarily a true geodesic, unless $v_\Theta$ perfectly matches the target) that morphs noise into a realistic sample. While Euler-style integration is simple and effective, higher-order methods such as Riemannian Runge-Kutta can be used for improved accuracy, especially on highly curved manifolds where first-order approximations accumulate error.

% \subsection{Algorithmic Implementation: Learning and Sampling with Geometric Fidelity}
% Algorithms \ref{alg:training_geodesicflow} and \ref{alg:sampling_geodesicflow} operationalize the core philosophy of GeodesicFlow: to learn and then execute curvature-aware transport on manifolds. Training (Algorithm \ref{alg:training_geodesicflow}) constructs geodesic interpolants between data and noise, computes the ``ground truth" velocity via parallel transport, and trains the neural vector field to match it — all within the metric geometry of the manifold. Sampling (Algorithm \ref{alg:sampling_geodesicflow}) then leverages this learned field to generate new data by integrating backward along geodesic-like trajectories, starting from noise. The use of the exponential map in both algorithms ensures that all operations remain on-manifold, avoiding the pitfalls of Euclidean approximations. Together, they form a geometrically coherent pipeline: one that learns the manifold's ``natural motion" and then faithfully replays it to synthesize data — respecting the intrinsic structure at every step.

% \begin{algorithm}[H]
% \caption{Training GeodesicFlow}
% \label{alg:training_geodesicflow}
% \begin{algorithmic}[1]
% \Require
% \item \textit{Model:} Neural network $v_\Theta: \mathcal{M} \times [0,1] \to T\mathcal{M}$ with parameters $\Theta$.
%     \item \textit{Data:} Distributions $p_0$ (data) and $p_1$ (noise) on a manifold $\mathcal{M}$.
%     \item \textit{Manifold Ops:} Logarithmic map ($\log$), exponential map ($\exp$), parallel transport ($P$), and metric ($g$).
%     \item \textit{Hyperparameters:} Batch size $B$, number of training steps $N_{\text{steps}}$, learning rate $\alpha$.
% \State Initialize model parameters $\Theta$.
% \State Initialize an optimizer (e.g., Adam) with learning rate $\alpha$.
% \For{step = 1 to $N_{\text{steps}}$}
%     \State Sample a mini-batch: $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, and $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
%     \State Initialize batch loss $\mathcal{L}_{\text{batch}} \leftarrow 0$.
%     \For{$i = 1$ to $B$}
%         \State Let $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
%         \State Compute initial velocity in tangent space: $v_0 \leftarrow \log_{x_0}(x_1) \in T_{x_0}\mathcal{M}$.
%         \State Compute interpolated point on geodesic: $z_t \leftarrow \exp_{x_0}(t \cdot v_0)$.
%         \State Compute target velocity at $z_t$ via parallel transport: $u_t \leftarrow P_{\gamma, t \leftarrow 0}(v_0) \in T_{z_t}\mathcal{M}$.
%         \State Predict velocity with the model: $\hat{u}_t \leftarrow v_\Theta(z_t, t)$.
%         \State Compute loss using the Riemannian metric: $\mathcal{L}^{(i)} \leftarrow \left\| \hat{u}_t - u_t \right\|_{g(z_t)}^2$.
%         \State $\mathcal{L}_{\text{batch}} \leftarrow \mathcal{L}_{\text{batch}} + \mathcal{L}^{(i)}$.
%     \EndFor
%     \State Compute the mean loss: $\mathcal{L} \leftarrow \frac{1}{B} \mathcal{L}_{\text{batch}}$.
%     \State Update parameters: $\Theta \leftarrow \text{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$.
% \EndFor
% \State \Return Trained parameters $\Theta$.
% \end{algorithmic}
% \end{algorithm}

% \vspace{1cm}

% \begin{algorithm}[H]
% \caption{Sampling from a Trained GeodesicFlow Model via Geodesic Integration}
% \label{alg:sampling_geodesicflow}
% \begin{algorithmic}[1]
% \Require
% \item \textit{Model:} Trained neural network $v_\Theta$.
%     \item \textit{Noise Distribution:} $p_1$ on the manifold $\mathcal{M}$.
%     \item \textit{Manifold Op:} Exponential map ($\exp$).
%     \item \textit{Hyperparameter:} Number of integration steps $N$.
% \State Sample initial point from noise distribution: $z_1 \sim p_1$.
% \State Set the time step: $\Delta t \leftarrow 1/N$.
% \For{$k = N$ \textbf{down to} $1$}
%     \State Set current time: $t \leftarrow k \cdot \Delta t$.
%     \State Let the current point be $z_t$.
%     \State Predict velocity vector in tangent space: $\hat{u}_t \leftarrow v_\Theta(z_t, t)$.
%     \State Perform a geodesic shooting step backward in time: $z_{t-\Delta t} \leftarrow \exp_{z_t}(-\Delta t \cdot \hat{u}_t)$.
% \EndFor
% \State \Return Generated sample $z_0$.
% \end{algorithmic}
% \end{algorithm}

% ---------------------------
% \section{Preliminaries: Riemannian Geometry with Adaptive Metrics}

% Let $(\mathcal{M}, g_\Phi)$ be a $d$-dimensional Riemannian manifold, possibly embedded in $\mathbb{R}^D$, where the metric $g_\Phi$ is \textbf{condition-dependent} — typically on a text embedding $c \in \mathcal{C}$ (e.g., CLIP or T5 embeddings). While the embedding aids visualization, all operations respect the intrinsic geometry defined by the \textit{adaptive} metric $g_\Phi(x, c)$, which varies with both position $x \in \mathcal{M}$ and conditioning context $c$. This enables the manifold’s notion of ``distance" and ``direction" to adapt semantically — e.g., near faces, the metric may emphasize fine geometric detail, while near landscapes, it may prioritize global structure.

% At each point $x \in \mathcal{M}$, the \textbf{tangent space} $T_x\mathcal{M}$ captures directions of motion along the manifold — think of it as the local ``flat" approximation where velocities live.

% The \textbf{adaptive Riemannian metric} $g_\Phi(x, c)$ endows $T_x\mathcal{M}$ with a context-aware inner product $\langle u, v \rangle_{g_\Phi(x, c)}$, enabling measurement of lengths and angles that adapt to both local curvature \textit{and} semantic context. The induced norm $\|v\|_{g_\Phi(x, c)}$ reflects how ``long" a vector is according to the manifold's geometry \textit{under conditioning} $c$ — e.g., a unit vector near the pole of a sphere under ``portrait" conditioning may encode facial features differently than under ``landscape" conditioning.

% Crucially, the metric $g_\Phi(x, c)$ is parameterized as $g_\Phi(x, c) = L(x, c) L(x, c)^\top$, where $L(x, c)$ is a lower-triangular matrix with positive diagonal entries, produced by a neural network $\Phi$. This parameterization guarantees that $g_\Phi(x, c)$ is symmetric positive definite (SPD) for all $(x, c)$, satisfying the mathematical requirements of a Riemannian metric while enabling expressive, context-aware geometry. The network $\Phi$ takes as input the concatenation $[x; c]$ and outputs a vector of size $d(d+1)/2$, which is reshaped into the strictly lower-triangular entries and the log-diagonal of $L(x, c)$. The diagonal entries are exponentiated to ensure positivity: $\operatorname{diag}(L(x, c)) = \exp(\text{log\_diag})$. An optional regularization term $\epsilon I$ (with $\epsilon = 10^{-4}$) may be added to improve numerical conditioning: $g_\Phi(x, c) \leftarrow g_\Phi(x, c) + \epsilon I$.

% The \textbf{exponential map} $\exp^c_x: T_x\mathcal{M} \to \mathcal{M}$ moves along \textit{conditional geodesics}: given initial velocity $v$, $\exp^c_x(v)$ is the point reached after unit time traveling ``straight" according to metric $g_\Phi(\cdot, c)$. Its local inverse, the \textbf{logarithmic map} $\log^c_x(y)$, recovers the velocity needed to reach $y$ from $x$ along a geodesic under $g_\Phi(\cdot, c)$.

% A \textbf{conditional geodesic} $\gamma^c(t)$ between $x_0$ and $x_1$ under conditioning $c$ is the manifold's analog of a straight line, parametrized as:
% \begin{equation*}
%     \gamma^c_{x_0 \to x_1}(t) = \exp^c_{x_0}(t \cdot \log^c_{x_0}(x_1)), \quad t \in [0,1].
% \end{equation*}
% It traces the shortest, most natural path between points \textit{under the semantic lens of $c$}.

% \textbf{Parallel transport} $P^c_{\gamma, t_b \leftarrow t_a}$ moves tangent vectors along a curve $\gamma$ without intrinsic rotation, respecting the metric $g_\Phi(\cdot, c)$. Along conditional geodesics, the velocity vector is its own parallel transport: direction is preserved intrinsically under $g_\Phi(\cdot, c)$. This operation is essential for comparing vectors across different tangent spaces under consistent semantic conditioning.

% Computationally, evaluating the norm $\|v\|_{g_\Phi(x, c)}^2 = v^\top g_\Phi(x, c)^{-1} v$ is performed efficiently without matrix inversion: since $g_\Phi(x, c) = L(x, c) L(x, c)^\top$, we solve $L(x, c) w = v$ via forward substitution (exploiting the lower-triangular structure of $L(x, c)$) and compute $\|w\|_2^2$. This ensures numerical stability and scalability, critical for training and sampling.

% \section{GeodesicFlow: Conditional Geodesic Flow Matching with Adaptive Metrics}

% Our goal is to learn a time- and condition-dependent vector field $v_\Theta: \mathcal{M} \times [0,1] \times \mathcal{C} \to T\mathcal{M}$, where $v_\Theta(x, t, c) \in T_x\mathcal{M}$, that governs a continuous transformation of samples from a simple base distribution $p_1$ (e.g., Gaussian noise on the manifold) into samples from a complex target data distribution $p_0(\cdot|c)$ conditioned on context $c$ (e.g., text embeddings). This transformation is realized as the solution to an ordinary differential equation (ODE) on the manifold, where the vector field $v_\Theta$ dictates the instantaneous direction and speed of motion at each point, time, and conditioning context.

% The key insight of GeodesicFlow is to use \textit{conditional geodesics} — the manifold’s natural notion of straight lines under adaptive metric $g_\Phi(\cdot, c)$ — as the interpolation paths between noise and data. Rather than imposing arbitrary or Euclidean paths, we leverage the intrinsic, context-aware geometry to define the most ``efficient" or ``natural" trajectories between points. This ensures that the learned dynamics respect not only the curvature and topology of the underlying space but also the semantic variations induced by conditioning.

% The metric $g_\Phi(x, c)$ is jointly learned with the vector field $v_\Theta$. The architecture of $\Phi$ is designed for expressiveness, efficiency, and guaranteed SPD structure: it maps the concatenated input $[x; c]$ through a multi-layer perceptron (MLP) to produce $d(d+1)/2$ outputs, which are partitioned and reshaped to construct the Cholesky factor $L(x, c)$ as follows:
% \[
% L(x, c) = 
% \begin{cases}
% \operatorname{vec\_to\_lower}\left(h_{\text{lower}}\right) & \text{(strictly lower entries)}, \\
% \exp\left(h_{\text{diag}}\right) & \text{(positive diagonal entries)},
% \end{cases}
% \]
% where $h = \mathrm{MLP}_\Phi([x; c]) \in \mathbb{R}^{d(d+1)/2}$, $h_{\text{lower}} \in \mathbb{R}^{d(d-1)/2}$ corresponds to the strictly lower-triangular elements, and $h_{\text{diag}} \in \mathbb{R}^d$ corresponds to the log-diagonal elements. The Cholesky parameterization ensures geometric validity while enabling rich adaptation to semantic context — e.g., near faces, the learned $L(x, c)$ may emphasize local feature directions, while near landscapes, it may align with global spatial gradients.

% \subsection{Conditional Geodesic Probability Path and Target Velocity Field}

% Suppose we draw a triplet: $c \sim p_{\text{text}}$, $x_0 \sim p_0(\cdot|c)$ (a data point conditioned on $c$), and $x_1 \sim p_1$ (a noise point). The path connecting them is not a straight line in $\mathbb{R}^D$, but the conditional geodesic $\gamma^c_{x_0 \to x_1}(t)$ on $\mathcal{M}$ under metric $g_\Phi(\cdot, c)$. At time $t$, the interpolant point $z_t$ along this path is given by:
% \begin{equation*}
%     z_t = \exp^c_{x_0}(t \cdot \log^c_{x_0}(x_1)).
% \end{equation*}
% This embodies the geometric principle that motion on a manifold should follow its curvature \textit{as modulated by semantic context $c$}. The logarithmic map $\log^c_{x_0}(x_1)$ gives us the ``launch vector" from $x_0$ under $c$, and scaling it by $t$ and exponentiating traces out the conditional geodesic proportionally.

% The \textbf{target velocity field} $u_t(z_t | x_0, x_1, c)$ is the instantaneous velocity of this conditional geodesic at point $z_t$. Since the geodesic's velocity vector is parallel-transported along the path under $g_\Phi(\cdot, c)$, the velocity at time $t$ is the parallel transport of the initial velocity $\log^c_{x_0}(x_1)$ from $T_{x_0}\mathcal{M}$ to $T_{z_t}\mathcal{M}$:
% \begin{equation*}
%     u_t(z_t | x_0, x_1, c) = P^c_{\gamma, t \leftarrow 0}(\log^c_{x_0}(x_1)).
% \end{equation*}
% This is geometrically intuitive: under conditioning $c$, you're moving along the most natural path, ``carrying" your initial direction with you via context-aware parallel transport. The vector field $u_t$ thus represents the ``gold standard" of motion — the most natural, curvature- and semantics-aware way to move from noise to data.

% \subsection{The GeodesicFlow Objective}

% To train the model $v_\Theta$, we minimize the discrepancy between its predicted velocity $v_\Theta(z_t, t, c)$ and the target conditional geodesic velocity $u_t(z_t | x_0, x_1, c)$. Since both vectors live in the tangent space $T_{z_t}\mathcal{M}$, we measure their difference using the adaptive Riemannian metric $g_\Phi(z_t, c)$, which ensures the comparison respects local geometry \textit{and} semantic context:
% \begin{equation}
%     \mathcal{L}_{\text{GeodesicFlow}}(\Theta, \Phi) = \mathbb{E}_{\substack{c \sim p_{\text{text}} \\ t \sim \mathcal{U}[0,1] \\ x_0 \sim p_0(\cdot|c) \\ x_1 \sim p_1}} \left[ \left\| v_\Theta(z_t, t, c) - u_t(z_t | x_0, x_1, c) \right\|_{g_\Phi(z_t, c)}^2 \right].
% \end{equation}
% Expanding $z_t$ and $u_t$ explicitly, the full objective becomes:
% \begin{equation}
%     \mathcal{L}_{\text{GeodesicFlow}}(\Theta, \Phi) = \mathbb{E}_{c, t, x_0, x_1} \left[ \left\| v_\Theta(\exp^c_{x_0}(t \cdot \log^c_{x_0}(x_1)), t, c) - P^c_{\gamma, t \leftarrow 0}(\log^c_{x_0}(x_1)) \right\|_{g_\Phi(\exp^c_{x_0}(t \cdot \log^c_{x_0}(x_1)), c)}^2 \right].
% \end{equation}
% Here, $\|\cdot\|_{g_\Phi(z_t, c)}^2$ is computed efficiently as $\|L(z_t, c)^{-1} v\|_2^2$ via forward substitution, avoiding explicit matrix inversion. We jointly optimize $\Theta$ and $\Phi$. The loss encourages the model to learn a vector field that mimics conditional geodesic motion — the most efficient transport according to the semantics-modulated geometry. In essence, GeodesicFlow teaches the model to ``flow along straight lines" on curved, context-aware spaces, ensuring that generated samples traverse the manifold in the most natural, semantically coherent way possible.

% \subsection{Generative Sampling via Conditional Geodesic Integration}

% Once trained, the vector field $v_\Theta$ and metric $g_\Phi$ define a dynamical system on $\mathcal{M}$: given a conditioning context $c$, we start from a sample $z_1 \sim p_1$, and integrate the ODE backward in time to generate a sample from $p_0(\cdot|c)$:
% \begin{equation*}
%     \frac{d z_t}{dt} = v_\Theta(z_t, t, c).
% \end{equation*}
% Numerically, this is achieved via \textbf{conditional geodesic shooting}: at each step, we use the exponential map under $g_\Phi(\cdot, c)$ to move along the direction predicted by the model. Specifically, from time $t$ to $t - \Delta t$, we update:
% \begin{equation*}
%     z_{t-\Delta t} = \exp^c_{z_t}(-\Delta t \cdot v_\Theta(z_t, t, c)).
% \end{equation*}
% This is the manifold analog of Euler’s method under adaptive geometry. The minus sign reflects backward integration: we start in noise and flow toward data under conditioning $c$.

% The resulting trajectory is a conditional geodesic-like path (not necessarily a true geodesic, unless $v_\Theta$ perfectly matches the target) that morphs noise into a realistic, semantically aligned sample. Higher-order methods such as Riemannian Runge-Kutta under $g_\Phi(\cdot, c)$ can be used for improved accuracy on highly curved or semantically complex regions.

% \subsection{Algorithmic Implementation: Learning and Sampling with Semantic-Geometric Fidelity}

% Algorithms \ref{alg:training_geodesicflow} and \ref{alg:sampling_geodesicflow} operationalize the core philosophy of GeodesicFlow: to learn and then execute curvature- and semantics-aware transport on manifolds. Training (Algorithm \ref{alg:training_geodesicflow}) constructs conditional geodesic interpolants between data and noise under text embeddings, computes the ``ground truth" velocity via context-aware parallel transport, and trains the neural vector field (and metric network) to match it — all within the adaptive metric geometry defined by $g_\Phi$. Sampling (Algorithm \ref{alg:sampling_geodesicflow}) then leverages this learned field to generate new data by integrating backward along conditional geodesic-like trajectories, starting from noise and conditioned on text. The use of the conditional exponential map ensures that all operations remain on-manifold and semantically grounded. Together, they form a geometrically and semantically coherent pipeline: one that learns the manifold’s ``natural motion under context" and then faithfully replays it to synthesize data — respecting intrinsic structure and semantic intent at every step.

% \begin{algorithm}[H]
% \caption{Training GeodesicFlow with Adaptive Metric}
% \label{alg:training_geodesicflow}
% \begin{algorithmic}[1]
% \Require
% \item \textit{Model:} Neural network $v_\Theta: \mathcal{M} \times [0,1] \times \mathcal{C} \to T\mathcal{M}$ with parameters $\Theta$.
% \item \textit{Metric Network:} $g_\Phi(x, c) = L(x, c) L(x, c)^\top$, where $L(x, c)$ is lower-triangular with positive diagonal, parameterized by $\Phi$.
%     \item \textit{Data:} Conditional distribution $p_0(\cdot|c)$, noise distribution $p_1$, and text prior $p_{\text{text}}$ on manifold $\mathcal{M}$.
%     \item \textit{Manifold Ops:} Conditional logarithmic map ($\log^c$), exponential map ($\exp^c$), parallel transport ($P^c$).
%     \item \textit{Hyperparameters:} Batch size $B$, number of training steps $N_{\text{steps}}$, learning rate $\alpha$, regularization $\epsilon = 10^{-4}$.
% \State Initialize model parameters $\Theta$ and metric parameters $\Phi$.
% \State Initialize optimizer (i.e., AdamW \cite{loshchilov2018decoupled}) with learning rate $\alpha$.
% \For{step = 1 to $N_{\text{steps}}$}
%     \State Sample a mini-batch: $\{c^{(i)}\}_{i=1}^B \sim p_{\text{text}}$, $\{x_0^{(i)}\}_{i=1}^B \sim p_0(\cdot|c^{(i)})$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, and $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
%     \State Initialize batch loss $\mathcal{L}_{\text{batch}} \leftarrow 0$.
%     \For{$i = 1$ to $B$}
%         \State Let $c \leftarrow c^{(i)}$, $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
%         \State Compute initial velocity under $g_\Phi(\cdot, c)$: $v_0 \leftarrow \log^c_{x_0}(x_1) \in T_{x_0}\mathcal{M}$.
%         \State Compute interpolated point: $z_t \leftarrow \exp^c_{x_0}(t \cdot v_0)$.
%         \State Compute target velocity via parallel transport: $u_t \leftarrow P^c_{\gamma, t \leftarrow 0}(v_0) \in T_{z_t}\mathcal{M}$.
%         \State Predict velocity: $\hat{u}_t \leftarrow v_\Theta(z_t, t, c)$.
%         \State Compute $L = L_\Phi(z_t, c)$, ensure $\operatorname{diag}(L) > 0$ via $\exp(\cdot)$.
%         \State Compute residual: $r \leftarrow \hat{u}_t - u_t$.
%         \State Solve $L(z_t, c) \, w = r$ for $w$ via forward substitution.
%         \State Compute loss: $\mathcal{L}^{(i)} \leftarrow \|w\|_2^2$.
%         \State $\mathcal{L}_{\text{batch}} \leftarrow \mathcal{L}_{\text{batch}} + \mathcal{L}^{(i)}$.
%     \EndFor
%     \State Compute mean loss: $\mathcal{L} \leftarrow \frac{1}{B} \mathcal{L}_{\text{batch}}$.
%     \State Update parameters: $\Theta \leftarrow \text{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$, $\Phi \leftarrow \text{OptimizerStep}(\Phi, \nabla_\Phi \mathcal{L})$.
% \EndFor
% \State \Return Trained parameters $\Theta$, $\Phi$.
% \end{algorithmic}
% \end{algorithm}

% \vspace{1cm}

% \begin{algorithm}[H]
% \caption{Sampling from a Trained GeodesicFlow Model via Conditional Geodesic Integration}
% \label{alg:sampling_geodesicflow}
% \begin{algorithmic}[1]
% \Require
% \item \textit{Model:} Trained neural network $v_\Theta$.
% \item \textit{Metric:} Trained $g_\Phi(x, c) = L(x, c)L(x, c)^\top$.
%     \item \textit{Conditioning:} Text embedding $c \in \mathcal{C}$.
%     \item \textit{Noise Distribution:} $p_1$ on the manifold $\mathcal{M}$.
%     \item \textit{Manifold Op:} Conditional exponential map ($\exp^c$).
%     \item \textit{Hyperparameter:} Number of integration steps $N$.
% \State Sample initial point: $z_1 \sim p_1$.
% \State Set time step: $\Delta t \leftarrow 1/N$.
% \For{$k = N$ \textbf{down to} $1$}
%     \State Set current time: $t \leftarrow k \cdot \Delta t$.
%     \State Let current point be $z_t$.
%     \State Predict velocity: $\hat{u}_t \leftarrow v_\Theta(z_t, t, c)$.
%     \State Perform conditional geodesic shooting: $z_{t-\Delta t} \leftarrow \exp^c_{z_t}(-\Delta t \cdot \hat{u}_t)$.
% \EndFor
% \State \Return Generated sample $z_0$ conditioned on $c$.
% \end{algorithmic}
% \end{algorithm}

% ---------------------------
% T2I setting
% \section{GeodesicFlow: Geodesic Flow Matching on Manifolds}

% Our goal is to learn a \textit{text-conditioned} time-dependent vector field $v_\Theta: \mathcal{M} \times [0,1] \times \mathcal{C} \to T\mathcal{M}$, where $v_\Theta(x, t, c) \in T_x\mathcal{M}$, that governs a continuous transformation of samples from a simple base distribution $p_1$ (e.g., Gaussian noise on the manifold) into samples from a complex, \textit{text-conditioned} target data distribution $p_0(\cdot \mid c)$. This transformation is realized as the solution to an ordinary differential equation (ODE) on the manifold, where the vector field $v_\Theta$ dictates the instantaneous direction and speed of motion at each point, time, and given text condition $c$.

% The key insight remains: we use \textit{geodesics} — the manifold’s natural notion of straight lines — as interpolation paths. However, now these paths are not only between noise and data, but between noise and \textit{text-aligned data}. The text condition $c$ guides the geometry of the flow, ensuring generated samples are semantically aligned with the provided description.

% \subsection{Geodesic Probability Path and Target Velocity Field}

% Suppose we draw a triplet: $x_0 \sim p_0(\cdot \mid c)$ (a data point matching caption $c$), $x_1 \sim p_1$ (a noise point), and a text embedding $c \sim p_{\text{text}}$. The path connecting $x_0$ and $x_1$ is still the geodesic $\gamma_{x_0 \to x_1}(t)$ on $\mathcal{M}$, but now the entire trajectory is implicitly conditioned on $c$ through the data distribution. At time $t$, the interpolant point $z_t$ is:
% \begin{equation*}
%     z_t = \exp_{x_0}(t \cdot \log_{x_0}(x_1)).
% \end{equation*}
% This path remains geometrically intrinsic — but now, $x_0$ is drawn from a distribution shaped by $c$, making the path semantically meaningful.

% The \textbf{text-conditioned target velocity field} $u_t(z_t | x_0, x_1, c)$ is again the instantaneous velocity of this geodesic at $z_t$, obtained via parallel transport of the initial launch vector:
% \begin{equation*}
%     u_t(z_t | x_0, x_1, c) = P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1)).
% \end{equation*}
% Note that while the velocity field formula does not explicitly depend on $c$, its statistical dependence arises because $x_0$ is sampled from $p_0(\cdot \mid c)$. Thus, the target velocity field is implicitly conditioned on $c$ through the selection of $x_0$.

% \subsection{The GeodesicFlow-T2I Objective}

% To train the text-conditioned model $v_\Theta(\cdot, \cdot, c)$, we minimize the discrepancy between its predicted velocity and the target geodesic velocity, now conditioned on text:
% \begin{equation}
%     \mathcal{L}_{\text{GeodesicFlow-T2I}}(\Theta) = \mathbb{E}_{\substack{t \sim \mathcal{U}[0,1] \\ x_0 \sim p_0(\cdot \mid c) \\ x_1 \sim p_1 \\ c \sim p_{\text{text}}}} \left[ \left\| v_\Theta(z_t, t, c) - u_t(z_t | x_0, x_1, c) \right\|_{g(z_t)}^2 \right].
% \end{equation}
% Expanding $z_t$ and $u_t$ explicitly:
% \begin{equation}
%     \mathcal{L}_{\text{GeodesicFlow-T2I}}(\Theta) = \mathbb{E}_{t, x_0, x_1, c} \left[ \left\| v_\Theta(\exp_{x_0}(t \cdot \log_{x_0}(x_1)), t, c) - P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1)) \right\|_{g(\exp_{x_0}(t \cdot \log_{x_0}(x_1)))}^2 \right].
% \end{equation}
% Minimizing this loss encourages the model to learn a vector field that mimics geodesic motion \textit{conditioned on text semantics}. The model learns to modulate its velocity predictions based on $c$, ensuring that the generated trajectory flows toward samples that are not only geometrically natural but also textually aligned.

% \subsection{Generative Sampling via Geodesic Integration}

% Once trained, sampling from the model for a given text $c$ proceeds by integrating the text-conditioned ODE backward in time:
% \begin{equation*}
%     \frac{d z_t}{dt} = v_\Theta(z_t, t, c).
% \end{equation*}
% Starting from noise $z_1 \sim p_1$, we generate a sample aligned with $c$ by numerically integrating backward using \textbf{geodesic shooting}:
% \begin{equation*}
%     z_{t-\Delta t} = \exp_{z_t}(-\Delta t \cdot v_\Theta(z_t, t, c)).
% \end{equation*}
% The text embedding $c$ is held fixed throughout the integration, acting as a semantic guide that steers the flow toward the desired region of the data manifold.

% The resulting trajectory is a text-conditioned, geodesic-like path that morphs noise into a realistic, caption-aligned sample. As before, higher-order Riemannian integrators can be employed for improved fidelity on highly curved manifolds.

% \subsection{Algorithmic Implementation: Learning and Sampling with Geometric Fidelity}

% Algorithms~\ref{alg:training_geodesicflow_t2i} and~\ref{alg:sampling_geodesicflow_t2i} extend the original GeodesicFlow framework to the text-to-image setting. Training now samples text-conditioned data points and feeds the text embedding $c$ into the neural vector field. Sampling accepts a user-provided text embedding and generates an image by integrating the text-conditioned dynamics. Crucially, all geometric operations — logarithmic/exponential maps, parallel transport, and metric evaluations — remain unchanged; only the functional form of the vector field becomes conditioned on $c$. This ensures geometric fidelity is preserved while enabling semantic control.

% \begin{algorithm}[H]
% \caption{Training GeodesicFlow}
% \label{alg:training_geodesicflow_t2i}
% \begin{algorithmic}[1]
% \Require
% \Statex \textit{Model:} Neural network $v_\Theta: \mathcal{M} \times [0,1] \times \mathcal{C} \to T\mathcal{M}$ with parameters $\Theta$.
% \Statex \textit{Data:} Text-conditioned distribution $p_0(\cdot \mid c)$, noise distribution $p_1$, and text prior $p_{\text{text}}$.
% \Statex \textit{Manifold Ops:} Logarithmic map ($\log$), exponential map ($\exp$), parallel transport ($P$), and metric ($g$).
% \Statex \textit{Hyperparameters:} Batch size $B$, number of training steps $N_{\text{steps}}$, learning rate $\alpha$.
% \State Initialize model parameters $\Theta$.
% \State Initialize an optimizer (e.g., Adam) with learning rate $\alpha$.
% \For{step = 1 to $N_{\text{steps}}$}
%     \State Sample a mini-batch: $\{c^{(i)}\}_{i=1}^B \sim p_{\text{text}}$, $\{x_0^{(i)}\}_{i=1}^B \sim p_0(\cdot \mid c^{(i)})$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, and $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
%     \State Initialize batch loss $\mathcal{L}_{\text{batch}} \leftarrow 0$.
%     \For{$i = 1$ to $B$}
%         \State Let $c \leftarrow c^{(i)}$, $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
%         \State Compute initial velocity: $v_0 \leftarrow \log_{x_0}(x_1) \in T_{x_0}\mathcal{M}$.
%         \State Compute interpolated point: $z_t \leftarrow \exp_{x_0}(t \cdot v_0)$.
%         \State Compute target velocity via parallel transport: $u_t \leftarrow P_{\gamma, t \leftarrow 0}(v_0) \in T_{z_t}\mathcal{M}$.
%         \State Predict conditioned velocity: $\hat{u}_t \leftarrow v_\Theta(z_t, t, c)$.
%         \State Compute loss: $\mathcal{L}^{(i)} \leftarrow \left\| \hat{u}_t - u_t \right\|_{g(z_t)}^2$.
%         \State $\mathcal{L}_{\text{batch}} \leftarrow \mathcal{L}_{\text{batch}} + \mathcal{L}^{(i)}$.
%     \EndFor
%     \State Compute mean loss: $\mathcal{L} \leftarrow \frac{1}{B} \mathcal{L}_{\text{batch}}$.
%     \State Update parameters: $\Theta \leftarrow \text{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$.
% \EndFor
% \State \Return Trained parameters $\Theta$.
% \end{algorithmic}
% \end{algorithm}

% \vspace{1cm}

% \begin{algorithm}[H]
% \caption{Sampling from a Trained GeodesicFlow Model}
% \label{alg:sampling_geodesicflow_t2i}
% \begin{algorithmic}[1]
% \Require
% \Statex \textit{Model:} Trained neural network $v_\Theta$.
% \Statex \textit{Text Embedding:} Condition $c \in \mathcal{C}$ (e.g., from CLIP text encoder).
% \Statex \textit{Noise Distribution:} $p_1$ on the manifold $\mathcal{M}$.
% \Statex \textit{Manifold Op:} Exponential map ($\exp$).
% \Statex \textit{Hyperparameter:} Number of integration steps $N$.
% \State Sample initial point: $z_1 \sim p_1$.
% \State Set time step: $\Delta t \leftarrow 1/N$.
% \For{$k = N$ \textbf{downto} $1$}
%     \State Set current time: $t \leftarrow k \cdot \Delta t$.
%     \State Predict conditioned velocity: $\hat{u}_t \leftarrow v_\Theta(z_t, t, c)$.
%     \State Geodesic shooting backward: $z_{t-\Delta t} \leftarrow \exp_{z_t}(-\Delta t \cdot \hat{u}_t)$.
% \EndFor
% \State \Return Generated sample $z_0$ aligned with text $c$.
% \end{algorithmic}
% \end{algorithm}

% ------------------------
\section{GeodesicFlow: Geodesic Flow Matching on Manifolds}

Our goal is to learn a \textit{text-conditioned} time-dependent vector field $v_\Theta: \mathcal{M} \times [0,1] \times \mathcal{C} \to T\mathcal{M}$, where $v_\Theta(x, t, c) \in T_x\mathcal{M}$, that governs a continuous transformation of samples from a simple base distribution $p_1$ (e.g., Gaussian noise on the manifold) into samples from a complex, \textit{text-conditioned} target data distribution $p_0(\cdot \mid c)$. This transformation is realized as the solution to an ordinary differential equation (ODE) on the manifold, where the vector field $v_\Theta$ dictates the instantaneous direction and speed of motion at each point, time, and given text condition $c$.

The key insight remains: we use \textit{geodesics} — the manifold’s natural notion of straight lines — as interpolation paths. However, now these paths are not only between noise and data, but between noise and \textit{text-aligned data}. The text condition $c$ guides the geometry of the flow, ensuring generated samples are semantically aligned with the provided description.

\subsection{Geodesic Probability Path and Target Velocity Field}

Suppose we draw a triplet: $x_0 \sim p_0(\cdot \mid c)$ (a data point matching caption $c$), $x_1 \sim p_1$ (a noise point), and a text embedding $c \sim p_{\text{text}}$. The path connecting $x_0$ and $x_1$ is still the geodesic $\gamma_{x_0 \to x_1}(t)$ on $\mathcal{M}$, but now the entire trajectory is implicitly conditioned on $c$ through the data distribution. At time $t$, the interpolant point $z_t$ is:
\begin{equation*}
    z_t = \exp_{x_0}(t \cdot \log_{x_0}(x_1)).
\end{equation*}
This path remains geometrically intrinsic — but now, $x_0$ is drawn from a distribution shaped by $c$, making the path semantically meaningful.

The \textbf{text-conditioned target velocity field} $u_t(z_t | x_0, x_1, c)$ is again the instantaneous velocity of this geodesic at $z_t$, obtained via parallel transport of the initial launch vector:
\begin{equation*}
    u_t(z_t | x_0, x_1, c) = P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1)).
\end{equation*}
Note that while the velocity field formula does not explicitly depend on $c$, its statistical dependence arises because $x_0$ is sampled from $p_0(\cdot \mid c)$. Thus, the target velocity field is implicitly conditioned on $c$ through the selection of $x_0$.

\subsection{The GeodesicFlow Objective}

To train the text-conditioned model $v_\Theta(\cdot, \cdot, c)$, we minimize the discrepancy between its predicted velocity and the target geodesic velocity, now conditioned on text:
\begin{equation}
    \mathcal{L}_{\text{GeodesicFlow}}(\Theta) = \mathbb{E}_{\substack{t \sim \mathcal{U}[0,1] \\ x_0 \sim p_0(\cdot \mid c) \\ x_1 \sim p_1 \\ c \sim p_{\text{text}}}} \left[ \left\| v_\Theta(z_t, t, c) - u_t(z_t | x_0, x_1, c) \right\|_{g(z_t)}^2 \right].
\end{equation}
Expanding $z_t$ and $u_t$ explicitly:
\begin{equation}
    \mathcal{L}_{\text{GeodesicFlow}}(\Theta) = \mathbb{E}_{t, x_0, x_1, c} \left[ \left\| v_\Theta(\exp_{x_0}(t \cdot \log_{x_0}(x_1)), t, c) - P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1)) \right\|_{g(\exp_{x_0}(t \cdot \log_{x_0}(x_1)))}^2 \right].
\end{equation}
Minimizing this loss encourages the model to learn a vector field that mimics geodesic motion \textit{conditioned on text semantics}. The model learns to modulate its velocity predictions based on $c$, ensuring that the generated trajectory flows toward samples that are not only geometrically natural but also textually aligned.


\begin{hypothesis}[Jacobian-Free Learning via Geodesic Velocity Regression]
\label{hyp:jacobian_free}
Let $\mathcal{M}$ be a Riemannian manifold with metric $g$, and let $v_\Theta: \mathcal{M} \times [0,1] \times \mathcal{C} \to T\mathcal{M}$ be a parametric vector field. Suppose the target velocity field $u_t(\cdot | x_0, x_1, c)$ along the geodesic path $\gamma_{x_0 \to x_1}(t)$ is explicitly computable via parallel transport, i.e., $u_t = P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1))$. Then, minimizing the Riemannian tangent-space regression loss
\[
\mathbb{E}_{t, x_0, x_1, c} \left[ \left\| v_\Theta(z_t, t, c) - u_t \right\|_{g(z_t)}^2 \right]
\]
does not require computation of the spatial Jacobian $\nabla_x v_\Theta(x,t,c)$, and gradients w.r.t. parameters $\Theta$ can be computed solely via backpropagation through the functional output of $v_\Theta$. Thus, the optimal vector field can be learned in a Jacobian-free manner.
\end{hypothesis}

This hypothesis is not restricted to specific manifolds or data modalities — it holds whenever geodesics and parallel transport are well-defined, making it applicable to spheres, hyperbolic spaces, SPD matrices, and other common Riemannian manifolds used in machine learning. Moreover, its reliance on direct velocity regression rather than probabilistic score matching renders it broadly compatible with any conditional generative setting where geometric interpolation paths can be constructed.

This hypothesis ensures computational tractability: because the loss is a simple regression in the tangent bundle and targets are geometrically precomputed, no differential operators (e.g., divergence, Hessian, or Jacobian trace) need to be evaluated during training. This is a significant advantage over score-based or continuous normalizing flow methods, which often require expensive Jacobian computations or stochastic trace estimators.

\subsection{Generative Sampling via Geodesic Integration}

Once trained, sampling from the model for a given text $c$ proceeds by integrating the text-conditioned ODE backward in time:
\begin{equation*}
    \frac{d z_t}{dt} = v_\Theta(z_t, t, c).
\end{equation*}
Starting from noise $z_1 \sim p_1$, we generate a sample aligned with $c$ by numerically integrating backward using \textbf{geodesic shooting}:
\begin{equation*}
    z_{t-\Delta t} = \exp_{z_t}(-\Delta t \cdot v_\Theta(z_t, t, c)).
\end{equation*}
The text embedding $c$ is held fixed throughout the integration, acting as a semantic guide that steers the flow toward the desired region of the data manifold.

The resulting trajectory is a text-conditioned, geodesic-like path that morphs noise into a realistic, caption-aligned sample. As before, higher-order Riemannian integrators can be employed for improved fidelity on highly curved manifolds.

\subsection{Algorithmic Implementation: Learning and Sampling with Geometric Fidelity}

Algorithms~\ref{alg:training_geodesicflow_t2i} and~\ref{alg:sampling_geodesicflow_t2i} extend the original GeodesicFlow framework to the text-to-image setting. Training now samples text-conditioned data points and feeds the text embedding $c$ into the neural vector field. Sampling accepts a user-provided text embedding and generates an image by integrating the text-conditioned dynamics. Crucially, all geometric operations — logarithmic/exponential maps, parallel transport, and metric evaluations — remain unchanged; only the functional form of the vector field becomes conditioned on $c$. This ensures geometric fidelity is preserved while enabling semantic control.


\begin{algorithm}[H]
\caption{Training GeodesicFlow}
\label{alg:training_geodesicflow_t2i}
\begin{algorithmic}[1]
\Require
\Statex \textit{Model:} Neural network $v_\Theta: \mathcal{M} \times [0,1] \times \mathcal{C} \to T\mathcal{M}$ with parameters $\Theta$.
\Statex \textit{Data:} Text-conditioned distribution $p_0(\cdot \mid c)$, noise distribution $p_1$, and text prior $p_{\text{text}}$.
\Statex \textit{Manifold Ops:} Logarithmic map ($\log$), exponential map ($\exp$), parallel transport ($P$), and metric ($g$).
\Statex \textit{Hyperparameters:} Batch size $B$, number of training steps $N_{\text{steps}}$, learning rate $\alpha$.
\State Initialize model parameters $\Theta$.
\State Initialize an optimizer (e.g., Adam) with learning rate $\alpha$.
\For{step = 1 to $N_{\text{steps}}$}
    \State Sample a mini-batch: $\{c^{(i)}\}_{i=1}^B \sim p_{\text{text}}$, $\{x_0^{(i)}\}_{i=1}^B \sim p_0(\cdot \mid c^{(i)})$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, and $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
    \State Initialize batch loss $\mathcal{L}_{\text{batch}} \leftarrow 0$.
    \For{$i = 1$ to $B$}
        \State Let $c \leftarrow c^{(i)}$, $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
        \State Compute initial velocity: $v_0 \leftarrow \log_{x_0}(x_1) \in T_{x_0}\mathcal{M}$.
        \State Compute interpolated point: $z_t \leftarrow \exp_{x_0}(t \cdot v_0)$.
        \State Compute target velocity via parallel transport: $u_t \leftarrow P_{\gamma, t \leftarrow 0}(v_0) \in T_{z_t}\mathcal{M}$.
        \State Predict conditioned velocity: $\hat{u}_t \leftarrow v_\Theta(z_t, t, c)$.
        \State Compute loss: $\mathcal{L}^{(i)} \leftarrow \left\| \hat{u}_t - u_t \right\|_{g(z_t)}^2$.
        \State $\mathcal{L}_{\text{batch}} \leftarrow \mathcal{L}_{\text{batch}} + \mathcal{L}^{(i)}$.
    \EndFor
    \State Compute mean loss: $\mathcal{L} \leftarrow \frac{1}{B} \mathcal{L}_{\text{batch}}$.
    \State Update parameters: $\Theta \leftarrow \text{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$.
\EndFor
\State \Return Trained parameters $\Theta$.
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
\caption{Sampling from a Trained GeodesicFlow Model}
\label{alg:sampling_geodesicflow_t2i}
\begin{algorithmic}[1]
\Require
\Statex \textit{Model:} Trained neural network $v_\Theta$.
\Statex \textit{Text Embedding:} Condition $c \in \mathcal{C}$ (e.g., from CLIP text encoder).
\Statex \textit{Noise Distribution:} $p_1$ on the manifold $\mathcal{M}$.
\Statex \textit{Manifold Op:} Exponential map ($\exp$).
\Statex \textit{Hyperparameter:} Number of integration steps $N$.
\State Sample initial point: $z_1 \sim p_1$.
\State Set time step: $\Delta t \leftarrow 1/N$.
\For{$k = N$ \textbf{downto} $1$}
    \State Set current time: $t \leftarrow k \cdot \Delta t$.
    \State Predict conditioned velocity: $\hat{u}_t \leftarrow v_\Theta(z_t, t, c)$.
    \State Geodesic shooting backward: $z_{t-\Delta t} \leftarrow \exp_{z_t}(-\Delta t \cdot \hat{u}_t)$.
\EndFor
\State \Return Generated sample $z_0$ aligned with text $c$.
\end{algorithmic}
\end{algorithm}

% --------------------------
% Metric-free GFlow
% \section{GeodesicFlow: Metric-Free Geodesic Flow Matching on Manifolds}

% Our goal is to learn a \textit{text-conditioned} time-dependent vector field $v_\Theta: \mathcal{M} \times [0,1] \times \mathcal{C} \to T\mathcal{M}$, where $v_\Theta(x, t, c) \in T_x\mathcal{M}$, that governs a continuous transformation of samples from a simple base distribution $p_1$ (e.g., isotropic Gaussian noise on the manifold) into samples from a complex, \textit{text-conditioned} target data distribution $p_0(\cdot \mid c)$. This transformation is realized as the solution to an ordinary differential equation (ODE) on the manifold, where the vector field $v_\Theta$ dictates the instantaneous direction and speed of motion at each point, time, and given text condition $c$.

% The core geometric insight remains: we use \textit{geodesics} — the manifold’s natural notion of shortest paths — as interpolation trajectories. However, these paths now connect noise to \textit{text-aligned data}, with the text condition $c$ implicitly shaping the statistical geometry of the flow. This ensures that generated samples are not only geometrically plausible but also semantically aligned with the provided description.

% \subsection{Geodesic Probability Path and Target Velocity Field}

% We sample a triplet: $x_0 \sim p_0(\cdot \mid c)$ (a data point matching caption $c$), $x_1 \sim p_1$ (a noise point), and a text embedding $c \sim p_{\text{text}}$. The path connecting $x_0$ and $x_1$ is the geodesic $\gamma_{x_0 \to x_1}(t)$ on $\mathcal{M}$, implicitly conditioned on $c$ through the sampling of $x_0$. At time $t$, the interpolant point $z_t$ is given by:
% \begin{equation*}
%     z_t = \exp_{x_0}(t \cdot \log_{x_0}(x_1)).
% \end{equation*}
% This path is geometrically intrinsic — and semantically meaningful — because $x_0$ is drawn from a distribution shaped by $c$.

% The \textbf{text-conditioned target velocity field} $u_t(z_t | x_0, x_1, c)$ is the instantaneous velocity of this geodesic at $z_t$, obtained via parallel transport of the initial tangent vector:
% \begin{equation*}
%     u_t(z_t | x_0, x_1, c) = P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1)).
% \end{equation*}
% Although $c$ does not appear explicitly in the formula, it influences the velocity field statistically through the dependence of $x_0 \sim p_0(\cdot \mid c)$. Thus, the target velocity field is implicitly conditioned on $c$.

% \subsection{Metric-Free Learning Objective}

% Computing the Riemannian norm $\|\cdot\|_{g(z_t)}$ requires evaluating the metric tensor $g$ at each point $z_t$, which is often intractable or computationally expensive for general manifolds. To circumvent this, we introduce the following key hypothesis:

% \begin{hypothesis}[Metric-Free Approximation]
% The tangent bundle $T\mathcal{M}$ is equipped with a smoothly varying inner product, but for the purpose of optimization, the squared Riemannian norm $\|\cdot\|_{g(z)}^2$ can be approximated by the Euclidean norm in local coordinates of the tangent space $T_z\mathcal{M}$, i.e.,
% \[
% \|v\|_{g(z)}^2 \approx \|v\|_2^2 = \langle v, v \rangle_{\mathbb{R}^d},
% \]
% where $d = \dim(\mathcal{M})$, and $v$ is expressed in an orthonormal basis of $T_z\mathcal{M}$ induced by a local chart or embedding. This approximation holds when the curvature-induced distortion of the metric is negligible within mini-batch scales or when the model compensates for metric variation implicitly through training.
% \end{hypothesis}

% Under this hypothesis, we define the \textbf{metric-free GeodesicFlow-T2I objective}:
% \begin{equation}
%     \mathcal{L}_{\text{GeodesicFlow-T2I}}(\Theta) = \mathbb{E}_{\substack{t \sim \mathcal{U}[0,1] \\ x_0 \sim p_0(\cdot \mid c) \\ x_1 \sim p_1 \\ c \sim p_{\text{text}}}} \left[ \left\| v_\Theta(z_t, t, c) - u_t(z_t | x_0, x_1, c) \right\|_2^2 \right],
% \end{equation}
% where $\|\cdot\|_2$ denotes the standard Euclidean norm in the tangent space $T_{z_t}\mathcal{M}$, computed after expressing both vectors in the same local basis (e.g., via coordinate representation from a chosen chart or embedding).

% Expanding $z_t$ and $u_t$ explicitly:
% \begin{equation}
%     \mathcal{L}_{\text{GeodesicFlow-T2I}}(\Theta) = \mathbb{E}_{t, x_0, x_1, c} \left[ \left\| v_\Theta(\exp_{x_0}(t \cdot \log_{x_0}(x_1)), t, c) - P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1)) \right\|_2^2 \right].
% \end{equation}

% This objective encourages the model to learn a vector field that mimics geodesic motion \textit{conditioned on text semantics}, without requiring explicit metric evaluations. The model learns to modulate its velocity predictions based on $c$, ensuring that the generated trajectory flows toward samples that are geometrically natural and textually aligned — all while remaining computationally tractable.

% \subsection{Generative Sampling via Geodesic Integration}

% Once trained, sampling for a given text $c$ proceeds by integrating the text-conditioned ODE backward in time:
% \begin{equation*}
%     \frac{d z_t}{dt} = v_\Theta(z_t, t, c).
% \end{equation*}
% Starting from noise $z_1 \sim p_1$, we generate a sample aligned with $c$ by numerically integrating backward using \textbf{geodesic shooting}:
% \begin{equation*}
%     z_{t-\Delta t} = \exp_{z_t}(-\Delta t \cdot v_\Theta(z_t, t, c)).
% \end{equation*}
% The text embedding $c$ is held fixed throughout integration, acting as a semantic guide that steers the flow toward the desired region of the data manifold.

% The resulting trajectory is a text-conditioned, geodesic-like path that morphs noise into a realistic, caption-aligned sample. Higher-order Riemannian integrators (e.g., Riemannian Euler or Munthe-Kaas methods) can still be employed for improved fidelity on highly curved manifolds — but crucially, they do not require metric tensor evaluations during training.

% \subsection{Algorithmic Implementation: Metric-Free Learning and Sampling}

% Algorithms~\ref{alg:training_geodesicflow_t2i} and~\ref{alg:sampling_geodesicflow_t2i} extend the GeodesicFlow framework to the text-to-image setting under the metric-free hypothesis. Training samples text-conditioned data points and feeds the text embedding $c$ into the neural vector field. Sampling accepts a user-provided text embedding and generates an image by integrating the text-conditioned dynamics. All geometric operations — logarithmic/exponential maps and parallel transport — are preserved to maintain geometric fidelity; only the loss computation is simplified by replacing the Riemannian norm with the Euclidean norm in local tangent space coordinates.

% \begin{algorithm}[H]
% \caption{Training GeodesicFlow (Metric-Free)}
% \label{alg:training_geodesicflow_t2i}
% \begin{algorithmic}[1]
% \Require
% \Statex \textit{Model:} Neural network $v_\Theta: \mathcal{M} \times [0,1] \times \mathcal{C} \to T\mathcal{M}$ with parameters $\Theta$.
% \Statex \textit{Data:} Text-conditioned distribution $p_0(\cdot \mid c)$, noise distribution $p_1$, text prior $p_{\text{text}}$.
% \Statex \textit{Manifold Ops:} Logarithmic map ($\log$), exponential map ($\exp$), parallel transport ($P$). \textbf{No metric $g$ required.}
% \Statex \textit{Hyperparameters:} Batch size $B$, number of training steps $N_{\text{steps}}$, learning rate $\alpha$.
% \State Initialize model parameters $\Theta$.
% \State Initialize an optimizer (e.g., Adam) with learning rate $\alpha$.
% \For{step = 1 to $N_{\text{steps}}$}
%     \State Sample mini-batch: $\{c^{(i)}\}_{i=1}^B \sim p_{\text{text}}$, $\{x_0^{(i)}\}_{i=1}^B \sim p_0(\cdot \mid c^{(i)})$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
%     \State Initialize batch loss $\mathcal{L}_{\text{batch}} \leftarrow 0$.
%     \For{$i = 1$ to $B$}
%         \State Let $c \leftarrow c^{(i)}$, $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
%         \State Compute initial velocity: $v_0 \leftarrow \log_{x_0}(x_1) \in T_{x_0}\mathcal{M}$.
%         \State Compute interpolated point: $z_t \leftarrow \exp_{x_0}(t \cdot v_0)$.
%         \State Compute target velocity via parallel transport: $u_t \leftarrow P_{\gamma, t \leftarrow 0}(v_0) \in T_{z_t}\mathcal{M}$.
%         \State Predict conditioned velocity: $\hat{u}_t \leftarrow v_\Theta(z_t, t, c)$.
%         \State \textbf{Compute metric-free loss:} $\mathcal{L}^{(i)} \leftarrow \left\| \hat{u}_t - u_t \right\|_2^2$ (Euclidean norm in $T_{z_t}\mathcal{M}$).
%         \State $\mathcal{L}_{\text{batch}} \leftarrow \mathcal{L}_{\text{batch}} + \mathcal{L}^{(i)}$.
%     \EndFor
%     \State Compute mean loss: $\mathcal{L} \leftarrow \frac{1}{B} \mathcal{L}_{\text{batch}}$.
%     \State Update parameters: $\Theta \leftarrow \text{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$.
% \EndFor
% \State \Return Trained parameters $\Theta$.
% \end{algorithmic}
% \end{algorithm}

% \vspace{1cm}

% \begin{algorithm}[H]
% \caption{Sampling from a Trained GeodesicFlow Model (Metric-Free)}
% \label{alg:sampling_geodesicflow_t2i}
% \begin{algorithmic}[1]
% \Require
% \Statex \textit{Model:} Trained neural network $v_\Theta$.
% \Statex \textit{Text Embedding:} Condition $c \in \mathcal{C}$ (e.g., from CLIP text encoder).
% \Statex \textit{Noise Distribution:} $p_1$ on the manifold $\mathcal{M}$.
% \Statex \textit{Manifold Op:} Exponential map ($\exp$). \textbf{No metric $g$ required.}
% \Statex \textit{Hyperparameter:} Number of integration steps $N$.
% \State Sample initial point: $z_1 \sim p_1$.
% \State Set time step: $\Delta t \leftarrow 1/N$.
% \For{$k = N$ \textbf{downto} $1$}
%     \State Set current time: $t \leftarrow k \cdot \Delta t$.
%     \State Predict conditioned velocity: $\hat{u}_t \leftarrow v_\Theta(z_t, t, c)$.
%     \State Geodesic shooting backward: $z_{t-\Delta t} \leftarrow \exp_{z_t}(-\Delta t \cdot \hat{u}_t)$.
% \EndFor
% \State \Return Generated sample $z_0$ aligned with text $c$.
% \end{algorithmic}
% \end{algorithm}

% ------------------------
% Metric-free v2
\section{GeodesicFlow: Metric-Free Geodesic Flow Matching on Sphere Manifolds}

Our goal is to learn a \textit{text-conditioned} time-dependent vector field $v_\Theta: \mathcal{M} \times [0,1] \times \mathcal{C} \to T\mathcal{M}$, where $v_\Theta(x, t, c) \in T_x\mathcal{M}$, that governs a continuous transformation of samples from a simple base distribution $p_1$ (e.g., uniform noise on the sphere) into samples from a complex, \textit{text-conditioned} target data distribution $p_0(\cdot \mid c)$. This transformation is realized as the solution to an ordinary differential equation (ODE) on the manifold, where the vector field $v_\Theta$ dictates the instantaneous direction and speed of motion at each point, time, and given text condition $c$.

We restrict $\mathcal{M}$ to be the unit sphere $\mathbb{S}^n \subset \mathbb{R}^{n+1}$ endowed with its canonical round metric. Although $\mathbb{S}^n$ is a curved Riemannian manifold, its isometric embedding in Euclidean space allows us to compute all necessary geometric operations — exponential/logarithmic maps, parallel transport, and norm evaluations — using only ambient-space linear algebra, \textit{without ever explicitly evaluating or storing the metric tensor}. This yields a computationally efficient, \textbf{metric-free} implementation while preserving geometric fidelity.

Critically, this approach is \textit{not equivalent} to performing flow matching in Euclidean space. While we employ the Euclidean norm $\|\cdot\|$ in the loss, the vectors involved lie in tangent spaces $T_x\mathbb{S}^n \subset \mathbb{R}^{n+1}$, and due to the induced metric, we have:
\[
\|v\|_{g(x)} = \|v\|_2 \quad \text{for all } v \in T_x\mathbb{S}^n.
\]
Although the loss employs the Euclidean norm $\|\cdot\|_2$, it is not a Euclidean objective: the vectors $v_\Theta(z_t, t, c)$ and $u_t$ are constrained to lie in the tangent space $T_{z_t}\mathbb{S}^n$, and their evolution follows curved geodesics governed by the sphere’s intrinsic geometry. In contrast, a true Euclidean flow would use linear interpolation and constant (non-parallel-transported) velocities — violating the manifold structure. Here, the Euclidean norm is merely a \textit{computational proxy}: because the Riemannian metric on $\mathbb{S}^n$ is induced from the ambient $\mathbb{R}^{n+1}$, we have $\|v\|_{g(x)} = \|v\|_2$ for all $v \in T_x\mathbb{S}^n$. Thus, the optimization remains geometrically faithful to the curved manifold — it is efficient, not approximate.


The key insight remains: we use \textit{geodesics} — great circles on $\mathbb{S}^n$ — as interpolation paths between noise and \textit{text-aligned data}. The text condition $c$ guides the statistical selection of endpoints, thereby shaping the semantic content of the generated flow without altering its geometric structure.

\subsection{Geodesic Probability Path and Target Velocity Field (Metric-Free)}

Given $x_0 \sim p_0(\cdot \mid c)$, $x_1 \sim p_1$, and $c \sim p_{\text{text}}$, the geodesic path $\gamma_{x_0 \to x_1}(t)$ is given by spherical linear interpolation (Slerp):
\begin{equation*}
    z_t = \frac{\sin((1-t)\theta)}{\sin\theta} x_0 + \frac{\sin(t\theta)}{\sin\theta} x_1,
    \quad \text{where } \theta = \arccos(x_0^\top x_1).
\end{equation*}

The initial tangent vector is:
\begin{equation*}
    v_0 = \log_{x_0}(x_1) = \theta \cdot \frac{x_1 - (x_0^\top x_1)x_0}{\|x_1 - (x_0^\top x_1)x_0\|}.
\end{equation*}

The target velocity at $z_t$, obtained via parallel transport along the geodesic, is computed without metric evaluation:
\begin{equation*}
    u_t = P_{\gamma, t \leftarrow 0}(v_0) = v_0 - \frac{v_0^\top z_t}{1 - (x_0^\top x_1)^2} (x_1 - (x_0^\top x_1) x_0).
\end{equation*}

This expression leverages the sphere’s symmetry and requires only inner products and vector arithmetic in $\mathbb{R}^{n+1}$.

\subsection{The GeodesicFlow Objective (Metric-Free and Geometrically Faithful)}

The training objective minimizes the squared Euclidean norm between predicted and target velocities — which, as justified above, equals the squared Riemannian norm on the sphere:
\begin{equation}
    \mathcal{L}_{\text{GeodesicFlow}}(\Theta) = \mathbb{E}_{\substack{t \sim \mathcal{U}[0,1] \\ x_0 \sim p_0(\cdot \mid c) \\ x_1 \sim p_1 \\ c \sim p_{\text{text}}}} \left[ \left\| v_\Theta(z_t, t, c) - u_t \right\|^2 \right].
\end{equation}

Expanding explicitly:
\begin{equation}
    \mathcal{L}_{\text{GeodesicFlow}}(\Theta) = \mathbb{E}_{t, x_0, x_1, c} \left[ \left\| v_\Theta(z_t, t, c) - \left( v_0 - \frac{v_0^\top z_t}{1 - (x_0^\top x_1)^2} (x_1 - (x_0^\top x_1) x_0) \right) \right\|^2 \right],
\end{equation}
with $z_t$ and $v_0$ as defined above.

This objective encourages the model to learn curvature-aware, text-conditioned dynamics — not flat Euclidean flows. The use of the Euclidean norm is a computational convenience enabled by the embedding, not a geometric approximation.

\subsection{Generative Sampling via Geodesic Integration (Metric-Free)}

Sampling for a fixed text $c$ proceeds by numerically integrating the learned ODE backward in time:
\begin{equation*}
    \frac{d z_t}{dt} = v_\Theta(z_t, t, c),
\end{equation*}
starting from $z_1 \sim p_1$. Each step uses geodesic shooting via the exponential map:
\begin{equation*}
    z_{t-\Delta t} = \cos(\|\xi\|) z_t + \sin(\|\xi\|) \frac{\xi}{\|\xi\|},
    \quad \text{where } \xi = -\Delta t \cdot v_\Theta(z_t, t, c) \in T_{z_t}\mathbb{S}^n.
\end{equation*}

All operations remain within $\mathbb{R}^{n+1}$ and require no metric tensor computations. The result is a semantically guided, geometrically natural trajectory from noise to data.

\subsection{Algorithmic Implementation: Metric-Free Learning and Sampling}

Algorithms~\ref{alg:training_geodesicflow_t2i} and~\ref{alg:sampling_geodesicflow_t2i} implement the above using only ambient Euclidean operations. The Riemannian structure of $\mathbb{S}^n$ is fully respected — geodesics, parallel transport, and tangent norms are all correctly modeled — while avoiding any explicit metric tensor handling. This ensures scalability without sacrificing geometric integrity.

\begin{algorithm}[H]
\caption{Training GeodesicFlow (Metric-Free on Sphere)}
\label{alg:training_geodesicflow_t2i}
\begin{algorithmic}[1]
\Require
\Statex \textit{Model:} Neural network $v_\Theta: \mathbb{S}^n \times [0,1] \times \mathcal{C} \to T\mathbb{S}^n$ with parameters $\Theta$.
\Statex \textit{Data:} Text-conditioned distribution $p_0(\cdot \mid c)$, uniform noise $p_1$ on $\mathbb{S}^n$, text prior $p_{\text{text}}$.
\Statex \textit{Sphere Ops (Metric-Free):} Slerp ($\exp/\log$), parallel transport via vector rejection.
\Statex \textit{Hyperparameters:} Batch size $B$, steps $N_{\text{steps}}$, learning rate $\alpha$.
\State Initialize model parameters $\Theta$.
\State Initialize optimizer (e.g., Adam) with learning rate $\alpha$.
\For{step = 1 to $N_{\text{steps}}$}
    \State Sample mini-batch: $\{c^{(i)}\}_{i=1}^B \sim p_{\text{text}}$, $\{x_0^{(i)}\}_{i=1}^B \sim p_0(\cdot \mid c^{(i)})$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
    \State Initialize batch loss $\mathcal{L}_{\text{batch}} \leftarrow 0$.
    \For{$i = 1$ to $B$}
        \State Let $c \leftarrow c^{(i)}$, $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
        \State Compute angle: $\theta \leftarrow \arccos(x_0^\top x_1)$.
        \State Compute initial log vector: $v_0 \leftarrow \theta \cdot \frac{x_1 - (x_0^\top x_1)x_0}{\|x_1 - (x_0^\top x_1)x_0\|}$.
        \State Compute interpolated point: $z_t \leftarrow \frac{\sin((1-t)\theta)}{\sin\theta} x_0 + \frac{\sin(t\theta)}{\sin\theta} x_1$.
        \State Compute parallel transport (metric-free):
            \[
            u_t \leftarrow v_0 - \frac{v_0^\top z_t}{1 - (x_0^\top x_1)^2} (x_1 - (x_0^\top x_1) x_0)
            \]
        \State Predict velocity: $\hat{u}_t \leftarrow v_\Theta(z_t, t, c)$.
        \State Compute loss (Euclidean = Riemannian norm): $\mathcal{L}^{(i)} \leftarrow \| \hat{u}_t - u_t \|^2$.
        \State $\mathcal{L}_{\text{batch}} \leftarrow \mathcal{L}_{\text{batch}} + \mathcal{L}^{(i)}$.
    \EndFor
    \State Compute mean loss: $\mathcal{L} \leftarrow \frac{1}{B} \mathcal{L}_{\text{batch}}$.
    \State Update parameters: $\Theta \leftarrow \text{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$.
\EndFor
\State \Return Trained parameters $\Theta$.
\end{algorithmic}
\end{algorithm}

\vspace{1cm}

\begin{algorithm}[H]
\caption{Sampling from Trained GeodesicFlow (Metric-Free)}
\label{alg:sampling_geodesicflow_t2i}
\begin{algorithmic}[1]
\Require
\Statex \textit{Model:} Trained $v_\Theta$.
\Statex \textit{Text Embedding:} Condition $c \in \mathcal{C}$.
\Statex \textit{Noise:} $z_1 \sim \text{Uniform}(\mathbb{S}^n)$.
\Statex \textit{Hyperparameter:} Integration steps $N$.
\State Set $\Delta t \leftarrow 1/N$.
\For{$k = N$ \textbf{downto} $1$}
    \State Set $t \leftarrow k \cdot \Delta t$.
    \State Predict velocity: $\xi \leftarrow -\Delta t \cdot v_\Theta(z_t, t, c)$.
    \State Normalize direction: $\hat{\xi} \leftarrow \xi / \|\xi\|$ if $\|\xi\| > 0$, else $\hat{\xi} \leftarrow 0$.
    \State Geodesic shooting: $z_{t-\Delta t} \leftarrow \cos(\|\xi\|) z_t + \sin(\|\xi\|) \hat{\xi}$.
\EndFor
\State \Return Generated sample $z_0$ aligned with text $c$.
\end{algorithmic}
\end{algorithm}


% \subsection{Mathematical Equivalence in the Geodesic Case}
% GeodesicFlow can be interpreted as a specific, geometrically principal instance of the more general RFM framework. When RFM is configured to use the \textbf{geodesic distance} $d_g(x,y)$ as its premetric, the target vector fields of the two methods become mathematically equivalent.

% Let us adopt the GeodesicFlow convention (path from $x_0$ to $x_1$) for RFM. We choose the scheduler $\kappa(t) = 1-t$, so the path $\psi_t$ satisfies $d_g(\psi_t, x_1) = (1-t)d_g(x_0, x_1)$, matching the linear decrease in distance of a constant-speed geodesic. The RFM velocity field from the original paper \cite{chen2024flow} is:
% $$
% u_t^{\text{RFM}}(x | x_1) = \frac{-1}{1-t} d_g(x, x_1) \frac{\nabla_x d_g(x, x_1)}{\|\nabla_x d_g(x, x_1)\|_g^2}.
% $$
% On a Riemannian manifold, it is known that $\|\nabla_x d_g(x, y)\|_g = 1$ and $\nabla_x d_g(x, y) = -\frac{\log_x(y)}{d_g(x, y)}$. Let $x_t$ be a point on the geodesic path. Substituting these properties, the RFM velocity at $x_t$ simplifies to:
% $$
% u_t^{\text{RFM}}(x_t | x_1) = \frac{-1}{1-t} d_g(x_t, x_1) \left( -\frac{\log_{x_t}(x_1)}{d_g(x_t, x_1)} \right) = \frac{\log_{x_t}(x_1)}{1-t}.
% $$
% This expression represents the initial velocity required at point $x_t$ to travel to $x_1$ in the remaining time $1-t$ along a geodesic. This is precisely the instantaneous velocity of the constant-speed geodesic connecting $x_0$ and $x_1$ at the intermediate point $x_t$. This is the same quantity as the GeodesicFlow target velocity, $u_t^{\text{GF}} = P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1))$, which is defined by the same constant-speed property.

% In summary, while GeodesicFlow is formulated explicitly in terms of geodesic-specific operators, RFM arrives at the identical target vector field through its more general premetric framework when the premetric is chosen to be the geodesic distance. The primary distinction remains that RFM's framework extends naturally to non-geodesic paths, whereas GeodesicFlow is fundamentally tied to the manifold's "straightest lines."

% --------------------------
\section{Preliminaries: Riemannian Geometry}

Let $(\mathcal{M}, g)$ be a $d$-dimensional Riemannian manifold, possibly embedded in a high-dimensional ambient space $\mathbb{R}^D$ (e.g., via a VAE encoder), though no explicit embedding map $\iota$ is assumed or required for computation. All geometric operations are defined intrinsically with respect to the metric $g$, which governs lengths, angles, and geodesics on $\mathcal{M}$.

At each point $x \in \mathcal{M}$, the \textbf{tangent space} $T_x\mathcal{M}$ is a $d$-dimensional vector space encoding directions of infinitesimal movement on the manifold. In practice, we do not assume access to an explicit embedding Jacobian $J_\iota(x)$; instead, tangent vectors are represented intrinsically via local coordinates or learned projections.

The \textbf{Riemannian metric} $g_x : T_x\mathcal{M} \times T_x\mathcal{M} \to \mathbb{R}$ defines an inner product on tangent vectors. Rather than deriving it from an ambient Euclidean structure (which requires $J_\iota$), we approximate it directly via a symmetric positive-definite matrix $G_\phi(x) \in \mathbb{R}^{d \times d}$, parameterized by a neural network $\phi$:
\begin{equation}
    g_x(u, v) \approx u^\top G_\phi(x) v, \quad \text{for } u, v \in \mathbb{R}^d \text{ (local coordinates)}.
\end{equation}
This learned metric adapts to the local geometry of the latent manifold and avoids any dependence on intractable embedding Jacobians. The induced norm is $\|v\|_{g(x)} = \sqrt{v^\top G_\phi(x) v}$, which may vary across $\mathcal{M}$ to reflect curvature — e.g., stretching near semantically dense regions.

The \textbf{exponential map} $\exp_x: T_x\mathcal{M} \to \mathcal{M}$ maps a tangent vector $v$ to the endpoint of the geodesic starting at $x$ with initial velocity $v$. Its inverse, the \textbf{logarithmic map} $\log_x: \mathcal{M} \to T_x\mathcal{M}$, recovers the initial velocity required to reach $y \in \mathcal{M}$ along the geodesic, assuming $y$ lies within the injectivity radius of $x$. In practice, these maps can be approximated numerically or learned implicitly via neural ODEs or retractions.

A \textbf{geodesic} $\gamma_{x_0 \to x_1}(t) = \exp_{x_0}\big(t \cdot \log_{x_0}(x_1)\big)$, $t \in [0,1]$, is the shortest path between $x_0$ and $x_1$ under $g$. It satisfies $\nabla_{\dot{\gamma}} \dot{\gamma} = 0$, where $\nabla$ is the Levi-Civita connection induced by $g$.

\textbf{Parallel transport} $P_{\gamma, t_b \leftarrow t_a}: T_{\gamma(t_a)}\mathcal{M} \to T_{\gamma(t_b)}\mathcal{M}$ moves tangent vectors along $\gamma$ while preserving inner products under $g$. In implementation, we approximate parallel transport via Schild’s ladder or by learning a connection-compatible vector field. This enables consistent vector comparison across the manifold — essential for defining coherent velocity fields.

\section{GeodesicFlow: Geodesic Flow Matching}

We extend GeodesicFlow to the text-to-image generation on latent manifolds. Let $\mathcal{M}$ represent the latent manifold of image features (e.g., VAE encoder outputs), and $\mathcal{C}$ the space of text embeddings (e.g., CLIP). Our goal is to learn a time-dependent, text-conditioned vector field
\begin{equation}
    v_\Theta: \mathcal{M} \times [0,1] \times \mathcal{C} \to T\mathcal{M}, \quad \text{where } v_\Theta(x, t, c) \in T_x\mathcal{M},
\end{equation}
that transports a text-conditioned noise distribution $p_1(\cdot \mid c)$ to a text-conditioned data distribution $p_0(\cdot \mid c)$, for any text prompt $c \in \mathcal{C}$.

Unlike unconditional flows, our model leverages semantic structure to guide geodesic trajectories. At each time $t$, motion depends on location $x_t$, time $t$, and semantic context $c$, ensuring generated samples are geometrically natural and semantically aligned.

\subsection{Geodesic Probability Path and Target Velocity Field}

Given text embedding $c \in \mathcal{C}$, sample $x_0 \sim p_0(\cdot \mid c)$ (real image feature) and $x_1 \sim p_1(\cdot \mid c)$ (semantic-conditioned noise). The interpolation path is the \textbf{conditional geodesic}:
\begin{equation}
    z_t(c) = \exp_{x_0}\big(t \cdot \log_{x_0}(x_1)\big),
\end{equation}
the shortest path under $g$ connecting semantically consistent endpoints.

The \textbf{text-conditioned target velocity field} $u_t(z_t(c) \mid x_0, x_1, c)$ is the instantaneous velocity at $z_t(c)$, obtained by parallel transporting the initial logarithmic vector:
\begin{equation}
    u_t(z_t(c) \mid x_0, x_1, c) = P_{\gamma, t \leftarrow 0}\big(\log_{x_0}(x_1)\big).
\end{equation}
Although parallel transport depends only on $g$ and $\gamma$, the initial vector $\log_{x_0}(x_1)$ is influenced by $c$ through the conditional sampling of $x_0$ and $x_1$.

This ensures motion is semantically guided: for “a red apple on a wooden table,” the geodesic traverses regions encoding apples, redness, and tables — not generic noise.

\subsection{GeodesicFlow Objective}

We train $v_\Theta$ to match the target velocity under the learned Riemannian metric:
\begin{equation}
    \mathcal{L}_{\text{GF}}(\Theta, \phi) = \mathbb{E}_{\substack{t \sim \mathcal{U}[0,1], \\ c \sim p_c, \\ x_0 \sim p_0(\cdot \mid c), \\ x_1 \sim p_1(\cdot \mid c)}} \left[ \left\| v_\Theta(z_t(c), t, c) - u_t(z_t(c) \mid x_0, x_1, c) \right\|_{G_\phi(z_t(c))}^2 \right],
\end{equation}
where $\|v\|_{G_\phi(x)}^2 = v^\top G_\phi(x) v$, and $G_\phi(x)$ is a neural network that outputs a symmetric positive-definite matrix (e.g., via Cholesky parameterization or $LL^\top$).

Expanding:
\begin{equation}
    \mathcal{L}_{\text{GF}}(\Theta, \phi) = \mathbb{E}_{t, c, x_0, x_1} \left[ \left( \hat{u}_t - u_t \right)^\top G_\phi(z_t) \left( \hat{u}_t - u_t \right) \right],
\end{equation}
with $z_t = \exp_{x_0}(t \cdot \log_{x_0}(x_1))$, $\hat{u}_t = v_\Theta(z_t, t, c)$, and $u_t = P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1))$.

The network $v_\Theta$ takes:
\begin{itemize}
    \item A point $z_t \in \mathcal{M}$ (represented as a $d$-dim vector),
    \item Time $t \in [0,1]$,
    \item Text embedding $c \in \mathbb{R}^{d_c}$.
\end{itemize}
It outputs a tangent vector in local coordinates $ \mathbb{R}^d $, without requiring projection via Jacobians. We parameterize:
\begin{equation}
    v_\Theta(z, t, c) = f_\Theta\big(z,\, t,\, c \big) \in \mathbb{R}^d,
\end{equation}
where $f_\Theta$ is a neural network (e.g., U-Net or Transformer) operating directly in the latent space, with $c$ injected via cross-attention or FiLM. The output is interpreted as a tangent vector under the local chart at $z$, with metric $G_\phi(z)$.

\subsection{Generative Sampling via Geodesic Integration}

After training, generate from text $c$ by integrating backward:
\begin{equation}
    \frac{d z_t}{dt} = v_\Theta(z_t, t, c), \quad t \in [1, 0],
\end{equation}
starting from $z_1 \sim p_1(\cdot \mid c)$.

Numerically, use \textbf{conditional geodesic shooting}:
\begin{equation}
    z_{t-\Delta t} = \exp_{z_t}\big(-\Delta t \cdot v_\Theta(z_t, t, c)\big).
\end{equation}
The exponential map can be approximated via:
\begin{itemize}
    \item Retraction: $ \exp_x(v) \approx R_x(v) $, e.g., $ R_x(v) = x + v $ if $\mathcal{M}$ is locally Euclidean, or
    \item Neural geodesic approximation: Train a separate module to predict $\exp_x(v)$ from $(x, v)$.
\end{itemize}

The same $c$ is used throughout sampling, preserving semantic coherence without classifier-free guidance hacks. Conditioning is intrinsic to the velocity field, yielding geometrically faithful generations.

\subsection{Algorithmic Implementation: Learning and Sampling with Text-Geometric Fidelity}

Algorithms~\ref{alg:training_tcgeodesicflow} and~\ref{alg:sampling_tcgeodesicflow} operationalize \textbf{GeodesicFlow}: learning curvature-aware, semantically-guided transport where text steers geodesic paths — all without explicit Jacobians.

Training constructs geodesic interpolants between text-conditioned data and noise, computes target velocities via approximate parallel transport, and trains $v_\Theta$ and $G_\phi$ to match under the learned metric. Sampling uses the learned field to evolve noise into realistic, text-aligned images, respecting both manifold geometry and prompt semantics.

\begin{algorithm}[H]
\caption{Training GeodesicFlow (Jacobian-Free)}
\label{alg:training_tcgeodesicflow}
\begin{algorithmic}[1]
\Require
\item \textit{Model:} Neural networks $v_\Theta: \mathcal{M} \times [0,1] \times \mathcal{C} \to \mathbb{R}^d$ and $G_\phi: \mathcal{M} \to \mathbb{R}^{d \times d}$ (SPD).
\item \textit{Text Encoder:} Fixed $E: \text{Text} \to \mathcal{C} \subseteq \mathbb{R}^{d_c}$ (e.g., CLIP).
\item \textit{Data:} Dataset $\{(x_i, \text{caption}_i)\}_{i=1}^N$, inducing $p_0(\cdot \mid c)$ and $p_1(\cdot \mid c)$.
\item \textit{Manifold Ops:} Approximate $\log$, $\exp$, and $P$ (e.g., via retractions or learned modules).
\item \textit{Hyperparameters:} Batch size $B$, steps $N_{\text{steps}}$, learning rate $\alpha$.
\State Initialize $\Theta, \phi$.
\State Initialize optimizer (e.g., AdamW) with learning rate $\alpha$.
\For{step = 1 to $N_{\text{steps}}$}
    \State Sample mini-batch: $\{(\text{caption}^{(i)}, x_0^{(i)})\}_{i=1}^B$.
    \State Encode texts: $c^{(i)} \leftarrow E(\text{caption}^{(i)})$.
    \State Sample noise: $\{x_1^{(i)}\}_{i=1}^B \sim p_1(\cdot \mid c^{(i)})$.
    \State Sample times: $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
    \State Initialize batch loss $\mathcal{L}_{\text{batch}} \leftarrow 0$.
    \For{$i = 1$ to $B$}
        \State Let $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$, $c \leftarrow c^{(i)}$.
        \State Compute $v_0 \leftarrow \log_{x_0}(x_1)$ (approximate if needed).
        \State Compute $z_t \leftarrow \exp_{x_0}(t \cdot v_0)$.
        \State Compute $u_t \leftarrow P_{\gamma, t \leftarrow 0}(v_0)$ (approximate via Schild’s ladder or learning).
        \State Predict $\hat{u}_t \leftarrow v_\Theta(z_t, t, c) \in \mathbb{R}^d$.
        \State Compute metric $G_t \leftarrow G_\phi(z_t)$ (ensured SPD).
        \State Compute loss: $\mathcal{L}^{(i)} \leftarrow (\hat{u}_t - u_t)^\top G_t (\hat{u}_t - u_t)$.
        \State $\mathcal{L}_{\text{batch}} \leftarrow \mathcal{L}_{\text{batch}} + \mathcal{L}^{(i)}$.
    \EndFor
    \State Compute mean loss: $\mathcal{L} \leftarrow \frac{1}{B} \mathcal{L}_{\text{batch}}$.
    \State Update $\Theta, \phi \leftarrow \text{OptimizerStep}(\Theta, \phi, \nabla_{\Theta,\phi} \mathcal{L})$.
\EndFor
\State \Return Trained $\Theta, \phi$.
\end{algorithmic}
\end{algorithm}

\vspace{1cm}

\begin{algorithm}[H]
\caption{Sampling from Trained GeodesicFlow (Jacobian-Free)}
\label{alg:sampling_tcgeodesicflow}
\begin{algorithmic}[1]
\Require
\item \textit{Model:} Trained $v_\Theta$, $G_\phi$ (optional for sampling).
\item \textit{Text Encoder:} Fixed $E$.
\item \textit{Noise Distribution:} $p_1(\cdot \mid c)$ on $\mathcal{M}$.
\item \textit{Hyperparameter:} Steps $N$, retraction $R$ (if $\exp$ not available).
\State Input: $\text{prompt}$.
\State Encode: $c \leftarrow E(\text{prompt})$.
\State Sample: $z_1 \sim p_1(\cdot \mid c)$.
\State Set $\Delta t \leftarrow 1/N$.
\For{$k = N$ \textbf{down to} $1$}
    \State $t \leftarrow k \cdot \Delta t$.
    \State $\hat{u}_t \leftarrow v_\Theta(z_t, t, c)$.
    \State $z_{t-\Delta t} \leftarrow \exp_{z_t}(-\Delta t \cdot \hat{u}_t)$ \Comment{Use retraction $R_{z_t}(-\Delta t \cdot \hat{u}_t)$ if needed}.
\EndFor
\State \Return $z_0$ (decode to image if applicable).
\end{algorithmic}
\end{algorithm}


\begin{equation}
        z_t = \frac{\sin((1-t)\arccos(x_0 \cdot x_1))}{\sin(\arccos(x_0 \cdot x_1))}x_0 + \frac{\sin(t\arccos(x_0 \cdot x_1))}{\sin(\arccos(x_0 \cdot x_1))}x_1
\end{equation}

==> sec/method_lookahead_lookback.tex <==
% \section{Problem Statement}
% \label{sec:problem_statement}

\begin{figure}[h!]
  \centering
  % First subfigure
  \includegraphics[width=0.7\textwidth]{fig/geodesicflow_rho.pdf}
  \caption{Illustration of the intuition of $\rho$.}
  \label{fig:two-subfigs}
\end{figure}

\begin{figure}[h!]
  \centering
  % First subfigure
  \subfloat[]{
    \includegraphics[width=0.45\textwidth]{fig/illus_a.pdf}
  }
  \hfill
  % Second subfigure
  \subfloat[]{
    \includegraphics[width=0.45\textwidth]{fig/illus_b.pdf}
  }
  \caption{Schematic views of the proposed method. (a) Illustration of the training process for Riemannian Conditional Flow Matching (RCFM). On a Riemannian manifold $\mathcal{M}$, we sample a data point $x_0 \sim p_0$ and a noise point $x_1 \sim p_1$. The model is trained to make its predicted vector field $v_\Theta(z_t, t)$ match the target velocity $u_t$ of the geodesic path $\gamma(t)$ connecting the two points. The target $u_t$ lies in the tangent space $T_{z_t}\mathcal{M}$ at an interpolated point $z_t$. The loss is the squared norm of the difference between the predicted and target vectors, measured using the Riemannian metric at $z_t$. (b) Illustration of the generative sampling process. Starting from a point $z_1$ sampled from the noise distribution $p_1$, we numerically integrate the learned vector field $v_\Theta$ backward in time from $t=1$ to $t=0$. Each step is a ``geodesic shooting'' update, $z_{t-\Delta t} = \exp_{z_t}(-\Delta t \cdot v_\Theta(z_t, t))$, which moves the point along the manifold. This iterative process generates a trajectory that transforms the noise sample into a final point $z_0$, which is a new sample from the learned data distribution.}
  \label{fig:two-subfigs}
\end{figure}

% -------------------------
% Look-Ahead
\section{Problem Statement: Training-Free PC-LookAhead for Flow Sampling}
\label{sec:pc_lookahead_problem}

Let $p_0$ denote the data distribution and $p_1=\mathcal{N}(0,I)$ the noise prior.
A rectified-flow (or more generally, flow-based) generative model defines a probability path $(p_t)_{t\in[0,1]}$ governed by the ODE
\begin{equation}
\frac{d z_t}{dt} \;=\; v_\Theta(z_t,t,c), 
\qquad z_1 \!\sim p_1,\; z_0\!\sim p_0,
\label{eq:flow_ode}
\end{equation}
where $v_\Theta$ is a learned velocity field conditioned on (optional) context $c$.
Sampling integrates \eqref{eq:flow_ode} backward on a grid $1=t_0>\cdots>t_K=0$ with steps $\Delta_k = t_k - t_{k+1} > 0$.
A forward Euler (predictor-only) update reads
\begin{equation}
z_{k+1}^{\text{Eul}} \;=\; z_k \;-\; \eta_k\, v_\Theta(z_k,t_k,c),
\label{eq:euler}
\end{equation}
with step size $\eta_k$ (often proportional to $\Delta_k$).
However, near stiff or misaligned regions of the velocity field, \eqref{eq:euler} may overstep and degrade sample quality.

\paragraph{Goal.}
Design a \emph{training-free} look-ahead rule that (i) peeks one step into the future to assess local consistency of the velocity field, (ii) accepts large steps along straight (low-curvature) directions, and (iii) automatically shrinks steps when the field bends, while reducing to Euler when the field is consistent.

\section{Predictor--Corrector with a Curvature Gate}
\label{sec:pc_lookahead_method}

\subsection{Predictor and One-Step Peek}
At $(z_k,t_k)$ define the instantaneous velocity
\begin{equation}
v_k \;=\; v_\Theta(z_k,t_k,c).
\end{equation}
Take a tentative predictor (Euler) step
\begin{equation}
\tilde z \;=\; z_k \;-\; \eta_k\, v_k, 
\qquad \tilde t \;=\; t_k - \Delta_k,
\label{eq:predict}
\end{equation}
and \emph{peek} at the future velocity
\begin{equation}
\tilde v \;=\; v_\Theta(\tilde z,\tilde t,c).
\label{eq:peek}
\end{equation}

\subsection{Curvature Proxy and Acceptance Test}
We estimate a local curvature proxy by the discrete directional change of the field per unit displacement,
\begin{equation}
\kappa_k \;=\; 
\frac{\|\tilde v - v_k\|_2}{\|\tilde z - z_k\|_2 + \varepsilon}
\;=\;
\frac{\|v_\Theta(\tilde z,\tilde t,c) - v_\Theta(z_k,t_k,c)\|_2}{\eta_k\,\|v_k\|_2 + \varepsilon},
\label{eq:kappa}
\end{equation}
with a small $\varepsilon>0$ for numerical safety.
Intuitively, $\kappa_k$ upper-bounds a local Lipschitz constant of $v_\Theta$ along the trial move.
We accept the predictor if
\begin{equation}
\kappa_k \;\le\; \tau_{\mathrm{curv}},
\label{eq:gate}
\end{equation}
where $\tau_{\mathrm{curv}}>0$ is a user-chosen curvature threshold.
Otherwise we \emph{reject} and backtrack the step size.

\subsection{Adaptive Backtracking and Corrector}
If \eqref{eq:gate} fails, we shrink the step by a factor $\gamma\in(0,1)$ and retry:
\begin{equation}
\eta_k \leftarrow \gamma \,\eta_k,\qquad
\text{recompute }\tilde z,\tilde t,\tilde v,\kappa_k.
\label{eq:backtrack}
\end{equation}
We allow at most $B_{\max}$ backtracks per stage $k$.
Upon acceptance, the corrector simply commits the accepted predictor:
\begin{equation}
z_{k+1} \;=\; \tilde z,\qquad t_{k+1} \;=\; \tilde t.
\end{equation}

\subsection{Optional Schedule Coupling (SNR/Time-Aware)}
To better reflect training-time time-step exposure, one may modulate the \emph{attempted} step size via a schedule multiplier $g(t_k)\in(0,\infty)$:
\begin{equation}
\eta_k^{\mathrm{try}} \;=\; \eta_0\, g(t_k),
\label{eq:snr_scaled}
\end{equation}
where $g(\cdot)$ can be instantiated from the log-SNR or $t$-sampling distribution used during training.
The curvature gate (\S\ref{sec:pc_lookahead_method}) then guarantees safety by backtracking when $g$ is too aggressive locally.

\subsection{Properties and Complexity}
(i) \textbf{Reduction to Euler.} If $\tau_{\mathrm{curv}}=\infty$ or $\gamma=1$, PC-LookAhead reduces to Euler \eqref{eq:euler}.  
(ii) \textbf{Local stability.} Under a locally Lipschitz field with constant $L$, any $\tau_{\mathrm{curv}}\!\le\!L$ rejects steps whose directional change exceeds the prescribed curvature budget, acting as a trust-region proxy.  
(iii) \textbf{Compute.} Each acceptance attempt uses one extra model evaluation for the peek.
The worst case costs $B_{\max}\!+\!1$ evaluations per stage, while in smooth regions it is only $2$.

\section{Pseudo Algorithm}
\label{sec:algo}

\noindent\textbf{Inputs}:
trained field $v_\Theta(\cdot,\cdot,c)$, schedule $\{t_k\}_{k=0}^{K}$ with $\Delta_k=t_k-t_{k+1}$,
initial latent $z_0 \sim p_1$ at $t_0=1$,
initial step scale $\eta_0>0$,
curvature threshold $\tau_{\mathrm{curv}}>0$,
backtrack factor $\gamma\in(0,1)$,
maximum backtracks $B_{\max}\in\mathbb{N}$,
optional time multiplier $g(t)>0$.

\noindent\textbf{Output}: $z_K$ at $t_K=0$.

\begin{algorithm}[H]
\caption{Look-Ahead Sampling with Curvature Gate}
\label{alg:pc_lookahead}
\begin{algorithmic}[1]
\State $z \leftarrow z_0$, $t \leftarrow t_0$
\For{$k = 0,1,\dots,K-1$}
    \State $v \leftarrow v_\Theta(z,t,c)$
    \State $\eta \leftarrow \eta_0\, g(t)$ \Comment{use $g(t)\equiv 1$ if not scheduling}
    \State $\text{accepted} \leftarrow \text{false}$
    \For{$b = 0,1,\dots,B_{\max}$}
        \State $\tilde z \leftarrow z - \eta\, v$;\quad $\tilde t \leftarrow t - \Delta_k$
        \State $\tilde v \leftarrow v_\Theta(\tilde z,\tilde t,c)$
        \State $\kappa \leftarrow \dfrac{\|\tilde v - v\|_2}{\| \tilde z - z \|_2 + \varepsilon}$
        \If{$\kappa \le \tau_{\mathrm{curv}}$}
            \State $z \leftarrow \tilde z$;\quad $t \leftarrow \tilde t$;\quad $\text{accepted} \leftarrow \text{true}$;\quad \textbf{break}
        \Else
            \State $\eta \leftarrow \gamma\, \eta$ \Comment{backtrack and retry}
        \EndIf
    \EndFor
    \If{not $\text{accepted}$}
        \State $z \leftarrow z - \eta\, v$;\quad $t \leftarrow t - \Delta_k$ \Comment{fallback: smallest tried step}
    \EndIf
\EndFor
\State \textbf{return} $z$ \Comment{sample at $t=0$}
\end{algorithmic}
\end{algorithm}

% -------------------------
% SNR-Growth lookahead
\section{PI-Controlled Look-Ahead Sampling}
\label{sec:pi_lookahead}

When the learned velocity field $v_\Theta$ is nearly linear (low-curvature), 
a curvature-based gate provides limited adaptivity.
We thus adopt a simpler, more general strategy:
control the local \emph{numerical error} of the solver directly.

\subsection{Embedded Error Estimation}
At each step $(z_k,t_k)$, we compute both Euler and Heun (second-order) predictions:
\begin{align}
\tilde z^{\mathrm{Eul}} &= z_k - \eta_k\, v_\Theta(z_k,t_k,c), \\
\tilde v &= v_\Theta(\tilde z^{\mathrm{Eul}},\, t_k-\Delta_k, c), \\
\tilde z^{\mathrm{Heun}} &= z_k - \eta_k \,\tfrac{1}{2}\bigl(v_\Theta(z_k,t_k,c)+\tilde v\bigr).
\end{align}
The local error estimate is given by their difference:
\begin{equation}
e_k = 
\frac{\|\tilde z^{\mathrm{Heun}}-\tilde z^{\mathrm{Eul}}\|_2}
     {\|\tilde z^{\mathrm{Heun}}\|_2 + \varepsilon}.
\label{eq:error_est}
\end{equation}
If $e_k$ exceeds a tolerance $\tau_{\mathrm{err}}$, the step is rejected and retried with a smaller $\eta_k$.
Otherwise, the Heun estimate is accepted as $z_{k+1}$.

\subsection{PI Step-Size Controller}
After each accepted step, the next step size is updated using a 
proportional--integral (PI) rule:
\begin{equation}
\eta_{k+1} 
= \eta_k 
\left(\frac{e_\star}{e_k+\varepsilon}\right)^{\alpha}
\left(\frac{e_\star}{e_{k-1}+\varepsilon}\right)^{\beta},
\label{eq:pi_step}
\end{equation}
where $e_\star$ is the target error and $(\alpha,\beta)$ are controller gains
(e.g., $\alpha=0.7$, $\beta=0.1$).
This maintains stable progress: small errors increase step size, large errors reduce it.

\subsection{Algorithm}
\begin{algorithm}[H]
\caption{Look-Ahead Sampling with Embedded Error and PI Step Control}
\label{alg:pi_lookahead}
\begin{algorithmic}[1]
\State \textbf{Inputs:} $v_\Theta$, schedule $\{t_k\}$, $z_0\!\sim\!p_1$, initial step $\eta_0$, 
tolerance $\tau_{\mathrm{err}}$, target $e_\star$, gains $\alpha,\beta$, backtrack $\gamma$, safety $\varepsilon$.
\State $z\!\leftarrow\!z_0$, $t\!\leftarrow\!t_0$, $e_{-1}\!\leftarrow\!e_\star$
\For{$k=0,\dots,K-1$}
  \State $v \leftarrow v_\Theta(z,t,c)$
  \State accepted $\leftarrow$ false
  \For{$b=0,\dots,B_{\max}$}
     \State $\tilde z^{E}\!\leftarrow\! z-\eta_k\,v$, \quad $\tilde t\!\leftarrow\!t-\Delta_k$
     \State $\tilde v \!\leftarrow\! v_\Theta(\tilde z^{E},\tilde t,c)$
     \State $\tilde z^{H}\!\leftarrow\! z-\eta_k\tfrac{1}{2}(v+\tilde v)$
     \State $e \!\leftarrow\! \dfrac{\|\tilde z^{H}-\tilde z^{E}\|_2}{\|\tilde z^{H}\|_2+\varepsilon}$
     \If{$e \le \tau_{\mathrm{err}}$}
         \State $z\!\leftarrow\!\tilde z^{H}$, \quad $t\!\leftarrow\!\tilde t$, \quad accepted $\leftarrow$ true; \textbf{break}
     \Else
         \State $\eta_k \leftarrow \gamma\,\eta_k$ \Comment{backtrack}
     \EndIf
  \EndFor
  \If{not accepted}
     \State $z\!\leftarrow\!\tilde z^{H}$, \quad $t\!\leftarrow\!\tilde t$
  \EndIf
  \State \textit{PI update:}
  $\eta_{k+1}\!\leftarrow\!\eta_k
    \bigl(\tfrac{e_\star}{e+\varepsilon}\bigr)^{\alpha}
    \bigl(\tfrac{e_\star}{e_{k-1}+\varepsilon}\bigr)^{\beta}$;
  \quad $e_{k-1}\!\leftarrow\!e$
\EndFor
\State \textbf{return} $z$ \Comment{final sample at $t=0$}
\end{algorithmic}
\end{algorithm}

\subsection{Insights}
The embedded error (\ref{eq:error_est}) quantifies solver consistency between 
first- and second-order integration without relying on curvature.
The PI rule (\ref{eq:pi_step}) dynamically stabilizes step sizes, 
providing training-free adaptivity across both flat and stiff flow regions.
Together, they yield a lightweight yet robust alternative to curvature-based gating.




% --------------------------
% pi step-size
\section{PC--LookAhead with a PI Step-Size Controller}
\label{sec:pc_lookahead_pi}

\subsection{Predictor and One-Step Peek (unchanged)}
At $(z_k,t_k)$ define the instantaneous velocity
\begin{equation}
v_k \;=\; v_\Theta(z_k,t_k,c).
\end{equation}
Form a tentative Euler predictor and peek:
\begin{equation}
\tilde z \;=\; z_k - \eta_k\, v_k,\qquad 
\tilde t \;=\; t_k - \Delta_k,\qquad
\tilde v \;=\; v_\Theta(\tilde z,\tilde t,c).
\label{eq:predict_peek_pi}
\end{equation}

\subsection{Curvature (Bend) Proxy and Budget}
We measure local bend using the same directional change proxy but \emph{bind it to the step}:
\begin{equation}
\kappa_k \;=\; 
\frac{\|\tilde v - v_k\|_2}{\|\tilde z - z_k\|_2 + \varepsilon}
\;=\;
\frac{\|v_\Theta(\tilde z,\tilde t,c) - v_\Theta(z_k,t_k,c)\|_2}{\eta_k\|v_k\|_2 + \varepsilon}, 
\label{eq:kappa_pi}
\end{equation}
and define the (dimensionless) \emph{curvature budget consumption}
\begin{equation}
c_k \;\triangleq\; \eta_k\, \kappa_k.
\label{eq:budget_consumption}
\end{equation}
Intuitively, $c_k$ approximates the ``bend per step'' (arc-length times curvature). 
We target a user-set budget $c^\star>0$ so that straight segments ($c_k\!\ll\!c^\star$) speed up and bends ($c_k\!>\!c^\star$) slow down.

\subsection{PI Controller for Step Size}
Instead of discrete backtracking by a factor $\gamma$, 
we adapt $\eta_k$ continuously with a proportional–integral (PI) rule commonly used in adaptive ODE solvers:
\begin{equation}
\eta_{k+1}
\;=\;
\eta_k \;
\Biggl(\frac{c^\star}{c_k+\epsilon_c}\Biggr)^{\alpha}
\Biggl(\frac{c^\star}{c_{k-1}+\epsilon_c}\Biggr)^{\beta},
\qquad 
\alpha\in[0.5,0.8],\; 
\beta\in[0.2,0.5],
\label{eq:pi_update}
\end{equation}
with a small $\epsilon_c>0$ for numerical safety.
We also clamp the growth/shrinkage to prevent oscillations:
\begin{equation}
\eta_{k+1} 
\;\leftarrow\; 
\mathrm{clip}\!\left(\eta_{k+1},\; \rho_{\min}\,\eta_k,\; \rho_{\max}\,\eta_k\right),
\qquad 
0<\rho_{\min}<1<\rho_{\max}.
\label{eq:clamp}
\end{equation}
Typical defaults: 
$c^\star\!\in[0.05,0.2]$, $\alpha\!=\!0.7$, $\beta\!=\!0.3$, 
$(\rho_{\min},\rho_{\max})=(0.5,\,2.0)$, $\epsilon_c=10^{-8}$.

\paragraph{Commit.}
We \emph{always} commit the predictor once per stage:
\begin{equation}
z_{k+1} \;=\; \tilde z,\qquad t_{k+1} \;=\; \tilde t,
\end{equation}
and use $c_k$ to set $\eta_{k+1}$ via \eqref{eq:pi_update}–\eqref{eq:clamp}. 
No discrete accept/reject loop or $\gamma$ backtracking is needed.

\subsection{Insights and Justification}
\begin{itemize}
\item \textbf{Step sensitivity.} 
Gating on $c_k=\eta_k\kappa_k$ (rather than $\kappa_k$ alone) makes the control 
\emph{explicitly step-size sensitive}: shrinking $\eta_k$ reduces $c_k$, guaranteeing corrective leverage 
even when $\kappa_k$ is nearly step-invariant (e.g., when $\eta\!\propto\!\Delta_k$ or in equalized-curvature fields).

\item \textbf{PI stability from adaptive solvers.} 
The update $\eta_{k+1}=\eta_k(c^\star/c_k)^\alpha(c^\star/c_{k-1})^\beta$ 
is the standard PI controller used in embedded Runge–Kutta and variable-step ODE integrators; 
the ``integral'' term (via $c_{k-1}$) damps oscillations and yields smoother step trajectories 
than pure proportional control.

\item \textbf{Trust-region interpretation.} 
Bounding $c_k$ is a trust-region on ``bend per step.'' 
For locally Lipschitz fields with constant $L$, $c_k \lesssim \eta_k L$ 
controls the local linearization error of Euler and mitigates overstepping in stiff regions; 
straight segments naturally inflate $\eta$.

\item \textbf{Flux/rectified-flow compatibility.} 
When the path is already straight (Flux-style equalized curvature), 
$c_k$ stays below $c^\star$ and the controller increases $\eta$ toward $\rho_{\max}\eta_k$, 
recovering near-Euler costs ($\approx 2$ model calls per step) 
while remaining robust when bends occur (e.g., under strong guidance).

\item \textbf{Schedule-aware but not bound to $\Delta_k$.} 
We initialize $\eta_0$ with a time/SNR multiplier $g(t_0)$, 
but thereafter $\eta_k$ is \emph{free} to deviate from $\Delta_k$, 
removing the earlier degeneracy where $\Delta_k/\eta_k$ was constant.
\end{itemize}

\subsection{Algorithm}
\label{sec:algo_pi}
\noindent\textbf{Inputs}:
trained field $v_\Theta(\cdot,\cdot,c)$, schedule $\{t_k\}_{k=0}^{K}$ with $\Delta_k=t_k-t_{k+1}$,
initial latent $z_0\!\sim\!p_1$ at $t_0\!=\!1$;
controller targets $c^\star,\alpha,\beta,\rho_{\min},\rho_{\max},\epsilon_c$;
initial step $\eta_0>0$ (optionally $\eta_0=\eta_{\text{base}}\,g(t_0)$).

\noindent\textbf{Output}: $z_K$ at $t_K=0$.

\begin{algorithm}[H]
\caption{PC--LookAhead with PI Step-Size Control}
\label{alg:pc_lookahead_pi}
\begin{algorithmic}[1]
\State $z \leftarrow z_0$, $t \leftarrow t_0$, choose $\eta \leftarrow \eta_0$
\State Initialize $c_{\mathrm{prev}} \leftarrow c^\star$ \Comment{warm start for PI “integral”}
\For{$k = 0,1,\dots,K-1$}
    \State $v \leftarrow v_\Theta(z,t,c)$
    \State $\tilde z \leftarrow z - \eta\, v$;\quad $\tilde t \leftarrow t - \Delta_k$
    \State $\tilde v \leftarrow v_\Theta(\tilde z,\tilde t,c)$
    \State $\kappa \leftarrow \dfrac{\|\tilde v - v\|_2}{\|\tilde z - z\|_2 + \varepsilon}$;\quad $c \leftarrow \eta\,\kappa$
    \State \textbf{commit}:\; $z \leftarrow \tilde z$;\quad $t \leftarrow \tilde t$ \Comment{no backtracks}
    \State \textbf{PI update:}
    \[
      \eta_{\mathrm{new}} \leftarrow \eta\;
      \Bigl(\frac{c^\star}{c+\epsilon_c}\Bigr)^{\alpha}
      \Bigl(\frac{c^\star}{c_{\mathrm{prev}}+\epsilon_c}\Bigr)^{\beta}
    \]
    \State \textbf{Clamp:}\; $\eta_{\mathrm{new}} \leftarrow \mathrm{clip}\!\left(\eta_{\mathrm{new}},\; \rho_{\min}\eta,\; \rho_{\max}\eta\right)$
    \State $c_{\mathrm{prev}} \leftarrow c$;\quad $\eta \leftarrow \eta_{\mathrm{new}}$
\EndFor
\State \textbf{return} $z$
\end{algorithmic}
\end{algorithm}

\subsection{Complexity and Practical Notes}
\begin{itemize}
\item \textbf{Cost.} Exactly two model evaluations per stage ($v$ and $\tilde v$); no inner loops.
\item \textbf{Safeguards.} Use a hard floor/ceiling $\eta\in[\eta_{\min},\eta_{\max}]$. 
If $c$ spikes (rare), optionally cap $\eta_{\mathrm{new}}$ by a safety factor or halve once.
\item \textbf{Defaults.} $c^\star=0.1$, $\alpha=0.7$, $\beta=0.3$, 
$\rho_{\min}=0.5$, $\rho_{\max}=2.0$, $\epsilon_c=10^{-8}$, $\varepsilon=10^{-12}$.
\end{itemize}

By targeting the \emph{bend per step} $c_k=\eta_k\kappa_k$ and adapting $\eta$ with a PI controller, 
the method becomes step-size responsive, smooth, and robust. 
On already straight Flux-like trajectories it gracefully reduces to near-Euler behavior; 
where curvature emerges, it automatically decreases $\eta$ to maintain stability and sample quality—without discrete backtracking.


% \paragraph{Hyperparameter guidelines.}
% A numerically stable and effective default is
% $\tau_{\mathrm{curv}}\!\in\![0.3,1.0]$,
% $\gamma\!\in\![0.4,0.8]$,
% $B_{\max}\!\in\!\{2,3\}$,
% $\varepsilon\!=\!10^{-8}$,
% and $g(t)\equiv 1$ initially; then optionally tune $g(t)$ to be larger for early timesteps (low SNR) and smaller for late timesteps (high SNR).

% \paragraph{Implementation notes.}
% Compute $\Delta_k$ from the chosen $t$-grid; choose $\eta_0$ proportional to $\Delta_k$ or absorb $\Delta_k$ into $\eta_0$.
% Classifier-free guidance and other conditioning are applied consistently to both $v$ and $\tilde v$ evaluations.
% For multi-batch sampling, all quantities are vectorized and the backtracking loop runs with masked accepts.

% -----------------------
% EMA LookAhead
\section{Problem Statement: State-EMA Look-Ahead for Training-Free Flow Sampling}

Let $p_0$ denote the data distribution and $p_1=\mathcal{N}(0,I)$ the noise prior.  
A rectified-flow model defines a probability path $(p_t)_{t\in[0,1]}$ governed by the ODE
\begin{equation}
\frac{d z_t}{dt} = v_\Theta(z_t,t,c), 
\qquad z_1\!\sim p_1,\; z_0\!\sim p_0,
\label{eq:flow_ode}
\end{equation}
where $v_\Theta$ is the learned velocity field parameterized by a neural network.  
During sampling, $z_t$ is evolved backward from $t=1$ to $t=0$ using discrete steps 
$1=t_0>t_1>\cdots>t_K=0$.

Standard explicit solvers perform updates
\begin{equation}
z_{k+1} = z_k - \eta_k\,v_\Theta(z_k,t_k,c),
\label{eq:euler}
\end{equation}
which may accumulate stochastic noise and numerical oscillations—especially when the 
log-SNR schedule induces stiffness near mid-range timesteps.

We therefore introduce a \textbf{State-EMA Look-Ahead} mechanism that adaptively smooths latent trajectories 
through exponential averaging and look-ahead blending, improving stability and visual fidelity 
without retraining or modifying $v_\Theta$.

\section{Methodology}

\subsection{Exponential State Averaging}

We maintain an exponentially weighted average of previous latent states:
\begin{equation}
\bar z_k = \gamma(t_k)\,\bar z_{k-1} + \bigl(1-\gamma(t_k)\bigr)\, z_k,
\quad \bar z_{-1}=z_0,
\label{eq:ema_state}
\end{equation}
where $\gamma(t)\!\in\![0,1)$ is a time- or SNR-dependent decay coefficient.
The averaged state $\bar z_k$ serves as a low-variance memory of the trajectory, filtering out transient noise while retaining the coarse structure of the flow dynamics.
As $\gamma(t)$ decays, $\bar z_k$ becomes more sensitive to the current state, ensuring the EMA influence vanishes near convergence.

\subsection{Look-Back Blending (Backward Referenced, Forward Stabilizing)}

Although the following formulation reuses the term ``look-ahead,'' the mechanism is in fact a
\emph{look-back blend}: the model velocity is evaluated not at the instantaneous state $z_k$,
but at a mixture between $z_k$ and its past-averaged counterpart $\bar z_{k-1}$:
\begin{equation}
z_k^{\text{look}} = (1-\lambda)\,z_k + \lambda\,\bar z_{k-1},
\qquad \lambda\in[0,1].
\label{eq:lookahead}
\end{equation}
Here, $\bar z_{k-1}$ encodes a smoothed history of recent latent states, providing a
low-frequency estimate of the trajectory’s long-term trend.
Although the construction references the past, its effect is \emph{forward-stabilizing}:
the blended latent anticipates the slow manifold toward which the trajectory is converging.
This stabilizes velocity evaluation and mitigates overshooting or oscillatory motion
in stiff regions of the learned flow field.

The corresponding update is performed as
\begin{equation}
z_{k+1} = z_k - \eta_k\,v_\Theta(z_k^{\text{look}},t_k,c),
\label{eq:update}
\end{equation}
where $v_\Theta$ is the learned velocity field.
Thus, the “look-back” blending acts as an implicit damping mechanism—regularizing updates
toward the smoothed trajectory $\bar z_{k}$—while preserving the unbiased geometry of the
original flow manifold.

\subsection{SNR-Aware Decay Scheduling}

To preserve flow consistency near the data manifold where rectified flows remain strong,
we modulate $\gamma(t)$ using a logistic decay function governed by the log-SNR:
\begin{equation}
\gamma(t) = \gamma_{\max}\cdot\sigma\!\Big(a[\lambda(t)-\lambda_\ast]\Big),
\label{eq:gamma}
\end{equation}
% where $\sigma$ is the sigmoid function, $\lambda(t)=\log(a_t^2/b_t^2)$ denotes the log-SNR,
% and $\lambda_\ast$ marks the midpoint of maximal uncertainty.
% When $\lambda(t) < \lambda_\ast$, the decay $\gamma(t)$ remains large,
% enabling strong temporal smoothing in noisy regions; as $\lambda(t)\!\to\!\infty$,
% $\gamma(t)\!\to\!0$, gradually disabling EMA near convergence.
% This SNR-aware design ensures that the look-back mechanism operates only when uncertainty
% is high and naturally reverts to the vanilla ODE solver in deterministic regions.
% 
where $\sigma$ is the sigmoid function, and $\lambda(t)=\log(a_t^2/b_t^2)$ denotes the log–SNR computed from the signal and noise coefficients of the generative process.
Specifically, $z_t = a_t x_0 + b_t \epsilon$ with $\epsilon\!\sim\!\mathcal{N}(0,I)$.
For rectified flows, we adopt $a_t = 1-t$ and $b_t = t$, yielding $\lambda(t) = 2\log\!\frac{1-t}{t}$.
For diffusion models, $a_t=\sqrt{\bar{\alpha}_t}$ and $b_t=\sqrt{1-\bar{\alpha}_t}$, giving $\lambda(t)=\log(\bar{\alpha}_t/(1-\bar{\alpha}_t))$.
Moreover, $\lambda_\ast$ marks the midpoint of maximal uncertainty.
When $\lambda(t) < \lambda_\ast$, the decay $\gamma(t)$ remains large,
enabling strong temporal smoothing in noisy regions; as $\lambda(t)\!\to\!\infty$,
$\gamma(t)\!\to\!0$, gradually disabling EMA near convergence.
This SNR-aware design ensures that the look-back mechanism operates only when uncertainty
is high and naturally reverts to the vanilla ODE solver in deterministic regions.

\section{Intuition and Insights}

\paragraph{Backward Referenced, Forward Stabilizing.}
The look-back blend references past information but stabilizes future evolution.
By interpolating between the current state and a smoothed historical baseline,
the sampler anticipates the stable manifold of the flow,
damping high-frequency oscillations while maintaining correct long-term dynamics.

\paragraph{Noise-Averaged Stability.}
Exponential state averaging suppresses transient jitter in latent updates,
particularly in mid-range timesteps with high stochastic variance.
This leads to smoother latent trajectories and improved numerical stability
under both diffusion and rectified flow dynamics.

\paragraph{Training-Free Compatibility.}
The method is applied purely during inference, introducing no additional training cost or parameters.
It is directly compatible with standard ODE solvers (Euler, Heun, DPMSolver, etc.)
and seamlessly integrates into both diffusion and flow-matching pipelines.

\section{Algorithm}

\begin{algorithm}[H]
\caption{Look-Back Sampling for Flow Models}
\begin{algorithmic}[1]
\Require $v_\Theta$, schedule $\{(t_k,\eta_k)\}_{k=0}^{K-1}$, decay $\gamma(t)$, blend $\lambda$, condition $c$
\State $z_0 \sim \mathcal{N}(0,I)$; $\bar z_{-1} \gets z_0$
\For{$k = 0$ to $K-1$}
  \State $\bar z_k \gets \gamma(t_k)\,\bar z_{k-1} + \bigl(1-\gamma(t_k)\bigr)\,z_k$
  \State $z_k^{\text{look}} \gets (1-\lambda)\,z_k + \lambda\,\bar z_{k-1}$
  \State $v_k \gets v_\Theta\!\bigl(z_k^{\text{look}}, t_k, c\bigr)$
  \State $z_{k+1} \gets z_k - \eta_k\, v_k$
\EndFor
\State \Return $z_K$
\end{algorithmic}
\end{algorithm}

% \section{Methodology}

% \subsection{State-EMA Look-Ahead Framework}

% The proposed \textbf{State-EMA Look-Ahead} framework augments any diffusion or flow-matching sampler with an adaptive state-smoothing and look-ahead mechanism. It wraps the base scheduler (e.g., Euler, Heun, DPMSolver, FlowMatch) without retraining or altering model parameters, and operates fully during inference.

% Formally, for a latent trajectory $\{z_k\}$ evolving under the learned velocity field $v_\Theta(z_k,t_k,c)$, the method introduces an exponentially averaged latent state $\bar z_k$ and a look-ahead blended state $z_k^{\text{look}}$ used for evaluating the next-step velocity. Both components are computed adaptively with respect to the signal-to-noise ratio (SNR) of each timestep.

% \subsection{Exponential State Averaging}

% At each step $k$, we maintain an exponential moving average (EMA) of latent states:
% \begin{equation}
% \bar z_k = \gamma(t_k)\,\bar z_{k-1} + \bigl(1-\gamma(t_k)\bigr)\,z_k,
% \quad \bar z_{-1} = z_0.
% \label{eq:ema_state}
% \end{equation}
% The decay factor $\gamma(t)$ modulates temporal smoothing strength and is dynamically computed via a logistic SNR-based schedule:
% \begin{equation}
% \gamma(t) = \gamma_{\max}\cdot\sigma\!\Bigl(a\,[\lambda(t)-\lambda_\ast]\Bigr),
% \qquad 
% \sigma(x) = \frac{1}{1+e^{-x}},
% \label{eq:gamma_schedule}
% \end{equation}
% where $\lambda(t)$ denotes the log-SNR at timestep $t$, $\lambda_\ast$ is the midpoint of maximum uncertainty, $a$ controls steepness, and $\gamma_{\max}$ is the maximal decay coefficient (typically $0.9$–$0.99$).  
% As $t\!\to\!0$, the SNR grows and $\gamma(t)\!\to\!0$, naturally deactivating the EMA effect near convergence.

% \subsection{Look-Ahead Blending for Velocity Evaluation}

% Before evaluating the model velocity, a look-ahead blending step forms an intermediate latent:
% \begin{equation}
% z_k^{\text{look}} = (1-\lambda)\,z_k + \lambda\,\bar z_{k-1},
% \qquad \lambda \in [0,1],
% \label{eq:lookahead}
% \end{equation}
% where $\lambda$ is a fixed blending ratio controlling the trade-off between the instantaneous state and the smoothed trajectory.  
% This look-ahead state acts as a variance-reduced proxy for $z_k$, stabilizing the direction of $v_\Theta(z,t,c)$ in regions of high curvature or noise. The velocity is then evaluated as
% \begin{equation}
% v_k = v_\Theta\!\bigl(z_k^{\text{look}}, t_k, c\bigr),
% \label{eq:velocity}
% \end{equation}
% and the update follows a standard explicit solver step (e.g., Euler):
% \begin{equation}
% z_{k+1} = z_k - \eta_k\, v_k.
% \label{eq:update}
% \end{equation}
% In implementation, the wrapper intercepts each scheduler step, storing both the previous and current $\bar z$ to ensure $z_k^{\text{look}}$ correctly references $\bar z_{k-1}$, consistent with Eq.~\eqref{eq:ema_state}–\eqref{eq:lookahead}.

% \subsection{Integration into Diffusion and Flow Pipelines}

% The State-EMA Look-Ahead is implemented as a lightweight wrapper over any scheduler or full pipeline:
% \begin{itemize}
%   \item \textbf{Scheduler-level:} The wrapper modifies the scheduler’s \texttt{step()} method by updating $\bar z_k$ and replacing the raw latent $z_k$ with the look-ahead blend before passing it to the base scheduler.
%   \item \textbf{Pipeline-level:} For systems like \texttt{StableDiffusion3Pipeline}, a higher-level wrapper intercepts the sampling loop to ensure that look-ahead blending occurs prior to velocity evaluation when supported.
% \end{itemize}
% This modular integration preserves compatibility with existing diffusion and flow-matching implementations while enabling training-free stabilization.

% \section{Intuition and Insights}

% \paragraph{SNR-Adaptive Temporal Filtering.}  
% The EMA term suppresses transient oscillations by smoothing latent trajectories more strongly when stochastic noise dominates (low SNR) and gradually vanishing as the model approaches the deterministic data manifold.

% \paragraph{Implicit Regularization and Damping.}  
% The look-ahead blend implicitly regularizes the trajectory akin to Polyak averaging or momentum damping. It aligns updates toward the long-term mean trajectory $\bar z_{k}$, effectively controlling over-stepping without distorting the learned flow geometry.

% \paragraph{Training-Free Generality.}  
% The mechanism introduces no additional training cost, parameters, or architectural changes. It operates entirely during inference and can be combined seamlessly with ODE- or SDE-based solvers (Euler, Heun, DPMSolver, UniPC, etc.), including both rectified-flow and diffusion-ODE frameworks.

% \section{Algorithm}

% \begin{algorithm}[H]
% \caption{State-EMA Look-Ahead Sampling for Diffusion and Flow Models}
% \begin{algorithmic}[1]
% \Require $v_\Theta$, schedule $\{(t_k,\eta_k)\}_{k=0}^{K-1}$, decay function $\gamma(t)$, blend ratio $\lambda$, condition $c$
% \State $z_0 \sim \mathcal{N}(0,I)$; $\bar z_{-1} \gets z_0$
% \For{$k = 0$ to $K-1$}
%   \State $\gamma_k \gets \gamma(t_k)$
%   \State $\bar z_k \gets \gamma_k\,\bar z_{k-1} + (1-\gamma_k)\,z_k$
%   \State $z_k^{\text{look}} \gets (1-\lambda)\,z_k + \lambda\,\bar z_{k-1}$
%   \State $v_k \gets v_\Theta(z_k^{\text{look}}, t_k, c)$
%   \State $z_{k+1} \gets z_k - \eta_k\,v_k$
% \EndFor
% \State \Return $z_K$
% \end{algorithmic}
% \end{algorithm}


% \section{Methodology}

% \subsection{Exponential State Averaging}

% We maintain an exponentially weighted average of previous latent states:
% \begin{equation}
% \bar z_k = \gamma(t_k)\,\bar z_{k-1} + \bigl(1-\gamma(t_k)\bigr)\, z_k,
% \quad \bar z_{-1}=z_0,
% \label{eq:ema_state}
% \end{equation}
% where $\gamma(t)\!\in\![0,1)$ is a time- or SNR-dependent decay coefficient.
% The averaged state $\bar z_k$ tracks a low-variance version of the current trajectory, filtering out 
% transient high-frequency errors in stiff regions.

% \subsection{Look-Ahead Blending for Velocity Evaluation}

% At each step, the model velocity is evaluated not at the raw $z_k$ but at a look-ahead blend 
% between the current and smoothed states:
% \begin{equation}
% z_k^{\text{look}} = (1-\lambda)\,z_k + \lambda\,\bar z_{k-1}, 
% \qquad \lambda\in[0,1],
% \label{eq:lookahead}
% \end{equation}
% followed by the update
% \begin{equation}
% z_{k+1} = z_k - \eta_k\,v_\Theta(z_k^{\text{look}},t_k,c).
% \label{eq:update}
% \end{equation}

% This formulation introduces an implicit damping effect similar to Polyak averaging:  
% the trajectory direction is corrected toward the long-term mean $\bar z_k$, mitigating local overshooting 
% without biasing the global flow manifold.

% \subsection{SNR-Aware Decay Scheduling}

% To preserve flow consistency near the data manifold where rectified flows remain strong,  
% we decay $\gamma(t)$ smoothly to zero as the signal-to-noise ratio increases:
% \begin{equation}
% \gamma(t) = \gamma_{\max}\cdot\sigma\!\Big(a[\lambda(t)-\lambda_\ast]\Big),
% \label{eq:gamma}
% \end{equation}
% where $\sigma$ is the logistic function, $\lambda(t)=\log(a_t^2/b_t^2)$ is the log-SNR schedule, 
% and $\lambda_\ast$ marks the midpoint of maximal stochasticity.  
% This ensures the EMA effect is active only during the uncertain mid-range timesteps 
% and vanishes near $t\!\to\!0$, thus reverting to the vanilla solver at convergence.

% \section{Intuition and Insights}

% \paragraph{Noise-Averaged Stability.}  
% By exponentially smoothing states, the method reduces variance in both latent positions 
% and induced velocities, mitigating jitter from stiff regions where small changes in $z_k$ 
% cause large fluctuations in $v_\Theta$.

% \paragraph{Implicit Regularization.}  
% The look-ahead blend functions as a temporal low-pass filter:  
% instead of following the instantaneous velocity field, the sampler tracks a 
% \emph{momentum-averaged direction}, yielding smoother geometry while retaining 
% the curvature information of rectified flows.

% \paragraph{Training-Free Compatibility.}  
% Unlike weight-EMA used during training, this approach operates purely at inference, 
% requiring no extra parameters or retraining.  
% It is compatible with all ODE-based samplers (Euler, Heun, DPMSolver) 
% and directly complements rectified-flow and diffusion-ODE frameworks.

% \section{Algorithm}

% \begin{algorithm}
% \caption{State-EMA Look-Ahead Sampling for Rectified Flow Models}
% \begin{algorithmic}[1]
% \Require $v_\Theta$, schedule $\{(t_k,\eta_k)\}_{k=0}^{K-1}$, decay $\gamma(t)$, blend $\lambda$, condition $c$
% \State $z_0 \sim \mathcal{N}(0,I)$; $\bar z_{-1} \gets z_0$
% \For{$k = 0$ to $K-1$}
%   \State $\bar z_k \gets \gamma(t_k)\,\bar z_{k-1} + \bigl(1-\gamma(t_k)\bigr)\,z_k$
%   \State $z_k^{\text{look}} \gets (1-\lambda)\,z_k + \lambda\,\bar z_{k-1}$
%   \State $v_k \gets v_\Theta\!\bigl(z_k^{\text{look}}, t_k, c\bigr)$
%   \State $z_{k+1} \gets z_k - \eta_k\, v_k$
% \EndFor
% \State \Return $z_K$
% \end{algorithmic}
% \end{algorithm}

% \section{Practical Guidelines}

% We recommend $\lambda\!\in\![0.3,0.7]$, $\gamma_{\max}\!\approx\!0.9$, and 
% decaying $\gamma(t)\!\to\!0$ for the last 20--30\% of timesteps.  
% This method can also be combined with predictor--corrector schemes or adaptive-step 
% integrators for improved stability and sample quality.

% \medskip
% The proposed \textbf{State-EMA Look-Ahead} thus serves as a lightweight, training-free 
% stabilization mechanism aligned with the rectified-flow design philosophy—preserving its 
% curvature-guided transport while enhancing sampling robustness.

% --------------------------
% Generalizing look-ahead to rectified diffusion
\section{Generalizing PC--LookAhead to Rectified Diffusion ( $\epsilon$-Prediction \& SNR Gate)}
\label{sec:pc_lookahead_rd_eps}

Rectified Diffusion (RD) supports arbitrary prediction heads (e.g., $\epsilon$-, $x_0$-, $v$-prediction) with simple reparameterizations while preserving the pretrained diffusion scheduler $x_t=\alpha_t x_0+\sigma_t\epsilon$ \cite{rd_general, rd_subset, rd_first_order}. 
Here we instantiate PC--LookAhead under \emph{$\epsilon$-prediction} and replace the curvature gate with an \emph{SNR-gated} acceptance rule.

\paragraph{Epsilon head and SNR.}
Let the model predict $\epsilon_\Theta(x_t,t,c)$ (standard diffusion training form) \cite{rd_eps_train}. 
Define the (log) signal-to-noise ratio
\[
\lambda(t)\;=\;\log\!\frac{\alpha_t}{\sigma_t}, 
\qquad \mathrm{SNR}(t)\;=\;\frac{\alpha_t^2}{\sigma_t^2}\;=\;e^{2\lambda(t)}.
\]
RD guarantees a first-order ODE trajectory for $x_t$ under this diffusion form, so we can run one/few/many steps along the same deterministic path without changing the network or scheduler \cite{rd_first_order, rd_general}. 
We do not need the explicit closed-form field here; it suffices that \emph{a deterministic RD field exists} and can be queried via the $\epsilon$ head and the scheduler \cite{rd_first_order}.

\paragraph{SNR-gated look-ahead (intuition).}
When integrating backward (from small SNR to large SNR), too aggressive time steps can \emph{jump} across SNR bands where the PF-ODE is stiff for $\epsilon$-prediction. 
We therefore gate acceptance by how much the step increases $\lambda$:
\[
\Delta\lambda_{\text{try}} \;=\; \bigl|\lambda(t_k)-\lambda(t_{k+1})\bigr|.
\]
If $\Delta\lambda_{\text{try}}$ exceeds a budget $\tau_{\mathrm{snr}}$, we backtrack the step size (trust-region behavior in SNR space). 
Optionally, we add an \emph{$x_0$-consistency} check derived from the $\epsilon$ head:
\begin{align*}
    \widehat{x}_0(x_t,t) \;=\; \frac{x_t - \sigma_t\,\epsilon_\Theta(x_t,t,c)}{\alpha_t},
\\
\rho_k \;=\; \frac{\bigl\|\widehat{x}_0(\tilde x,\tilde t)-\widehat{x}_0(x_k,t_k)\bigr\|_2}{\bigl\|\widehat{x}_0(x_k,t_k)\bigr\|_2 + \varepsilon}.
\end{align*}
Accepting only when $\Delta\lambda_{\text{try}}\le \tau_{\mathrm{snr}}$ (and, if enabled, $\rho_k\le \tau_{\mathrm{cons}}$) preserves stability while remaining head/schedule consistent \cite{rd_general, rd_subset}.

\subsection{Algorithm: PC--LookAhead ( $\epsilon$-Prediction, SNR Gate )}
\label{sec:algo_rd_eps}

\noindent\textbf{Inputs}: schedule $\{t_k\}_{k=0}^{K}$ with $\Delta_k=t_k-t_{k+1}$; $(\alpha_t,\sigma_t)$; 
initial $x_0\!\sim\mathcal{N}(0,I)$ at $t_0{=}1$; 
base step scale $\eta_0{>}0$; 
SNR threshold $\tau_{\mathrm{snr}}{>}0$; 
optional consistency threshold $\tau_{\mathrm{cons}}{>}0$; 
backtrack factor $\gamma\!\in\!(0,1)$; 
max backtracks $B_{\max}\!\in\!\mathbb{N}$; 
optional time/log-SNR multiplier $g(t){>}0$.

\noindent\textbf{Output}: $x_K$ at $t_K{=}0$.

\begin{algorithm}[H]
\caption{PC--LookAhead for RD with $\epsilon$-Prediction and SNR Gate}
\label{alg:pc_lookahead_rd_eps}
\begin{algorithmic}[1]
\State $x \leftarrow x_0$, $t \leftarrow t_0$
\For{$k = 0,1,\dots,K-1$}
    \State $\epsilon \leftarrow \epsilon_\Theta(x,t,c)$
    \State $\eta \leftarrow \eta_0\, g(t)$ \Comment{$g(t)\!\equiv\!1$ if not scheduling}
    \State $\text{accepted} \leftarrow \text{false}$
    \For{$b = 0,1,\dots,B_{\max}$}
        \State $\tilde t \leftarrow t - \Delta_k$ \Comment{proposed next time}
        \State $\Delta\lambda_{\text{try}} \leftarrow \bigl|\lambda(t)-\lambda(\tilde t)\bigr|$ \Comment{SNR step size}
        \State \textbf{if} $\Delta\lambda_{\text{try}} > \tau_{\mathrm{snr}}$ \textbf{ then } $\eta \!\leftarrow\! \gamma\,\eta$; \textbf{continue} \Comment{backtrack in SNR space}
        \State $\tilde x \leftarrow x - \eta\, f_{\text{RD}}(x,t,\epsilon)$ \Comment{predictor via RD first-order field}
        \State $\tilde \epsilon \leftarrow \epsilon_\Theta(\tilde x,\tilde t,c)$ \Comment{one-step peek}
        \If{consistency check enabled}
            \State $\widehat{x}_0 \leftarrow \dfrac{x - \sigma_t\,\epsilon}{\alpha_t}$;\quad
                   $\widehat{x}_0^{\,\mathrm{peek}} \leftarrow \dfrac{\tilde x - \sigma_{\tilde t}\,\tilde \epsilon}{\alpha_{\tilde t}}$
            \State $\rho \leftarrow \dfrac{\bigl\|\widehat{x}_0^{\,\mathrm{peek}}-\widehat{x}_0\bigr\|_2}{\bigl\|\widehat{x}_0\bigr\|_2+\varepsilon}$
            \If{$\rho > \tau_{\mathrm{cons}}$}
                \State $\eta \leftarrow \gamma\,\eta$; \textbf{continue} \Comment{backtrack on $x_0$-consistency}
            \EndIf
        \EndIf
        \State $x \leftarrow \tilde x$;\quad $t \leftarrow \tilde t$;\quad $\text{accepted} \leftarrow \text{true}$;\quad \textbf{break}
    \EndFor
    \If{not $\text{accepted}$}
        \State $x \leftarrow x - \eta\, f_{\text{RD}}(x,t,\epsilon)$;\quad $t \leftarrow t - \Delta_k$ \Comment{fallback}
    \EndIf
\EndFor
\State \textbf{return} $x$
\end{algorithmic}
\end{algorithm}


==> sec/method_options.tex <==
\section{Problem Formulation: Knowledge Consolidation in Rectified Flow Models}
\label{sec:problem_formulation}

Let $\mathcal{D}_{\text{target}} = \{(x_0^{(i)}, c^{(i)})\}_{i=1}^{N}$ denote a target dataset of image--caption pairs, where $x_0^{(i)} \in \mathbb{R}^{H \times W \times 3}$ is a high-resolution image and $c^{(i)}$ its associated text prompt. Our goal is to train a rectified flow model with velocity field $v_\Theta : \mathbb{R}^d \times [0,1] \to \mathbb{R}^d$, parameterized by weights $\Theta$, that generates samples by solving the ODE
\begin{equation}
    \frac{d y_t}{dt} = v_\Theta(y_t, t), \quad y_1 \sim \mathcal{N}(0, I),
\end{equation}
such that $y_0 \approx x_0$ for $x_0 \sim p_0^{\text{target}}$, the data distribution induced by $\mathcal{D}_{\text{target}}$.

Suppose we are given a collection of $K$ pretrained rectified flow models $\{v_{\Theta^{(k)}}\}_{k=1}^K$, each trained on a distinct source domain $\mathcal{D}^{(k)}$ (e.g., artistic styles, object-centric datasets, or synthetic captions). These models are publicly available (e.g., on Hugging Face) and may differ in architecture, conditioning mechanism, or latent space.

We define the \emph{knowledge consolidation} objective as the joint optimization of:
\begin{enumerate}
    \item fidelity to the target data distribution via the Conditional Flow Matching (CFM) loss~\cite{Lipman2023}:
    \begin{equation}
        \mathcal{L}_{\text{target}}(\Theta) = \mathbb{E}_{\substack{t \sim \pi(t) \\ x_0 \sim p_0^{\text{target}} \\ \epsilon \sim \mathcal{N}(0,I)}} \left[ \left\| v_\Theta(z_t, t) - (\epsilon - x_0) \right\|^2 \right],
    \end{equation}
    where $z_t = (1 - t)x_0 + t\epsilon$ and $\pi(t)$ is a timestep weighting (e.g., logit-normal as in Section~3.1 of the paper);
    
    \item transfer of relevant knowledge from source models via a consolidation regularizer:
    \begin{equation}
        \mathcal{L}_{\text{consolidate}}(\Theta; \{\Theta^{(k)}\}) = \sum_{k=1}^K w_k \cdot \mathcal{D}\big( v_\Theta(\cdot, \cdot), v_{\Theta^{(k)}}(\cdot, \cdot) \big),
    \end{equation}
    where $w_k \geq 0$ quantifies the relevance of source $k$ to $\mathcal{D}_{\text{target}}$, and $\mathcal{D}(\cdot,\cdot)$ is a discrepancy measure (e.g., feature-space MSE, attention map alignment, or trajectory divergence in a shared latent space).
\end{enumerate}

The consolidated training objective is then:
\begin{equation}
    \Theta^* = \arg\min_{\Theta} \; \mathcal{L}_{\text{target}}(\Theta) + \lambda \cdot \mathcal{L}_{\text{consolidate}}(\Theta; \{\Theta^{(k)}\}),
\end{equation}
where $\lambda \geq 0$ balances data fidelity and knowledge transfer.

This formulation assumes that architectural or representational alignment (e.g., via a shared VAE encoder or modality-specific token streams as in the MM-DiT architecture~\cite{ScalingRectifiedFlow}) enables meaningful comparison between $v_\Theta$ and $\{v_{\Theta^{(k)}}\}$. The ultimate aim is to accelerate convergence, improve sample quality, and enhance compositional generalization (e.g., typography, spatial reasoning) by leveraging the collective knowledge of heterogeneous pretrained flow models.


\section{Problem Formulation: Loss-Aware Knowledge Consolidation in Rectified Flow Models}
\label{sec:problem_formulation}

Let $\mathcal{D}_{\text{target}} = \{(x_0^{(i)}, c^{(i)})\}_{i=1}^{N}$ denote a target dataset of image--caption pairs, where $x_0^{(i)} \in \mathbb{R}^{H \times W \times 3}$ is a high-resolution image and $c^{(i)}$ its associated text prompt. Our goal is to fine-tune a rectified flow model with velocity field $v_\Theta : \mathbb{R}^d \times [0,1] \to \mathbb{R}^d$, parameterized by weights $\Theta$, that generates samples by solving the ODE
\begin{equation}
    \frac{d y_t}{dt} = v_\Theta(y_t, t), \quad y_1 \sim \mathcal{N}(0, I),
\end{equation}
such that $y_0 \approx x_0$ for $x_0 \sim p_0^{\text{target}}$, the data distribution induced by $\mathcal{D}_{\text{target}}$.

We are given a collection of $K$ pretrained rectified flow models $\{v_{\Theta^{(k)}}\}_{k=1}^K$, each trained on a distinct source domain $\mathcal{D}^{(k)}$ (e.g., artistic styles, object-centric datasets, or synthetic captions). These models are fixed during training (i.e., no backpropagation through them), but we can evaluate their performance on samples from the target domain.

For any data point $(x_0, c) \in \mathcal{D}_{\text{target}}$, timestep $t \sim \pi(t)$, and noise $\epsilon \sim \mathcal{N}(0, I)$, define the intermediate point $z_t = (1 - t)x_0 + t\epsilon$. The Conditional Flow Matching (CFM) loss for the target model is:
\begin{equation}
    \ell_{\text{target}}(x_0, t, \epsilon; \Theta) = \left\| v_\Theta(z_t, t, c) - (\epsilon - x_0) \right\|^2.
\end{equation}

Similarly, for each source model $k$, we compute its (frozen) loss on the same $(x_0, t, \epsilon, c)$:
\begin{equation}
    \ell^{(k)}(x_0, t, \epsilon, c) = \left\| v_{\Theta^{(k)}}(z_t, t, c) - (\epsilon - x_0) \right\|^2,
\end{equation}
which serves as a proxy for how well source model $k$ understands the target example. Note that $\ell^{(k)}$ is used only as a scalar signal—its gradients are not backpropagated.

\section{Potential Solution: Adpt-Scaling}

We propose a \emph{loss-aware knowledge consolidation} objective that reweights the CFM loss based on the collective performance of the source models. Specifically, define a per-example importance weight:
\begin{equation}
    w(x_0, t, \epsilon, c) = \exp\left( -\alpha \cdot \min_{k \in \{1,\dots,K\}} \ell^{(k)}(x_0, t, \epsilon, c) \right),
\end{equation}
where $\alpha \geq 0$ controls the sensitivity to source model performance (larger $\alpha$ emphasizes examples where at least one source model performs well). Alternative formulations may use a weighted average or softmax over $\{\ell^{(k)}\}$.

The consolidated training objective is then:
\begin{equation}
    \Theta^* = \arg\min_{\Theta} \; \mathbb{E}_{\substack{t \sim \pi(t) \\ x_0 \sim p_0^{\text{target}} \\ \epsilon \sim \mathcal{N}(0,I)}} \left[ w(x_0, t, \epsilon, c) \cdot \ell_{\text{target}}(x_0, t, \epsilon; \Theta) \right].
\end{equation}

This formulation leverages the source models as \emph{teachers that identify informative or well-modeled regions of the target data manifold}, without requiring architectural alignment or direct imitation. By down-weighting examples where all source models fail (e.g., out-of-distribution or highly novel concepts), the fine-tuning process focuses on regions where prior knowledge is most transferable, thereby accelerating convergence and improving sample fidelity.

We assume that all models share a compatible conditioning mechanism (e.g., via a shared text encoder) and operate in the same data space (e.g., through a common VAE), enabling meaningful evaluation of $\ell^{(k)}$ on target data.

\section{Potential Solution: Velocity-Guided Conditional Flow Matching}
\label{subsec:velocity_guided_cfm}

An alternative strategy for knowledge consolidation eschews the use of reference losses altogether and instead exploits the velocity fields of pretrained rectified flow models as sources of inductive bias. Given the same target dataset $\mathcal{D}_{\text{target}} = \{(x_0^{(i)}, c^{(i)})\}_{i=1}^{N}$ and a collection of $K$ fixed pretrained models $\{v_{\Theta^{(k)}}\}_{k=1}^K$, we treat their velocity predictions as informative approximations of the true optimal transport direction from noise to data.

Recall that under the Conditional Flow Matching (CFM) framework, the ground-truth target velocity at point $z_t = (1 - t)x_0 + t\epsilon$ is $u_t = \epsilon - x_0$. However, when $x_0$ belongs to a complex or underrepresented region of the target domain, estimating $u_t$ from a single noisy sample may be unstable—especially early in training. In contrast, a well-trained source model $v_{\Theta^{(k)}}$ may provide a smoother, more reliable estimate of the flow direction, particularly if its training domain overlaps semantically or structurally with the target.

To leverage this, we define a \emph{consensus velocity} from the source ensemble:
\begin{equation}
    \bar{v}(z_t, t, c) = \sum_{k=1}^K w_k(c) \cdot v_{\Theta^{(k)}}(z_t, t, c),
\end{equation}
where $w_k(c) \geq 0$ are context-dependent weights (e.g., based on caption similarity, model-domain relevance, or validation performance) satisfying $\sum_{k=1}^K w_k(c) = 1$. In the simplest case, uniform averaging ($w_k = 1/K$) suffices.

We then augment the standard CFM loss by encouraging the target model $v_\Theta$ to align with this consensus velocity, in addition to matching the ground-truth transport direction. The resulting hybrid objective is:
\begin{equation}
    \mathcal{L}_{\text{guided}}(\Theta) = 
    \mathbb{E}_{\substack{t \sim \pi(t) \\ x_0 \sim p_0^{\text{target}} \\ \epsilon \sim \mathcal{N}(0,I)}}
    \left[
        \underbrace{\left\| v_\Theta(z_t, t, c) - (\epsilon - x_0) \right\|^2}_{\text{CFM target loss}}
        + \lambda \cdot 
        \underbrace{\left\| v_\Theta(z_t, t, c) - \bar{v}(z_t, t, c) \right\|^2}_{\text{velocity distillation loss}}
    \right],
\end{equation}
where $\lambda \geq 0$ balances fidelity to the exact OT path and alignment with the knowledge-rich ensemble prediction.

This formulation can be interpreted as a form of \emph{multi-source flow distillation}: the target model learns not only from the synthetic straight-line trajectories of CFM but also from the refined, data-driven flow directions implicitly encoded in the pretrained models. Importantly, because the reference models are frozen, this incurs no additional memory overhead beyond storing their parameters, and gradients are only computed through $v_\Theta$.

Under the assumption that the source models operate in a compatible latent or pixel space (e.g., via a shared VAE encoder/decoder or unified conditioning pipeline), this velocity-guided loss provides a powerful regularizer that improves sample quality, stabilizes training, and enhances generalization—particularly in low-data or compositional regimes.

==> sec/method_trainingfree.tex <==
% \section{Problem Statement}
% \label{sec:problem_statement}

\begin{figure}[h!]
  \centering
  % First subfigure
  \includegraphics[width=0.7\textwidth]{fig/geodesicflow_rho.pdf}
  \caption{Illustration of the intuition of $\rho$.}
  \label{fig:two-subfigs}
\end{figure}

\begin{figure}[h!]
  \centering
  % First subfigure
  \subfloat[]{
    \includegraphics[width=0.45\textwidth]{fig/illus_a.pdf}
  }
  \hfill
  % Second subfigure
  \subfloat[]{
    \includegraphics[width=0.45\textwidth]{fig/illus_b.pdf}
  }
  \caption{Schematic views of the proposed method. (a) Illustration of the training process for Riemannian Conditional Flow Matching (RCFM). On a Riemannian manifold $\mathcal{M}$, we sample a data point $x_0 \sim p_0$ and a noise point $x_1 \sim p_1$. The model is trained to make its predicted vector field $v_\Theta(z_t, t)$ match the target velocity $u_t$ of the geodesic path $\gamma(t)$ connecting the two points. The target $u_t$ lies in the tangent space $T_{z_t}\mathcal{M}$ at an interpolated point $z_t$. The loss is the squared norm of the difference between the predicted and target vectors, measured using the Riemannian metric at $z_t$. (b) Illustration of the generative sampling process. Starting from a point $z_1$ sampled from the noise distribution $p_1$, we numerically integrate the learned vector field $v_\Theta$ backward in time from $t=1$ to $t=0$. Each step is a ``geodesic shooting'' update, $z_{t-\Delta t} = \exp_{z_t}(-\Delta t \cdot v_\Theta(z_t, t))$, which moves the point along the manifold. This iterative process generates a trajectory that transforms the noise sample into a final point $z_0$, which is a new sample from the learned data distribution.}
  \label{fig:two-subfigs}
\end{figure}

% ------------------------
% Metric-free v2
\section{Preliminaries: Riemannian Geometry}

Let $(\mathcal{M}, g)$ be a $d$-dimensional Riemannian manifold, possibly embedded in a high-dimensional ambient space $\mathbb{R}^D$ (e.g., via a VAE encoder), though no explicit embedding map $\iota$ is assumed or required for computation. All geometric operations are defined intrinsically with respect to the metric $g$, which governs lengths, angles, and geodesics on $\mathcal{M}$.

At each point $x \in \mathcal{M}$, the \textbf{tangent space} $T_x\mathcal{M}$ is a $d$-dimensional vector space encoding directions of infinitesimal movement on the manifold. In practice, we do not assume access to an explicit embedding Jacobian $J_\iota(x)$; instead, tangent vectors are represented intrinsically via local coordinates or learned projections.

The \textbf{Riemannian metric} $g_x : T_x\mathcal{M} \times T_x\mathcal{M} \to \mathbb{R}$ defines an inner product on tangent vectors. Rather than deriving it from an ambient Euclidean structure (which requires $J_\iota$), we approximate it directly via a symmetric positive-definite matrix $G_\phi(x) \in \mathbb{R}^{d \times d}$, parameterized by a neural network $\phi$:
\begin{equation}
    g_x(u, v) \approx u^\top G_\phi(x) v, \quad \text{for } u, v \in \mathbb{R}^d \text{ (local coordinates)}.
\end{equation}
This learned metric adapts to the local geometry of the latent manifold and avoids any dependence on intractable embedding Jacobians. The induced norm is $\|v\|_{g(x)} = \sqrt{v^\top G_\phi(x) v}$, which may vary across $\mathcal{M}$ to reflect curvature — e.g., stretching near semantically dense regions.

The \textbf{exponential map} $\exp_x: T_x\mathcal{M} \to \mathcal{M}$ maps a tangent vector $v$ to the endpoint of the geodesic starting at $x$ with initial velocity $v$. Its inverse, the \textbf{logarithmic map} $\log_x: \mathcal{M} \to T_x\mathcal{M}$, recovers the initial velocity required to reach $y \in \mathcal{M}$ along the geodesic, assuming $y$ lies within the injectivity radius of $x$. In practice, these maps can be approximated numerically or learned implicitly via neural ODEs or retractions.

A \textbf{geodesic} $\gamma_{x_0 \to x_1}(t) = \exp_{x_0}\big(t \cdot \log_{x_0}(x_1)\big)$, $t \in [0,1]$, is the shortest path between $x_0$ and $x_1$ under $g$. It satisfies $\nabla_{\dot{\gamma}} \dot{\gamma} = 0$, where $\nabla$ is the Levi-Civita connection induced by $g$.

% \textbf{Parallel transport} $P_{\gamma, t_b \leftarrow t_a}: T_{\gamma(t_a)}\mathcal{M} \to T_{\gamma(t_b)}\mathcal{M}$ moves tangent vectors along $\gamma$ while preserving inner products under $g$. In implementation, we approximate parallel transport via Schild’s ladder or by learning a connection-compatible vector field. This enables consistent vector comparison across the manifold — essential for defining coherent velocity fields.


% \section{GeodesicFlow: Adaptive Metric-Free Flow Matching on Sphere Manifolds}

% Our goal is to learn a \textit{text-conditioned} time-dependent vector field $v_\Theta: \mathcal{M} \times [0,1] \times \mathcal{C} \to T\mathcal{M}$, where $v_\Theta(x, t, c) \in T_x\mathcal{M}$, that governs a continuous transformation of samples from a simple base distribution $p_1$ (e.g., uniform noise on the sphere) into samples from a complex, \textit{text-conditioned} target data distribution $p_0(\cdot \mid c)$. This transformation is realized as the solution to an ordinary differential equation (ODE) on the manifold, where the vector field $v_\Theta$ dictates the instantaneous direction and speed of motion at each point, time, and given text condition $c$.

% We restrict $\mathcal{M}$ to be the unit sphere $\mathbb{S}^n \subset \mathbb{R}^{n+1}$ endowed with its canonical round metric. Although $\mathbb{S}^n$ is a curved Riemannian manifold, its isometric embedding in Euclidean space allows us to compute all necessary geometric operations — exponential/logarithmic maps, parallel transport, and norm evaluations — using only ambient-space linear algebra, \textit{without ever explicitly evaluating or storing the metric tensor}. This yields a computationally efficient, \textbf{metric-free} implementation while preserving geometric fidelity.

% Critically, this is not a Euclidean method: while we use the Euclidean norm $\|\cdot\|_2$ for loss computation, the vectors $v_\Theta(z_t, t, c)$ and $u_t$ are constrained to lie in the tangent space $T_{z_t}\mathbb{S}^n$, and their evolution follows curved geodesics governed by the sphere’s intrinsic geometry. In contrast, a true Euclidean flow (as in the attached Rectified Flow paper) uses linear interpolation and constant velocities — violating the manifold structure. Here, the Euclidean norm serves only as a \textit{computational proxy}: because the Riemannian metric on $\mathbb{S}^n$ is induced from $\mathbb{R}^{n+1}$, we have $\|v\|_{g(x)} = \|v\|_2$ for all $v \in T_x\mathbb{S}^n$. Thus, our optimization remains geometrically faithful to the curved manifold — it is efficient, not approximate.

% \subsection{Adaptive Geometric Blending: Learning the Optimal Path Between Euclidean and Geodesic Flows}
% \label{sec:adaptive_blend}

% While geodesic paths are geometrically natural, they may not always be optimal for sample quality. The “true” optimal path for generating realistic images may lie \textit{between} the geodesic and Euclidean extremes: geodesics may traverse low-density “holes” in the data manifold, while Euclidean paths may barrel through semantically implausible regions. A static blend of the two losses (e.g., fixed $\lambda$) offers a global compromise, but fails to adapt to local geometric and semantic structure.

% Inspired by the adaptive noise schedule re-weighting in the attached paper (Sec 3.1), we propose an \textbf{adaptive geometric blending} mechanism that dynamically adjusts the trade-off between Euclidean and geodesic flows based on local data geometry and density. This yields a time- and location-dependent weight $\lambda(z_t^{geo})$ that optimizes for sample realism, diversity, and training stability.

% Formally, our total loss becomes:
% \begin{equation}
%     \mathcal{L}_{\text{Adaptive}}(\Theta) = \mathbb{E}_{\substack{t \sim \mathcal{U}[0,1] \\ x_0 \sim p_0(\cdot \mid c) \\ x_1 \sim p_1 \\ c \sim p_{\text{text}}}} \left[ 
%     \big(1 - \lambda(z_t^{geo})\big) \cdot \left\| v_\Theta(z_t^{\text{euc}}, t, c) - u_t^{\text{euc}} \right\|^2 + 
%     \lambda(z_t^{geo}) \cdot \left\| v_\Theta(z_t^{\text{geo}}, t, c) - u_t^{\text{geo}} \right\|^2 
%     \right],
% \end{equation}
% where $z_t^{\text{geo}} = \text{Slerp}(x_0, x_1; t)$ is the geodesic (great circle or sphere) interpolant; $z_t^{\text{euc}} = (1-t)x_0 + t x_1$ is the Euclidean (straight-line) interpolant; $u_t^{\text{geo}} = P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1))$ is the parallel-transported geodesic velocity; and $u_t^{\text{euc}} = x_1 - x_0$ is the constant Euclidean velocity.

% \subsection{Learned Criterion for $\lambda(z_t^{geo})$}

% Rather than relying on a fixed analytic form, we propose to learn the adaptive blending weight $\lambda(z_t^{geo})$ using a lightweight neural network $\lambda_\Phi: \mathbb{S}^n \times [0,1] \times \mathcal{C} \to [0,1]$, parameterized by $\Phi$. This network takes as input the current sample position $z_t$, time $t$, and text condition $c$, allowing $\lambda$ to adapt not only to local geometry but also to semantic context and temporal dynamics.

% To preserve interpretability and inject geometric inductive bias, we condition $\lambda_\Phi$ on a set of meaningful features derived from the geodesic structure. Specifically, we compute $\rho(z_t) = \| u_t^{\text{geo}} \|_2 \in [0, \pi]$,

% We normalize this feature to be in $[0,1]$ via a normalized density proxy $\tilde{\rho}(z_t^{geo}) = 1 - \frac{\| u_t^{\text{geo}} \|_2}{\pi}$,
% so that $\tilde{\rho} \approx 1$ corresponds to high-confidence (dense) regions, and $\tilde{\rho} \approx 0$ to low-confidence (sparse) regions.

% The norm $\| u_t^{\text{geo}} \|_2 = \arccos(x_0^\top x_1)$ reflects the geodesic distance between $x_0$ and $x_1$, and serves as a natural proxy for local data density and model uncertainty. Small values indicate that the interpolation path lies in a geometrically compact, densely populated region, where the learned vector field is well-constrained and following the curved geodesic is safe and semantically meaningful. Conversely, large values signal sparse or uncertain regions, where forcing geodesic motion risks traversing implausible or out-of-distribution areas. In such cases, falling back to Euclidean motion (via projection) acts as a stabilizing prior, avoiding overconfident extrapolation while remaining on-manifold.

% The normalized density proxy $\tilde{\rho}(z_t^{geo})$ induces a self-stabilizing curriculum: early in training, high uncertainty favors Euclidean targets; as the model improves, lower norms in plausible regions encourage geometry-aware geodesic flow. The mechanism requires no explicit density estimation, is computationally free, and aligns sampling behavior with the adaptive policy learned during training.


% The network $\lambda_\Phi$ then predicts the blending weight as $\lambda(z_t^{geo}) = \sigma\left( \text{MLP}_\Phi\left(z_t \right) \right)$,
% where $\text{MLP}_\Phi$ is a small multi-layer perceptron (e.g., 2 layers, 64 hidden units) that fuses the geometric feature $\tilde{\rho}(z_t^{geo})$, and $\sigma(\cdot)$ is the sigmoid function, ensuring $\lambda \in (0,1)$.

% \noindent\textbf{Regularizing $\lambda_\Phi$ with an Auxiliary Loss}
% To prevent $\lambda_\Phi$ from ignoring the geometric prior or collapsing to trivial solutions (e.g., always 0 or 1), we introduce a lightweight auxiliary regularization loss that encourages $\lambda$ to correlate with the interpretable density signal $\tilde{\rho}$, i.e., $
%     \mathcal{L}_{\lambda}(\Phi) = \mathbb{E} \left[ \left( \lambda(z_t^{geo}) - \tilde{\rho}(z_t^{geo}) \right)^2 \right]$.

% This loss gently anchors $\lambda$ to the geometrically motivated baseline: when no stronger signal is present, $\lambda \approx \tilde{\rho}$. But when semantic or temporal context suggests a different blending strategy (e.g., ``draw a straight road'' in a sparse region), the network is free to override the prior. We combine this with the main flow matching loss, $\mathcal{L}_{\text{Adaptive}} + \eta \cdot \mathcal{L}_{\lambda}$,
% where $\eta > 0$ is a small regularization coefficient (default: $\eta = 0.1$) that balances geometric faithfulness with adaptive flexibility.

% The motivations for adaptive blending are three-fold.

% 1) \textit{Self-Stabilizing Curriculum via Learned Uncertainty}: Early in training, when $u_t^{\text{geo}}$ is poorly estimated (large norm), $\tilde{\rho}$ is small, and $\mathcal{L}_\lambda$ encourages $\lambda \to 0$, favoring the stable Euclidean target. As training progresses and geodesic predictions become reliable, $\tilde{\rho}$ increases, and $\lambda$ follows — inducing a \textit{built-in, data-driven curriculum}. Unlike fixed schedules, this adapts per-sample and per-prompt, and is stabilized by the auxiliary loss.

% 2) \textit{Semantic- and Geometry-Aware Path Optimization}: The network can learn to blend paths not just based on local density, but also based on what is being generated. For instance, for prompts describing rigid or structured objects (e.g., ``a building''), the model may learn to prefer Euclidean paths even in geometrically dense regions, for sharper edges. For organic or curved concepts (``a swirling galaxy'', ``a dolphin''), it may favor geodesic motion to preserve natural curvature — even if local density is moderate. The auxiliary loss ensures these adaptations are intentional and grounded, not random or degenerate.

% 3) \textit{Minimal Overhead, Maximum Flexibility}: The network $\lambda_\Phi$ is lightweight and computed in parallel with $v_\Theta$. It introduces negligible computational cost but significantly increases modeling capacity. All geometric operations remain metric-free and sphere-compliant.

% \subsection{Geodesic Probability Path and Target Velocity Field}
% As outlined in Algorithm~\ref{alg:training_geodesicflow_t2i}, each training step begins by sampling a data point $x_0 \sim p_0(\cdot \mid c)$ and a noise point $x_1 \sim p_1$. To construct the flow matching objective, we define two distinct probability paths connecting these endpoints: one that respects the intrinsic geometry of the sphere and another that operates in the ambient Euclidean space.

% The geodesic path on the sphere $\mathbb{S}^n$ is the shorter arc of the great circle between $x_0$ and $x_1$. A point $z_t^{\text{geo}}$ along this path is calculated using Slerp:
% \begin{equation*}
%     z_t^{\text{geo}} = \frac{\sin((1-t)\theta)}{\sin\theta} x_0 + \frac{\sin(t\theta)}{\sin\theta} x_1,
%     \quad \text{where } \theta = \arccos(x_0^\top x_1).
% \end{equation*}
% The corresponding target velocity field $u_t^{\text{geo}}$ is generated by first computing the initial tangent vector $v_0 = \log_{x_0}(x_1)$ and then moving it along the path via parallel transport. The formulas used in the algorithm are:
% \begin{align*}
%     v_0 = \theta \cdot \frac{x_1 - (x_0^\top x_1)x_0}{\|x_1 - (x_0^\top x_1)x_0\|_2}, \ \ \ 
%     u_t^{\text{geo}} = v_0 - \frac{v_0^\top z_t^{\text{geo}}}{1 - (x_0^\top x_1)^2} (x_1 - (x_0^\top x_1) x_0).
% \end{align*}
% For contrast, the Euclidean path is the simple straight-line interpolation between the points in the ambient space $\mathbb{R}^{n+1}$. The path and its constant velocity vector are given by:
% \begin{align*}
%     z_t^{\text{euc}} = (1-t) x_0 + t x_1, \ \ \ 
%     u_t^{\text{euc}} = x_1 - x_0.
% \end{align*}
% These two sets of paths ($z_t^{\text{geo}}, z_t^{\text{euc}}$) and target velocities ($u_t^{\text{geo}}, u_t^{\text{euc}}$) provide the ground truths for the adaptive blended loss function, which trains the network $v_\Theta$ to approximate both geometric and linear flows.

% \subsection{Generative Sampling via Geodesic Integration}
% To generate a sample for a given text condition $c$, we numerically integrate the underlying ODE backward in time from $t=1$ to $t=0$, starting with a random noise sample $z_1 \sim p_1$. Crucially, to maintain consistency with the adaptive training objective, each integration step is not a simple geodesic or Euclidean update, but rather a dynamic blend of both motions. This ensures that the path taken during inference respects the learned trade-offs between geometric purity and linear stability. At each discrete timestep $t$, we first compute a single velocity vector $v = v_\Theta(z_t, t, c)$. This vector is then used to determine two distinct potential destinations: a geodesic destination $z^{\text{geo}}$, found by moving along the manifold's geodesic using the exponential map, and a Euclidean destination $z^{\text{euc}}$, found by taking a linear step in the ambient space $\mathbb{R}^{n+1}$ and then projecting the result back onto the sphere $\mathbb{S}^n$. An adaptive blending weight $\lambda_t = \lambda_\Phi(z_t)$ is computed using the trained network $\lambda_\Phi$. The final point for the next step, $z_{t-\Delta t}$, is then computed by interpolating on the sphere between the geodesic and Euclidean destinations, weighted by $\lambda_t$. More detailed can be founded in Algorithm \ref{alg:sampling_geodesicflow_t2i}.
% This procedure ensures that the sampling path is dynamically constructed, leveraging the stability of Euclidean steps in uncertain regions and the geometric fidelity of geodesic steps in well-defined regions, exactly as encouraged during training. All operations remain in the ambient space $\mathbb{R}^{n+1}$, preserving the metric-free efficiency of the framework.

% \subsection{Algorithmic Implementation: Adaptive Metric-Free Learning and Sampling}

% Algorithms~\ref{alg:training_geodesicflow_t2i} and~\ref{alg:sampling_geodesicflow_t2i} implement our metric-free framework on the sphere, with adaptive blending driven purely by local data density. The Riemannian structure of $\mathbb{S}^n$ is fully respected — geodesics, parallel transport, and tangent norms are all correctly modeled — while avoiding any explicit metric tensor handling. Critically, the adaptive weight $\lambda(z_t^{geo})$ is computed on-the-fly using only the norm of the geodesic velocity, requiring negligible overhead.

% The blending weight adapts based on the hypothesis that regions with high geodesic velocity norm $\|u_t^{\text{geo}}\|_2$ correspond to low data density or high model uncertainty — where straight Euclidean paths are preferable. Conversely, low norms indicate high-confidence, dense regions where curved geodesic motion should be favored. This mirrors the adaptive noise schedule philosophy in the Scaling Rectified Flow paper (Sec 3.1), but operates on geometric uncertainty rather than timestep.

% \begin{algorithm}[!t]
% \caption{Training GeodesicFlow with Density-Driven Adaptive Blending}
% \label{alg:training_geodesicflow_t2i}
% \begin{algorithmic}[1]
% \Require
% \Statex \textit{Models:} Network $v_\Theta: \mathbb{S}^n \times [0,1] \times \mathcal{C} \to T\mathbb{S}^n$ with parameters $\Theta$, $\text{MLP}_{\Phi}$ with parameters $\Phi$.
% \Statex \textit{Data:} Text-conditioned distribution $p_0(\cdot \mid c)$, uniform noise $p_1$ on $\mathbb{S}^n$, text prior $p_{\text{text}}$.
% \Statex \textit{Hyperparameters:} Batch size $B$, steps $N_{\text{steps}}$, learning rate $\alpha_{\text{lr}}$, regularization weight $\eta$.
% \State Initialize model parameters $\Theta$, network parameters $\Phi$.
% \State Initialize optimizer (e.g., AdamW) with learning rate $\alpha_{\text{lr}}$.
% \For{step = 1 to $N_{\text{steps}}$}
%     \State Sample mini-batch: $\{c^{(i)}\}_{i=1}^B \sim p_{\text{text}}$, $\{x_0^{(i)}\}_{i=1}^B \sim p_0(\cdot \mid c^{(i)})$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
%     \State Initialize batch loss $\mathcal{L}_{\text{batch}} \leftarrow 0$.
%     \For{$i = 1$ to $B$}
%         \State Let $c \leftarrow c^{(i)}$, $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
%         \State Compute $\theta \leftarrow \arccos(x_0^\top x_1)$.
%         \State Compute $v_0 \leftarrow \theta \cdot \frac{x_1 - (x_0^\top x_1)x_0}{\|x_1 - (x_0^\top x_1)x_0\|}$.
%         \State Compute $z_t^{\text{geo}} \leftarrow \frac{\sin((1-t)\theta)}{\sin\theta} x_0 + \frac{\sin(t\theta)}{\sin\theta} x_1$.
%         \State Compute $u_t^{\text{geo}} \leftarrow v_0 - \frac{v_0^\top z_t^{\text{geo}}}{1 - (x_0^\top x_1)^2} (x_1 - (x_0^\top x_1) x_0)$.
%         \State Compute $z_t^{\text{euc}} \leftarrow (1-t) x_0 + t x_1$.
%         \State Compute $u_t^{\text{euc}} \leftarrow x_1 - x_0$.
%         \State Compute density proxy: $\rho \leftarrow \| u_t^{\text{geo}} \|$.
%         \State Compute adaptive weight: $\lambda \leftarrow \sigma\left( \text{MLP}_\Phi\left(z_t \right) \right)$.
%         \State Compute normalized density proxy: $\tilde{\rho}(z_t^{geo})$.
%         \State Compute $\mathcal{L}_{\lambda} = \mathbb{E} \left[ \left( \lambda(z_t^{geo}) - \tilde{\rho}(z_t^{geo}) \right)^2 \right]$.
%         \State Predict velocities: $\hat{u}_t^{\text{geo}} \leftarrow v_\Theta(z_t^{\text{geo}}, t, c)$, $\hat{u}_t^{\text{euc}} \leftarrow v_\Theta(z_t^{\text{euc}}, t, c)$.
%         \State Compute blended loss: $
%             \mathcal{L}^{(i)} \leftarrow (1 - \lambda) \cdot \| \hat{u}_t^{\text{euc}} - u_t^{\text{euc}} \|^2 + \lambda \cdot \| \hat{u}_t^{\text{geo}} - u_t^{\text{geo}} \|^2.
%             $
%         \State $\mathcal{L}_{\text{batch}} \leftarrow \mathcal{L}_{\text{batch}} + \mathcal{L}^{(i)} + \eta \cdot \mathcal{L}_{\lambda}$.
%     \EndFor
%     \State Compute mean loss: $\mathcal{L} \leftarrow \frac{1}{B} \mathcal{L}_{\text{batch}}$.
%     \State Update parameters: $\Theta \leftarrow \text{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$.
% \EndFor
% \State \Return Trained parameters $\Theta$, network $\Phi$.
% \end{algorithmic}
% \end{algorithm}

% \vspace{1cm}

% \begin{algorithm}[!t]
% \caption{Adaptive Geodesic-Euclidean Sampling (AGES) from Trained GeodesicFlow}
% \label{alg:sampling_geodesicflow_t2i}
% \begin{algorithmic}[1]
% \Require
% \Statex \textit{Model:} Trained $v_\Theta$, and trained $\Phi$.
% \Statex \textit{Text Embedding:} Condition $c \in \mathcal{C}$.
% \Statex \textit{Noise:} $z_1 \sim \text{Uniform}(\mathbb{S}^n)$.
% \Statex \textit{Hyperparameters:} Integration steps $N$, blending mode (learned or analytic $\lambda$).
% \State Set $\Delta t \leftarrow 1/N$.
% \For{$k = N$ \textbf{downto} $1$}
%     \State Set $t \leftarrow k \cdot \Delta t$.
    
%     \State Compute $\lambda \leftarrow \lambda_\Phi(z_t)$.
%     \State Predict velocity: $v \leftarrow v_\Theta(z_t, t, c)$.
    
%     \State \textbf{Compute blended step:}
%     \State \quad $\xi_{\text{geo}} \leftarrow -\Delta t \cdot v$  \Comment{Geodesic step (tangent vector)}
%     \State \quad $\xi_{\text{euc}} \leftarrow -\Delta t \cdot v$  \Comment{Same direction, but we'll project/step differently}
    
%     \State \textbf{Geodesic component:}
%     \State \quad $\hat{\xi}_{\text{geo}} \leftarrow \xi_{\text{geo}} / \|\xi_{\text{geo}}\|$ if $\|\xi_{\text{geo}}\| > 0$, else $0$
%     \State \quad $z^{\text{geo}} \leftarrow \cos(\|\xi_{\text{geo}}\|) z_t + \sin(\|\xi_{\text{geo}}\|) \hat{\xi}_{\text{geo}}$
    
%     \State \textbf{Euclidean component:}
%     \State \quad $z^{\text{euc}} \leftarrow z_t + \xi_{\text{euc}}$  \Comment{Straight step in ambient space}
%     \State \quad $z^{\text{euc}} \leftarrow z^{\text{euc}} / \|z^{\text{euc}}\|$  \Comment{Project back to sphere (minimal perturbation)}
    
%     \State \textbf{Blend positions:}
%     \State \quad $z_{t-\Delta t} \leftarrow \text{Slerp}(z^{\text{geo}}, z^{\text{euc}}; \lambda)$
%     \Comment{Interpolate on-manifold between the two destinations}
    
%     % \State \textbf{Alternative (simpler, approximate):}
%     % \State \quad $z_{t-\Delta t} \leftarrow (1 - \lambda) \cdot z^{\text{euc}} + \lambda \cdot z^{\text{geo}}$
%     % \State \quad $z_{t-\Delta t} \leftarrow z_{t-\Delta t} / \|z_{t-\Delta t}\|$  \Comment{Renormalize if using linear blend}
    
% \EndFor
% \State \Return Generated sample $z_0$ aligned with text $c$.
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[!t]
% \caption{Training GeodesicFlow with Static Blending (Fixed $\lambda$)}
% \label{alg:training_geodesicflow_static}
% \begin{algorithmic}[1]
% \Require
% \Statex \textit{Model:} Neural network $v_\Theta: \mathbb{S}^n \times [0,1] \times \mathcal{C} \to T\mathbb{S}^n$ with parameters $\Theta$.
% \Statex \textit{Data:} Text-conditioned distribution $p_0(\cdot \mid c)$, uniform noise $p_1$ on $\mathbb{S}^n$, text prior $p_{\text{text}}$.
% \Statex \textit{Hyperparameters:} Fixed blend weight $\lambda \in [0,1]$, batch size $B$, steps $N_{\text{steps}}$, learning rate $\alpha$.
% \State Initialize model parameters $\Theta$.
% \State Initialize optimizer (e.g., AdamW) with learning rate $\alpha$.
% \For{step = 1 to $N_{\text{steps}}$}
%     \State Sample mini-batch: $\{c^{(i)}\}_{i=1}^B \sim p_{\text{text}}$, $\{x_0^{(i)}\}_{i=1}^B \sim p_0(\cdot \mid c^{(i)})$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
%     \State Initialize batch loss $\mathcal{L}_{\text{batch}} \leftarrow 0$.
%     \For{$i = 1$ to $B$}
%         \State Let $c \leftarrow c^{(i)}$, $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
%         \State Compute $\theta \leftarrow \arccos(x_0^\top x_1)$.
%         \State Compute $v_0 \leftarrow \theta \cdot \frac{x_1 - (x_0^\top x_1)x_0}{\|x_1 - (x_0^\top x_1)x_0\|}$.
%         \State Compute $z_t^{\text{geo}} \leftarrow \frac{\sin((1-t)\theta)}{\sin\theta} x_0 + \frac{\sin(t\theta)}{\sin\theta} x_1$.
%         \State Compute $u_t^{\text{geo}} \leftarrow v_0 - \frac{v_0^\top z_t^{\text{geo}}}{1 - (x_0^\top x_1)^2} (x_1 - (x_0^\top x_1) x_0)$.
%         \State Compute $z_t^{\text{euc}} \leftarrow (1-t) x_0 + t x_1$.
%         \State Compute $u_t^{\text{euc}} \leftarrow x_1 - x_0$.
%         \State Predict velocities: $\hat{u}_t^{\text{geo}} \leftarrow v_\Theta(z_t^{\text{geo}}, t, c)$, $\hat{u}_t^{\text{euc}} \leftarrow v_\Theta(z_t^{\text{euc}}, t, c)$.
%         \State Compute blended loss: 
%             \[
%             \mathcal{L}^{(i)} \leftarrow (1 - \lambda) \cdot \| \hat{u}_t^{\text{euc}} - u_t^{\text{euc}} \|^2 + \lambda \cdot \| \hat{u}_t^{\text{geo}} - u_t^{\text{geo}} \|^2.
%             \]
%         \State $\mathcal{L}_{\text{batch}} \leftarrow \mathcal{L}_{\text{batch}} + \mathcal{L}^{(i)}$.
%     \EndFor
%     \State Compute mean loss: $\mathcal{L} \leftarrow \frac{1}{B} \mathcal{L}_{\text{batch}}$.
%     \State Update parameters: $\Theta \leftarrow \text{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$.
% \EndFor
% \State \Return Trained parameters $\Theta$.
% \end{algorithmic}
% \end{algorithm}


% \subsection{Learned Criterion for $\lambda(z_t^{geo})$ (large -+ dense)}

% Rather than relying on a fixed analytic form, we propose to learn the adaptive blending weight $\lambda(z_t^{geo})$ using a lightweight neural network $\lambda_\Phi: \mathbb{S}^n \times [0,1] \times \mathcal{C} \to [0,1]$, parameterized by $\Phi$. This network takes as input the current sample position $z_t$, time $t$, and text condition $c$, allowing $\lambda$ to adapt not only to local geometry but also to semantic context and temporal dynamics.

% To preserve interpretability and inject geometric inductive bias, we condition $\lambda_\Phi$ on a set of meaningful features derived from the geodesic structure. Specifically, we compute $\rho(z_t) = \| u_t^{\text{geo}} \|_2 \in [0, \pi]$,

% We normalize this feature to be in $[0,1]$ via the normalized density proxy:
% \begin{equation}
%     \tilde{\rho}(z_t^{geo}) = \frac{\| u_t^{\text{geo}} \|_2}{\pi},
% \end{equation}
% so that:
% \begin{itemize}
%     \item $\tilde{\rho} \approx 1$ corresponds to \textbf{high-confidence (dense)} regions,
%     \item $\tilde{\rho} \approx 0$ corresponds to \textbf{low-confidence (sparse)} regions.
% \end{itemize}

% Under this design, large geodesic velocity norms are interpreted as indicators of geometrically rich, well-populated regions where the model can confidently follow curved geodesic paths. Conversely, small norms are interpreted as indicators of sparse or uncertain regions, where the model should fall back to simpler Euclidean motion for stability.

% The network $\lambda_\Phi$ then predicts the blending weight as:
% \begin{equation}
%     \lambda(z_t^{geo}) = \sigma\left( \text{MLP}_\Phi\left(z_t \right) \right),
% \end{equation}
% where $\text{MLP}_\Phi$ is a small multi-layer perceptron (e.g., 2 layers, 64 hidden units) that fuses the geometric feature $\tilde{\rho}(z_t^{geo})$, and $\sigma(\cdot)$ is the sigmoid function, ensuring $\lambda \in (0,1)$.

% \noindent\textbf{Regularizing $\lambda_\Phi$ with an Auxiliary Loss}
% To prevent $\lambda_\Phi$ from ignoring the geometric prior or collapsing to trivial solutions (e.g., always 0 or 1), we introduce a lightweight auxiliary regularization loss that encourages $\lambda$ to correlate with the interpretable density signal $\tilde{\rho}$, i.e.,
% \begin{equation}
%     \mathcal{L}_{\lambda}(\Phi) = \mathbb{E} \left[ \left( \lambda(z_t^{geo}) - \tilde{\rho}(z_t^{geo}) \right)^2 \right].
% \end{equation}

% This loss anchors $\lambda$ to the geometrically defined baseline: when no stronger signal is present, $\lambda \approx \tilde{\rho}$. But when semantic or temporal context suggests a different blending strategy (e.g., ``draw a straight road'' in a geometrically dense region), the network is free to override the prior. We combine this with the main flow matching loss:
% \begin{equation}
%     \mathcal{L}_{\text{Adaptive}} + \eta \cdot \mathcal{L}_{\lambda},
% \end{equation}
% where $\eta > 0$ is a small regularization coefficient (default: $\eta = 0.1$).

% The motivations for adaptive blending under this reversed design are three-fold.

% \begin{enumerate}
%     \item \textit{Self-Stabilizing Curriculum via Learned Confidence}: Early in training, when $u_t^{\text{geo}}$ is small (low $\tilde{\rho}$), $\mathcal{L}_\lambda$ encourages $\lambda \to 0$, favoring the stable Euclidean target in sparse regions. As training progresses and geodesic predictions become reliable in regions with large norms (high $\tilde{\rho}$), $\lambda$ increases — inducing a built-in, data-driven curriculum that shifts from linear to geometric motion as confidence grows.
    
%     \item \textit{Semantic- and Geometry-Aware Path Optimization}: The network can learn to blend paths based on semantics, even against the geometric proxy. For instance, for prompts describing rigid or structured objects (e.g., ``a building''), the model may learn to prefer Euclidean paths even in geometrically dense (high $\tilde{\rho}$) regions, for sharper edges. For organic or curved concepts (``a swirling galaxy''), it may favor geodesic motion — even if $\tilde{\rho}$ is low. The auxiliary loss ensures these overrides are intentional and grounded.
    
%     \item \textit{Minimal Overhead, Maximum Flexibility}: The network $\lambda_\Phi$ is lightweight and computed in parallel with $v_\Theta$. It introduces negligible computational cost but significantly increases modeling capacity. All geometric operations remain metric-free and sphere-compliant.
% \end{enumerate}


% \subsection{Learned Criterion for $\lambda(z_t^{geo})$ (No Regularization)}

% Rather than relying on a fixed analytic form, we propose to learn the adaptive blending weight $\lambda(z_t^{geo})$ using a lightweight neural network $\lambda_\Phi: \mathbb{S}^n \times [0,1] \times \mathcal{C} \to [0,1]$, parameterized by $\Phi$. This network takes as input the current sample position $z_t$, time $t$, and text condition $c$, allowing $\lambda$ to adapt not only to local geometry but also to semantic context and temporal dynamics.

% The network $\lambda_\Phi$ then predicts the blending weight as:
% \begin{equation}
%     \lambda(z_t^{geo}) = \sigma\left( \text{MLP}_\Phi\left(z_t \right) \right),
% \end{equation}
% where $\text{MLP}_\Phi$ is a small multi-layer perceptron (e.g., 2 layers, 64 hidden units) that fuses the geometric feature $\tilde{\rho}(z_t^{geo})$, and $\sigma(\cdot)$ is the sigmoid function, ensuring $\lambda \in (0,1)$.


% % ---------------------
% % NLerp

% \section{GeodesicFlow: Adaptive Metric-Free Flow Matching on Sphere Manifolds}

% Our goal is to learn a \textit{text-conditioned} time-dependent vector field $v_\Theta: \mathcal{M} \times [0,1] \times \mathcal{C} \to T\mathcal{M}$, where $v_\Theta(x, t, c) \in T_x\mathcal{M}$, that governs a continuous transformation of samples from a simple base distribution $p_1$ (e.g., uniform noise on the sphere) into samples from a complex, \textit{text-conditioned} target data distribution $p_0(\cdot \mid c)$. This transformation is realized as the solution to an ordinary differential equation (ODE) on the manifold, where the vector field $v_\Theta$ dictates the instantaneous direction and speed of motion at each point, time, and given text condition $c$.

% We restrict $\mathcal{M}$ to be the unit sphere $\mathbb{S}^n \subset \mathbb{R}^{n+1}$ endowed with its canonical round metric. Although $\mathbb{S}^n$ is a curved Riemannian manifold, its isometric embedding in Euclidean space allows us to compute all necessary geometric operations — exponential/logarithmic maps, parallel transport, and norm evaluations — using only ambient-space linear algebra, \textit{without ever explicitly evaluating or storing the metric tensor}. This yields a computationally efficient, \textbf{metric-free} implementation while preserving geometric fidelity.

% Critically, this is not a Euclidean method: while we use the Euclidean norm $\|\cdot\|_2$ for loss computation, the vectors $v_\Theta(z_t, t, c)$ and $u_t$ are constrained to lie in the tangent space $T_{z_t}\mathbb{S}^n$, and their evolution follows curved geodesics governed by the sphere’s intrinsic geometry. In contrast, a true Euclidean flow (as in the attached Rectified Flow paper) uses linear interpolation and constant velocities — violating the manifold structure. Here, the Euclidean norm serves only as a \textit{computational proxy}: because the Riemannian metric on $\mathbb{S}^n$ is induced from $\mathbb{R}^{n+1}$, we have $\|v\|_{g(x)} = \|v\|_2$ for all $v \in T_x\mathbb{S}^n$. Thus, our optimization remains geometrically faithful to the curved manifold — it is efficient, not approximate.

% \subsection{Adaptive Geometric Blending: Learning the Optimal Path Between Euclidean and Geodesic Flows}
% \label{sec:adaptive_blend}

% While geodesic paths are geometrically natural, they may not always be optimal for sample quality. The “true” optimal path for generating realistic images may lie \textit{between} the geodesic and Euclidean extremes: geodesics may traverse low-density “holes” in the data manifold, while Euclidean paths may barrel through semantically implausible regions. A static blend of the two losses (e.g., fixed $\lambda$) offers a global compromise, but fails to adapt to local geometric and semantic structure.

% Inspired by the adaptive noise schedule re-weighting in the attached paper (Sec 3.1), we propose an \textbf{adaptive geometric blending} mechanism that dynamically adjusts the trade-off between Euclidean and geodesic flows based on local data geometry and density. This yields a time- and location-dependent weight $\lambda(z_t^{geo})$ that optimizes for sample realism, diversity, and training stability.

% Formally, our total loss becomes:
% \begin{equation}
%     \mathcal{L}_{\text{Adaptive}}(\Theta) = \mathbb{E}_{\substack{t \sim \mathcal{U}[0,1] \\ x_0 \sim p_0(\cdot \mid c) \\ x_1 \sim p_1 \\ c \sim p_{\text{text}}}} \left[ 
%     \big(1 - \lambda(z_t^{geo})\big) \cdot \left\| v_\Theta(z_t^{\text{euc}}, t, c) - u_t^{\text{euc}} \right\|^2 + 
%     \lambda(z_t^{geo}) \cdot \left\| v_\Theta(z_t^{\text{geo}}, t, c) - u_t^{\text{geo}} \right\|^2 
%     \right],
% \end{equation}
% where $z_t^{\text{geo}} = \text{NLerp}(x_0, x_1; t)$ is the normalized linear interpolant (approximating the geodesic); $z_t^{\text{euc}} = (1-t)x_0 + t x_1$ is the Euclidean (straight-line) interpolant; $u_t^{\text{geo}} = P_{\gamma, t \leftarrow 0}(\log_{x_0}(x_1))$ is the parallel-transported geodesic velocity; and $u_t^{\text{euc}} = x_1 - x_0$ is the constant Euclidean velocity.

% \subsection{Learned Criterion for $\lambda(z_t^{geo})$}

% Rather than relying on a fixed analytic form, we propose to learn the adaptive blending weight $\lambda(z_t^{geo})$ using a lightweight neural network $\lambda_\Phi: \mathbb{S}^n \times [0,1] \times \mathcal{C} \to [0,1]$, parameterized by $\Phi$. This network takes as input the current sample position $z_t$, time $t$, and text condition $c$, allowing $\lambda$ to adapt not only to local geometry but also to semantic context and temporal dynamics.

% To preserve interpretability and inject geometric inductive bias, we condition $\lambda_\Phi$ on a set of meaningful features derived from the geodesic structure. Specifically, we compute $\rho(z_t) = \| u_t^{\text{geo}} \|_2 \in [0, \pi]$,

% We normalize this feature to be in $[0,1]$ via a normalized density proxy $\tilde{\rho}(z_t^{geo}) = 1 - \frac{\| u_t^{\text{geo}} \|_2}{\pi}$,
% so that $\tilde{\rho} \approx 1$ corresponds to high-confidence (dense) regions, and $\tilde{\rho} \approx 0$ to low-confidence (sparse) regions.

% The norm $\| u_t^{\text{geo}} \|_2 = \arccos(x_0^\top x_1)$ reflects the geodesic distance between $x_0$ and $x_1$, and serves as a natural proxy for local data density and model uncertainty. Small values indicate that the interpolation path lies in a geometrically compact, densely populated region, where the learned vector field is well-constrained and following the curved geodesic is safe and semantically meaningful. Conversely, large values signal sparse or uncertain regions, where forcing geodesic motion risks traversing implausible or out-of-distribution areas. In such cases, falling back to Euclidean motion (via projection) acts as a stabilizing prior, avoiding overconfident extrapolation while remaining on-manifold.

% The normalized density proxy $\tilde{\rho}(z_t^{geo})$ induces a self-stabilizing curriculum: early in training, high uncertainty favors Euclidean targets; as the model improves, lower norms in plausible regions encourage geometry-aware geodesic flow. The mechanism requires no explicit density estimation, is computationally free, and aligns sampling behavior with the adaptive policy learned during training.


% The network $\lambda_\Phi$ then predicts the blending weight as $\lambda(z_t^{geo}) = \sigma\left( \text{MLP}_\Phi\left(z_t \right) \right)$,
% where $\text{MLP}_\Phi$ is a small multi-layer perceptron (e.g., 2 layers, 64 hidden units) that fuses the geometric feature $\tilde{\rho}(z_t^{geo})$, and $\sigma(\cdot)$ is the sigmoid function, ensuring $\lambda \in (0,1)$.

% \noindent\textbf{Regularizing $\lambda_\Phi$ with an Auxiliary Loss}
% To prevent $\lambda_\Phi$ from ignoring the geometric prior or collapsing to trivial solutions (e.g., always 0 or 1), we introduce a lightweight auxiliary regularization loss that encourages $\lambda$ to correlate with the interpretable density signal $\tilde{\rho}$, i.e., 
% \[
%     \mathcal{L}_{\lambda}(\Phi) = \mathbb{E} \left[ \left( \lambda(z_t^{geo}) - \tilde{\rho}(z_t^{geo}) \right)^2 \right].
% \]

% This loss gently anchors $\lambda$ to the geometrically motivated baseline: when no stronger signal is present, $\lambda \approx \tilde{\rho}$. But when semantic or temporal context suggests a different blending strategy (e.g., ``draw a straight road'' in a sparse region), the network is free to override the prior. We combine this with the main flow matching loss, $\mathcal{L}_{\text{Adaptive}} + \eta \cdot \mathcal{L}_{\lambda}$,
% where $\eta > 0$ is a small regularization coefficient (default: $\eta = 0.1$) that balances geometric faithfulness with adaptive flexibility.

% The motivations for adaptive blending are three-fold.

% 1) \textit{Self-Stabilizing Curriculum via Learned Uncertainty}: Early in training, when $u_t^{\text{geo}}$ is poorly estimated (large norm), $\tilde{\rho}$ is small, and $\mathcal{L}_\lambda$ encourages $\lambda \to 0$, favoring the stable Euclidean target. As training progresses and geodesic predictions become reliable, $\tilde{\rho}$ increases, and $\lambda$ follows — inducing a \textit{built-in, data-driven curriculum}. Unlike fixed schedules, this adapts per-sample and per-prompt, and is stabilized by the auxiliary loss.

% 2) \textit{Semantic- and Geometry-Aware Path Optimization}: The network can learn to blend paths not just based on local density, but also based on what is being generated. For instance, for prompts describing rigid or structured objects (e.g., ``a building''), the model may learn to prefer Euclidean paths even in geometrically dense regions, for sharper edges. For organic or curved concepts (``a swirling galaxy'', ``a dolphin''), it may favor geodesic motion to preserve natural curvature — even if local density is moderate. The auxiliary loss ensures these adaptations are intentional and grounded, not random or degenerate.

% 3) \textit{Minimal Overhead, Maximum Flexibility}: The network $\lambda_\Phi$ is lightweight and computed in parallel with $v_\Theta$. It introduces negligible computational cost but significantly increases modeling capacity. All geometric operations remain metric-free and sphere-compliant.

% \subsection{Geodesic Probability Path and Target Velocity Field}
% As outlined in Algorithm~\ref{alg:training_geodesicflow_t2i}, each training step begins by sampling a data point $x_0 \sim p_0(\cdot \mid c)$ and a noise point $x_1 \sim p_1$. To construct the flow matching objective, we define two distinct probability paths connecting these endpoints: one that respects the intrinsic geometry of the sphere (approximated via NLerp) and another that operates in the ambient Euclidean space.

% The geodesic path on the sphere $\mathbb{S}^n$ is approximated by normalizing the linear interpolation between $x_0$ and $x_1$. A point $z_t^{\text{geo}}$ along this path is calculated using NLerp:
% \begin{equation*}
%     z_t^{\text{geo}} = \frac{(1-t) x_0 + t x_1}{\|(1-t) x_0 + t x_1\|_2}.
% \end{equation*}
% Note: This is valid as long as $(1-t)x_0 + t x_1 \neq 0$, which holds almost surely for $x_0, x_1 \in \mathbb{S}^n$ and $t \in (0,1)$, since antipodal points have measure zero under typical distributions.

% The corresponding target velocity field $u_t^{\text{geo}}$ is generated by first computing the initial tangent vector $v_0 = \log_{x_0}(x_1)$ and then moving it along the path via parallel transport. The formulas used in the algorithm are:
% \begin{align*}
%     v_0 = \theta \cdot \frac{x_1 - (x_0^\top x_1)x_0}{\|x_1 - (x_0^\top x_1)x_0\|_2}, \quad 
%     u_t^{\text{geo}} = v_0 - \frac{v_0^\top z_t^{\text{geo}}}{1 - (x_0^\top x_1)^2} (x_1 - (x_0^\top x_1) x_0),
% \end{align*}
% where $\theta = \arccos(x_0^\top x_1)$.

% For contrast, the Euclidean path is the simple straight-line interpolation between the points in the ambient space $\mathbb{R}^{n+1}$. The path and its constant velocity vector are given by:
% \begin{align*}
%     z_t^{\text{euc}} = (1-t) x_0 + t x_1, \quad 
%     u_t^{\text{euc}} = x_1 - x_0.
% \end{align*}
% These two sets of paths ($z_t^{\text{geo}}, z_t^{\text{euc}}$) and target velocities ($u_t^{\text{geo}}, u_t^{\text{euc}}$) provide the ground truths for the adaptive blended loss function, which trains the network $v_\Theta$ to approximate both geometric and linear flows.

% \subsection{Generative Sampling via Geodesic Integration}
% To generate a sample for a given text condition $c$, we numerically integrate the underlying ODE backward in time from $t=1$ to $t=0$, starting with a random noise sample $z_1 \sim p_1$. Crucially, to maintain consistency with the adaptive training objective, each integration step is not a simple geodesic or Euclidean update, but rather a dynamic blend of both motions. This ensures that the path taken during inference respects the learned trade-offs between geometric purity and linear stability. At each discrete timestep $t$, we first compute a single velocity vector $v = v_\Theta(z_t, t, c)$. This vector is then used to determine two distinct potential destinations: a geodesic destination $z^{\text{geo}}$, found by moving along the manifold's geodesic using the exponential map, and a Euclidean destination $z^{\text{euc}}$, found by taking a linear step in the ambient space $\mathbb{R}^{n+1}$ and then projecting the result back onto the sphere $\mathbb{S}^n$. An adaptive blending weight $\lambda_t = \lambda_\Phi(z_t)$ is computed using the trained network $\lambda_\Phi$. The final point for the next step, $z_{t-\Delta t}$, is then computed by interpolating on the sphere between the \textit{Euclidean} and \textit{geodesic} destinations, weighted by $\lambda_t$, using normalized linear interpolation (NLerp) with arguments ordered to ensure $\lambda=0$ yields pure Euclidean motion. That is, we compute:
% \[
% z_{t-\Delta t} = \text{NLerp}(z^{\text{euc}}, z^{\text{geo}}; \lambda_t) = \frac{(1 - \lambda_t) z^{\text{euc}} + \lambda_t z^{\text{geo}}}{\|(1 - \lambda_t) z^{\text{euc}} + \lambda_t z^{\text{geo}}\|_2},
% \]
% which guarantees that when $\lambda_t = 0$, the update is purely Euclidean (after normalization), and when $\lambda_t = 1$, it is purely geodesic (approximated via NLerp). More details can be found in Algorithm \ref{alg:sampling_geodesicflow_t2i}.

% This procedure ensures that the sampling path is dynamically constructed, leveraging the stability of Euclidean steps in uncertain regions and the geometric fidelity of geodesic steps (via NLerp) in well-defined regions, exactly as encouraged during training. All operations remain in the ambient space $\mathbb{R}^{n+1}$, preserving the metric-free efficiency of the framework.

% \begin{algorithm}[!t]
% \caption{Training GeodesicFlow with Density-Driven Adaptive Blending}
% \label{alg:training_geodesicflow_t2i}
% \begin{algorithmic}[1]
% \Require
% \Statex \textit{Models:} Network $v_\Theta: \mathbb{S}^n \times [0,1] \times \mathcal{C} \to T\mathbb{S}^n$ with parameters $\Theta$, $\text{MLP}_{\Phi}$ with parameters $\Phi$.
% \Statex \textit{Data:} Text-conditioned distribution $p_0(\cdot \mid c)$, uniform noise $p_1$ on $\mathbb{S}^n$, text prior $p_{\text{text}}$.
% \Statex \textit{Hyperparameters:} Batch size $B$, steps $N_{\text{steps}}$, learning rate $\alpha_{\text{lr}}$, regularization weight $\eta$.
% \State Initialize model parameters $\Theta$, network parameters $\Phi$.
% \State Initialize optimizer (e.g., AdamW) with learning rate $\alpha_{\text{lr}}$.
% \For{step = 1 to $N_{\text{steps}}$}
%     \State Sample mini-batch: $\{c^{(i)}\}_{i=1}^B \sim p_{\text{text}}$, $\{x_0^{(i)}\}_{i=1}^B \sim p_0(\cdot \mid c^{(i)})$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
%     \State Initialize batch loss $\mathcal{L}_{\text{batch}} \leftarrow 0$.
%     \For{$i = 1$ to $B$}
%         \State Let $c \leftarrow c^{(i)}$, $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
%         \State Compute $\theta \leftarrow \arccos(x_0^\top x_1)$.
%         \State Compute $v_0 \leftarrow \theta \cdot \frac{x_1 - (x_0^\top x_1)x_0}{\|x_1 - (x_0^\top x_1)x_0\|_2}$.
%         \State Compute $z_t^{\text{geo}} \leftarrow \frac{(1-t) x_0 + t x_1}{\|(1-t) x_0 + t x_1\|_2}$.
%         \State Compute $u_t^{\text{geo}} \leftarrow v_0 - \frac{v_0^\top z_t^{\text{geo}}}{1 - (x_0^\top x_1)^2} (x_1 - (x_0^\top x_1) x_0)$.
%         \State Compute $z_t^{\text{euc}} \leftarrow (1-t) x_0 + t x_1$.
%         \State Compute $u_t^{\text{euc}} \leftarrow x_1 - x_0$.
%         \State Compute density proxy: $\rho \leftarrow \| u_t^{\text{geo}} \|_2$.
%         \State Compute adaptive weight: $\lambda \leftarrow \sigma\left( \text{MLP}_\Phi\left(z_t \right) \right)$.
%         \State Compute normalized density proxy: $\tilde{\rho}(z_t^{geo}) = 1 - \rho / \pi$.
%         \State Compute $\mathcal{L}_{\lambda} = \left( \lambda - \tilde{\rho}(z_t^{geo}) \right)^2$.
%         \State Predict velocities: $\hat{u}_t^{\text{geo}} \leftarrow v_\Theta(z_t^{\text{geo}}, t, c)$, $\hat{u}_t^{\text{euc}} \leftarrow v_\Theta(z_t^{\text{euc}}, t, c)$.
%         \State Compute blended loss: 
%         \[
%             \mathcal{L}^{(i)} \leftarrow (1 - \lambda) \cdot \| \hat{u}_t^{\text{euc}} - u_t^{\text{euc}} \|^2 + \lambda \cdot \| \hat{u}_t^{\text{geo}} - u_t^{\text{geo}} \|^2.
%         \]
%         \State $\mathcal{L}_{\text{batch}} \leftarrow \mathcal{L}_{\text{batch}} + \mathcal{L}^{(i)} + \eta \cdot \mathcal{L}_{\lambda}$.
%     \EndFor
%     \State Compute mean loss: $\mathcal{L} \leftarrow \frac{1}{B} \mathcal{L}_{\text{batch}}$.
%     \State Update parameters: $\Theta \leftarrow \text{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$.
% \EndFor
% \State \Return Trained parameters $\Theta$, network $\Phi$.
% \end{algorithmic}
% \end{algorithm}

% \vspace{1cm}

% \begin{algorithm}[!t]
% \caption{Adaptive Geodesic-Euclidean Sampling (AGES) from Trained GeodesicFlow}
% \label{alg:sampling_geodesicflow_t2i}
% \begin{algorithmic}[1]
% \Require
% \Statex \textit{Model:} Trained $v_\Theta$, and trained $\Phi$.
% \Statex \textit{Text Embedding:} Condition $c \in \mathcal{C}$.
% \Statex \textit{Noise:} $z_1 \sim \text{Uniform}(\mathbb{S}^n)$.
% \Statex \textit{Hyperparameters:} Integration steps $N$, blending mode (learned or analytic $\lambda$).
% \State Set $\Delta t \leftarrow 1/N$.
% \For{$k = N$ \textbf{downto} $1$}
%     \State Set $t \leftarrow k \cdot \Delta t$.
    
%     \State Compute $\lambda \leftarrow \lambda_\Phi(z_t)$.
%     \State Predict velocity: $v \leftarrow v_\Theta(z_t, t, c)$.
    
%     \State \textbf{Compute blended step:}
%     \State \quad $\xi \leftarrow -\Delta t \cdot v$  \Comment{Shared tangent vector for both paths}
    
%     \State \textbf{Geodesic component:}
%     \State \quad \textbf{if} $\|\xi\| > 0$ \textbf{then}
%     \State \quad \quad $\hat{\xi} \leftarrow \xi / \|\xi\|$
%     \State \quad \quad $z^{\text{geo}} \leftarrow \cos(\|\xi\|) z_t + \sin(\|\xi\|) \hat{\xi}$
%     \State \quad \textbf{else}
%     \State \quad \quad $z^{\text{geo}} \leftarrow z_t$  \Comment{No movement if velocity is zero}
%     \State \quad \textbf{end if}
    
%     \State \textbf{Euclidean component:}
%     \State \quad $z^{\text{euc}} \leftarrow z_t + \xi$  \Comment{Straight step in ambient space}
%     \State \quad $z^{\text{euc}} \leftarrow z^{\text{euc}} / \|z^{\text{euc}}\|_2$  \Comment{Project back to sphere}
    
%     \State \textbf{Blend positions on-manifold:}
%     \State \quad $z_{t-\Delta t} \leftarrow \text{NLerp}(z^{\text{euc}}, z^{\text{geo}}; \lambda) = \frac{(1 - \lambda) z^{\text{euc}} + \lambda z^{\text{geo}}}{\|(1 - \lambda) z^{\text{euc}} + \lambda z^{\text{geo}}\|_2}$
%     \Comment{Interpolate: $\lambda=0$ → Euclidean, $\lambda=1 \rightarrow$ Geodesic (via NLerp)}
    
% \EndFor
% \State \Return Generated sample $z_0$ aligned with text $c$.
% \end{algorithmic}
% \end{algorithm}

% ------------------------
% \section{GeodesicFlow: Dual-Target Ambient Flow Matching via Slerp}

% We introduce \textbf{GeodesicFlow}, a generative modeling framework for data lying on or near Riemannian manifolds embedded in Euclidean space. Our approach learns an ambient time-dependent velocity field $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$ that governs a continuous transformation from a simple base distribution $p_1$ (e.g., uniform noise on the manifold) to a complex data distribution $p_0$. 

% Crucially, while the model operates in ambient space $\mathbb{R}^D$, its training objective is designed to respect the underlying manifold geometry — without requiring explicit Riemannian operators (e.g., exponential maps, parallel transport, or metric tensors). This enables:
% \begin{itemize}
%     \item \textbf{Geometric fidelity}: The model learns to replicate curvature-aware motion intrinsic to the manifold.
%     \item \textbf{Euclidean flexibility}: The same model can generate samples in $\mathbb{R}^D$ without manifold constraints — useful for interpolation, robustness, or hybrid modeling.
%     \item \textbf{Plug-and-play compatibility}: Sampling uses standard ODE solvers from Euclidean Flow Matching, with optional projection for manifold adherence.
% \end{itemize}


% The core innovation of GeodesicFlow is \textbf{Dual-Target Flow Matching}: we train the model to simultaneously match two distinct but complementary velocity targets:
% \begin{enumerate}
%     \item A \textbf{Riemannian target} derived from Spherical Linear Interpolation (Slerp) — a computationally efficient surrogate for geodesics on spherical and rotation manifolds.
%     \item An \textbf{Euclidean target} derived from linear interpolation — preserving smooth, semantically meaningful structure in the ambient space.
% \end{enumerate}

% This dual-target design ensures that the learned flow respects both the intrinsic geometry of the manifold \textit{and} the extrinsic structure of the embedding space — yielding a more robust, flexible, and semantically coherent generative model.

% \subsection{Slerp as a Geodesic Surrogate}

% Let $x_0 \sim p_0$ (data point) and $x_1 \sim p_1$ (noise point), both lying on a manifold $\mathcal{M} \subset \mathbb{R}^D$. While computing true geodesics may be intractable or expensive, Slerp provides a geometrically faithful, computationally efficient approximation — particularly on hyperspheres and rotation groups.

% The Slerp interpolation path is defined as:
% \begin{equation}
%     z_t^{\text{riem}} = \mathrm{Slerp}(x_0, x_1; t) := \frac{\sin((1-t)\theta)}{\sin(\theta)} x_0 + \frac{\sin(t\theta)}{\sin(\theta)} x_1,
% \end{equation}
% where $\theta = \cos^{-1}(\langle x_0, x_1 \rangle)$ is the angle between $x_0$ and $x_1$ (assuming unit norm or appropriate normalization). Slerp traces the shortest arc on the great circle connecting $x_0$ and $x_1$, making it a natural geodesic proxy for spherical geometries.

% The \textbf{Riemannian target velocity} is the time derivative of this path:
% \begin{equation}
%     u_t^{\text{riem}} = \frac{d}{dt} \mathrm{Slerp}(x_0, x_1; t) = \frac{\theta}{\sin(\theta)} \left[ \cos(t\theta) x_1 - \cos((1-t)\theta) x_0 \right].
% \end{equation}
% By construction, $u_t^{\text{riem}} \in T_{z_t^{\text{riem}}}\mathcal{M}$ — it is tangent to the manifold. However, we treat it as an unconstrained vector in $\mathbb{R}^D$ during training, allowing the model to learn geometry-aware motion without hard tangent-space constraints.

% \subsection{Euclidean Target via Linear Interpolation}

% To preserve meaningful structure in the ambient space, we also include the Euclidean target that defined by linear interpolation:
% \begin{equation}
%     z_t^{\text{euc}} = (1-t) x_0 + t x_1, \quad u_t^{\text{euc}} = x_0 - x_1.
% \end{equation}
% This constant-velocity path ignores manifold curvature but ensures smooth, intuitive motion in $\mathbb{R}^D$ — useful for off-manifold interpolation, semantic consistency, or downstream Euclidean tasks.

% \subsection{Dual-Target Training Objective}

% We train the model $v_\Theta$ to minimize a composite loss that balances fidelity to both targets:
% \begin{equation}
%     \mathcal{L}_{\mathrm{GeodesicFlow}}(\Theta) = 
%     \lambda_{\text{riem}} \cdot \mathbb{E}_{t, x_0, x_1} \left[ \left\| v_\Theta(z_t^{\text{riem}}, t) - u_t^{\text{riem}} \right\|^2 \right]
%     + \lambda_{\text{euc}} \cdot \mathbb{E}_{t, x_0, x_1} \left[ \left\| v_\Theta(z_t^{\text{euc}}, t) - u_t^{\text{euc}} \right\|^2 \right],
% \end{equation}
% where:
% \begin{itemize}
%     \item $z_t^{\text{riem}} = \mathrm{Slerp}(x_0, x_1; t)$, $u_t^{\text{riem}} = \frac{d}{dt} \mathrm{Slerp}(x_0, x_1; t)$,
%     \item $z_t^{\text{euc}} = (1-t) x_0 + t x_1$, $u_t^{\text{euc}} = x_0 - x_1$,
%     \item $\lambda_{\text{riem}}, \lambda_{\text{euc}} \geq 0$ are tunable weights controlling the trade-off between geometric and ambient priors.
% \end{itemize}


% This objective encourages the model to learn a velocity field that:
% \begin{itemize}
%     \item Flows along approximately geodesic paths when near the manifold (via Slerp target),
%     \item Flows along semantically smooth paths in ambient space (via linear target),
%     \item Generalizes gracefully between on- and off-manifold regions.
% \end{itemize}


% In the special case $\lambda_{\text{euc}} = 0$, this reduces to the original Ambient GeodesicFlow — preserving backward compatibility.

% \subsection{Generative Sampling: Plug-and-Play with Flow Matching}

% Once trained, sampling from GeodesicFlow is identical to standard Euclidean Flow Matching — with optional manifold projection for geometric fidelity.

% Starting from $z_1 \sim p_1$, we integrate the ODE backward in time:
% \begin{equation}
%     \frac{d z_t}{dt} = v_\Theta(z_t, t).
% \end{equation}

% We support two sampling modes:

% \begin{description}
%     \item[\textbf{Euclidean-Unconstrained}] Integrate directly in $\mathbb{R}^D$:
%     \begin{equation}
%         z_{t - \Delta t} = z_t - \Delta t \cdot v_\Theta(z_t, t).
%     \end{equation}
%     This allows off-manifold generation — useful for interpolation, anomaly detection, or hybrid modeling.

%     \item[\textbf{Manifold-Constrained}] Project after each step to enforce manifold adherence:
%     \begin{equation}
%         z_{t - \Delta t} = \Pi_{\mathcal{M}}\left( z_t - \Delta t \cdot v_\Theta(z_t, t) \right),
%     \end{equation}
%     where $\Pi_{\mathcal{M}}$ is a cheap, manifold-specific projection (e.g., normalization for spheres, QR for Stiefel).
% \end{description}

% Higher-order ODE solvers (e.g., Dopri5, RK4) can be used without modification — making GeodesicFlow a true drop-in replacement for existing Flow Matching pipelines.

% \subsection{Algorithmic Implementation}

% Algorithms~\ref{alg:training_geodesicflow} and~\ref{alg:sampling_geodesicflow} summarize the training and sampling procedures. Training constructs both Slerp and linear interpolants, computes their respective velocities, and trains the model to match both — all within the ambient Euclidean space. Sampling leverages the same velocity field used in vanilla Flow Matching, with optional projection for geometric fidelity. This design ensures scalability, flexibility, and seamless integration with existing codebases — while preserving optional manifold structure.

% \begin{algorithm}[H]
% \caption{Training GeodesicFlow}
% \label{alg:training_geodesicflow}
% \begin{algorithmic}[1]
% \Require
% \Statex \textit{Model:} Neural network $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$.
% \Statex \textit{Data:} Distributions $p_0$ (data on $\mathcal{M}$), $p_1$ (noise on $\mathcal{M}$), $\mathcal{M} \subset \mathbb{R}^D$.
% \Statex \textit{Hyperparameters:} Weights $\lambda_{\text{riem}}, \lambda_{\text{euc}}$, batch size $B$, steps $N_{\text{steps}}$, learning rate $\alpha$.
% \State Initialize model parameters $\Theta$.
% \State Initialize optimizer (e.g., AdamW) with learning rate $\alpha$.
% \For{step = 1 to $N_{\text{steps}}$}
%     \State Sample mini-batch: $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
%     \State Initialize batch loss $\mathcal{L}_{\text{batch}} \leftarrow 0$.
%     \For{$i = 1$ to $B$}
%         \State Let $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
        
%         \State \textbf{// Riemannian (Slerp) target}
%         \State $\theta \leftarrow \cos^{-1}(\langle x_0, x_1 \rangle)$ \Comment{Clamp for stability}
%         \State $z_t^{\text{riem}} \leftarrow \frac{\sin((1-t)\theta)}{\sin(\theta)} x_0 + \frac{\sin(t\theta)}{\sin(\theta)} x_1$
%         \State $u_t^{\text{riem}} \leftarrow \frac{\theta}{\sin(\theta)} \left[ \cos(t\theta) x_1 - \cos((1-t)\theta) x_0 \right]$
%         \State $\hat{u}_t^{\text{riem}} \leftarrow v_\Theta(z_t^{\text{riem}}, t)$
%         \State $\mathcal{L}_{\text{riem}}^{(i)} \leftarrow \left\| \hat{u}_t^{\text{riem}} - u_t^{\text{riem}} \right\|^2$
        
%         \State \textbf{// Euclidean (Linear) target}
%         \State $z_t^{\text{euc}} \leftarrow (1-t) x_0 + t x_1$
%         \State $u_t^{\text{euc}} \leftarrow x_0 - x_1$
%         \State $\hat{u}_t^{\text{euc}} \leftarrow v_\Theta(z_t^{\text{euc}}, t)$
%         \State $\mathcal{L}_{\text{euc}}^{(i)} \leftarrow \left\| \hat{u}_t^{\text{euc}} - u_t^{\text{euc}} \right\|^2$
        
%         \State \textbf{// Composite loss}
%         \State $\mathcal{L}^{(i)} \leftarrow \lambda_{\text{riem}} \cdot \mathcal{L}_{\text{riem}}^{(i)} + \lambda_{\text{euc}} \cdot \mathcal{L}_{\text{euc}}^{(i)}$
%         \State $\mathcal{L}_{\text{batch}} \leftarrow \mathcal{L}_{\text{batch}} + \mathcal{L}^{(i)}$
%     \EndFor
%     \State $\mathcal{L} \leftarrow \frac{1}{B} \mathcal{L}_{\text{batch}}$
%     \State Update $\Theta \leftarrow \mathrm{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$.
% \EndFor
% \State \Return Trained parameters $\Theta$.
% \end{algorithmic}
% \end{algorithm}

% ---------------------------
% \section{GeodesicFlow: Adaptive Ambient Flow Matching via Blended Geodesic Interpolation}

% We introduce \textbf{GeodesicFlow}, a generative modeling framework for data lying on or near Riemannian manifolds embedded in Euclidean space. Our approach learns an ambient time-dependent velocity field $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$ that governs a continuous transformation from a simple base distribution $p_1$ (e.g., uniform noise on the manifold) to a complex data distribution $p_0$.

% Crucially, while the model operates in ambient space $\mathbb{R}^D$, its training objective is designed to respect the underlying manifold geometry—without requiring explicit Riemannian operators (e.g., exponential maps, parallel transport, or metric tensors). This enables:
% \begin{itemize}
%     \item \textbf{Geometric fidelity}: The model learns curvature-aware motion intrinsic to the manifold.
%     \item \textbf{Euclidean flexibility}: The same model can generate samples in $\mathbb{R}^D$ without manifold constraints—useful for interpolation, robustness, or hybrid modeling.
%     \item \textbf{Plug-and-play compatibility}: Sampling uses standard ODE solvers from Euclidean Flow Matching, with optional projection for manifold adherence.
% \end{itemize}


% The core innovation of GeodesicFlow is \textbf{Adaptive Path Flow Matching}: we define a \textit{single}, differentiable interpolation path that smoothly blends geodesic-like motion (via Slerp) and ambient linear interpolation. This unified path induces a unique target velocity field, ensuring coherent and stable training—while preserving the dual geometric and semantic desiderata of the original dual-target design.

% \subsection{Slerp as a Geodesic Surrogate}

% Let $x_0 \sim p_0$ (data point) and $x_1 \sim p_1$ (noise point), both assumed to lie on a manifold $\mathcal{M} \subset \mathbb{R}^D$ (e.g., the unit hypersphere $\mathbb{S}^{D-1}$ or rotation group $\mathrm{SO}(n)$). While computing true geodesics may be intractable, Spherical Linear Interpolation (Slerp) provides a geometrically faithful and computationally efficient approximation on spherical and rotation manifolds.

% Assuming unit-norm inputs (or appropriate normalization), the Slerp path is:
% \begin{equation}
%     z_t^{\text{riem}} = \mathrm{Slerp}(x_0, x_1; t) := \frac{\sin((1-t)\theta)}{\sin(\theta)} x_0 + \frac{\sin(t\theta)}{\sin(\theta)} x_1,
% \end{equation}
% where $\theta = \cos^{-1}(\langle x_0, x_1 \rangle) \in [0, \pi]$ is the angular distance. Slerp traces the shortest arc on the great circle connecting $x_0$ and $x_1$, making it a natural geodesic proxy.

% Its time derivative—the \textbf{Riemannian target velocity}—is:
% \begin{equation}
%     u_t^{\text{riem}} = \frac{d}{dt} \mathrm{Slerp}(x_0, x_1; t) = \frac{\theta}{\sin(\theta)} \left[ \cos(t\theta) x_1 - \cos((1-t)\theta) x_0 \right].
% \end{equation}
% By construction, $u_t^{\text{riem}}$ is tangent to $\mathcal{M}$ at $z_t^{\text{riem}}$, but we treat it as an unconstrained vector in $\mathbb{R}^D$ during training.

% \subsection{Unified Adaptive Interpolation Path}

% To reconcile geometric fidelity with ambient smoothness in a \textit{coherent} manner, we define a single interpolation path that blends Slerp and linear interpolation via a time-dependent mixing function $\alpha: [0,1] \to [0,1]$:
% \begin{equation}
%     z_t = (1 - \alpha(t)) \cdot z_t^{\text{riem}} + \alpha(t) \cdot z_t^{\text{euc}},
% \end{equation}
% where $z_t^{\text{euc}} = (1-t)x_0 + t x_1$ is the Euclidean linear interpolant.

% The corresponding \textbf{target velocity} is the exact time derivative of $z_t$:
% \begin{equation}
%     u_t = \frac{d}{dt} z_t = (1 - \alpha(t)) u_t^{\text{riem}} + \alpha(t) u_t^{\text{euc}} - \alpha'(t) \left( z_t^{\text{riem}} - z_t^{\text{euc}} \right),
% \end{equation}
% with $u_t^{\text{euc}} = x_0 - x_1$. The correction term $-\alpha'(t)(z_t^{\text{riem}} - z_t^{\text{euc}})$ is essential to ensure $u_t = \dot{z}_t$, satisfying the fundamental requirement of Flow Matching.

% We adopt the simple linear schedule $\alpha(t) = t$, which yields $\alpha'(t) = 1$. This choice emphasizes geometric fidelity near $t=0$ (where data resides) and ambient smoothness near $t=1$ (where noise resides), aligning naturally with the reverse-time sampling direction. Alternative schedules (e.g., $\alpha(t) = t^2$ or learnable $\alpha$) can be used for task-specific trade-offs.

% \subsection{Stable Slerp Computation}

% To ensure numerical stability, we clamp the angle $\theta$ away from singularities:
% \begin{equation}
%     \theta \leftarrow \mathrm{clamp}\big(\cos^{-1}(\langle \hat{x}_0, \hat{x}_1 \rangle),\, \epsilon,\, \pi - \epsilon\big),
% \end{equation}
% with $\epsilon = 10^{-3}$ and $\hat{x} = x / \|x\|$ (for non-unit inputs). For $\theta < \epsilon$, we use the first-order Taylor approximation $\mathrm{Slerp}(x_0,x_1;t) \approx (1-t)x_0 + t x_1$, ensuring smooth behavior in the Euclidean limit.

% \subsection{Training Objective}

% GeodesicFlow minimizes the standard Flow Matching loss with respect to the unified path:
% \begin{equation}
%     \mathcal{L}_{\mathrm{GeodesicFlow}}(\Theta) = 
%     \mathbb{E}_{t, x_0, x_1} \left[ \left\| v_\Theta(z_t, t) - u_t \right\|^2 \right],
% \end{equation}
% where $z_t$ and $u_t$ are defined as above. This objective ensures that $v_\Theta$ learns the velocity field of a well-defined continuous probability path $\{p_t = \mathrm{Law}(z_t)\}_{t\in[0,1]}$, guaranteeing that integrating the ODE $\frac{dz}{dt} = v_\Theta(z,t)$ recovers $p_0$ from $p_1$.

% \subsection{Generative Sampling: Plug-and-Play with Flow Matching}

% Sampling from GeodesicFlow is identical to standard Euclidean Flow Matching—with optional manifold projection for geometric fidelity.

% Starting from $z_1 \sim p_1$, we integrate the ODE backward in time:
% \begin{equation}
%     \frac{d z_t}{dt} = v_\Theta(z_t, t).
% \end{equation}

% We support two sampling modes:

% \begin{description}
%     \item[\textbf{Euclidean-Unconstrained}] Integrate directly in $\mathbb{R}^D$ using any standard ODE solver (e.g., Euler, RK4, Dopri5):
%     \begin{equation}
%         z_{t - \Delta t} = z_t - \Delta t \cdot v_\Theta(z_t, t).
%     \end{equation}
%     This enables off-manifold generation—useful for interpolation, anomaly detection, or hybrid modeling.

%     \item[\textbf{Manifold-Constrained}] Project after each step to enforce manifold adherence:
%     \begin{equation}
%         z_{t - \Delta t} = \Pi_{\mathcal{M}}\left( z_t - \Delta t \cdot v_\Theta(z_t, t) \right),
%     \end{equation}
%     where $\Pi_{\mathcal{M}}$ is a cheap, manifold-specific projection (e.g., normalization for spheres, QR decomposition for Stiefel manifolds).
% \end{description}

% Higher-order solvers require no modification, making GeodesicFlow a true drop-in replacement for existing Flow Matching pipelines.

% \subsection{Algorithmic Implementation}

% Algorithm~\ref{alg:training_geodesicflow} summarizes the training procedure. The method constructs a unified interpolation path blending Slerp and linear motion, computes its exact time derivative, and trains the model to match this single target—all within ambient Euclidean space. This design ensures scalability, stability, and seamless integration with existing codebases, while preserving optional manifold structure.

% \begin{algorithm}[H]
% \caption{Training GeodesicFlow (Unified Adaptive Path)}
% \label{alg:training_geodesicflow}
% \begin{algorithmic}[1]
% \Require
% \Statex \textit{Model:} Neural network $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$.
% \Statex \textit{Data:} Distributions $p_0$ (data on $\mathcal{M}$), $p_1$ (noise on $\mathcal{M}$), $\mathcal{M} \subset \mathbb{R}^D$.
% \Statex \textit{Hyperparameters:} Batch size $B$, steps $N_{\text{steps}}$, learning rate $\alpha$, stability $\epsilon = 10^{-3}$.
% \State Initialize model parameters $\Theta$.
% \State Initialize optimizer (e.g., AdamW) with learning rate $\alpha$.
% \For{step = 1 to $N_{\text{steps}}$}
%     \State Sample mini-batch: $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
%     \State Initialize batch loss $\mathcal{L}_{\text{batch}} \leftarrow 0$.
%     \For{$i = 1$ to $B$}
%         \State Let $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
%         \State Normalize: $\hat{x}_0 \leftarrow x_0 / \|x_0\|$, $\hat{x}_1 \leftarrow x_1 / \|x_1\|$.
        
%         \State \textbf{// Compute Slerp components}
%         \State $\theta \leftarrow \cos^{-1}(\langle \hat{x}_0, \hat{x}_1 \rangle)$
%         \State $\theta \leftarrow \mathrm{clamp}(\theta, \epsilon, \pi - \epsilon)$
%         \State $z_t^{\text{riem}} \leftarrow \frac{\sin((1-t)\theta)}{\sin(\theta)} \hat{x}_0 + \frac{\sin(t\theta)}{\sin(\theta)} \hat{x}_1$
%         \State $u_t^{\text{riem}} \leftarrow \frac{\theta}{\sin(\theta)} \left[ \cos(t\theta) \hat{x}_1 - \cos((1-t)\theta) \hat{x}_0 \right]$
        
%         \State \textbf{// Compute Euclidean components}
%         \State $z_t^{\text{euc}} \leftarrow (1-t) \hat{x}_0 + t \hat{x}_1$
%         \State $u_t^{\text{euc}} \leftarrow \hat{x}_0 - \hat{x}_1$
        
%         \State \textbf{// Unified path with $\alpha(t) = t$}
%         \State $\alpha \leftarrow t$, \quad $\alpha' \leftarrow 1$
%         \State $z_t \leftarrow (1 - \alpha) \cdot z_t^{\text{riem}} + \alpha \cdot z_t^{\text{euc}}$
%         \State $u_t \leftarrow (1 - \alpha) \cdot u_t^{\text{riem}} + \alpha \cdot u_t^{\text{euc}} - \alpha' \cdot (z_t^{\text{riem}} - z_t^{\text{euc}})$
        
%         \State \textbf{// Loss}
%         \State $\hat{u}_t \leftarrow v_\Theta(z_t, t)$
%         \State $\mathcal{L}^{(i)} \leftarrow \left\| \hat{u}_t - u_t \right\|^2$
%         \State $\mathcal{L}_{\text{batch}} \leftarrow \mathcal{L}_{\text{batch}} + \mathcal{L}^{(i)}$
%     \EndFor
%     \State $\mathcal{L} \leftarrow \frac{1}{B} \mathcal{L}_{\text{batch}}$
%     \State Update $\Theta \leftarrow \mathrm{OptimizerStep}(\Theta, \nabla_\Theta \mathcal{L})$.
% \EndFor
% \State \Return Trained parameters $\Theta$.
% \end{algorithmic}
% \end{algorithm}

% ---------------------
% improve self-containedness
\section{GeodesicFlow: Adaptive Ambient Flow Matching via Blended Geodesic Interpolation}

We introduce \textbf{GeodesicFlow}, a generative modeling framework designed for data that lies on or near a Riemannian manifold embedded in Euclidean space $\mathbb{R}^D$. The method learns an ambient, time-dependent velocity field $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$, parameterized by neural network weights $\Theta$, which governs a continuous transformation from a simple base distribution $p_1$—such as an isotropic Gaussian—to a complex data distribution $p_0$. Although the model operates entirely in the ambient Euclidean space $\mathbb{R}^D$, its training objective is constructed to respect the intrinsic geometry of the underlying data manifold without requiring explicit knowledge of Riemannian operators (e.g., the metric tensor, exponential map, or logarithmic map). This design preserves geometric structure while retaining compatibility with standard Euclidean flow architectures and solvers.

The core innovation of GeodesicFlow is \textbf{Adaptive Path Flow Matching}, which defines a single, differentiable interpolation trajectory between a data point and a noise sample by blending two geometrically motivated paths: one based on spherical linear interpolation (Slerp), which captures curvature-aware rotational motion on the unit sphere, and another based on standard linear interpolation in Euclidean space. The blending weight is not fixed but is instead dynamically determined from a local estimate of manifold curvature computed directly from the input pair. While the model operates in ambient space $\mathbb{R}^D$, its training objective leverages interpolation on the spherical manifold of directions, ensuring that the learned flow respects the intrinsic geometry of the data without requiring explicit Riemannian operators. This design achieves geometric fidelity by guiding the model along geodesic-like paths on the sphere of directions, while preserving meaningful scale through linear interpolation of vector magnitudes—a property especially important for latent representations such as those from variational autoencoders, where norm carries semantic information. Moreover, because the velocity field remains defined in Euclidean space and the sampling procedure is unchanged, GeodesicFlow maintains full compatibility with standard ODE solvers used in conventional Euclidean Flow Matching.

% The core innovation of GeodesicFlow is \textbf{Adaptive Path Flow Matching}, which defines a single, differentiable interpolation trajectory between a data point and a noise sample by blending two geometrically motivated paths: one based on spherical linear interpolation (Slerp), which captures curvature-aware rotational motion on the unit sphere, and another based on standard linear interpolation in Euclidean space. The blending weight is not fixed but is instead dynamically determined from a local estimate of manifold curvature, computed directly from the input pair.

% While the model operates in ambient space $\mathbb{R}^D$, its training objective is constructed using interpolation on the spherical manifold of directions, ensuring that the learned flow respects the intrinsic geometry of the data without requiring explicit Riemannian operators. This design achieves geometric fidelity by guiding the model along geodesic-like paths on the sphere of directions, thereby capturing curvature-aware motion. At the same time, it preserves meaningful scale by interpolating vector magnitudes linearly—a property especially important for latent representations such as those from variational autoencoders, where norm carries semantic information. Finally, because the velocity field is defined in Euclidean space and the sampling procedure remains unchanged, the method maintains full compatibility with standard ODE solvers used in Euclidean Flow Matching.

\subsection{Separating Magnitude and Direction}

The direction of a latent vector often encodes semantic or structural information about the data, while its magnitude reflects uncertainty, reconstruction quality, or scale. Moreover, the intrinsic geometry of the data manifold is primarily manifested in the directional component: for instance, clusters or continuous transformations in the data tend to correspond to paths on or near a sphere in latent space, even when magnitudes vary significantly. In contrast, standard Euclidean interpolation conflates changes in direction with changes in scale, potentially distorting the underlying manifold structure. To respect this geometric structure while preserving meaningful scale information, we explicitly decouple magnitude and direction.

Let $x_0 \in \mathbb{R}^D$ be a sample from the data distribution $p_0$ (e.g., a latent vector from a variational autoencoder), and let $x_1 \in \mathbb{R}^D$ be a sample from the base noise distribution $p_1$. While these vectors are not constrained to the unit hypersphere, their directions carry geometric information about the underlying manifold. To isolate this, we decompose each vector into its magnitude and direction:
$\|x_0\| = \sqrt{x_0^\top x_0}$, $\quad \|x_1\| = \sqrt{x_1^\top x_1}$, $\hat{x}_0 = \frac{x_0}{\|x_0\|}$, $\hat{x}_1 = \frac{x_1}{\|x_1\|}$,
% \[
% \|x_0\| = \sqrt{x_0^\top x_0}, \quad \|x_1\| = \sqrt{x_1^\top x_1}, \quad \hat{x}_0 = \frac{x_0}{\|x_0\|}, \quad \hat{x}_1 = \frac{x_1}{\|x_1\|},
% \]
where $\hat{x}_0, \hat{x}_1 \in \mathbb{S}^{D-1}$ denote the corresponding unit vectors on the $(D-1)$-dimensional unit sphere. The angular distance between these directions is defined as
\[
\theta = \cos^{-1}\big( \langle \hat{x}_0, \hat{x}_1 \rangle \big) \in [0, \pi],
\]
where $\langle \cdot, \cdot \rangle$ denotes the standard Euclidean inner product.

Using $\theta$, we define the unit spherical linear interpolation (Slerp) path between $\hat{x}_0$ and $\hat{x}_1$ as a function of time $t \in [0,1]$:
\[
z_t^{\text{riem\_unit}} = \mathrm{Slerp}(\hat{x}_0, \hat{x}_1; t) := \frac{\sin\big((1 - t)\theta\big)}{\sin(\theta)} \, \hat{x}_0 + \frac{\sin\big(t\theta\big)}{\sin(\theta)} \, \hat{x}_1.
\]
Its time derivative—the unit-direction velocity—is given by
\[
u_t^{\text{riem\_unit}} = \frac{d}{dt} z_t^{\text{riem\_unit}} = \frac{\theta}{\sin(\theta)} \Big[ \cos(t\theta) \, \hat{x}_1 - \cos\big((1 - t)\theta\big) \, \hat{x}_0 \Big].
\]
These expressions describe pure rotational motion on the sphere and form the directional backbone of our Riemannian-inspired path.

\subsection{Curvature-Aware Adaptive Blending}

To construct a full interpolation path in $\mathbb{R}^D$ that respects both geometry and scale, we blend two scale-aware trajectories: a Riemannian-inspired path that combines Slerp-based rotation with linear magnitude interpolation, and a standard Euclidean linear path that preserves the original vector norms.

The blending weights are derived from a nonparametric indicator of local flatness, computed solely from the normalized directions $\hat{x}_0$ and $\hat{x}_1$. Specifically, we consider the chord length $\|\hat{x}_0 - \hat{x}_1\|$ and the arc length $\theta$ between them, and define their ratio as
\[
\rho = \frac{\|\hat{x}_0 - \hat{x}_1\|}{\theta}.
\]
This quantity $\rho \in (0,1]$ serves as a measure of local flatness: when $\rho$ is close to 1, the segment between the points is nearly straight (low curvature), favoring Euclidean interpolation; when $\rho$ is significantly less than 1, the path is highly curved, favoring geodesic-like motion. We define the Riemannian blending weight as $w_{\text{riem}} = 1 - \rho$ and the Euclidean blending weight as $w_{\text{euc}} = \rho$, ensuring $w_{\text{riem}} + w_{\text{euc}} = 1$.

We now define the two constituent paths. First, the Scale-Aware Euclidean Path linearly interpolates the original, unnormalized vectors:
\[
z_t^{\text{euc}} = (1 - t) x_0 + t x_1, \quad u_t^{\text{euc}} = x_1 - x_0.
\]
Second, the Scale-Aware Riemannian Path combines the unit Slerp trajectory with a linearly interpolated magnitude. Let the time-dependent magnitude be
\[
\mathrm{mag}(t) = (1 - t) \|x_0\| + t \|x_1\|,
\]
and its time derivative be
\[
\frac{d}{dt} \mathrm{mag}(t) = \|x_1\| - \|x_0\|.
\]
The full Riemannian path is then
\[
z_t^{\text{riem}} = \mathrm{mag}(t) \cdot z_t^{\text{riem\_unit}},
\]
and its velocity, obtained via the product rule, accounts for changes in both magnitude and direction:
\[
u_t^{\text{riem}} = \big( \|x_1\| - \|x_0\| \big) \cdot z_t^{\text{riem\_unit}} + \mathrm{mag}(t) \cdot u_t^{\text{riem\_unit}}.
\]

The final blended interpolation path $z_t$ and its target velocity $u_t$ are convex combinations of these two components:
\[
z_t = w_{\text{riem}} \cdot z_t^{\text{riem}} + w_{\text{euc}} \cdot z_t^{\text{euc}}, \quad
u_t = w_{\text{riem}} \cdot u_t^{\text{riem}} + w_{\text{euc}} \cdot u_t^{\text{euc}}.
\]
This construction ensures that the learned flow adapts to local geometry while preserving the meaningful scale of ambient latent representations.

\subsection{Stable Slerp and Distance Computation}

To avoid numerical instability in Slerp when $\theta$ approaches $0$ or $\pi$ (where $\sin(\theta) \to 0$), we clamp the angle away from these singularities. Specifically, we define
\[
\theta \leftarrow \mathrm{clamp}\big( \cos^{-1}( \langle \hat{x}_0, \hat{x}_1 \rangle ),\, \epsilon,\, \pi - \epsilon \big),
\]
where $\mathrm{clamp}(a, l, u) = \min(\max(a, l), u)$ and $\epsilon = 10^{-3}$ is a small constant. In the near-parallel case where the original (unclamped) $\theta < \epsilon$, we explicitly set $\rho = 1$ (i.e., $w_{\text{riem}} = 0$) and use only the Euclidean path, as the local geometry is effectively flat at this scale. The chord distance $\|\hat{x}_0 - \hat{x}_1\|$ used in $\rho$ is always computed from the normalized vectors to maintain consistency with the definition of $\theta$.

\subsection{Training and Sampling}

The model is trained by minimizing the standard Flow Matching loss:
\[
\mathcal{L}(\Theta) = \mathbb{E}_{t \sim \mathcal{U}(0,1),\, x_0 \sim p_0,\, x_1 \sim p_1} \left[ \big\| v_\Theta(z_t, t) - u_t \big\|^2 \right],
\]
where $z_t$ and $u_t$ are constructed via the adaptive blending procedure described above. During sampling, we draw an initial noise sample $z_1 \sim p_1$ and numerically integrate the ordinary differential equation
\[
\frac{dz}{dt} = v_\Theta(z, t)
\]
backward in time from $t = 1$ to $t = 0$ using any standard ODE solver (e.g., Runge–Kutta methods), exactly as in Euclidean Flow Matching. No modifications to the sampling pipeline, solver, or architecture are required. This plug-and-play compatibility ensures that GeodesicFlow can be readily integrated into existing flow matching frameworks without altering their inference workflow.

\subsection{Algorithmic Implementation}

The complete training procedure is summarized in Algorithm~\ref{alg:training_geodesicflow}. For each training iteration, we sample a mini-batch of data points $\{x_0^{(i)}\}$, noise samples $\{x_1^{(i)}\}$, and time steps $\{t^{(i)}\}$. For each sample pair, we compute magnitudes and unit directions, estimate local flatness via $\rho$, construct both scale-aware interpolation paths, blend them using adaptive weights, and evaluate the Flow Matching loss between the model’s predicted velocity and the target velocity $u_t$. The model parameters $\Theta$ are updated using the average loss over the batch.

\begin{algorithm}[H]
\caption{Training GeodesicFlow}
\label{alg:training_geodesicflow}
\begin{algorithmic}[1]
\Require
\Statex \textit{Model:} Neural network $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$.
\Statex \textit{Data:} Distributions $p_0$ (data), $p_1$ (noise) in $\mathbb{R}^D$.
\Statex \textit{Hyperparameters:} Batch size $B$, stability constant $\epsilon = 10^{-3}$.
\For{each training step}
    \State Sample mini-batch: $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
    \For{$i = 1$ to $B$}
        \State Let $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
        \State \textbf{// Compute magnitudes and directions}
        \State $\text{mag}_{x0} \leftarrow \|x_0\|$, \quad $\text{mag}_{x1} \leftarrow \|x_1\|$
        \State $\hat{x}_0 \leftarrow x_0 / \text{mag}_{x0}$, \quad $\hat{x}_1 \leftarrow x_1 / \text{mag}_{x1}$
        
        \State \textbf{// Compute curvature-based weights from directions}
        \State $\theta \leftarrow \cos^{-1}(\langle \hat{x}_0, \hat{x}_1 \rangle)$
        \State $\theta \leftarrow \mathrm{clamp}(\theta, \epsilon, \pi - \epsilon)$
        \State $d_{\text{chord}} \leftarrow \|\hat{x}_0 - \hat{x}_1\|$
        \State $\rho \leftarrow d_{\text{chord}} / \theta$
        \State $w_{\text{riem}} \leftarrow 1 - \rho$, \quad $w_{\text{euc}} \leftarrow \rho$
        
        \State \textbf{// Compute scale-aware Riemannian components}
        \State $z_t^{\text{riem\_unit}} \leftarrow \frac{\sin((1-t)\theta)}{\sin(\theta)} \hat{x}_0 + \frac{\sin(t\theta)}{\sin(\theta)} \hat{x}_1$
        \State $u_t^{\text{riem\_unit}} \leftarrow \frac{\theta}{\sin(\theta)} \left[ \cos(t\theta) \hat{x}_1 - \cos((1-t)\theta) \hat{x}_0 \right]$
        \State $\text{mag}_t \leftarrow (1-t)\text{mag}_{x0} + t \cdot \text{mag}_{x1}$
        \State $\text{mag}_{dt} \leftarrow \text{mag}_{x1} - \text{mag}_{x0}$
        \State $z_t^{\text{riem}} \leftarrow \text{mag}_t \cdot z_t^{\text{riem\_unit}}$
        \State $u_t^{\text{riem}} \leftarrow \text{mag}_{dt} \cdot z_t^{\text{riem\_unit}} + \text{mag}_t \cdot u_t^{\text{riem\_unit}}$
        
        \State \textbf{// Compute scale-aware Euclidean components}
        \State $z_t^{\text{euc}} \leftarrow (1-t) x_0 + t x_1$
        \State $u_t^{\text{euc}} \leftarrow x_1 - x_0$
        
        \State \textbf{// Unified curvature-adaptive path and velocity}
        \State $z_t \leftarrow w_{\text{riem}} \cdot z_t^{\text{riem}} + w_{\text{euc}} \cdot z_t^{\text{euc}}$
        \State $u_t \leftarrow w_{\text{riem}} \cdot u_t^{\text{riem}} + w_{\text{euc}} \cdot u_t^{\text{euc}}$
        
        \State \textbf{// Compute loss}
        \State $\mathcal{L}^{(i)} \leftarrow \left\| v_\Theta(z_t, t) - u_t \right\|^2$
    \EndFor
    \State Update $\Theta$ using batch loss $\frac{1}{B}\sum_{i=1}^B \mathcal{L}^{(i)}$.
\EndFor
\end{algorithmic}
\end{algorithm}

% ----------------------------
% basic version
% \section{GeodesicFlow: Adaptive Ambient Flow Matching via Blended Geodesic Interpolation}

% We introduce \textbf{GeodesicFlow}, a generative modeling framework for data lying on or near Riemannian manifolds embedded in Euclidean space. Our approach learns an ambient time-dependent velocity field $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$ that governs a continuous transformation from a simple base distribution $p_1$ (e.g., Gaussian noise) to a complex data distribution $p_0$.

% Crucially, while the model operates in ambient space $\mathbb{R}^D$, its training objective is designed to respect the underlying manifold geometry—without requiring explicit Riemannian operators. This enables:
% \begin{itemize}
%     \item \textbf{Geometric fidelity}: The model learns curvature-aware motion intrinsic to the data manifold.
%     \item \textbf{Euclidean flexibility}: The model operates on standard VAE latents, which have meaningful magnitude, rather than being restricted to a hypersphere.
%     \item \textbf{Plug-and-play compatibility}: Sampling uses standard ODE solvers from Euclidean Flow Matching.
% \end{itemize}

% The core innovation of GeodesicFlow is \textbf{Adaptive Path Flow Matching}: we define a \textit{single}, differentiable interpolation path that smoothly blends geodesic-like rotational motion (via Slerp) and ambient linear motion. The blending weight is \textbf{dynamically determined by a local curvature estimate}, ensuring that the interpolation adapts to the intrinsic geometry of the data manifold.

% \subsection{Separating Magnitude and Direction}

% Let $x_0 \sim p_0$ be a data point (e.g., a VAE latent) and $x_1 \sim p_1$ be a noise point in $\mathbb{R}^D$. While these vectors are not restricted to a unit hypersphere, their \textit{directions} define a great circle on which we can measure local curvature. Spherical Linear Interpolation (Slerp) provides a geometrically faithful way to interpolate between these directions.

% Our approach separates the interpolation of vector \textbf{magnitude} from the interpolation of vector \textbf{direction}. We first normalize the inputs to get their directions, $\hat{x}_0 = x_0 / \|x_0\|$ and $\hat{x}_1 = x_1 / \|x_1\|$. The unit Slerp path and its velocity are:
% \begin{equation}
% z_t^{\text{riem\_unit}} = \mathrm{Slerp}(\hat{x}_0, \hat{x}_1; t) := \frac{\sin((1-t)\theta)}{\sin(\theta)} \hat{x}_0 + \frac{\sin(t\theta)}{\sin(\theta)} \hat{x}_1
% \end{equation}
% \begin{equation}
% u_t^{\text{riem\_unit}} = \frac{d}{dt} z_t^{\text{riem\_unit}} = \frac{\theta}{\sin(\theta)} \left[ \cos(t\theta) \hat{x}_1 - \cos((1-t)\theta) \hat{x}_0 \right]
% \end{equation}
% where $\theta = \cos^{-1}(\langle \hat{x}_0, \hat{x}_1 \rangle) \in [0, \pi]$ is the angular distance between the vector directions. These components capture the rotational part of the transformation.

% \subsection{Curvature-Aware Adaptive Blending}

% To create a unified path, we blend a scale-aware Riemannian path and a standard Euclidean path. The blending weights are determined by the local curvature between the \textit{directions} of $x_0$ and $x_1$.

% The ratio of the chord length to the arc length between the normalized vectors,
% \begin{equation}
% \rho = \frac{\|\hat{x}_0 - \hat{x}_1\|}{\theta}
% \end{equation}
% serves as a \textbf{nonparametric local flatness indicator}:
% \begin{itemize}
%     \item $\rho \approx 1$: The path is locally straight $\rightarrow$ trust the Euclidean interpolant.
%     \item $\rho \ll 1$: The path has high curvature $\rightarrow$ trust the Riemannian interpolant.
% \end{itemize}

% We define the \textbf{Riemannian weight} as $w_{\text{riem}} = 1 - \rho$ and the Euclidean weight as $w_{\text{euc}} = \rho$. These weights, computed once per pair $(x_0, x_1)$, guide the blending of two scale-aware interpolation paths:

% \begin{enumerate}
%     \item \textbf{Scale-Aware Euclidean Path}: This is the standard linear interpolation between the \textit{original}, unnormalized vectors, preserving their magnitudes.
%     \begin{equation}
%     z_t^{\text{euc}} = (1-t)x_0 + t x_1 \quad \text{with velocity} \quad u_t^{\text{euc}} = x_1 - x_0
%     \end{equation}

%     \item \textbf{Scale-Aware Riemannian Path}: This path combines the rotational motion from Slerp with a linear interpolation of the vector magnitudes. We define a time-dependent magnitude $\text{mag}(t) = (1-t)\|x_0\| + t\|x_1\|$. The path is:
%     \begin{equation}
%         z_t^{\text{riem}} = \text{mag}(t) \cdot z_t^{\text{riem\_unit}}
%     \end{equation}
%     Its velocity, derived via the product rule, accounts for changes in both magnitude and direction:
%     \begin{equation}
%         u_t^{\text{riem}} = \frac{d}{dt}\text{mag}(t) \cdot z_t^{\text{riem\_unit}} + \text{mag}(t) \cdot u_t^{\text{riem\_unit}}
%     \end{equation}
% \end{enumerate}

% The final blended path and target velocity are convex combinations of these two scale-aware components:
% \begin{equation}
% z_t = w_{\text{riem}} \cdot z_t^{\text{riem}} + w_{\text{euc}} \cdot z_t^{\text{euc}}
% \end{equation}
% \begin{equation}
% u_t = w_{\text{riem}} \cdot u_t^{\text{riem}} + w_{\text{euc}} \cdot u_t^{\text{euc}}
% \end{equation}
% This formulation ensures that the model learns a flow that respects both the intrinsic geometry of the data directions and the extrinsic magnitudes of the latent space.

% \subsection{Stable Slerp and Distance Computation}

% To ensure numerical stability, we clamp the angle $\theta$ away from singularities:
% \begin{equation}
% \theta \leftarrow \mathrm{clamp}\big(\cos^{-1}(\langle \hat{x}_0, \hat{x}_1 \rangle),\, \epsilon,\, \pi - \epsilon\big),
% \end{equation}
% with a small $\epsilon = 10^{-3}$. If $\theta < \epsilon$, we set $\rho = 1$ (i.e., $w_{\text{riem}} = 0$) and use the Euclidean path exclusively, as the manifold is effectively flat at this scale. The chord distance for computing $\rho$ is $\|\hat{x}_0 - \hat{x}_1\|$, using the normalized inputs for consistency with $\theta$.

% \subsection{Training and Sampling}
% The model is trained by minimizing the standard Flow Matching loss $\mathcal{L}(\Theta) = \mathbb{E}_{t, x_0, x_1} \left[ \left\| v_\Theta(z_t, t) - u_t \right\|^2 \right]$, where $z_t$ and $u_t$ are defined by the adaptive blending procedure above. Sampling is identical to standard Euclidean Flow Matching, where one integrates the learned ODE $\frac{dz}{dt} = v_\Theta(z,t)$ from $t=1$ to $t=0$ starting from a noise sample $z_1 \sim p_1$.

% \subsection{Algorithmic Implementation}

% \begin{algorithm}[H]
% \caption{Training GeodesicFlow}
% \label{alg:training_geodesicflow_revised}
% \begin{algorithmic}[1]
% \Require
% \Statex \textit{Model:} Neural network $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$.
% \Statex \textit{Data:} Distributions $p_0$ (data), $p_1$ (noise) in $\mathbb{R}^D$.
% \Statex \textit{Hyperparameters:} Batch size $B$, stability $\epsilon = 10^{-3}$.
% \For{each training step}
%     \State Sample mini-batch: $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
%     \For{$i = 1$ to $B$}
%         \State Let $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
%         \State \textbf{// Compute magnitudes and directions}
%         \State $\text{mag}_{x0} \leftarrow \|x_0\|$, \quad $\text{mag}_{x1} \leftarrow \|x_1\|$
%         \State $\hat{x}_0 \leftarrow x_0 / \text{mag}_{x0}$, \quad $\hat{x}_1 \leftarrow x_1 / \text{mag}_{x1}$
        
%         \State \textbf{// Compute curvature-based weights from directions}
%         \State $\theta \leftarrow \cos^{-1}(\langle \hat{x}_0, \hat{x}_1 \rangle)$
%         \State $\theta \leftarrow \mathrm{clamp}(\theta, \epsilon, \pi - \epsilon)$
%         \State $d_{\text{chord}} \leftarrow \|\hat{x}_0 - \hat{x}_1\|$
%         \State $\rho \leftarrow d_{\text{chord}} / \theta$
%         \State $w_{\text{riem}} \leftarrow 1 - \rho$, \quad $w_{\text{euc}} \leftarrow \rho$
        
%         \State \textbf{// Compute scale-aware Riemannian components}
%         \State $z_t^{\text{riem\_unit}} \leftarrow \frac{\sin((1-t)\theta)}{\sin(\theta)} \hat{x}_0 + \frac{\sin(t\theta)}{\sin(\theta)} \hat{x}_1$
%         \State $u_t^{\text{riem\_unit}} \leftarrow \frac{\theta}{\sin(\theta)} \left[ \cos(t\theta) \hat{x}_1 - \cos((1-t)\theta) \hat{x}_0 \right]$
%         \State $\text{mag}_t \leftarrow (1-t)\text{mag}_{x0} + t \cdot \text{mag}_{x1}$
%         \State $\text{mag}_{dt} \leftarrow \text{mag}_{x1} - \text{mag}_{x0}$
%         \State $z_t^{\text{riem}} \leftarrow \text{mag}_t \cdot z_t^{\text{riem\_unit}}$
%         \State $u_t^{\text{riem}} \leftarrow \text{mag}_{dt} \cdot z_t^{\text{riem\_unit}} + \text{mag}_t \cdot u_t^{\text{riem\_unit}}$
        
%         \State \textbf{// Compute scale-aware Euclidean components}
%         \State $z_t^{\text{euc}} \leftarrow (1-t) x_0 + t x_1$
%         \State $u_t^{\text{euc}} \leftarrow x_1 - x_0$
        
%         \State \textbf{// Unified curvature-adaptive path and velocity}
%         \State $z_t \leftarrow w_{\text{riem}} \cdot z_t^{\text{riem}} + w_{\text{euc}} \cdot z_t^{\text{euc}}$
%         \State $u_t \leftarrow w_{\text{riem}} \cdot u_t^{\text{riem}} + w_{\text{euc}} \cdot u_t^{\text{euc}}$
        
%         \State \textbf{// Compute loss}
%         \State $\mathcal{L}^{(i)} \leftarrow \left\| v_\Theta(z_t, t) - u_t \right\|^2$
%     \EndFor
%     \State Update $\Theta$ using batch loss $\frac{1}{B}\sum_i \mathcal{L}^{(i)}$.
% \EndFor
% \end{algorithmic}
% \end{algorithm}

% ----------------------------
% spherical manifold only
\section{GeodesicFlow: Ambient Flow Matching via Spherical Manifold Interpolation}

We introduce \textbf{GeodesicFlow}, a generative modeling framework for data lying on or near Riemannian manifolds embedded in Euclidean space. Our approach learns an ambient time-dependent velocity field $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$ that governs a continuous transformation from a simple base distribution $p_1$ (e.g., Gaussian noise) to a complex data distribution $p_0$.

While the model operates in ambient space $\mathbb{R}^D$, its training objective is constructed using interpolation on the spherical manifold of directions, ensuring that the learned flow respects the intrinsic geometry of the data without requiring explicit Riemannian operators. This enables:
\begin{itemize}
    \item \textbf{Geometric fidelity}: The model follows geodesic-like paths on the sphere of directions, capturing curvature-aware motion.
    \item \textbf{Magnitude preservation}: Vector norms are interpolated linearly, accommodating meaningful scale in VAE latents.
    \item \textbf{Euclidean compatibility}: Sampling uses standard ODE solvers from Euclidean Flow Matching.
\end{itemize}


The core of GeodesicFlow is \textbf{Spherical Path Flow Matching}: we define a single, differentiable interpolation path that evolves on the spherical manifold for directions while linearly interpolating magnitudes. This yields a geometrically principled trajectory in ambient space.

\subsection{Separating Magnitude and Direction}

Let $x_0 \sim p_0$ be a data point (e.g., a VAE latent) and $x_1 \sim p_1$ be a noise point in $\mathbb{R}^D$. Although these vectors are not constrained to the unit hypersphere, their \textit{directions} naturally lie on $\mathbb{S}^{D-1}$, where spherical interpolation is well-defined.

We decompose each vector into magnitude and direction:
\[
\text{mag}_0 = \|x_0\|, \quad \hat{x}_0 = \frac{x_0}{\|x_0\|}, \qquad
\text{mag}_1 = \|x_1\|, \quad \hat{x}_1 = \frac{x_1}{\|x_1\|}.
\]

We interpolate the directions using Spherical Linear Interpolation (Slerp), which follows the shortest geodesic on the unit sphere:
\begin{equation}
z_t^{\text{unit}} = \mathrm{Slerp}(\hat{x}_0, \hat{x}_1; t) := \frac{\sin((1-t)\theta)}{\sin(\theta)} \hat{x}_0 + \frac{\sin(t\theta)}{\sin(\theta)} \hat{x}_1,
\end{equation}
with angular distance $\theta = \cos^{-1}(\langle \hat{x}_0, \hat{x}_1 \rangle) \in [0, \pi]$. The corresponding unit-sphere velocity is:
\begin{equation}
u_t^{\text{unit}} = \frac{d}{dt} z_t^{\text{unit}} = \frac{\theta}{\sin(\theta)} \left[ \cos(t\theta) \hat{x}_1 - \cos((1-t)\theta) \hat{x}_0 \right].
\end{equation}

\subsection{Scale-Aware Spherical Interpolation}

To account for the full ambient-space trajectory, we combine the spherical direction path with a linear interpolation of magnitudes:
\begin{equation}
\text{mag}(t) = (1 - t)\, \text{mag}_0 + t\, \text{mag}_1.
\end{equation}

The final interpolation path and its velocity are defined as:
\begin{equation}
z_t = \text{mag}(t) \cdot z_t^{\text{unit}},
\end{equation}
\begin{equation}
u_t = \frac{d}{dt}\text{mag}(t) \cdot z_t^{\text{unit}} + \text{mag}(t) \cdot u_t^{\text{unit}} = (\text{mag}_1 - \text{mag}_0) \cdot z_t^{\text{unit}} + \text{mag}(t) \cdot u_t^{\text{unit}}.
\end{equation}

This formulation ensures that the model evolves along a path that is geodesic in direction (on the sphere) and linear in scale—fully respecting the spherical geometry of normalized latents while preserving magnitude information.

\subsection{Stable Slerp and Edge Cases}

To ensure numerical stability near antipodal or identical directions, we clamp the angle $\theta$:
\begin{equation}
\theta \leftarrow \mathrm{clamp}\big(\cos^{-1}(\langle \hat{x}_0, \hat{x}_1 \rangle),\, \epsilon,\, \pi - \epsilon\big),
\end{equation}
with $\epsilon = 10^{-3}$. When $\theta < \epsilon$, the directions are nearly identical, and Slerp reduces to linear interpolation on the sphere; the above formula remains well-defined due to the clamping and the smooth limit $\lim_{\theta \to 0} \mathrm{Slerp}(\hat{x}_0, \hat{x}_1; t) = (1-t)\hat{x}_0 + t\hat{x}_1$.

\subsection{Training and Sampling}

The model is trained by minimizing the standard Flow Matching loss:
\begin{equation}
\mathcal{L}(\Theta) = \mathbb{E}_{t, x_0, x_1} \left[ \left\| v_\Theta(z_t, t) - u_t \right\|^2 \right],
\end{equation}
where $z_t$ and $u_t$ are computed exclusively via the scale-aware spherical interpolation described above. Sampling proceeds identically to standard Euclidean Flow Matching: integrate the learned ODE $\frac{dz}{dt} = v_\Theta(z,t)$ backward from $t=1$ to $t=0$, starting from $z_1 \sim p_1$.

\subsection{Algorithmic Implementation}

\begin{algorithm}[H]
\caption{Training GeodesicFlow (Pure Spherical Interpolation)}
\label{alg:training_geodesicflow_spherical}
\begin{algorithmic}[1]
\Require
\Statex \textit{Model:} Neural network $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$.
\Statex \textit{Data:} Distributions $p_0$ (data), $p_1$ (noise) in $\mathbb{R}^D$.
\Statex \textit{Hyperparameters:} Batch size $B$, stability $\epsilon = 10^{-3}$.
\For{each training step}
    \State Sample mini-batch: $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
    \For{$i = 1$ to $B$}
        \State Let $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
        \State \textbf{// Compute magnitudes and directions}
        \State $\text{mag}_0 \leftarrow \|x_0\|$, \quad $\text{mag}_1 \leftarrow \|x_1\|$
        \State $\hat{x}_0 \leftarrow x_0 / \max(\text{mag}_0, \epsilon)$, \quad $\hat{x}_1 \leftarrow x_1 / \max(\text{mag}_1, \epsilon)$
        
        \State \textbf{// Compute spherical interpolation parameters}
        \State $\theta \leftarrow \cos^{-1}(\langle \hat{x}_0, \hat{x}_1 \rangle)$
        \State $\theta \leftarrow \mathrm{clamp}(\theta, \epsilon, \pi - \epsilon)$
        
        \State \textbf{// Unit-sphere Slerp path and velocity}
        \State $z_t^{\text{unit}} \leftarrow \frac{\sin((1-t)\theta)}{\sin(\theta)} \hat{x}_0 + \frac{\sin(t\theta)}{\sin(\theta)} \hat{x}_1$
        \State $u_t^{\text{unit}} \leftarrow \frac{\theta}{\sin(\theta)} \left[ \cos(t\theta) \hat{x}_1 - \cos((1-t)\theta) \hat{x}_0 \right]$
        
        \State \textbf{// Scale-aware spherical path}
        \State $\text{mag}_t \leftarrow (1-t)\text{mag}_0 + t \cdot \text{mag}_1$
        \State $\text{mag}_{dt} \leftarrow \text{mag}_1 - \text{mag}_0$
        \State $z_t \leftarrow \text{mag}_t \cdot z_t^{\text{unit}}$
        \State $u_t \leftarrow \text{mag}_{dt} \cdot z_t^{\text{unit}} + \text{mag}_t \cdot u_t^{\text{unit}}$
        
        \State \textbf{// Compute loss}
        \State $\mathcal{L}^{(i)} \leftarrow \left\| v_\Theta(z_t, t) - u_t \right\|^2$
    \EndFor
    \State Update $\Theta$ using batch loss $\frac{1}{B}\sum_i \mathcal{L}^{(i)}$.
\EndFor
\end{algorithmic}
\end{algorithm}

% ---------------------------
% Hyperbolic space only
% \section{GeodesicFlow: Ambient Flow Matching via Hyperbolic Geodesic Interpolation}

% We introduce \textbf{GeodesicFlow}, a generative modeling framework for data that exhibits hierarchical or tree-like structure, naturally embedded in hyperbolic space. Our approach learns an ambient time-dependent velocity field $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$ that governs a continuous transformation from a simple base distribution $p_1$ (e.g., Gaussian noise) to a complex data distribution $p_0$.

% Although the model operates in ambient Euclidean space $\mathbb{R}^D$, its training objective is constructed using **geodesics of the Poincaré ball model** of hyperbolic space. This ensures that the learned flow respects the intrinsic negative curvature of the data manifold—without requiring explicit manifold-constrained sampling. The method enables:
% \begin{itemize}
%     \item \textbf{Hyperbolic fidelity}: The model follows true geodesics in hyperbolic space, capturing exponential volume growth and hierarchical relationships.
%     \item \textbf{Ambient compatibility}: Training and sampling use standard Euclidean networks and ODE solvers.
%     \item \textbf{Curvature awareness}: The interpolation accounts for the non-linear metric of hyperbolic space via the Poincaré ball formalism.
% \end{itemize}


% The core of GeodesicFlow is \textbf{Hyperbolic Geodesic Flow Matching}: we define a single, differentiable interpolation path that follows the geodesic (gyroline) between two points in the Poincaré ball of curvature $c > 0$. This path and its time derivative serve as regression targets for the ambient velocity field.

% \subsection{Poincaré Ball Preliminaries}

% We model the latent space as the Poincaré ball $\mathbb{D}_c^D = \{ x \in \mathbb{R}^D : \|x\| < 1/\sqrt{c} \}$ equipped with the Riemannian metric
% \[
% g_x^c = \left( \frac{2}{1 - c\|x\|^2} \right)^2 I.
% \]
% The distance between two points $x, y \in \mathbb{D}_c^D$ is
% \begin{equation}
% d_c(x, y) = \frac{2}{\sqrt{c}} \tanh^{-1}\left( \sqrt{c} \, \| \ominus_c x \oplus_c y \| \right),
% \end{equation}
% where $\oplus_c$ and $\ominus_c$ denote Möbius addition and negation:
% \begin{align}
% x \oplus_c y &= \frac{(1 + 2c\langle x, y \rangle + c\|y\|^2)x + (1 - c\|x\|^2)y}{1 + 2c\langle x, y \rangle + c^2\|x\|^2\|y\|^2}, \\
% \ominus_c x &= -x.
% \end{align}

% The geodesic (gyroline) between $x_0$ and $x_1$ in $\mathbb{D}_c^D$ is given by the **gyrolinear interpolation**:
% \begin{equation}
% z_t = x_0 \oplus_c \left( \tanh\left( t \cdot \xi \right) \oslash_c \xi \cdot (\ominus_c x_0 \oplus_c x_1) \right),
% \end{equation}
% where $\xi = \tanh^{-1}(\sqrt{c} \, \|\ominus_c x_0 \oplus_c x_1\|)$, and scalar multiplication $\oslash_c$ is defined as
% \[
% r \otimes_c v = \frac{\tanh(r \tanh^{-1}(\sqrt{c}\|v\|))}{\sqrt{c}\|v\|} v, \quad v \neq 0.
% \]

% However, for computational efficiency and differentiability, we use the equivalent **exponential-logarithmic map formulation**.

% \subsection{Hyperbolic Geodesic Path and Velocity}

% Let $x_0 \sim p_0$ and $x_1 \sim p_1$ be data and noise samples, assumed to lie within the open ball $\mathbb{D}_c^D$ (we enforce this via clipping or normalization during preprocessing). The hyperbolic geodesic from $x_0$ to $x_1$ is:
% \begin{equation}
% z_t = \exp_{x_0}^c \left( t \cdot \log_{x_0}^c (x_1) \right),
% \end{equation}
% where $\exp_x^c(\cdot)$ and $\log_x^c(\cdot)$ are the exponential and logarithmic maps of the Poincaré ball:
% \begin{align}
% \log_x^c(y) &= \frac{2}{\sqrt{c} \lambda_x^c} \tanh^{-1}\left( \sqrt{c} \, \| \ominus_c x \oplus_c y \| \right) \frac{\ominus_c x \oplus_c y}{\| \ominus_c x \oplus_c y \|}, \\
% \exp_x^c(v) &= x \oplus_c \left( \tanh\left( \frac{\sqrt{c}}{2} \lambda_x^c \|v\| \right) \frac{v}{\sqrt{c} \|v\|} \right),
% \end{align}
% with conformal factor $\lambda_x^c = \frac{2}{1 - c\|x\|^2}$.

% The time derivative of the geodesic gives the target velocity:
% \begin{equation}
% u_t = \frac{d}{dt} z_t = \left. \frac{d}{ds} \exp_{z_t}^c(s \cdot w_t) \right|_{s=0} = w_t,
% \end{equation}
% where $w_t = \frac{d}{dt} \exp_{x_0}^c(t \cdot \log_{x_0}^c(x_1))$. Using properties of geodesics in constant curvature spaces, this simplifies to parallel transport of the initial velocity:
% \begin{equation}
% u_t = \mathcal{P}_{x_0 \to z_t}^c \left( \log_{x_0}^c(x_1) \right),
% \end{equation}
% where $\mathcal{P}$ denotes parallel transport along the geodesic. In the Poincaré ball, parallel transport of a vector $v$ from $x$ to $y$ is:
% \begin{equation}
% \mathcal{P}_{x \to y}^c(v) = \frac{\lambda_x^c}{\lambda_y^c} v.
% \end{equation}

% Thus, letting $v_0 = \log_{x_0}^c(x_1)$, we compute:
% \begin{align}
% z_t &= \exp_{x_0}^c(t v_0), \\
% u_t &= \frac{\lambda_{x_0}^c}{\lambda_{z_t}^c} v_0.
% \end{align}

% This $(z_t, u_t)$ pair defines the hyperbolic geodesic trajectory and its instantaneous velocity in ambient coordinates.

% \subsection{Stable Computation and Boundary Handling}

% To ensure numerical stability:
% \begin{itemize}
%     \item We clamp inputs to satisfy $\|x\| \leq R < 1/\sqrt{c}$ (e.g., $R = 0.99 / \sqrt{c}$).
%     \item When $\| \ominus_c x_0 \oplus_c x_1 \|$ is near zero, we use the Euclidean limit: $z_t \approx (1-t)x_0 + t x_1$, $u_t \approx x_1 - x_0$.
%     \item The conformal factor $\lambda_x^c$ is always positive and smooth within the ball.
% \end{itemize}


% \subsection{Training and Sampling}

% The model is trained by minimizing the Flow Matching loss using the hyperbolic geodesic targets:
% \begin{equation}
% \mathcal{L}(\Theta) = \mathbb{E}_{t, x_0, x_1} \left[ \left\| v_\Theta(z_t, t) - u_t \right\|^2 \right],
% \end{equation}
% where $z_t$ and $u_t$ are computed via the Poincaré geodesic as above. Sampling proceeds as in standard Flow Matching: draw $z_1 \sim p_1$ (ensuring $z_1 \in \mathbb{D}_c^D$), then solve the ODE $\frac{dz}{dt} = v_\Theta(z, t)$ backward from $t=1$ to $t=0$. The resulting $z_0$ approximates a sample from $p_0$, implicitly respecting hyperbolic geometry through the trained velocity field.

% \subsection{Algorithmic Implementation}

% \begin{algorithm}[H]
% \caption{Training GeodesicFlow (Hyperbolic Geodesic Interpolation)}
% \label{alg:training_geodesicflow_hyperbolic}
% \begin{algorithmic}[1]
% \Require
% \Statex \textit{Model:} Neural network $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$.
% \Statex \textit{Data:} Distributions $p_0$, $p_1$ supported in $\mathbb{D}_c^D$.
% \Statex \textit{Hyperparameters:} Curvature $c > 0$, radius margin $\delta = 0.01$, batch size $B$.
% \For{each training step}
%     \State Sample mini-batch: $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
%     \For{$i = 1$ to $B$}
%         \State Let $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
%         \State \textbf{// Ensure points are inside Poincaré ball}
%         \State $R \leftarrow (1 - \delta)/\sqrt{c}$
%         \State $x_0 \leftarrow \mathrm{clip\_norm}(x_0, R)$, \quad $x_1 \leftarrow \mathrm{clip\_norm}(x_1, R)$
        
%         \State \textbf{// Compute Möbius difference}
%         \State $v \leftarrow \ominus_c x_0 \oplus_c x_1$
%         \State $\|v\| \leftarrow \max(\|v\|, 10^{-8})$
        
%         \State \textbf{// Logarithmic map at $x_0$}
%         \State $\lambda_{x_0} \leftarrow 2 / (1 - c \|x_0\|^2)$
%         \State $\xi \leftarrow \tanh^{-1}(\sqrt{c} \|v\|)$
%         \State $v_0 \leftarrow \frac{2 \xi}{\sqrt{c} \lambda_{x_0} \|v\|} \cdot v$  \Comment{$v_0 = \log_{x_0}^c(x_1)$}
        
%         \State \textbf{// Exponential map for $z_t$}
%         \State $w \leftarrow t \cdot v_0$
%         \State $\|w\| \leftarrow \max(\|w\|, 10^{-8})$
%         \State $\alpha \leftarrow \tanh\left( \frac{\sqrt{c}}{2} \lambda_{x_0} \|w\| \right) / (\sqrt{c} \|w\|)$
%         \State $z_t \leftarrow x_0 \oplus_c (\alpha \cdot w)$
        
%         \State \textbf{// Parallel transport for velocity $u_t$}
%         \State $\lambda_{z_t} \leftarrow 2 / (1 - c \|z_t\|^2)$
%         \State $u_t \leftarrow (\lambda_{x_0} / \lambda_{z_t}) \cdot v_0$
        
%         \State \textbf{// Compute loss}
%         \State $\mathcal{L}^{(i)} \leftarrow \left\| v_\Theta(z_t, t) - u_t \right\|^2$
%     \EndFor
%     \State Update $\Theta$ using batch loss $\frac{1}{B}\sum_i \mathcal{L}^{(i)}$.
% \EndFor
% \end{algorithmic}
% \end{algorithm}

% ---------------------
% revised method, wait for testing
\section{GeodesicFlow: Adaptive Ambient Flow Matching via Blended Geodesic Interpolation}

We introduce \textbf{GeodesicFlow}, a generative modeling framework designed for data that lies on or near a Riemannian manifold embedded in Euclidean space $\mathbb{R}^D$. The method learns an ambient, time-dependent velocity field $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$, parameterized by neural network weights $\Theta$, which governs a continuous transformation from a simple base distribution $p_1$ to a complex data distribution $p_0$.

The core innovation of GeodesicFlow is to define a conditional interpolation trajectory by \textbf{adaptively blending two geometrically motivated paths}: a standard linear path in Euclidean space, and a geodesic path defined by Spherical Linear Interpolation (Slerp) applied directly to the ambient vectors. The blending weight is dynamically determined from a local estimate of manifold curvature computed from the directional components of the endpoint vectors. This design allows the model to smoothly transition from straight-line trajectories in flat regions of the space to curvature-aware geodesic arcs where the data manifold requires it, without requiring explicit knowledge of Riemannian operators. This preserves geometric structure while retaining full compatibility with standard Euclidean flow architectures and solvers.

\subsection{Geometric Curvature Estimation}

To adapt the interpolation path to the local data geometry, we require a metric that can be computed directly from an endpoint pair $(x_0, x_1)$. The intrinsic curvature of the manifold is primarily manifested in the directional component of the data vectors. Therefore, we base our estimation on the directions of the vectors, which we isolate by decomposing each vector into its magnitude and direction:
$$
\|x_0\| = \sqrt{x_0^\top x_0}, \quad \|x_1\| = \sqrt{x_1^\top x_1}, \quad \hat{x}_0 = \frac{x_0}{\|x_0\|}, \quad \hat{x}_1 = \frac{x_1}{\|x_1\|},
$$
where $\hat{x}_0, \hat{x}_1 \in \mathbb{S}^{D-1}$ are unit vectors. The angular distance between these directions is the length of the geodesic arc on the unit sphere:
$$
\theta = \cos^{-1}\big( \langle \hat{x}_0, \hat{x}_1 \rangle \big) \in [0, \pi]
$$
This arc length can be compared to the length of the straight-line chord between the directions, $\|\hat{x}_0 - \hat{x}_1\|$. The ratio of these lengths provides a robust, scale-invariant measure of local flatness that will determine our blending strategy.

\subsection{Adaptive Blending of Euclidean and Geodesic Paths}

Having a measure of local curvature, we construct the interpolation path as a convex combination of two fundamental trajectories: a \textbf{Euclidean path} (a straight line) and a \textbf{Geodesic path} (a circular arc). This blending allows the model to default to the simplest possible trajectory in flat regions while seamlessly adopting a curved path to respect the manifold's geometry when necessary.

The \textbf{Euclidean Path} is the standard linear interpolation between the endpoints:
$$
z_t^{\text{euc}} = (1 - t) x_0 + t x_1
$$
Its corresponding velocity is constant:
$$
u_t^{\text{euc}} = x_1 - x_0
$$
The \textbf{Geodesic Path} is constructed using Spherical Linear Interpolation (Slerp) applied directly to the ambient vectors $x_0$ and $x_1$. This generates the shortest possible path along a circular arc connecting the two points. Using the angle $\theta$ computed from the unit vectors, the Slerp path is defined as:
$$
z_t^{\text{geo}} = \mathrm{Slerp}(x_0, x_1; t) := \frac{\sin\big((1 - t)\theta\big)}{\sin(\theta)} \, x_0 + \frac{\sin\big(t\theta\big)}{\sin(\theta)} \, x_1
$$
This formulation provides a unified interpolation of both direction and magnitude, tracing a smooth arc in the 2D plane spanned by $x_0$ and $x_1$. Its time derivative—the geodesic velocity—is given by:
$$
u_t^{\text{geo}} = \frac{d}{dt} z_t^{\text{geo}} = \frac{\theta}{\sin(\theta)} \Big[ \cos(t\theta) \, x_1 - \cos\big((1 - t)\theta\big) \, x_0 \Big]
$$
To blend these paths, we define a local flatness ratio $\rho = \frac{\|\hat{x}_0 - \hat{x}_1\|}{\theta}$. We then define the geodesic blending weight as $w_{\text{geo}} = 1 - \rho$ and the Euclidean blending weight as $w_{\text{euc}} = \rho$. When the path is straight ($\theta \to 0, \rho \to 1$), $w_{\text{euc}} \to 1$ and we recover the linear path. When the path is highly curved ($\theta \gg 0, \rho \ll 1$), $w_{\text{geo}} \to 1$ and we follow the geodesic arc.

The final blended interpolation path $z_t$ and its target velocity $u_t$ are:
$$
z_t = w_{\text{geo}} \cdot z_t^{\text{geo}} + w_{\text{euc}} \cdot z_t^{\text{euc}}
$$
$$
u_t = w_{\text{geo}} \cdot u_t^{\text{geo}} + w_{\text{euc}} \cdot u_t^{\text{euc}}
$$
This formulation is simpler and more geometrically principled. By blending two well-defined paths in the ambient space, we create a more stable and effective target for the flow matching objective.

\subsection{Stable Slerp and Distance Computation}
\subsection{Training and Sampling}

\subsection{Algorithmic Implementation}

The simplified formulation leads to a cleaner algorithm.

\begin{algorithm}[H]
\caption{Training GeodesicFlow}
\label{alg:training_geodesicflow_revised}
\begin{algorithmic}[1]
\Require
\Statex \textit{Model:} Neural network $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$.
\Statex \textit{Data:} Distributions $p_0$ (data), $p_1$ (noise) in $\mathbb{R}^D$.
\Statex \textit{Hyperparameters:} Batch size $B$, stability constant $\epsilon = 10^{-3}$.
\For{each training step}
    \State Sample mini-batch: $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
    \For{$i = 1$ to $B$}
        \State Let $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
        \State \textbf{// Compute directions for curvature estimation}
        \State $\hat{x}_0 \leftarrow x_0 / \|x_0\|$, \quad $\hat{x}_1 \leftarrow x_1 / \|x_1\|$
        
        \State \textbf{// Compute curvature-based weights}
        \State $\theta_{\text{raw}} \leftarrow \cos^{-1}(\langle \hat{x}_0, \hat{x}_1 \rangle)$
        \State $\theta \leftarrow \mathrm{clamp}(\theta_{\text{raw}}, \epsilon, \pi - \epsilon)$
        \State If $\theta_{\text{raw}} < \epsilon$: $\rho \leftarrow 1$ else: $\rho \leftarrow \|\hat{x}_0 - \hat{x}_1\| / \theta$
        \State $w_{\text{geo}} \leftarrow 1 - \rho$, \quad $w_{\text{euc}} \leftarrow \rho$
        
        \State \textbf{// Compute Geodesic components (Full Slerp on ambient vectors)}
        \State $z_t^{\text{geo}} \leftarrow \frac{\sin((1-t)\theta)}{\sin(\theta)} x_0 + \frac{\sin(t\theta)}{\sin(\theta)} x_1$
        \State $u_t^{\text{geo}} \leftarrow \frac{\theta}{\sin(\theta)} \left[ \cos(t\theta) x_1 - \cos((1-t)\theta) x_0 \right]$
        
        \State \textbf{// Compute Euclidean components}
        \State $z_t^{\text{euc}} \leftarrow (1-t) x_0 + t x_1$
        \State $u_t^{\text{euc}} \leftarrow x_1 - x_0$
        
        \State \textbf{// Unified curvature-adaptive path and velocity}
        \State $z_t \leftarrow w_{\text{geo}} \cdot z_t^{\text{geo}} + w_{\text{euc}} \cdot z_t^{\text{euc}}$
        \State $u_t \leftarrow w_{\text{geo}} \cdot u_t^{\text{geo}} + w_{\text{euc}} \cdot u_t^{\text{euc}}$
        
        \State \textbf{// Compute loss}
        \State $\mathcal{L}^{(i)} \leftarrow \left\| v_\Theta(z_t, t) - u_t \right\|^2$
    \EndFor
    \State Update $\Theta$ using batch loss $\frac{1}{B}\sum_{i=1}^B \mathcal{L}^{(i)}$.
\EndFor
\end{algorithmic}
\end{algorithm}

% ------------------------
% improved version, wait for testing
\section{GeodesicFlow: Adaptive Ambient Flow Matching via Blended Geodesic Interpolation}

We introduce \textbf{GeodesicFlow}, a generative modeling framework designed for data that lies on or near a Riemannian manifold embedded in Euclidean space $\mathbb{R}^D$. The method learns an ambient, time-dependent velocity field $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$, parameterized by neural network weights $\Theta$, which governs a continuous transformation from a simple base distribution $p_1$—such as an isotropic Gaussian—to a complex data distribution $p_0$. Although the model operates entirely in the ambient Euclidean space $\mathbb{R}^D$, its training objective is constructed to respect the intrinsic geometry of the underlying data manifold without requiring explicit knowledge of Riemannian operators (e.g., the metric tensor, exponential map, or logarithmic map). This design preserves geometric structure while retaining compatibility with standard Euclidean flow architectures and solvers.

The core innovation of GeodesicFlow is \textbf{Adaptive Path Flow Matching}, which defines a single, differentiable interpolation trajectory between a data point and a noise sample by blending two geometrically motivated paths: one based on spherical linear interpolation (Slerp), which captures curvature-aware rotational motion on the unit sphere, and another based on standard linear interpolation in Euclidean space. The blending weight is not fixed but is instead dynamically determined from a smooth, differentiable estimate of local directional curvature computed directly from the input pair. While the model operates in ambient space $\mathbb{R}^D$, its training objective leverages interpolation on the spherical manifold of directions, ensuring that the learned flow respects the intrinsic geometry of the data without requiring explicit Riemannian operators. This design achieves geometric fidelity by guiding the model along geodesic-like paths on the sphere of directions, while preserving meaningful scale through linear interpolation of vector magnitudes—a property especially important for latent representations such as those from variational autoencoders, where norm carries semantic information. Moreover, because the velocity field remains defined in Euclidean space and the sampling procedure is unchanged, GeodesicFlow maintains full compatibility with standard ODE solvers used in conventional Euclidean Flow Matching.

\subsection{Separating Magnitude and Direction}

The direction of a latent vector often encodes semantic or structural information about the data, while its magnitude reflects uncertainty, reconstruction quality, or scale. Moreover, the intrinsic geometry of the data manifold is primarily manifested in the directional component: for instance, clusters or continuous transformations in the data tend to correspond to paths on or near a sphere in latent space, even when magnitudes vary significantly. In contrast, standard Euclidean interpolation conflates changes in direction with changes in scale, potentially distorting the underlying manifold structure. To respect this geometric structure while preserving meaningful scale information, we explicitly decouple magnitude and direction.

Let $x_0 \in \mathbb{R}^D$ be a sample from the data distribution $p_0$ (e.g., a latent vector from a variational autoencoder), and let $x_1 \in \mathbb{R}^D$ be a sample from the base noise distribution $p_1$. To ensure numerical stability, we add a small constant $\varepsilon_{\text{norm}} = 10^{-8}$ to the norm before normalization. We decompose each vector into its magnitude and direction:
\[
\|x_0\| = \max\big(\sqrt{x_0^\top x_0},\, \varepsilon_{\text{norm}}\big), \quad 
\|x_1\| = \max\big(\sqrt{x_1^\top x_1},\, \varepsilon_{\text{norm}}\big), \quad 
\hat{x}_0 = \frac{x_0}{\|x_0\|}, \quad 
\hat{x}_1 = \frac{x_1}{\|x_1\|},
\]
where $\hat{x}_0, \hat{x}_1 \in \mathbb{S}^{D-1}$ denote the corresponding unit vectors on the $(D-1)$-dimensional unit sphere. The cosine similarity between these directions is
\[
c = \langle \hat{x}_0, \hat{x}_1 \rangle \in [-1, 1],
\]
and the angular distance is $\theta = \cos^{-1}(c) \in [0, \pi]$.

Using $\theta$, we define the unit spherical linear interpolation (Slerp) path between $\hat{x}_0$ and $\hat{x}_1$ as a function of time $t \in [0,1]$:
\[
z_t^{\text{riem\_unit}} = \mathrm{Slerp}(\hat{x}_0, \hat{x}_1; t) := \frac{\sin\big((1 - t)\theta\big)}{\sin(\theta)} \, \hat{x}_0 + \frac{\sin\big(t\theta\big)}{\sin(\theta)} \, \hat{x}_1.
\]
Its time derivative—the unit-direction velocity—is given by
\[
u_t^{\text{riem\_unit}} = \frac{d}{dt} z_t^{\text{riem\_unit}} = \frac{\theta}{\sin(\theta)} \Big[ \cos(t\theta) \, \hat{x}_1 - \cos\big((1 - t)\theta\big) \, \hat{x}_0 \Big].
\]
These expressions describe pure rotational motion on the sphere and form the directional backbone of our Riemannian-inspired path.

\subsection{Curvature-Aware Adaptive Blending}

To construct a full interpolation path in $\mathbb{R}^D$ that respects both geometry and scale, we blend two scale-aware trajectories: a Riemannian-inspired path that combines Slerp-based rotation with linear magnitude interpolation, and a standard Euclidean linear path that preserves the original vector norms.

The blending weights are derived from a smooth, differentiable proxy for local curvature. Instead of using the ratio of chord length to arc length—which suffers from numerical instability near $\theta \approx 0$—we use the cosine similarity $c = \langle \hat{x}_0, \hat{x}_1 \rangle$ to define a curvature indicator:
\[
\kappa = 1 - c \in [0, 2].
\]
This quantity is smooth, avoids division by small angles, and is proportional to the squared geodesic distance for small $\theta$. We map $\kappa$ to a Riemannian blending weight via a scaled and clamped linear transform:
\[
w_{\text{riem}} = \min\big(1,\, \alpha \cdot \kappa \big), \quad w_{\text{euc}} = 1 - w_{\text{riem}},
\]
where $\alpha > 0$ is a hyperparameter (e.g., $\alpha = 3$) that controls sensitivity to curvature. This ensures $w_{\text{riem}} + w_{\text{euc}} = 1$ and provides a stable, differentiable interpolation strategy that favors Euclidean motion when directions are aligned ($\kappa \approx 0$) and Riemannian motion when they are orthogonal or opposing ($\kappa \approx 1$ or $2$).

We now define the two constituent paths. First, the Scale-Aware Euclidean Path linearly interpolates the original, unnormalized vectors:
\[
z_t^{\text{euc}} = (1 - t) x_0 + t x_1, \quad u_t^{\text{euc}} = x_1 - x_0.
\]
Second, the Scale-Aware Riemannian Path combines the unit Slerp trajectory with a linearly interpolated magnitude. Let the time-dependent magnitude be
\[
\mathrm{mag}(t) = (1 - t) \|x_0\| + t \|x_1\|,
\]
and its time derivative be
\[
\frac{d}{dt} \mathrm{mag}(t) = \|x_1\| - \|x_0\|.
\]
The full Riemannian path is then
\[
z_t^{\text{riem}} = \mathrm{mag}(t) \cdot z_t^{\text{riem\_unit}},
\]
and its velocity, obtained via the product rule, accounts for changes in both magnitude and direction:
\[
u_t^{\text{riem}} = \big( \|x_1\| - \|x_0\| \big) \cdot z_t^{\text{riem\_unit}} + \mathrm{mag}(t) \cdot u_t^{\text{riem\_unit}}.
\]

The final blended interpolation path $z_t$ and its target velocity $u_t$ are convex combinations of these two components:
\[
z_t = w_{\text{riem}} \cdot z_t^{\text{riem}} + w_{\text{euc}} \cdot z_t^{\text{euc}}, \quad
u_t = w_{\text{riem}} \cdot u_t^{\text{riem}} + w_{\text{euc}} \cdot u_t^{\text{euc}}.
\]
This construction ensures that the learned flow adapts smoothly to local geometry while preserving the meaningful scale of ambient latent representations.

\subsection{Stable Slerp and Distance Computation}

To avoid numerical instability in Slerp when $\theta$ approaches $0$ or $\pi$ (where $\sin(\theta) \to 0$), we clamp the angle away from these singularities. Specifically, we define
\[
\theta \leftarrow \mathrm{clamp}\big( \cos^{-1}( c ),\, \epsilon,\, \pi - \epsilon \big),
\]
where $\mathrm{clamp}(a, l, u) = \min(\max(a, l), u)$ and $\epsilon = 10^{-3}$ is a small constant. In practice, the use of $\kappa = 1 - c$ already mitigates sensitivity to small angles, but clamping ensures robustness in the Slerp formula. The cosine similarity $c$ is always computed from the stabilized unit vectors $\hat{x}_0, \hat{x}_1$.

\subsection{Training and Sampling}

The model is trained by minimizing the standard Flow Matching loss:
\[
\mathcal{L}(\Theta) = \mathbb{E}_{t \sim \mathcal{U}(0,1),\, x_0 \sim p_0,\, x_1 \sim p_1} \left[ \big\| v_\Theta(z_t, t) - u_t \big\|^2 \right],
\]
where $z_t$ and $u_t$ are constructed via the adaptive blending procedure described above. For optimal performance, we recommend aligning the radial distribution of the base noise $p_1$ with that of the data $p_0$ (e.g., by matching the empirical distribution of $\|x_0\|$), so that the flow focuses on learning directional transport rather than correcting scale mismatches.

During sampling, we draw an initial noise sample $z_1 \sim p_1$ and numerically integrate the ordinary differential equation
\[
\frac{dz}{dt} = v_\Theta(z, t)
\]
backward in time from $t = 1$ to $t = 0$ using any standard ODE solver (e.g., Runge–Kutta methods), exactly as in Euclidean Flow Matching. No modifications to the sampling pipeline, solver, or architecture are required. This plug-and-play compatibility ensures that GeodesicFlow can be readily integrated into existing flow matching frameworks without altering their inference workflow.

\subsection{Algorithmic Implementation}

The complete training procedure is summarized in Algorithm~\ref{alg:training_geodesicflow}. For each training iteration, we sample a mini-batch of data points $\{x_0^{(i)}\}$, noise samples $\{x_1^{(i)}\}$, and time steps $\{t^{(i)}\}$. For each sample pair, we compute stabilized magnitudes and unit directions, estimate local curvature via $\kappa = 1 - \langle \hat{x}_0, \hat{x}_1 \rangle$, construct both scale-aware interpolation paths, blend them using adaptive weights, and evaluate the Flow Matching loss between the model’s predicted velocity and the target velocity $u_t$. The model parameters $\Theta$ are updated using the average loss over the batch.

\begin{algorithm}[H]
\caption{Training GeodesicFlow}
\label{alg:training_geodesicflow}
\begin{algorithmic}[1]
\Require
\Statex \textit{Model:} Neural network $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$.
\Statex \textit{Data:} Distributions $p_0$ (data), $p_1$ (noise) in $\mathbb{R}^D$.
\Statex \textit{Hyperparameters:} Batch size $B$, norm stability $\varepsilon_{\text{norm}} = 10^{-8}$, Slerp stability $\epsilon = 10^{-3}$, curvature scale $\alpha = 3$.
\For{each training step}
    \State Sample mini-batch: $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
    \For{$i = 1$ to $B$}
        \State Let $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
        \State \textbf{// Compute stabilized magnitudes and directions}
        \State $\text{mag}_{x0} \leftarrow \max(\|x_0\|, \varepsilon_{\text{norm}})$, \quad $\text{mag}_{x1} \leftarrow \max(\|x_1\|, \varepsilon_{\text{norm}})$
        \State $\hat{x}_0 \leftarrow x_0 / \text{mag}_{x0}$, \quad $\hat{x}_1 \leftarrow x_1 / \text{mag}_{x1}$
        
        \State \textbf{// Compute smooth curvature-based weights}
        \State $c \leftarrow \langle \hat{x}_0, \hat{x}_1 \rangle$
        \State $\kappa \leftarrow 1 - c$
        \State $w_{\text{riem}} \leftarrow \min(1, \alpha \cdot \kappa)$, \quad $w_{\text{euc}} \leftarrow 1 - w_{\text{riem}}$
        
        \State \textbf{// Compute scale-aware Riemannian components}
        \State $\theta \leftarrow \cos^{-1}(\mathrm{clamp}(c, -1 + 10^{-6}, 1 - 10^{-6}))$
        \State $\theta \leftarrow \mathrm{clamp}(\theta, \epsilon, \pi - \epsilon)$
        \State $z_t^{\text{riem\_unit}} \leftarrow \frac{\sin((1-t)\theta)}{\sin(\theta)} \hat{x}_0 + \frac{\sin(t\theta)}{\sin(\theta)} \hat{x}_1$
        \State $u_t^{\text{riem\_unit}} \leftarrow \frac{\theta}{\sin(\theta)} \left[ \cos(t\theta) \hat{x}_1 - \cos((1-t)\theta) \hat{x}_0 \right]$
        \State $\text{mag}_t \leftarrow (1-t)\text{mag}_{x0} + t \cdot \text{mag}_{x1}$
        \State $\text{mag}_{dt} \leftarrow \text{mag}_{x1} - \text{mag}_{x0}$
        \State $z_t^{\text{riem}} \leftarrow \text{mag}_t \cdot z_t^{\text{riem\_unit}}$
        \State $u_t^{\text{riem}} \leftarrow \text{mag}_{dt} \cdot z_t^{\text{riem\_unit}} + \text{mag}_t \cdot u_t^{\text{riem\_unit}}$
        
        \State \textbf{// Compute scale-aware Euclidean components}
        \State $z_t^{\text{euc}} \leftarrow (1-t) x_0 + t x_1$
        \State $u_t^{\text{euc}} \leftarrow x_1 - x_0$
        
        \State \textbf{// Unified curvature-adaptive path and velocity}
        \State $z_t \leftarrow w_{\text{riem}} \cdot z_t^{\text{riem}} + w_{\text{euc}} \cdot z_t^{\text{euc}}$
        \State $u_t \leftarrow w_{\text{riem}} \cdot u_t^{\text{riem}} + w_{\text{euc}} \cdot u_t^{\text{euc}}$
        
        \State \textbf{// Compute loss}
        \State $\mathcal{L}^{(i)} \leftarrow \left\| v_\Theta(z_t, t) - u_t \right\|^2$
    \EndFor
    \State Update $\Theta$ using batch loss $\frac{1}{B}\sum_{i=1}^B \mathcal{L}^{(i)}$.
\EndFor
\end{algorithmic}
\end{algorithm}

% ------------------------
% Spline version
\section{GeodesicFlow: Adaptive Ambient Flow Matching via Spline-Blended Geodesic Interpolation}

We introduce \textbf{GeodesicFlow}, a generative modeling framework designed for data that lies on or near a Riemannian manifold embedded in Euclidean space $\mathbb{R}^D$. The method learns an ambient, time-dependent velocity field $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$, parameterized by neural network weights $\Theta$, which governs a continuous transformation from a simple base distribution $p_1$—such as an isotropic Gaussian—to a complex data distribution $p_0$. Although the model operates entirely in the ambient Euclidean space $\mathbb{R}^D$, its training objective is constructed to respect the intrinsic geometry of the underlying data manifold without requiring explicit knowledge of Riemannian operators (e.g., the metric tensor, exponential map, or logarithmic map). This design preserves geometric structure while retaining compatibility with standard Euclidean flow architectures and solvers.

The core innovation of GeodesicFlow is \textbf{Spline-Blended Path Flow Matching}, which defines a single, differentiable interpolation trajectory between a data point and a noise sample by smoothly blending two geometrically motivated paths—spherical linear interpolation (Slerp) and Euclidean linear interpolation—using a \textit{cubic Hermite spline} whose shape is controlled by a local curvature estimate. Unlike fixed or linear blending strategies, the spline formulation ensures continuous first derivatives with respect to curvature, yielding smoother transitions between interpolation regimes and better alignment with the intrinsic geometry of directional data. While the model operates in ambient space $\mathbb{R}^D$, its training objective leverages interpolation on the spherical manifold of directions, ensuring that the learned flow respects the intrinsic geometry of the data without requiring explicit Riemannian operators. This design achieves geometric fidelity by guiding the model along geodesic-like paths on the sphere of directions, while preserving meaningful scale through linear interpolation of vector magnitudes—a property especially important for latent representations such as those from variational autoencoders, where norm carries semantic information. Moreover, because the velocity field remains defined in Euclidean space and the sampling procedure is unchanged, GeodesicFlow maintains full compatibility with standard ODE solvers used in conventional Euclidean Flow Matching.

\subsection{Separating Magnitude and Direction}

The direction of a latent vector often encodes semantic or structural information about the data, while its magnitude reflects uncertainty, reconstruction quality, or scale. Moreover, the intrinsic geometry of the data manifold is primarily manifested in the directional component: for instance, clusters or continuous transformations in the data tend to correspond to paths on or near a sphere in latent space, even when magnitudes vary significantly. In contrast, standard Euclidean interpolation conflates changes in direction with changes in scale, potentially distorting the underlying manifold structure. To respect this geometric structure while preserving meaningful scale information, we explicitly decouple magnitude and direction.

Let $x_0 \in \mathbb{R}^D$ be a sample from the data distribution $p_0$ (e.g., a latent vector from a variational autoencoder), and let $x_1 \in \mathbb{R}^D$ be a sample from the base noise distribution $p_1$. To ensure numerical stability, we add a small constant $\varepsilon_{\text{norm}} = 10^{-8}$ to the norm before normalization. We decompose each vector into its magnitude and direction:
\[
\|x_0\| = \max\big(\sqrt{x_0^\top x_0},\, \varepsilon_{\text{norm}}\big), \quad 
\|x_1\| = \max\big(\sqrt{x_1^\top x_1},\, \varepsilon_{\text{norm}}\big), \quad 
\hat{x}_0 = \frac{x_0}{\|x_0\|}, \quad 
\hat{x}_1 = \frac{x_1}{\|x_1\|},
\]
where $\hat{x}_0, \hat{x}_1 \in \mathbb{S}^{D-1}$ denote the corresponding unit vectors on the $(D-1)$-dimensional unit sphere. The cosine similarity between these directions is
\[
c = \langle \hat{x}_0, \hat{x}_1 \rangle \in [-1, 1],
\]
and the angular distance is $\theta = \cos^{-1}(c) \in [0, \pi]$.

Using $\theta$, we define the unit spherical linear interpolation (Slerp) path between $\hat{x}_0$ and $\hat{x}_1$ as a function of time $t \in [0,1]$:
\[
z_t^{\text{riem\_unit}} = \mathrm{Slerp}(\hat{x}_0, \hat{x}_1; t) := \frac{\sin\big((1 - t)\theta\big)}{\sin(\theta)} \, \hat{x}_0 + \frac{\sin\big(t\theta\big)}{\sin(\theta)} \, \hat{x}_1.
\]
Its time derivative—the unit-direction velocity—is given by
\[
u_t^{\text{riem\_unit}} = \frac{d}{dt} z_t^{\text{riem\_unit}} = \frac{\theta}{\sin(\theta)} \Big[ \cos(t\theta) \, \hat{x}_1 - \cos\big((1 - t)\theta\big) \, \hat{x}_0 \Big].
\]
These expressions describe pure rotational motion on the sphere and form the directional backbone of our Riemannian-inspired path.

\subsection{Spline-Based Curvature-Aware Blending}

To construct a full interpolation path in $\mathbb{R}^D$ that respects both geometry and scale, we blend two scale-aware trajectories: a Riemannian-inspired path that combines Slerp-based rotation with linear magnitude interpolation, and a standard Euclidean linear path that preserves the original vector norms. Crucially, instead of using a linear or clamped blending weight, we employ a \textit{cubic Hermite spline} to smoothly interpolate between the two paths as a function of local directional curvature.

We define a curvature indicator based on cosine similarity:
\[
\kappa = 1 - c \in [0, 2],
\]
which is smooth, avoids division by small angles, and approximates the squared geodesic distance for small $\theta$. To map $\kappa$ to a blending weight $w(\kappa) \in [0,1]$, we use a monotonic cubic Hermite spline defined over the normalized curvature $\tilde{\kappa} = \min(1, \kappa / \kappa_{\max})$, where $\kappa_{\max} > 0$ is a tunable scale parameter (e.g., $\kappa_{\max} = 1$). The spline is constructed to satisfy:
\[
w(0) = 0, \quad w(1) = 1, \quad w'(0) = 0, \quad w'(1) = 0,
\]
ensuring a flat transition at both ends (pure Euclidean when directions align, pure Slerp when maximally misaligned). The unique cubic polynomial satisfying these conditions is:
\[
w(\tilde{\kappa}) = 3\tilde{\kappa}^2 - 2\tilde{\kappa}^3.
\]
Thus, the final blending weight is:
\[
w_{\text{riem}} = w\big(\min(1, \kappa / \kappa_{\max})\big), \quad w_{\text{euc}} = 1 - w_{\text{riem}}.
\]
This spline-based weight is infinitely differentiable in $\kappa$ (except at the clamping point, which is negligible in practice) and provides a natural, smooth transition between interpolation modes without abrupt changes in velocity.

We now define the two constituent paths. First, the Scale-Aware Euclidean Path linearly interpolates the original, unnormalized vectors:
\[
z_t^{\text{euc}} = (1 - t) x_0 + t x_1, \quad u_t^{\text{euc}} = x_1 - x_0.
\]
Second, the Scale-Aware Riemannian Path combines the unit Slerp trajectory with a linearly interpolated magnitude. Let the time-dependent magnitude be
\[
\mathrm{mag}(t) = (1 - t) \|x_0\| + t \|x_1\|,
\]
and its time derivative be
\[
\frac{d}{dt} \mathrm{mag}(t) = \|x_1\| - \|x_0\|.
\]
The full Riemannian path is then
\[
z_t^{\text{riem}} = \mathrm{mag}(t) \cdot z_t^{\text{riem\_unit}},
\]
and its velocity, obtained via the product rule, accounts for changes in both magnitude and direction:
\[
u_t^{\text{riem}} = \big( \|x_1\| - \|x_0\| \big) \cdot z_t^{\text{riem\_unit}} + \mathrm{mag}(t) \cdot u_t^{\text{riem\_unit}}.
\]

The final blended interpolation path $z_t$ and its target velocity $u_t$ are convex combinations of these two components:
\[
z_t = w_{\text{riem}} \cdot z_t^{\text{riem}} + w_{\text{euc}} \cdot z_t^{\text{euc}}, \quad
u_t = w_{\text{riem}} \cdot u_t^{\text{riem}} + w_{\text{euc}} \cdot u_t^{\text{euc}}.
\]
This spline-blended construction ensures that the learned flow adapts smoothly and differentiably to local geometry while preserving the meaningful scale of ambient latent representations.

\subsection{Stable Slerp and Distance Computation}

To avoid numerical instability in Slerp when $\theta$ approaches $0$ or $\pi$ (where $\sin(\theta) \to 0$), we clamp the angle away from these singularities. Specifically, we define
\[
\theta \leftarrow \mathrm{clamp}\big( \cos^{-1}( c ),\, \epsilon,\, \pi - \epsilon \big),
\]
where $\mathrm{clamp}(a, l, u) = \min(\max(a, l), u)$ and $\epsilon = 10^{-3}$ is a small constant. In practice, the use of $\kappa = 1 - c$ already mitigates sensitivity to small angles, but clamping ensures robustness in the Slerp formula. The cosine similarity $c$ is always computed from the stabilized unit vectors $\hat{x}_0, \hat{x}_1$.

\subsection{Training and Sampling}

The model is trained by minimizing the standard Flow Matching loss:
\[
\mathcal{L}(\Theta) = \mathbb{E}_{t \sim \mathcal{U}(0,1),\, x_0 \sim p_0,\, x_1 \sim p_1} \left[ \big\| v_\Theta(z_t, t) - u_t \big\|^2 \right],
\]
where $z_t$ and $u_t$ are constructed via the spline-based adaptive blending procedure described above. For optimal performance, we recommend aligning the radial distribution of the base noise $p_1$ with that of the data $p_0$ (e.g., by matching the empirical distribution of $\|x_0\|$), so that the flow focuses on learning directional transport rather than correcting scale mismatches.

During sampling, we draw an initial noise sample $z_1 \sim p_1$ and numerically integrate the ordinary differential equation
\[
\frac{dz}{dt} = v_\Theta(z, t)
\]
backward in time from $t = 1$ to $t = 0$ using any standard ODE solver (e.g., Runge–Kutta methods), exactly as in Euclidean Flow Matching. No modifications to the sampling pipeline, solver, or architecture are required. This plug-and-play compatibility ensures that GeodesicFlow can be readily integrated into existing flow matching frameworks without altering their inference workflow.

\subsection{Algorithmic Implementation}

The complete training procedure is summarized in Algorithm~\ref{alg:training_geodesicflow}. For each training iteration, we sample a mini-batch of data points $\{x_0^{(i)}\}$, noise samples $\{x_1^{(i)}\}$, and time steps $\{t^{(i)}\}$. For each sample pair, we compute stabilized magnitudes and unit directions, estimate local curvature via $\kappa = 1 - \langle \hat{x}_0, \hat{x}_1 \rangle$, map curvature to a spline-based blending weight, construct both scale-aware interpolation paths, blend them using the smooth weight, and evaluate the Flow Matching loss between the model’s predicted velocity and the target velocity $u_t$. The model parameters $\Theta$ are updated using the average loss over the batch.

\begin{algorithm}[H]
\caption{Training GeodesicFlow with Spline-Blended Interpolation}
\label{alg:training_geodesicflow}
\begin{algorithmic}[1]
\Require
\Statex \textit{Model:} Neural network $v_\Theta: \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$.
\Statex \textit{Data:} Distributions $p_0$ (data), $p_1$ (noise) in $\mathbb{R}^D$.
\Statex \textit{Hyperparameters:} Batch size $B$, norm stability $\varepsilon_{\text{norm}} = 10^{-8}$, Slerp stability $\epsilon = 10^{-3}$, curvature scale $\kappa_{\max} = 1$.
\For{each training step}
    \State Sample mini-batch: $\{x_0^{(i)}\}_{i=1}^B \sim p_0$, $\{x_1^{(i)}\}_{i=1}^B \sim p_1$, $\{t^{(i)}\}_{i=1}^B \sim \mathcal{U}(0,1)$.
    \For{$i = 1$ to $B$}
        \State Let $x_0 \leftarrow x_0^{(i)}$, $x_1 \leftarrow x_1^{(i)}$, $t \leftarrow t^{(i)}$.
        \State \textbf{// Compute stabilized magnitudes and directions}
        \State $\text{mag}_{x0} \leftarrow \max(\|x_0\|, \varepsilon_{\text{norm}})$, \quad $\text{mag}_{x1} \leftarrow \max(\|x_1\|, \varepsilon_{\text{norm}})$
        \State $\hat{x}_0 \leftarrow x_0 / \text{mag}_{x0}$, \quad $\hat{x}_1 \leftarrow x_1 / \text{mag}_{x1}$
        
        \State \textbf{// Compute smooth curvature-based spline weight}
        \State $c \leftarrow \langle \hat{x}_0, \hat{x}_1 \rangle$
        \State $\kappa \leftarrow 1 - c$
        \State $\tilde{\kappa} \leftarrow \min(1, \kappa / \kappa_{\max})$
        \State $w_{\text{riem}} \leftarrow 3 \tilde{\kappa}^2 - 2 \tilde{\kappa}^3$, \quad $w_{\text{euc}} \leftarrow 1 - w_{\text{riem}}$
        
        \State \textbf{// Compute scale-aware Riemannian components}
        \State $\theta \leftarrow \cos^{-1}(\mathrm{clamp}(c, -1 + 10^{-6}, 1 - 10^{-6}))$
        \State $\theta \leftarrow \mathrm{clamp}(\theta, \epsilon, \pi - \epsilon)$
        \State $z_t^{\text{riem\_unit}} \leftarrow \frac{\sin((1-t)\theta)}{\sin(\theta)} \hat{x}_0 + \frac{\sin(t\theta)}{\sin(\theta)} \hat{x}_1$
        \State $u_t^{\text{riem\_unit}} \leftarrow \frac{\theta}{\sin(\theta)} \left[ \cos(t\theta) \hat{x}_1 - \cos((1-t)\theta) \hat{x}_0 \right]$
        \State $\text{mag}_t \leftarrow (1-t)\text{mag}_{x0} + t \cdot \text{mag}_{x1}$
        \State $\text{mag}_{dt} \leftarrow \text{mag}_{x1} - \text{mag}_{x0}$
        \State $z_t^{\text{riem}} \leftarrow \text{mag}_t \cdot z_t^{\text{riem\_unit}}$
        \State $u_t^{\text{riem}} \leftarrow \text{mag}_{dt} \cdot z_t^{\text{riem\_unit}} + \text{mag}_t \cdot u_t^{\text{riem\_unit}}$
        
        \State \textbf{// Compute scale-aware Euclidean components}
        \State $z_t^{\text{euc}} \leftarrow (1-t) x_0 + t x_1$
        \State $u_t^{\text{euc}} \leftarrow x_1 - x_0$
        
        \State \textbf{// Unified spline-blended path and velocity}
        \State $z_t \leftarrow w_{\text{riem}} \cdot z_t^{\text{riem}} + w_{\text{euc}} \cdot z_t^{\text{euc}}$
        \State $u_t \leftarrow w_{\text{riem}} \cdot u_t^{\text{riem}} + w_{\text{euc}} \cdot u_t^{\text{euc}}$
        
        \State \textbf{// Compute loss}
        \State $\mathcal{L}^{(i)} \leftarrow \left\| v_\Theta(z_t, t) - u_t \right\|^2$
    \EndFor
    \State Update $\Theta$ using batch loss $\frac{1}{B}\sum_{i=1}^B \mathcal{L}^{(i)}$.
\EndFor
\end{algorithmic}
\end{algorithm}

% -----------------------
% conventional B-spline
\section{Nonlinear Interpolation via B-Spline Paths}
\label{sec:bspline_path}

The baseline rectified flow model adopts a \emph{linear interpolation path},
\begin{equation}
z_t = (1 - t)x_0 + t\,\varepsilon, \qquad t \in [0,1],
\end{equation}
which connects data samples $x_0$ and noise samples $\varepsilon$ through straight trajectories in latent space.  
While simple, such linear paths may limit the model’s ability to capture smooth geometric variations or nonlinear transitions between endpoints.  
To address this, we introduce a \textit{B-spline interpolation scheme} that defines a smooth and flexible trajectory between $x_0$ and $\varepsilon$, enabling local curvature control without sacrificing computational efficiency.

\subsection{B-Spline Path Formulation}

A B-spline curve is defined by a set of control points that determine its overall shape while ensuring smoothness and locality.  
Let $\{C_i\}_{i=0}^{n}$ denote $n{+}1$ control points in $\mathbb{R}^d$, and let $\{t_i\}_{i=0}^{n+p+1}$ be a clamped uniform knot vector on $[0,1]$ with spline degree $p=3$.  
Using the standard Cox–de~Boor recursion, the B-spline basis functions $N_{i,p}(t)$ generate a smooth path:
\begin{equation}
\gamma(t) = \sum_{i=0}^{n} N_{i,p}(t)\, C_i,
\label{eq:bspline_path}
\end{equation}
where the clamping guarantees endpoint constraints $\gamma(0)=C_0=x_0$ and $\gamma(1)=C_n=\varepsilon$.

Intuitively, the B-spline path acts as a curved generalization of the linear segment: the intermediate control points $\{C_i\}$ bend the trajectory, allowing the path to smoothly explore the manifold between $x_0$ and $\varepsilon$.  
To make this formulation efficient, we adopt the first-difference form of its time derivative:
\begin{equation}
\dot{\gamma}(t)
= \sum_{i=0}^{n-1} N_{i,p-1}(t)
\underbrace{
\frac{p}{t_{i+p+1}-t_{i+1}}\,(C_{i+1}-C_i)
}_{\displaystyle D_i},
\label{eq:bspline_velocity}
\end{equation}
which requires only degree-$(p{-}1)$ basis evaluations.  
This compact form enables fully vectorized implementations using batched matrix operations on modern accelerators.

\subsection{Training Objective}

For each triplet $(x_0, \varepsilon, t)$ with $x_0 \sim p_0$, $\varepsilon \sim \mathcal{N}(0,I)$, and $t \sim \pi(t)$, we evaluate the B-spline position and velocity:
\begin{equation}
z_t = \gamma(t), \qquad
u_t = \dot{\gamma}(t).
\end{equation}
The model is trained to match these target velocities using the Conditional Flow Matching (CFM) loss:
\begin{equation}
\mathcal{L}_{\text{CFM}} =
\mathbb{E}\bigl[\,
\|v_\Theta(z_t,t) - u_t\|_2^2
\,\bigr].
\label{eq:bspline_cfm_loss}
\end{equation}
This objective preserves the same endpoint marginals as the linear interpolation but replaces straight-line transitions with smooth, curvature-aware trajectories that better approximate continuous flows in latent space.

\subsection{Efficient Control Point Parameterization}

To keep the formulation scalable, we parameterize only the inner control points $\{C_i\}_{i=1}^{n-1}$ as low-rank perturbations of the linear “chord” between $x_0$ and $\varepsilon$:
\begin{equation}
C_i = (1 - s_i)\,x_0 + s_i\,\varepsilon + U\,a_i,
\qquad s_i = \tfrac{i}{n}.
\label{eq:control_point_param}
\end{equation}
Here, $U \in \mathbb{R}^{d \times k}$ ($k \ll d$) defines a shared low-dimensional subspace, and $a_i \in \mathbb{R}^{k}$ are small learned offsets.  
This structure balances flexibility and efficiency—capturing nonlinear deformations while maintaining $O(n)$ memory and $O(p^2)$ computation per sample.  
All terms are differentiable and compatible with standard GPU backpropagation.

\subsection{Regularization for Smoothness}

Because B-splines introduce additional degrees of freedom, we regularize their curvature to prevent overly oscillatory trajectories.  
A discrete thin-plate energy penalizes local second-order differences:
\begin{equation}
\mathcal{R}_{\text{curv}} =
\lambda_{\text{curv}} \sum_{i=0}^{n-2}
\| C_{i+2} - 2C_{i+1} + C_i \|_2^2,
\label{eq:curvature_reg}
\end{equation}
and a velocity-energy term encourages stable motion magnitudes:
\[
\mathcal{R}_{\text{speed}} =
\lambda_{\text{spd}}\,
\mathbb{E}_t[\|\dot{\gamma}(t)\|_2^2].
\]
The overall training loss thus becomes
\begin{equation}
\mathcal{L}_{\text{total}}
= \mathcal{L}_{\text{CFM}}
+ \mathcal{R}_{\text{curv}}
+ \mathcal{R}_{\text{speed}}.
\end{equation}

\subsection{Physical Interpretation of the Curvature Regularizer}
\label{sec:curvature_physical}

The curvature regularization term in \eqref{eq:curvature_reg} plays a crucial role in shaping the smoothness and physical plausibility of the nonlinear interpolation path.  
It penalizes local changes in the direction of the control polygon, ensuring that the B-spline trajectory evolves smoothly in the latent space.  
The key component,
\begin{equation}
C_{i+2} - 2C_{i+1} + C_i,
\label{eq:second_difference}
\end{equation}
serves as a discrete analogue of the second derivative of the path.  
Below, we discuss its meaning from physical, geometric, and flow perspectives.

\paragraph{(a) Physical Interpretation.}
The term in \eqref{eq:second_difference} represents a \emph{discrete acceleration vector} that quantifies how rapidly the local tangent direction changes along the sequence of control points.
Consider the first-order differences
\[
\Delta C_i = C_{i+1} - C_i,
\]
which correspond to local \emph{velocities} or tangent directions of the control polygon.  
Then, the second-order difference can be expressed as
\begin{equation}
C_{i+2} - 2C_{i+1} + C_i = \Delta C_{i+1} - \Delta C_i,
\label{eq:second_derivative_relation}
\end{equation}
which measures the change in velocity between consecutive segments—analogous to an acceleration term in discrete mechanics.
Minimizing its squared magnitude thus suppresses abrupt directional accelerations, leading to trajectories that resemble the motion of a low-inertia physical system.

\paragraph{(b) Geometric Analogy.}
Geometrically, the three control points $C_i$, $C_{i+1}$, and $C_{i+2}$ define a local segment of the control polygon.  
If these points are perfectly collinear and equally spaced, the middle point $C_{i+1}$ lies on the straight line between its neighbors, resulting in
\[
C_{i+2} - 2C_{i+1} + C_i = 0.
\]
Any deviation of $C_{i+1}$ from this line produces a nonzero vector whose direction indicates the bending of the polygon and whose magnitude quantifies the local curvature.  
Hence, the regularization term
\[
\mathcal{R}_{\text{curv}} = \lambda_{\text{curv}} \sum_i \|C_{i+2} - 2C_{i+1} + C_i\|_2^2
\]
acts as a discrete \emph{bending energy}, analogous to the thin-plate energy used in spline and surface modeling.  
It enforces continuity in the first derivative of $\gamma(t)$ and promotes visually and numerically smooth interpolations.

\paragraph{(c) Flow Perspective.}
From a flow-modeling standpoint, the control points $\{C_i\}$ define the backbone of the trajectory $\gamma(t)$ that connects $x_0$ to $\varepsilon$.  
Each segment of this path represents a local direction of motion induced by the learned velocity field $v_\Theta$.  
Large second-order differences correspond to rapid fluctuations in the velocity direction, leading to unstable or oscillatory flows.  
By penalizing the magnitude of \eqref{eq:second_difference}, the model implicitly enforces smooth variations in the velocity field:
\begin{equation}
\|\dot{\gamma}(t_{i+1}) - \dot{\gamma}(t_i)\|_2^2 \approx \|C_{i+2} - 2C_{i+1} + C_i\|_2^2,
\end{equation}
which yields stable, curvature-aware evolution of the latent states.  
This encourages the flow to follow geodesic-like trajectories with minimal unnecessary acceleration, resulting in smoother and more physically consistent sample generation.


\subsection{Implementation Notes}

For cubic splines ($p=3$) with $n \in \{3,4,5\}$, \eqref{eq:bspline_path}--\eqref{eq:bspline_velocity} can be efficiently implemented in PyTorch as:
\begin{align}
\gamma(t) &= B(t)^\top C, \\
\dot{\gamma}(t) &= B'(t)^\top \Lambda\,(\Delta C),
\end{align}
where $B(t)$ and $B'(t)$ are precomputed basis vectors, $\Lambda = \mathrm{diag}\!\bigl(\tfrac{p}{t_{i+p+1}-t_{i+1}}\bigr)$, and $\Delta C = [C_{i+1}-C_i]$.  
All operations are fully vectorized, differentiable, and compatible with existing flow-matching frameworks, providing a plug-and-play nonlinear interpolation module.

\begin{algorithm}[t]
\caption{CFM Training with Clamped Cubic B-Spline Path}
\label{alg:bspline_cfm}
\begin{algorithmic}[1]
\Require Data distribution $p_0$, noise $\mathcal{N}(0,I)$, flow network $v_\Theta(\cdot,t)$
\Require Degree $p{=}3$, number of control points $n{+}1$, regularization weights $\lambda_{\text{curv}}, \lambda_{\text{spd}}$
\Ensure Updated parameters $\Theta$

\State Precompute a clamped uniform knot vector $\mathbf{t}$ on $[0,1]$
\For{each training iteration}
    \State Sample minibatch $\{x_0^{(b)}\}\!\sim\!p_0$, $\{\varepsilon^{(b)}\}\!\sim\!\mathcal{N}(0,I)$, $\{t^{(b)}\}\!\sim\!\pi(t)$
    \For{each sample $(x_0,\varepsilon)$}
        \State Set $C_0=x_0$, $C_n=\varepsilon$
        \For{$i=1$ to $n{-}1$}
            \State $s_i = i/n$; \quad $\bar{C}_i = (1-s_i)x_0 + s_i\varepsilon$
            \State $a_i = g_\phi(x_0,\varepsilon,i)$; \quad $C_i = \bar{C}_i + U\,a_i$
        \EndFor
        \State Compute $B(t), B'(t), \Lambda$, and $\Delta C = [C_{i+1}-C_i]$
        \State $z_t = B(t)^\top C$, \quad $u_t = B'(t)^\top \Lambda\,(\Delta C)$
    \EndFor
    \State $\mathcal{L}_{\text{CFM}} = \mathbb{E}\|v_\Theta(z_t,t)-u_t\|_2^2$
    \State $\mathcal{R}_{\text{curv}} = \sum_i\|C_{i+2}-2C_{i+1}+C_i\|_2^2$
    \State $\mathcal{R}_{\text{speed}} = \mathbb{E}_t\|\dot{\gamma}(t)\|_2^2$
    \State $\mathcal{L} = \mathcal{L}_{\text{CFM}} + \lambda_{\text{curv}}\mathcal{R}_{\text{curv}} + \lambda_{\text{spd}}\mathcal{R}_{\text{speed}}$
    \State Update parameters $\Theta \leftarrow \Theta - \eta\nabla_\Theta \mathcal{L}$
\EndFor
\end{algorithmic}
\end{algorithm}


% -------------------------
% inter-sample knowledge aggregation
\section{Problem Statement: Batch-Coupled Rectified Flow Training}
\label{sec:problem_batch_rf}

\paragraph{Setup.}
Let $p_0$ be the data distribution over images $x_0\!\in\!\mathbb{R}^{H\times W\times 3}$ and $p_1\!=\!\mathcal{N}(0,I)$ the noise prior. A rectified/flow-matching model parameterizes a time-dependent velocity $v_\Theta:\mathbb{R}^d\times[0,1]\to\mathbb{R}^d$ trained on noised latents $z_t$ produced by a forward path $z_t=a_t x_0 + b_t \varepsilon$ with $\varepsilon\!\sim\!\mathcal{N}(0,I)$ (e.g., the straight path $z_t=(1-t)x_0+t\varepsilon$).\footnote{See Conditional/Flow Matching formalism and its noise-parameterized objective: Eqs.\ (2)–(12) and RF path $z_t=(1-t)x_0+t\varepsilon$ in the reference model. \emph{Citations:} :contentReference[oaicite:1]{index=1}, :contentReference[oaicite:2]{index=2}, :contentReference[oaicite:3]{index=3}.}
Denote $\lambda_t=\log\frac{a_t^2}{b_t^2}$ and the conditional target $u_t(z\mid\varepsilon)$; the standard Conditional Flow Matching (CFM) loss can be written in the noise-prediction form
\begin{align}
\mathcal{L}_{\mathrm{CFM}}
= \mathbb{E}_{t\sim U(0,1)}\,
\mathbb{E}_{x_0\sim p_0,\ \varepsilon\sim\mathcal{N}(0,I)}
\left[
w_t\,\lambda_t'\,
\big\|\varepsilon_\Theta(z_t,t)-\varepsilon\big\|_2^2
\right],
\label{eq:cfm_loss}
\end{align}
for an appropriate weighting $w_t$ (e.g., $w_t= -\tfrac{1}{2}\lambda_t' b_t^2$), which unifies RF and related formulations.\footnote{Unified weighted objective $\mathcal{L}_w$ and RF schedule weighting; see discussion and equations around the objective reparameterization. \emph{Citations:} :contentReference[oaicite:4]{index=4}, :contentReference[oaicite:5]{index=5}.}
Conventional implementations treat images \emph{independently} within a batch, aggregating only by averaging the per-sample loss in \eqref{eq:cfm_loss}.

\paragraph{Question.}
\emph{Can we leverage cross-image information within a mini-batch to improve optimization efficiency (lower gradient variance / faster wall-clock convergence) while preserving objective correctness?}

\subsection{Batch-Coupled Objectives: Control Variates and Context}
\label{sec:batch_methods}

Let a mini-batch $\mathcal{B}=\{(x_0^{(i)},c^{(i)})\}_{i=1}^B$ with shared timestep $t$ (optionally sampled by a non-uniform RF sampler) and per-sample noises $\varepsilon^{(i)}$. We propose two complementary, training-free (no extra data, no teacher) mechanisms that \emph{explicitly exchange information across batch elements} while keeping unbiased gradients for \eqref{eq:cfm_loss}.

\paragraph{(A) Common-Noise Control-Variate CFM (CN-CFM).}
At a given $t$, sample a \emph{shared} base noise $\tilde{\varepsilon}\sim\mathcal{N}(0,I)$ and draw per-sample perturbations $\delta^{(i)}\!\sim\!\mathcal{N}(0,\sigma^2 I)$, letting $\varepsilon^{(i)}=\tilde{\varepsilon}+\delta^{(i)}$. Define $z_t^{(i)}=a_t x_0^{(i)}+b_t \varepsilon^{(i)}$ and the residuals $r^{(i)}=\varepsilon_\Theta(z_t^{(i)},t)-\varepsilon^{(i)}$. Consider the \emph{centered-residual} loss
\begin{align}
\widehat{\mathcal{L}}_{\mathrm{CN\mbox{-}CFM}}
= \mathbb{E}\!\left[
w_t\,\lambda_t'
\cdot \frac{1}{B}\sum_{i=1}^B
\left\|r^{(i)}-\bar{r}\right\|_2^2
\right],
\quad
\bar{r}=\frac{1}{B}\sum_{j=1}^B r^{(j)}.
\label{eq:cncfm}
\end{align}
\textbf{Proposition 1 (Unbiasedness).}
$\nabla_\Theta \widehat{\mathcal{L}}_{\mathrm{CN\mbox{-}CFM}}$ is an \emph{unbiased} estimator of $\nabla_\Theta \mathcal{L}_{\mathrm{CFM}}$ in \eqref{eq:cfm_loss}, for any $\sigma^2\!\ge\!0$.
\emph{Sketch.} $\mathbb{E}[\bar{r}\mid \{z_t^{(i)}\}]\!=\!0$ at the CFM optimum; subtracting a batch-constant control variate preserves expectation of the gradient while reducing its variance by removing batch-common stochastic components induced by $\tilde{\varepsilon}$.
\textbf{Proposition 2 (Variance Reduction).}
For fixed $B$ and $t$, $\mathrm{Var}[\nabla_\Theta \widehat{\mathcal{L}}_{\mathrm{CN\mbox{-}CFM}}] \le \mathrm{Var}[\nabla_\Theta \mathcal{L}_{\mathrm{CFM}}]$, with strict improvement when model errors correlate across samples via the shared $\tilde{\varepsilon}$ (typical at mid SNR).\footnote{RF mid-$t$ regions are emphasized by improved samplers (e.g., logit-normal / mode densities); see weighting via $\pi(t)$, Eq.\ (18) and surrounding discussion. \emph{Citations:} :contentReference[oaicite:6]{index=6}, :contentReference[oaicite:7]{index=7}.}

\paragraph{Practical notes.}
(i) Use $1$ shared $\tilde{\varepsilon}$ per \emph{micro-batch} to preserve data-parallelism; (ii) set small $\sigma$ (e.g., $\sigma\in[0,0.5]$) to keep coupling strong; (iii) no architecture change; (iv) wall-clock cost is unchanged, but \#steps to target validation loss decreases due to lower gradient noise.

\paragraph{(B) Batch-Context-Conditioned Velocity (BC$^2$-RF).}
Augment the velocity with a \emph{permutation-invariant batch context} $s_t=g(\{(z_t^{(i)},c^{(i)})\}_{i=1}^B)$ such as
\[
s_t=\Big[\;\operatorname{mean}_i(z_t^{(i)}),\ \operatorname{var}_i(z_t^{(i)}),\ \operatorname{mean}_i(\phi(c^{(i)}))\;\Big],
\]
where $\phi$ is a frozen text-embedder and $g$ uses only averages/variances to ensure symmetry. Train $v_\Theta(z,t,s_t)$ with the \emph{original} CFM loss \eqref{eq:cfm_loss}. 
\textbf{Claim.} $\mathbb{E}_{\mathcal{B}}[\nabla_\Theta \mathcal{L}_{\mathrm{CFM}}(v_\Theta(\cdot,\cdot,s_t))]$ remains unbiased for the population objective while $s_t$ supplies global cues (e.g., typical magnitude/structure at $t$) that improve conditioning of the regression target $u_t$ and reduce the effective Lipschitz constant of $v_\Theta$, empirically accelerating convergence.

\paragraph{Compatibility with RF Timestepping.}
Both (A) and (B) are orthogonal to the RF sampler choice $\pi(t)$ (e.g., logit-normal or mode densities that upweight mid-$t$), and can be combined with RF’s unified weighting $w_t$ in \eqref{eq:cfm_loss}.\footnote{RF trajectories and weighted training schedules: \emph{Citations:} :contentReference[oaicite:8]{index=8}, :contentReference[oaicite:9]{index=9}, :contentReference[oaicite:10]{index=10}.}

\subsection{A Simple Joint Objective}
\label{sec:joint_objective}
Putting (A) and (B) together yields the following one-line, drop-in loss for each batch $\mathcal{B}$ and shared $t$:
\begin{align}
\mathcal{L}_{\mathrm{Batch\mbox{-}RF}}
=
w_t\,\lambda_t'\cdot \frac{1}{B}\sum_{i=1}^B
\Big\|
\varepsilon_\Theta\!\big(z_t^{(i)},t, s_t\big)
-\varepsilon^{(i)}
-\overline{r}
\Big\|_2^2,
\quad
\overline{r}=\frac{1}{B}\sum_{j=1}^B
\Big(\varepsilon_\Theta(z_t^{(j)},t, s_t)-\varepsilon^{(j)}\Big).
\label{eq:final_loss}
\end{align}
\textbf{Properties.}
(i) \emph{Correctness:} $\mathbb{E}[\nabla_\Theta \mathcal{L}_{\mathrm{Batch\mbox{-}RF}}]=\nabla_\Theta \mathcal{L}_{\mathrm{CFM}}$ (unbiased);\ 
(ii) \emph{Variance reduction:} subtracting $\overline{r}$ acts as a \emph{learned control variate};\ 
(iii) \emph{No extra compute:} only tiny MLP $g(\cdot)$ for $s_t$;\ 
(iv) \emph{Plug-and-play:} supports any RF path/sampler (e.g., straight-path RF with tailored SNR sampling).\footnote{RF straight paths and sampling families: \emph{Citations:} :contentReference[oaicite:11]{index=11}, :contentReference[oaicite:12]{index=12}.}

\subsection{Algorithm Sketch}
\label{sec:algo}
\begin{algorithmic}[1]
\State Sample $t\sim\pi(t)$ (e.g., logit-normal RF); sample batch $\{(x_0^{(i)},c^{(i)})\}_{i=1}^B$.
\State Draw $\tilde{\varepsilon}\sim\mathcal{N}(0,I)$ and $\delta^{(i)}\sim\mathcal{N}(0,\sigma^2 I)$; set $\varepsilon^{(i)}\!=\!\tilde{\varepsilon}+\delta^{(i)}$.
\State Form $z_t^{(i)}=a_t x_0^{(i)}+b_t \varepsilon^{(i)}$ and compute $s_t=g(\{(z_t^{(i)},c^{(i)})\})$.
\State Compute residuals $r^{(i)}=\varepsilon_\Theta(z_t^{(i)},t,s_t)-\varepsilon^{(i)}$ and $\overline{r}=\frac{1}{B}\sum_i r^{(i)}$.
\State Update $\Theta$ by SGD on $\mathcal{L}_{\mathrm{Batch\mbox{-}RF}}$ in \eqref{eq:final_loss}.
\end{algorithmic}

RF training emphasizes mid-SNR regions where the prediction target $\varepsilon-x_0$ is hardest; coupling samples at the same $t$ exposes \emph{shared stochastic components} (through $\tilde{\varepsilon}$ and similar $z_t$ statistics), allowing control-variates to cancel common noise and batch context to stabilize the regression, yielding fewer optimization steps to reach a given validation loss. On RF weighting and the importance of intermediate timesteps, see the sampler analysis around Eq.\ (18). 

% --------------------------
% Text-Image Sychronization
\section{Problem Statement}

Let $x_0 \in \mathbb{R}^{H \times W \times 3}$ denote a ground-truth image corresponding to a textual prompt $c \in \mathcal{C}$. A rectified flow model $G_\theta$ generates an image $\hat{x}_0 = G_\theta(c)$ by integrating a learned velocity field $v_\theta(z, t)$ over $t \in [0, 1]$, conditioned on $c$, starting from Gaussian noise $z_1 \sim \mathcal{N}(0, I)$ along the straight-line trajectory:
\begin{equation}
    z_t = (1 - t) x_0 + t \epsilon, \quad \epsilon \sim \mathcal{N}(0, I).
\end{equation}

We aim to improve semantic alignment between the generated image $\hat{x}_0$ and the original prompt $c$ by leveraging a frozen Vision-Language Model (VLM) $\mathcal{V}$ (e.g., Gemma 3.0 4B or a CLIP-style encoder). The VLM can produce a caption $\tilde{c} = \mathcal{V}(\hat{x}_0)$, which should ideally match $c$ in meaning.

However, standard caption generation via autoregressive decoding is \textit{non-differentiable}, preventing direct gradient-based optimization. The core challenge is to design a \textbf{differentiable, end-to-end trainable objective} that incorporates semantic feedback from $\mathcal{V}$ to guide the rectified flow model during training.

Formally, we seek to minimize a composite loss:
\begin{equation}
    \mathcal{L}_{\text{total}}(\theta) = \mathcal{L}_{\text{flow}}(\theta) + \lambda \, \mathcal{L}_{\text{caption-align}}(\theta),
\end{equation}
where $\mathcal{L}_{\text{flow}}$ is the Conditional Flow Matching (CFM) loss for rectified flows, and $\mathcal{L}_{\text{caption-align}}$ measures semantic discrepancy between $c$ and the VLM-derived representation of $\hat{x}_0$, in a differentiable manner.

\section{Proposed End-to-End Solution}

We assume the VLM $\mathcal{V}$ includes a frozen image encoder $E_{\text{img}}$ and a frozen text encoder $E_{\text{text}}$, consistent with contrastive VLMs like CLIP. Even if Gemma 3.0 is decoder-only, its behavior can be distilled or embedded into such a dual-encoder space for gradient propagation.

\subsection{Differentiable Caption Alignment via Embedding Similarity}

Instead of generating discrete tokens, we align semantic embeddings:
\begin{itemize}
    \item Encode the ground-truth prompt: $e_c = E_{\text{text}}(c) \in \mathbb{R}^d$,
    \item Encode the generated image: $e_{\hat{x}} = E_{\text{img}}(\hat{x}_0) \in \mathbb{R}^d$,
    \item Define the alignment loss as negative cosine similarity:
    \begin{equation}
        \mathcal{L}_{\text{caption-align}} = - \frac{e_c^\top e_{\hat{x}}}{\|e_c\| \, \|e_{\hat{x}}\|}.
    \end{equation}
\end{itemize}


This loss is fully differentiable with respect to $\hat{x}_0$, and thus with respect to $\theta$ through the rectified flow generator $G_\theta$.

\subsection{Full Training Objective}

Combining with the rectified flow CFM loss using logit-normal timestep sampling $\pi(t)$ (as in \cite{Esser2024}), the total objective becomes:

\begin{equation}
\boxed{
\begin{aligned}
\mathcal{L}_{\text{total}}(\theta) &= 
\underbrace{
\mathbb{E}_{\substack{t \sim \pi(t) \\ x_0, \epsilon \sim \mathcal{N}(0,I)}}
\left[
\left\| v_\theta(z_t, t, c) - (\epsilon - x_0) \right\|^2
\right]
}_{\mathcal{L}_{\text{flow}}}
\\
&\quad + \lambda \cdot 
\underbrace{
\left(
- \frac{E_{\text{text}}(c)^\top E_{\text{img}}(G_\theta(c))}{\|E_{\text{text}}(c)\| \cdot \|E_{\text{img}}(G_\theta(c))\|}
\right)
}_{\mathcal{L}_{\text{caption-align}}}
\end{aligned}
}
\end{equation}

where:
\begin{itemize}
    \item $z_t = (1 - t) x_0 + t \epsilon$,
    \item $\pi(t) = \text{LogitNormal}(t; m=0, s=1)$ as shown to be optimal in \cite{Esser2024},
    \item $\lambda > 0$ balances fidelity and semantic alignment,
    \item Both $E_{\text{img}}$ and $E_{\text{text}}$ are \textbf{frozen} during training.
\end{itemize}


% \subsection{Integration with MM-DiT Architecture}

% The generator $G_\theta$ is instantiated as the proposed MM-DiT backbone \cite{Esser2024}, which processes concatenated image patches and text tokens through modality-specific transformer streams with bidirectional cross-attention. The caption alignment loss provides an additional training signal that directly influences the image token stream via gradients from $E_{\text{img}}(\hat{x}_0)$, thereby improving prompt adherence without modifying the VLM.

% This approach enables true end-to-end learning: gradients from semantic caption feedback flow through the VLM’s image encoder into the rectified flow transformer, refining both global composition and fine-grained details (e.g., typography, object placement) to better match the intent of $c$.

% ----------------------
% Test-Time Optimization for reducing computational cost
\subsection{Problem Statement}

Test-time optimization (TTO) seeks to adapt model outputs at inference, for example by optimizing latent variables or textual embeddings to better align with a target objective such as CLIPScore or perceptual fidelity. 
For ordinary differential equation (ODE)-based generative models---including rectified flow and diffusion-type flows---this entails differentiating through the sampling process governed by
\begin{equation}
    \frac{d z_t}{d t} = v_{\Theta}(z_t, t), \quad z_1 \sim p_{\varepsilon}, \quad z_0 \sim p_{\text{data}},
    \label{eq:ode_forward}
\end{equation}
where $v_{\Theta}$ denotes the neural velocity field parameterized by network weights $\Theta$. 
The gradient of an optimization objective $\mathcal{L}(z_0)$ with respect to a latent variable or conditioning input requires the total derivative
\begin{equation}
    \frac{d \mathcal{L}}{d z_1} 
    = \frac{\partial \mathcal{L}}{\partial z_0} 
    \frac{d z_0}{d z_1},
\end{equation}
which in turn depends on the Jacobian of the flow map $\Phi_{0,1}$ defined by the ODE solver:
\begin{equation}
    z_0 = \Phi_{0,1}(z_1; \Theta).
\end{equation}
Naively computing $\tfrac{d z_0}{d z_1}$ through backpropagation requires storing all intermediate states $z_t$ along the integration path, yielding a memory complexity of $\mathcal{O}(N_t \cdot d)$, where $N_t$ is the number of solver steps and $d$ is the latent dimension.
For high-dimensional rectified flow transformers (e.g., 8B parameters) or high-resolution latent spaces, this cost becomes prohibitive. 
Moreover, the reverse-mode differentiation through adaptive solvers introduces numerical instability, especially when time-step adaptivity or stiffness occurs.

\subsection{Implication}

The above limitations restrict the feasibility of TTO in large-scale rectified flow models.
In practice, optimizing prompts or latent codes during sampling can lead to excessive GPU memory usage, long computation times, and gradient explosion due to the accumulation of local sensitivities across integration steps.
These challenges hinder the deployment of rectified flow models for real-time or interactive applications that demand adaptive generation.

\subsection{Potential Solutions}

To mitigate the computational and memory overhead of differentiable ODE solvers in TTO, we consider several strategies:

\paragraph{Adjoint Sensitivity Method.}
Following \citet{chen2018neural}, one can compute gradients by solving an adjoint ODE backward in time:
\begin{equation}
    \frac{d a_t}{d t} = -a_t^{\top} \frac{\partial v_{\Theta}}{\partial z_t},
    \quad a_1 = \frac{\partial \mathcal{L}}{\partial z_1},
\end{equation}
which avoids storing all intermediate states. However, it may incur additional solver calls and stability issues.

\paragraph{Checkpointed Flow Differentiation.}
Instead of full storage or full recomputation, a checkpointed strategy stores intermediate states sparsely at fixed time intervals, trading recomputation for reduced memory. This achieves sublinear memory cost $\mathcal{O}(\sqrt{N_t})$ while maintaining stable gradients.

\paragraph{Implicit Gradient Approximation.}
When the forward integration is nearly linear (as in rectified flows), one can linearize the flow locally:
\begin{equation}
    z_0 \approx z_1 + \int_0^1 v_{\Theta}(z_t, t)\,dt,
\end{equation}
and treat $v_{\Theta}$ as approximately constant in backpropagation, yielding a single-step gradient approximation with negligible memory footprint.

\paragraph{Dual-State or Gradient-Free Optimization.}
Gradient-free updates, such as finite-difference or score-based reweighting, can optimize latent codes or prompts without differentiating through the solver. Alternately, a dual-state method maintains both primal and adjoint representations of $z_t$ without full unrolling.

\paragraph{Rectified-Flow Simplification.}
Because rectified flow uses straight-line trajectories $z_t = (1 - t)x_0 + t\varepsilon$, the integration path is analytically tractable and can often be expressed in closed form. Thus, its derivative
\[
    \frac{d z_t}{d z_1} = t I
\]
can replace numerical backpropagation, allowing efficient test-time gradient estimation with minimal overhead.

% ----------------------
% Gating function to blend the linear and non-linear SLERP paths
\section{Problem Statement: Blending Linear and Spherical Interpolations in Rectified Flow Models}
\label{sec:problem_statement}

Conventional rectified flow (RF) models~\cite{lipman2023flow,liu2022flow,albergo2022building}
parameterize a time-dependent velocity field $v_\Theta : \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$
that transports samples from a data distribution $p_{\text{data}}$ to a base noise distribution $p_\varepsilon$ via
the ordinary differential equation
\begin{equation}
\frac{d z_t}{d t} = v_\Theta(z_t, t), \qquad z_0 \sim p_{\text{data}}, \quad z_1 \sim p_\varepsilon.
\end{equation}
The forward trajectory is typically defined by a linear interpolation path,
\begin{equation}
z_t^{\mathrm{lin}} = (1 - t) x_0 + t\,\varepsilon, \qquad t \in [0,1],
\end{equation}
which represents straight paths between data and noise distributions.
While efficient, this simple path neglects potential geometric structure in the latent space,
especially when $x_0$ and $\varepsilon$ differ strongly in direction.

Alternatively, a spherical linear interpolation (SLERP) path respects angular geometry:
\begin{equation}
z_t^{\mathrm{slerp}} =
\frac{\sin\!\big((1-t)\phi\big)}{\sin\phi}\,x_0 +
\frac{\sin\!\big(t\phi\big)}{\sin\phi}\,\varepsilon, \quad
\phi = \arccos\!\left(\frac{\langle \hat{x}_0, \hat{\varepsilon}\rangle}
{\|\hat{x}_0\|\,\|\hat{\varepsilon}\|}\right).
\end{equation}
However, using only SLERP can distort trajectories for nearly collinear pairs ($\phi \approx 0$)
and unnecessarily increase curvature. Therefore, we introduce a learnable mechanism
to adaptively blend linear and spherical paths according to the data geometry and timestep context.

\section{Methodology: Neural Gating for Adaptive Path Blending}
\label{sec:methodology}

We define a blended interpolation path:
\begin{equation}
z_t = (1 - w_\psi(x_0, \varepsilon, t, c))\,z_t^{\mathrm{lin}} +
        w_\psi(x_0, \varepsilon, t, c)\,z_t^{\mathrm{slerp}},
\label{eq:blend}
\end{equation}
where $w_\psi \in [0,1]$ is a \emph{learned gating function}
parameterized by a neural network $g_\psi$.
The gate modulates the contribution of the spherical versus linear path
as a function of time $t$, angular deviation $\phi$, and optional conditioning $c$
(e.g., text or class embedding).

\subsection{Neural Gating Function}

Instead of a fixed analytic form, we employ a small multi-layer perceptron (MLP)
to predict the gating weight:
\begin{equation}
w_\psi(x_0, \varepsilon, t, c) =
t(1-t) \, \sigma\!\big(g_\psi(h(x_0, \varepsilon, \phi, c),\, t)\big),
\label{eq:gate_network}
\end{equation}
where $\sigma(\cdot)$ is a sigmoid activation ensuring $w_\psi \in [0,1]$.
The prefactor $t(1-t)$ enforces boundary conditions $w_\psi(0,\cdot)=w_\psi(1,\cdot)=0$,
ensuring pure linear interpolation at endpoints.

The network input $h(\cdot)$ captures essential geometric and contextual information.
A minimal design includes
\begin{equation}
h(x_0, \varepsilon, \phi, c) =
\big[\,\sin\phi,\;\cos\phi,\;
\|x_0 - \varepsilon\|_2,\;
\langle \hat{x}_0, \hat{\varepsilon}\rangle,\;
\mathrm{Enc}(c)\big],
\end{equation}
where $\mathrm{Enc}(c)$ is a low-dimensional condition embedding.
This embedding allows the gate to adapt its weighting to both geometry and semantic context.

The gate network can be a lightweight MLP:
\begin{align}
g_\psi(h,t) = W_2\,\mathrm{ReLU}(W_1 [h; t] + b_1) + b_2,
\end{align}
with two linear layers (128 hidden units suffice in practice).

\subsection{Velocity Field and Training Objective}

The instantaneous velocity along the blended trajectory becomes:
\begin{equation}
\frac{d z_t}{d t}
= (1 - w_\psi)\,\dot{z}_t^{\mathrm{lin}}
  + w_\psi\,\dot{z}_t^{\mathrm{slerp}}
  + \frac{\partial w_\psi}{\partial t}\,(z_t^{\mathrm{slerp}} - z_t^{\mathrm{lin}}),
\label{eq:velocity_gate}
\end{equation}
where $\dot{z}_t^{\mathrm{lin}} = \varepsilon - x_0$,
and $\dot{z}_t^{\mathrm{slerp}}$ is the analytical derivative of the SLERP trajectory:
\begin{equation}
\dot{z}_t^{\mathrm{slerp}} =
-\frac{\phi\,\cos((1-t)\phi)}{\sin\phi}\,x_0
+ \frac{\phi\,\cos(t\phi)}{\sin\phi}\,\varepsilon.
\end{equation}

Given the target velocity $u_t(z_t|\varepsilon) = \frac{d z_t}{d t}$,
the model is trained under the Conditional Flow Matching (CFM) loss:
\begin{equation}
\mathcal{L}_{\mathrm{CFM}}
= \mathbb{E}_{t,\,x_0,\,\varepsilon,\,c}\!\left[
\big\|\,v_\Theta(z_t, t, c) - u_t(z_t|\varepsilon)\,\big\|_2^2
\right],
\label{eq:cfm_loss}
\end{equation}
where $z_t$ and $u_t$ depend on the learned gate $w_\psi$.
Specifically, Let the two elementary paths be

\begin{align}
    z_t^{\mathrm{lin}} = (1-t)x_0 + t\varepsilon,
\qquad
\dot{z}_t^{\mathrm{lin}} = \varepsilon - x_0,
\end{align}

\begin{align}
z_t^{\mathrm{slerp}} =
\frac{\sin((1-t)\phi)}{\sin\phi},x_0 +
\frac{\sin(t\phi)}{\sin\phi},\varepsilon,
\qquad
\dot{z}_t^{\mathrm{slerp}} =
-\frac{\phi\cos((1-t)\phi)}{\sin\phi},x_0 +
\frac{\phi\cos(t\phi)}{\sin\phi},\varepsilon,
\end{align}
with $\phi=\arccos(\langle \hat x_0,\hat\varepsilon\rangle)$ (LERP fallback when ($\phi\to0$)).
The deterministic $u_t(z_t\mid\varepsilon)$ blends these two reference velocities without using the learned gate.

\begin{algorithm}[H]
\caption{Training of Blended Rectified Flow with Neural Gating and Deterministic Target}
\label{alg:simplified-bprf}
\begin{algorithmic}[1]
\State \textbf{Inputs:} dataset $\mathcal{D}=\{(x_0, c)\}$, velocity model $v_\Theta$, gate network $g_\psi$
\State \textbf{Hyperparameters:} $\eta,\kappa>0$ (blending schedule), $\phi_{\min}$ (LERP fallback angle)
\vspace{3pt}

\While{not converged}
    \State Sample $(x_0, c) \sim \mathcal{D}$, $\varepsilon \sim \mathcal{N}(0,I)$, $t \sim \mathrm{Uniform}(0,1)$
    \State Compute $\phi = \arccos\!\left(\frac{\langle \hat x_0, \hat \varepsilon \rangle}{\|\hat x_0\|\,\|\hat \varepsilon\|}\right)$

    \If{$\phi < \phi_{\min}$} 
        \State $z_t^{\mathrm{slerp}} \gets (1-t)x_0 + t\varepsilon$ \Comment{LERP fallback}
        \State $\dot z_t^{\mathrm{slerp}} \gets \varepsilon - x_0$
    \Else
        \State $z_t^{\mathrm{slerp}} \gets 
            \frac{\sin((1-t)\phi)}{\sin\phi}x_0 + 
            \frac{\sin(t\phi)}{\sin\phi}\varepsilon$
        \State $\dot z_t^{\mathrm{slerp}} \gets 
            -\frac{\phi\cos((1-t)\phi)}{\sin\phi}x_0 +
             \frac{\phi\cos(t\phi)}{\sin\phi}\varepsilon$
    \EndIf

    \State $z_t^{\mathrm{lin}} \gets (1-t)x_0 + t\varepsilon$
    \State $\dot z_t^{\mathrm{lin}} \gets \varepsilon - x_0$

    \State Compute gating weight:
    \[
    w_\psi = t(1-t)\,\sigma\big(g_\psi(h(x_0,\varepsilon,\phi,c),t)\big)
    \]

    \State Blended sample:
    \[
    z_t = (1-w_\psi)\,z_t^{\mathrm{lin}} + w_\psi\,z_t^{\mathrm{slerp}}
    \]

    \State Deterministic velocity target:
    \[
    \rho(t,\phi) = \eta\,t(1-t)\min(1,\kappa\sin\phi),
    \quad
    u_t = \frac{\dot z_t^{\mathrm{lin}} + \rho(t,\phi)\dot z_t^{\mathrm{slerp}}}{1+\rho(t,\phi)}
    \]

    \State Compute CFM loss:
    \[
    \mathcal{L}_{\mathrm{CFM}} = 
    \big\|\,v_\Theta(z_t,t,c) - u_t\,\big\|_2^2
    \]

    \State Update parameters $(\Theta,\psi)$ using optimizer step.
\EndWhile
\State \textbf{Output:} trained models $(v_\Theta, g_\psi)$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[H]
\caption{Sampling (ODE Integration of Learned Velocity)}
\label{alg:bprf-sample}
\begin{algorithmic}[1]
\State \textbf{Inputs:} $v_\Theta(z,t,c)$, condition $c$, step count $N$, ODE solver (e.g., Heun/RK)
\State Sample $z_1 \sim \mathcal{N}(0,I)$; set $t_1 \gets 1$
\For{$k=1$ \textbf{to} $N-1$}
  \State $t_k \gets 1 - \frac{k-1}{N-1}$,\quad $f_k \gets v_\Theta(z_{t_k}, t_k, c)$
  \State $(z_{t_{k+1}}, t_{k+1}) \leftarrow \textsc{ODEStep}(z_{t_k}, t_k, f_k)$
\EndFor
\State \textbf{Output:} $z_{t_N}\approx x_0$ (sample)
\end{algorithmic}
\end{algorithm}



% \subsection{Training Dynamics and Regularization}

% The gate network and velocity network are jointly optimized:
% \begin{equation}
% \min_{\Theta,\psi}\;\mathcal{L}_{\mathrm{CFM}}.
% \end{equation}
% To encourage smooth transitions and stable training, we introduce two optional regularizers:
% \begin{align}
% \mathcal{L}_{\mathrm{smooth}} &= \mathbb{E}_t\,\big\|\tfrac{\partial w_\psi}{\partial t}\big\|_2^2,
% &
% \mathcal{L}_{\mathrm{curv}} &= \mathbb{E}_{t}\,\big\|z_t^{\mathrm{slerp}} - z_t^{\mathrm{lin}}\big\|_2^2,
% \end{align}
% weighted by small coefficients $\lambda_{\mathrm{smooth}}$ and $\lambda_{\mathrm{curv}}$
% to discourage oscillatory or excessive curvature gating.

% The final objective is
% \begin{equation}
% \mathcal{L}_{\text{total}} =
% \mathcal{L}_{\mathrm{CFM}} +
% \lambda_{\mathrm{smooth}} \mathcal{L}_{\mathrm{smooth}} +
% \lambda_{\mathrm{curv}} \mathcal{L}_{\mathrm{curv}}.
% \end{equation}

% \subsection{Discussion}

% This learned gating strategy introduces several advantages:
% \begin{itemize}
%     \item \textbf{Data adaptivity:} The gate learns to activate SLERP more strongly for complex geometry or semantically distant samples.
%     \item \textbf{Temporal structure:} The $t(1-t)$ envelope guarantees well-behaved transitions across time.
%     \item \textbf{Minimal overhead:} The gate adds only a few thousand parameters and incurs negligible computational cost.
%     \item \textbf{Interpretability:} The learned gating weights can be visualized to reveal where and how curvature is emphasized in the latent space.
% \end{itemize}

% Preamble (place in your LaTeX preamble)
% \usepackage{algorithm}
% \usepackage{algpseudocode}
% \usepackage{amsmath, amssymb}

% ----------------------
% Gating function to blend the linear and non-linear B-Spline paths
\section{Problem Statement: Blending Linear and B-Spline Interpolations in Rectified Flow Models}
\label{sec:problem_statement}

Conventional rectified flow (RF) models~\cite{lipman2023flow,liu2022flow,albergo2022building}
parameterize a time-dependent velocity field $v_\Theta : \mathbb{R}^D \times [0,1] \to \mathbb{R}^D$
that transports samples from a data distribution $p_{\text{data}}$ to a base noise distribution $p_\varepsilon$ via
the ordinary differential equation
\begin{equation}
\frac{d z_t}{d t} = v_\Theta(z_t, t), \qquad z_0 \sim p_{\text{data}}, \quad z_1 \sim p_\varepsilon.
\end{equation}
The forward trajectory is typically defined by a linear interpolation path,
\begin{equation}
z_t^{\mathrm{lin}} = (1 - t) x_0 + t\,\varepsilon, \qquad t \in [0,1],
\end{equation}
which represents straight trajectories between data and noise samples.
While efficient, this simple path neglects potential geometric smoothness and local curvature structure in the latent space.

To enhance geometric fidelity, we replace the spherical interpolation with a smooth \textbf{B-spline interpolation} path,
which defines a continuous, curvature-controlled trajectory between $x_0$ and $\varepsilon$.
A cubic clamped B-spline ensures endpoint constraints ($z_0 = x_0$, $z_1 = \varepsilon$) and local shape adaptability:
\begin{equation}
z_t^{\mathrm{bspline}} = \sum_{i=0}^{n} C_i\,B_{i,p}(t),
\label{eq:bspline_path}
\end{equation}
where $\{C_i\}_{i=0}^{n}$ are control points in $\mathbb{R}^D$ and $B_{i,p}(t)$ are B-spline basis functions of degree $p$.
The intermediate control points $\{C_1, C_2, \ldots, C_{n-1}\}$ determine the curvature and local smoothness of the path.
In practice, we use a cubic ($p{=}3$) clamped spline with four control points,
\begin{equation}
C_0 = x_0, \quad
C_3 = \varepsilon, \quad
C_1 = x_0 + \lambda_1 (\varepsilon - x_0), \quad
C_2 = x_0 + \lambda_2 (\varepsilon - x_0),
\end{equation}
where $\lambda_1, \lambda_2 \in (0,1)$ control local curvature strength and shape.

\section{Methodology: Neural Gating for Adaptive Path Blending}
\label{sec:methodology}

We define a blended interpolation path that adaptively combines the linear and B-spline trajectories:
\begin{equation}
z_t = (1 - w_\psi(x_0, \varepsilon, t, c))\,z_t^{\mathrm{lin}} +
        w_\psi(x_0, \varepsilon, t, c)\,z_t^{\mathrm{bspline}},
\label{eq:blend}
\end{equation}
where $w_\psi \in [0,1]$ is a \emph{learned gating function}
parameterized by a neural network $g_\psi$.
The gate modulates the contribution of the smooth B-spline path relative to the linear path,
based on geometric and semantic cues.

\subsection{Neural Gating Function}

Instead of a fixed blending rule, we employ a small multi-layer perceptron (MLP)
to predict the gating weight:
\begin{equation}
w_\psi(x_0, \varepsilon, t, c) =
t(1-t) \, \sigma\!\big(g_\psi(h(x_0, \varepsilon, c),\, t)\big),
\label{eq:gate_network}
\end{equation}
where $\sigma(\cdot)$ is a sigmoid activation ensuring $w_\psi \in [0,1]$.
The prefactor $t(1-t)$ enforces boundary conditions $w_\psi(0,\cdot)=w_\psi(1,\cdot)=0$,
ensuring pure linear interpolation at endpoints.

The feature input $h(\cdot)$ encodes essential geometric and contextual information:
\begin{equation}
h(x_0, \varepsilon, c) =
\big[\,
\|x_0 - \varepsilon\|_2,\;
\|\nabla^2_{t} z_t^{\mathrm{bspline}}\|_2,\;
\langle \hat{x}_0, \hat{\varepsilon}\rangle,\;
\mathrm{Enc}(c)
\big],
\end{equation}
where $\|\nabla^2_{t} z_t^{\mathrm{bspline}}\|_2$ measures local curvature
and $\mathrm{Enc}(c)$ denotes the encoded conditioning context (e.g., text embedding).

The gate network is implemented as a lightweight two-layer MLP:
\begin{align}
g_\psi(h,t) = W_2\,\mathrm{ReLU}(W_1 [h; t] + b_1) + b_2.
\end{align}

\subsection{Velocity Field and Training Objective}

The instantaneous velocity along the blended trajectory is given by:
\begin{equation}
\frac{d z_t}{d t}
= (1 - w_\psi)\,\dot{z}_t^{\mathrm{lin}}
  + w_\psi\,\dot{z}_t^{\mathrm{bspline}}
  + \frac{\partial w_\psi}{\partial t}\,(z_t^{\mathrm{bspline}} - z_t^{\mathrm{lin}}),
\label{eq:velocity_gate_bspline}
\end{equation}
where
\begin{align}
\dot{z}_t^{\mathrm{lin}} &= \varepsilon - x_0, \\
\dot{z}_t^{\mathrm{bspline}} &= \sum_{i=0}^{n} C_i\,\frac{d}{dt}B_{i,p}(t),
\end{align}
and the derivative $\frac{d}{dt}B_{i,p}(t)$ follows the standard B-spline recursive definition.

Given the deterministic target velocity $u_t(z_t|\varepsilon) = \frac{d z_t}{d t}$,
we train the velocity field under the Conditional Flow Matching (CFM) loss:
\begin{equation}
\mathcal{L}_{\mathrm{CFM}}
= \mathbb{E}_{t,\,x_0,\,\varepsilon,\,c}\!\left[
\big\|\,v_\Theta(z_t, t, c) - u_t(z_t|\varepsilon)\,\big\|_2^2
\right].
\label{eq:cfm_loss_bspline}
\end{equation}

\begin{algorithm}[H]
\caption{Training of Blended Rectified Flow with B-Spline Interpolation and Neural Gating}
\label{alg:bspline-bprf}
\begin{algorithmic}[1]
\State \textbf{Inputs:} dataset $\mathcal{D}=\{(x_0, c)\}$, velocity model $v_\Theta$, gate network $g_\psi$
\State \textbf{Hyperparameters:} $\lambda_1,\lambda_2$ (B-spline control parameters), $\eta,\kappa>0$ (blending schedule)
\vspace{3pt}

\While{not converged}
    \State Sample $(x_0, c) \sim \mathcal{D}$, $\varepsilon \sim \mathcal{N}(0,I)$, $t \sim \mathrm{Uniform}(0,1)$
    \State Define control points:
    \[
    C_0 = x_0,\;
    C_1 = x_0 + \lambda_1 (\varepsilon - x_0),\;
    C_2 = x_0 + \lambda_2 (\varepsilon - x_0),\;
    C_3 = \varepsilon
    \]
    \State Compute cubic B-spline path and derivative:
    \[
    z_t^{\mathrm{bspline}} = \sum_{i=0}^{3} C_i B_{i,3}(t), \quad
    \dot z_t^{\mathrm{bspline}} = \sum_{i=0}^{3} C_i B'_{i,3}(t)
    \]
    \State $z_t^{\mathrm{lin}} \gets (1-t)x_0 + t\varepsilon$, \quad $\dot z_t^{\mathrm{lin}} \gets \varepsilon - x_0$
    \State Compute gating weight:
    \[
    w_\psi = t(1-t)\,\sigma\big(g_\psi(h(x_0,\varepsilon,c),t)\big)
    \]
    \State Blended sample:
    \[
    z_t = (1-w_\psi)\,z_t^{\mathrm{lin}} + w_\psi\,z_t^{\mathrm{bspline}}
    \]
    \State Deterministic velocity target:
    \[
    \rho(t) = \eta\,t(1-t)\min(1,\kappa\|\nabla^2_t z_t^{\mathrm{bspline}}\|_2), \quad
    u_t = \frac{\dot z_t^{\mathrm{lin}} + \rho(t)\dot z_t^{\mathrm{bspline}}}{1+\rho(t)}
    \]
    \State Compute CFM loss:
    \[
    \mathcal{L}_{\mathrm{CFM}} = 
    \big\|\,v_\Theta(z_t,t,c) - u_t\,\big\|_2^2
    \]
    \State Update $(\Theta,\psi)$ via gradient step.
\EndWhile
\State \textbf{Output:} trained models $(v_\Theta, g_\psi)$
\end{algorithmic}
\end{algorithm}

% --------------------------
% linear CFM loss + BSpline CFM loss
\section{Methodology: Norm-Based Adaptive Dual Conditional Flow Matching}
\label{sec:norm_dual_cfm}

Norm-Based Adaptive norm-based dual conditional flow matching (Dual-CFM) automatically balances between linear and B-spline flow matching by comparing the magnitudes of their predicted velocity fields, letting the model emphasize the path with stronger or more confident dynamics.
% We propose a \textbf{norm-based dual conditional flow matching} (Dual-CFM) objective.
We define the relative importance of the linear and B-spline interpolation paths directly from the model's own velocity magnitudes.

\subsection{Norm-Based Weighting}

At each time step $t$, we compute the instantaneous velocity norms for the two paths:
\begin{equation}
\|v_\Theta(z_t^{\mathrm{lin}}, t, c)\|, 
\qquad
\|v_\Theta(z_t^{\mathrm{bspline}}, t, c)\|.
\end{equation}
The linear-path weight is obtained by a sigmoid comparison:
\begin{equation}
w_{\mathrm{lin}}
= \sigma\!\left(
\|v_\Theta(z_t^{\mathrm{lin}}, t, c)\|
- \|v_\Theta(z_t^{\mathrm{bspline}}, t, c)\|
\right),
\label{eq:w_lin}
\end{equation}
where $\sigma(\cdot)$ denotes the sigmoid function.
The complementary weight for the B-spline path is simply
\begin{equation}
w_{\mathrm{bspline}} = 1 - w_{\mathrm{lin}}.
\label{eq:w_bspline}
\end{equation}
Intuitively, when the velocity magnitude of the linear path dominates,
$w_{\mathrm{lin}}$ increases, emphasizing the linear CFM loss; conversely,
if the B-spline path yields smoother or stronger directional updates,
the balance naturally shifts toward $\mathcal{L}_{\mathrm{bspline}}$.

\subsection{Dual Conditional Flow Matching Objective}

We define the two conditional flow matching losses as:
\begin{align}
\mathcal{L}_{\mathrm{lin}}
&= \mathbb{E}_{t,\,x_0,\,\varepsilon,\,c}
\!\left[
\big\|\,v_\Theta(z_t^{\mathrm{lin}}, t, c)
- u_t^{\mathrm{lin}}(z_t^{\mathrm{lin}}|\varepsilon)\,\big\|_2^2
\right],
\\[3pt]
\mathcal{L}_{\mathrm{bspline}}
&= \mathbb{E}_{t,\,x_0,\,\varepsilon,\,c}
\!\left[
\big\|\,v_\Theta(z_t^{\mathrm{bspline}}, t, c)
- u_t^{\mathrm{bspline}}(z_t^{\mathrm{bspline}}|\varepsilon)\,\big\|_2^2
\right],
\end{align}
where $u_t^{\mathrm{lin}} = \varepsilon - x_0$
and $u_t^{\mathrm{bspline}} = \sum_i C_i B'_{i,p}(t)$
denote the deterministic target velocities for the two paths.

The total objective adaptively blends both terms based on the norm-derived weights:
\begin{equation}
\mathcal{L}_{\mathrm{dual\text{-}CFM}}
= w_{\mathrm{lin}}\,\mathcal{L}_{\mathrm{lin}}
  + w_{\mathrm{bspline}}\,\mathcal{L}_{\mathrm{bspline}}.
\label{eq:dual_cfm_norm}
\end{equation}
This formulation eliminates auxiliary gating parameters,
allowing the balance between linear and curvature-aware flow matching
to emerge directly from the dynamics of the learned velocity field.

\begin{algorithm}[H]
\caption{Norm-Based Dual Conditional Flow Matching}
\label{alg:norm-dual-cfm}
\begin{algorithmic}[1]
\State \textbf{Inputs:} dataset $\mathcal{D}=\{(x_0, c)\}$, velocity model $v_\Theta$
\State \textbf{Hyperparameters:} $\lambda_1,\lambda_2$ (B-spline control parameters)
\vspace{3pt}

\While{not converged}
    \State Sample $(x_0,c)\!\sim\!\mathcal{D}$, $\varepsilon\!\sim\!\mathcal{N}(0,I)$, $t\!\sim\!\mathrm{Uniform}(0,1)$
    \State Construct paths:
    \[
    z_t^{\mathrm{lin}} = (1-t)x_0 + t\varepsilon, \quad
    z_t^{\mathrm{bspline}} = \sum_{i=0}^{3} C_i B_{i,3}(t)
    \]
    \State Compute deterministic targets:
    \[
    u_t^{\mathrm{lin}} = \varepsilon - x_0, \quad
    u_t^{\mathrm{bspline}} = \sum_{i=0}^{3} C_i B'_{i,3}(t)
    \]
    \State Evaluate model velocities:
    \[
    v^{\mathrm{lin}} = v_\Theta(z_t^{\mathrm{lin}},t,c), \quad
    v^{\mathrm{bspline}} = v_\Theta(z_t^{\mathrm{bspline}},t,c)
    \]
    \State Compute norm-based weights:
    \[
    w_{\mathrm{lin}} = \sigma(\|v^{\mathrm{lin}}\| - \|v^{\mathrm{bspline}}\|), \quad
    w_{\mathrm{bspline}} = 1 - w_{\mathrm{lin}}
    \]
    \State Compute CFM losses:
    \[
    \mathcal{L}_{\mathrm{lin}} = \|v^{\mathrm{lin}} - u_t^{\mathrm{lin}}\|_2^2, \quad
    \mathcal{L}_{\mathrm{bspline}} = \|v^{\mathrm{bspline}} - u_t^{\mathrm{bspline}}\|_2^2
    \]
    \State Combine adaptively:
    \[
    \mathcal{L}_{\mathrm{dual\text{-}CFM}} = 
    w_{\mathrm{lin}}\mathcal{L}_{\mathrm{lin}} + w_{\mathrm{bspline}}\mathcal{L}_{\mathrm{bspline}}
    \]
    \State Update $\Theta$ via gradient step.
\EndWhile
\State \textbf{Output:} trained model $v_\Theta$
\end{algorithmic}
\end{algorithm}

% ---------------------------
% SNR-aware dual CFM loss
\section{Methodology: SNR-Based Adaptive Dual Conditional Flow Matching}
\label{sec:snr_dual_cfm}

We introducing a Signal-to-Noise Ratio (SNR) criterion that adaptively modulates the balance between linear and B-spline flow matching.
The key idea is that the magnitude of the predicted velocity reflects the signal strength of the flow field, while curvature-induced variations or residual uncertainty represent noise.
The ratio between the two provides a principled indicator
of how confident the model is in each interpolation regime.

\subsection{SNR-Based Weighting}

For each path, we compute an instantaneous signal-to-noise ratio:
\begin{equation}
\mathrm{SNR}_{\mathrm{lin}}
= \frac{\|v_\Theta(z_t^{\mathrm{lin}}, t, c)\|_2^2}
       {\|v_\Theta(z_t^{\mathrm{lin}}, t, c) - u_t^{\mathrm{lin}}\|_2^2 + \epsilon},
\qquad
\mathrm{SNR}_{\mathrm{bspline}}
= \frac{\|v_\Theta(z_t^{\mathrm{bspline}}, t, c)\|_2^2}
       {\|v_\Theta(z_t^{\mathrm{bspline}}, t, c) - u_t^{\mathrm{bspline}}\|_2^2 + \epsilon},
\label{eq:snr_def}
\end{equation}
where $\epsilon$ is a small stabilizing constant.
A higher SNR implies that the model’s predicted velocity
is well-aligned with the target velocity—i.e., a more confident flow direction.

The relative SNRs determine adaptive weighting coefficients via a softmax normalization:
\begin{equation}
w_{\mathrm{lin}}
= \frac{\exp(\gamma\,\mathrm{SNR}_{\mathrm{lin}})}
       {\exp(\gamma\,\mathrm{SNR}_{\mathrm{lin}}) + \exp(\gamma\,\mathrm{SNR}_{\mathrm{bspline}})},
\qquad
w_{\mathrm{bspline}} = 1 - w_{\mathrm{lin}},
\label{eq:snr_weights}
\end{equation}
where $\gamma > 0$ controls the sharpness of the weighting distribution.
This design ensures that the higher-SNR path dominates training,
while maintaining smooth differentiability and adaptive balancing
throughout learning.

\subsection{Dual Conditional Flow Matching Objective}

We define the two conditional flow matching losses as:
\begin{align}
\mathcal{L}_{\mathrm{lin}}
&= \mathbb{E}_{t,\,x_0,\,\varepsilon,\,c}
\!\left[
\big\|\,v_\Theta(z_t^{\mathrm{lin}}, t, c)
- u_t^{\mathrm{lin}}(z_t^{\mathrm{lin}}|\varepsilon)\,\big\|_2^2
\right],
\\[3pt]
\mathcal{L}_{\mathrm{bspline}}
&= \mathbb{E}_{t,\,x_0,\,\varepsilon,\,c}
\!\left[
\big\|\,v_\Theta(z_t^{\mathrm{bspline}}, t, c)
- u_t^{\mathrm{bspline}}(z_t^{\mathrm{bspline}}|\varepsilon)\,\big\|_2^2
\right].
\end{align}

The SNR-weighted total objective is then defined as:
\begin{equation}
\mathcal{L}_{\mathrm{SNR\text{-}Dual\text{-}CFM}}
= w_{\mathrm{lin}}\,\mathcal{L}_{\mathrm{lin}}
  + w_{\mathrm{bspline}}\,\mathcal{L}_{\mathrm{bspline}},
\label{eq:snr_dual_cfm}
\end{equation}
where the weights $w_{\mathrm{lin}}$ and $w_{\mathrm{bspline}}$
dynamically adapt based on the relative confidence of the learned velocity field.

\begin{algorithm}[H]
\caption{SNR-Based Dual Conditional Flow Matching}
\label{alg:snr-dual-cfm}
\begin{algorithmic}[1]
\State \textbf{Inputs:} dataset $\mathcal{D}=\{(x_0, c)\}$, velocity model $v_\Theta$
\State \textbf{Hyperparameters:} $\lambda_1,\lambda_2$ (B-spline controls), $\gamma$ (temperature)
\vspace{3pt}

\While{not converged}
    \State Sample $(x_0,c)\!\sim\!\mathcal{D}$, $\varepsilon\!\sim\!\mathcal{N}(0,I)$, $t\!\sim\!\mathrm{Uniform}(0,1)$
    \State Construct paths:
    \[
    z_t^{\mathrm{lin}} = (1-t)x_0 + t\varepsilon, \quad
    z_t^{\mathrm{bspline}} = \sum_{i=0}^{3} C_i B_{i,3}(t)
    \]
    \State Compute deterministic targets:
    \[
    u_t^{\mathrm{lin}} = \varepsilon - x_0, \quad
    u_t^{\mathrm{bspline}} = \sum_{i=0}^{3} C_i B'_{i,3}(t)
    \]
    \State Evaluate model velocities:
    \[
    v^{\mathrm{lin}} = v_\Theta(z_t^{\mathrm{lin}},t,c), \quad
    v^{\mathrm{bspline}} = v_\Theta(z_t^{\mathrm{bspline}},t,c)
    \]
    \State Compute SNRs:
    \[
    \mathrm{SNR}_{\mathrm{lin}} =
    \frac{\|v^{\mathrm{lin}}\|_2^2}{\|v^{\mathrm{lin}} - u_t^{\mathrm{lin}}\|_2^2 + \epsilon}, \quad
    \mathrm{SNR}_{\mathrm{bspline}} =
    \frac{\|v^{\mathrm{bspline}}\|_2^2}{\|v^{\mathrm{bspline}} - u_t^{\mathrm{bspline}}\|_2^2 + \epsilon}
    \]
    \State Compute SNR-based weights:
    \[
    w_{\mathrm{lin}} = 
    \frac{\exp(\gamma\,\mathrm{SNR}_{\mathrm{lin}})}
         {\exp(\gamma\,\mathrm{SNR}_{\mathrm{lin}}) + \exp(\gamma\,\mathrm{SNR}_{\mathrm{bspline}})}, \quad
    w_{\mathrm{bspline}} = 1 - w_{\mathrm{lin}}
    \]
    \State Compute CFM losses:
    \[
    \mathcal{L}_{\mathrm{lin}} = \|v^{\mathrm{lin}} - u_t^{\mathrm{lin}}\|_2^2, \quad
    \mathcal{L}_{\mathrm{bspline}} = \|v^{\mathrm{bspline}} - u_t^{\mathrm{bspline}}\|_2^2
    \]
    \State Combine adaptively:
    \[
    \mathcal{L}_{\mathrm{SNR\text{-}Dual\text{-}CFM}} =
    w_{\mathrm{lin}}\mathcal{L}_{\mathrm{lin}} + w_{\mathrm{bspline}}\mathcal{L}_{\mathrm{bspline}}
    \]
    \State Update $\Theta$ via gradient step.
\EndWhile
\State \textbf{Output:} trained model $v_\Theta$
\end{algorithmic}
\end{algorithm}


% --------------------------
% z_t = z_lin+z_bspline
\section{Methodology: Norm-Based Adaptive Dual Conditional Flow Matching}
\label{sec:norm_dual_cfm}

We propose a methhod, \textbf{Norm-Based Adaptive Dual Conditional Flow Matching (Dual-CFM)}, where the latent path itself is adaptively blended before evaluating the velocity. 
We construct a unified latent trajectory
\begin{equation}
z_t = w_{\mathrm{lin}}\,z_t^{\mathrm{lin}} + w_{\mathrm{bspline}}\,z_t^{\mathrm{bspline}},
\label{eq:zt_combined}
\end{equation}
which captures a weighted combination of the linear and B-spline interpolations. 
The model then predicts a single velocity $v_\Theta(z_t, t, c)$ that is consistently used in both the linear and B-spline conditional flow matching loss terms.

\subsection{Norm-Based Weighting from Path Magnitudes}

To determine the adaptive interpolation weights, we compare the magnitudes of the latent paths rather than their predicted velocities.
At each time step $t$, the linear-path weight is computed by a sigmoid comparison:
\begin{equation}
w_{\mathrm{lin}} 
= \sigma\!\left(
\|z_t^{\mathrm{lin}}\| - \|z_t^{\mathrm{bspline}}\|
\right),
\label{eq:w_lin_z}
\end{equation}
where $\sigma(\cdot)$ denotes the sigmoid function, ensuring $w_{\mathrm{lin}}\in(0,1)$.
The complementary weight for the B-spline path is given by
\begin{equation}
w_{\mathrm{bspline}} = 1 - w_{\mathrm{lin}}.
\label{eq:w_bspline_z}
\end{equation}

This norm-based weighting scheme adaptively emphasizes the trajectory with larger geometric magnitude—intuitively corresponding to a more dynamic or higher-energy latent path—while maintaining smooth transitions between the two interpolation modes.

\subsection{Dual Conditional Flow Matching Objective}

Given the unified latent $z_t$ in Eq.~\eqref{eq:zt_combined}, we compute a single model velocity 
\[
v_t = v_\Theta(z_t, t, c),
\]
and evaluate it against both deterministic target velocities derived from the individual interpolation paths:
\begin{align}
u_t^{\mathrm{lin}} &= \varepsilon - x_0, \\
u_t^{\mathrm{bspline}} &= \sum_{i} C_i B'_{i,p}(t),
\end{align}
where $B_{i,p}(t)$ denotes the B-spline basis of degree $p$ and $C_i$ are the control points.
The two conditional flow matching losses are defined as:
\begin{align}
\mathcal{L}_{\mathrm{lin}}
&= \mathbb{E}_{t,\,x_0,\,\varepsilon,\,c}
\!\left[
\|\,v_t - u_t^{\mathrm{lin}}(z_t^{\mathrm{lin}}|\varepsilon)\,\|_2^2
\right],
\\[2pt]
\mathcal{L}_{\mathrm{bspline}}
&= \mathbb{E}_{t,\,x_0,\,\varepsilon,\,c}
\!\left[
\|\,v_t - u_t^{\mathrm{bspline}}(z_t^{\mathrm{bspline}}|\varepsilon)\,\|_2^2
\right].
\end{align}

Finally, the overall Dual-CFM objective adaptively combines both terms:
\begin{equation}
\mathcal{L}_{\mathrm{dual\text{-}CFM}}
= w_{\mathrm{lin}}\,\mathcal{L}_{\mathrm{lin}}
  + w_{\mathrm{bspline}}\,\mathcal{L}_{\mathrm{bspline}}.
\label{eq:dual_cfm_final}
\end{equation}
This formulation eliminates the need for separate velocity evaluations, producing a unified representation that captures both linear and curvature-aware dynamics through the shared latent evolution $z_t$.

\begin{algorithm}[H]
\caption{Norm-Based Adaptive Dual Conditional Flow Matching}
\label{alg:norm-dual-cfm}
\begin{algorithmic}[1]
\State \textbf{Inputs:} dataset $\mathcal{D}=\{(x_0, c)\}$, velocity model $v_\Theta$
\State \textbf{Hyperparameters:} $\lambda_1,\lambda_2$ (B-spline control parameters)
\vspace{3pt}

\While{not converged}
    \State Sample $(x_0,c)\!\sim\!\mathcal{D}$, $\varepsilon\!\sim\!\mathcal{N}(0,I)$, $t\!\sim\!\mathrm{Uniform}(0,1)$
    \State Construct interpolation paths:
    \[
    z_t^{\mathrm{lin}} = (1-t)x_0 + t\varepsilon, \quad
    z_t^{\mathrm{bspline}} = \sum_{i=0}^{3} C_i B_{i,3}(t)
    \]
    \State Compute norm-based weights:
    \[
    w_{\mathrm{lin}} = \sigma(\|z_t^{\mathrm{lin}}\| - \|z_t^{\mathrm{bspline}}\|), \quad
    w_{\mathrm{bspline}} = 1 - w_{\mathrm{lin}}
    \]
    \State Construct the unified latent:
    \[
    z_t = w_{\mathrm{lin}} z_t^{\mathrm{lin}} + w_{\mathrm{bspline}} z_t^{\mathrm{bspline}}
    \]
    \State Evaluate model velocity:
    \[
    v_t = v_\Theta(z_t, t, c)
    \]
    \State Compute target velocities:
    \[
    u_t^{\mathrm{lin}} = \varepsilon - x_0, \quad
    u_t^{\mathrm{bspline}} = \sum_{i=0}^{3} C_i B'_{i,3}(t)
    \]
    \State Compute individual losses:
    \[
    \mathcal{L}_{\mathrm{lin}} = \|v_t - u_t^{\mathrm{lin}}\|_2^2, \quad
    \mathcal{L}_{\mathrm{bspline}} = \|v_t - u_t^{\mathrm{bspline}}\|_2^2
    \]
    \State Combine adaptively:
    \[
    \mathcal{L}_{\mathrm{dual\text{-}CFM}} = 
    w_{\mathrm{lin}}\mathcal{L}_{\mathrm{lin}} + w_{\mathrm{bspline}}\mathcal{L}_{\mathrm{bspline}}
    \]
    \State Update $\Theta$ via gradient descent.
\EndWhile
\State \textbf{Output:} trained model $v_\Theta$
\end{algorithmic}
\end{algorithm}


% ---------------------------
% z_t = z_lin + z_bspline, using |u_t| for w
\section{Methodology: Norm-Based Adaptive Dual Conditional Flow Matching}
\label{sec:norm_dual_cfm}

We propose a method, \textbf{Norm-Based Adaptive Dual Conditional Flow Matching (Dual-CFM)}, where the latent trajectory is adaptively blended prior to velocity evaluation. This approach adaptively emphasizes linear or B-spline dynamics based on the instantaneous magnitudes of their respective target velocities.

\subsection{Velocity-Norm-Based Weighting}

At each time step $t$, we first compute the target velocities for the two interpolation paths:
\begin{align}
u_t^{\mathrm{lin}} &= \varepsilon - x_0, \\
u_t^{\mathrm{bspline}} &= \sum_{i} C_i B'_{i,p}(t),
\end{align}
where $B_{i,p}(t)$ is the B-spline basis of degree $p$, and $C_i$ are the control points.

The relative strength of these two paths is determined by comparing their velocity norms.  
We define the linear-path weight using a sigmoid comparison:
\begin{equation}
w_{\mathrm{lin}} 
= \sigma\!\left(
\|u_t^{\mathrm{lin}}\| - \|u_t^{\mathrm{bspline}}\|
\right),
\label{eq:w_lin_u}
\end{equation}
where $\sigma(\cdot)$ is the sigmoid function that ensures $w_{\mathrm{lin}}\in(0,1)$.  
The complementary weight is
\begin{equation}
w_{\mathrm{bspline}} = 1 - w_{\mathrm{lin}}.
\label{eq:w_bspline_u}
\end{equation}

This velocity-norm-based weighting scheme adaptively prioritizes the interpolation path exhibiting stronger instantaneous dynamics, i.e., a larger velocity magnitude, reflecting higher flow energy or stronger transport directionality. It naturally transitions between linear and curvature-aware regimes as the relative flow strengths evolve over time.

\subsection{Unified Latent and Adaptive Loss Formulation}

Given the adaptive weights, we define a unified latent path as
\begin{equation}
z_t = w_{\mathrm{lin}}\,z_t^{\mathrm{lin}} + w_{\mathrm{bspline}}\,z_t^{\mathrm{bspline}},
\label{eq:zt_combined}
\end{equation}
where $z_t^{\mathrm{lin}} = (1-t)x_0 + t\varepsilon$ and 
$z_t^{\mathrm{bspline}} = \sum_i C_i B_{i,p}(t)$.

A single model-predicted velocity is then evaluated:
\begin{equation}
v_t = v_\Theta(z_t, t, c),
\end{equation}
which is shared by both conditional flow matching loss terms.

The two conditional flow matching losses are defined as:
\begin{align}
\mathcal{L}_{\mathrm{lin}}
&= \mathbb{E}_{t,\,x_0,\,\varepsilon,\,c}
\!\left[
\|\,v_t - u_t^{\mathrm{lin}}\,\|_2^2
\right],
\\[3pt]
\mathcal{L}_{\mathrm{bspline}}
&= \mathbb{E}_{t,\,x_0,\,\varepsilon,\,c}
\!\left[
\|\,v_t - u_t^{\mathrm{bspline}}\,\|_2^2
\right].
\end{align}

Finally, the overall Dual-CFM objective adaptively merges both losses according to the velocity-based weights:
\begin{equation}
\mathcal{L}_{\mathrm{dual\text{-}CFM}}
= w_{\mathrm{lin}}\,\mathcal{L}_{\mathrm{lin}}
  + w_{\mathrm{bspline}}\,\mathcal{L}_{\mathrm{bspline}}.
\label{eq:dual_cfm_final}
\end{equation}

This formulation eliminates the need for separate velocity evaluations while dynamically adapting to the instantaneous energy of each flow mode, producing a unified representation that fuses linear and curvature-aware dynamics in a norm-consistent manner.

\begin{algorithm}[H]
\caption{Velocity-Norm-Based Adaptive Dual Conditional Flow Matching}
\label{alg:velocity-norm-dual-cfm}
\begin{algorithmic}[1]
\State \textbf{Inputs:} dataset $\mathcal{D}=\{(x_0, c)\}$, model $v_\Theta$
\State \textbf{Hyperparameters:} B-spline control parameters $\{C_i\}$
\vspace{3pt}

\While{not converged}
    \State Sample $(x_0,c)\!\sim\!\mathcal{D}$, $\varepsilon\!\sim\!\mathcal{N}(0,I)$, $t\!\sim\!\mathrm{Uniform}(0,1)$
    \State Construct interpolation paths:
    \[
    z_t^{\mathrm{lin}} = (1-t)x_0 + t\varepsilon, \quad
    z_t^{\mathrm{bspline}} = \sum_{i=0}^{3} C_i B_{i,3}(t)
    \]
    \State Compute target velocities:
    \[
    u_t^{\mathrm{lin}} = \varepsilon - x_0, \quad
    u_t^{\mathrm{bspline}} = \sum_{i=0}^{3} C_i B'_{i,3}(t)
    \]
    \State Compute velocity-norm-based weights:
    \[
    w_{\mathrm{lin}} = \sigma(\|u_t^{\mathrm{lin}}\| - \|u_t^{\mathrm{bspline}}\|), \quad
    w_{\mathrm{bspline}} = 1 - w_{\mathrm{lin}}
    \]
    \State Construct unified latent:
    \[
    z_t = w_{\mathrm{lin}} z_t^{\mathrm{lin}} + w_{\mathrm{bspline}} z_t^{\mathrm{bspline}}
    \]
    \State Evaluate model velocity:
    \[
    v_t = v_\Theta(z_t, t, c)
    \]
    \State Compute individual losses:
    \[
    \mathcal{L}_{\mathrm{lin}} = \|v_t - u_t^{\mathrm{lin}}\|_2^2, \quad
    \mathcal{L}_{\mathrm{bspline}} = \|v_t - u_t^{\mathrm{bspline}}\|_2^2
    \]
    \State Combine adaptively:
    \[
    \mathcal{L}_{\mathrm{dual\text{-}CFM}} =
    w_{\mathrm{lin}}\mathcal{L}_{\mathrm{lin}} + 
    w_{\mathrm{bspline}}\mathcal{L}_{\mathrm{bspline}}
    \]
    \State Update $\Theta$ via gradient descent.
\EndWhile
\State \textbf{Output:} trained model $v_\Theta$
\end{algorithmic}
\end{algorithm}


% ---------------------------
% z_t = z_lin + z_bspline, using |v_t - u_t| for w
\section{Methodology: Residual-Norm Adaptive Dual Conditional Flow Matching}
\label{sec:residual_dual_cfm}

We propose a method, \textbf{Residual-Norm Adaptive Dual Conditional Flow Matching (Dual-CFM)}, which adaptively blends linear and B-spline flow dynamics by measuring their alignment with the model-predicted velocity. 
Instead of comparing raw velocity magnitudes, we compute weights based on the residual norms between the predicted and target velocities, allowing the model to emphasize the interpolation path that is better aligned with its current flow estimate.

\subsection{Residual-Norm-Based Weighting}

At each time step $t$, we compute the deterministic target velocities for both paths:
\begin{align}
u_t^{\mathrm{lin}} &= \varepsilon - x_0, \\
u_t^{\mathrm{bspline}} &= \sum_{i} C_i B'_{i,p}(t),
\end{align}
where $B_{i,p}(t)$ denotes the B-spline basis of degree $p$, and $C_i$ are the control points.

Given the model-predicted velocity $v_t = v_\Theta(z_t, t, c)$, 
we define the linear-path weight using a sigmoid function over the difference of residual norms:
\begin{equation}
w_{\mathrm{lin}}
= \sigma\!\left(
\|v_t - u_t^{\mathrm{lin}}\|
-
\|v_t - u_t^{\mathrm{bspline}}\|
\right),
\label{eq:w_lin_residual}
\end{equation}
where $\sigma(\cdot)$ ensures $w_{\mathrm{lin}}\in(0,1)$.  
The complementary weight is
\begin{equation}
w_{\mathrm{bspline}} = 1 - w_{\mathrm{lin}}.
\label{eq:w_bspline_residual}
\end{equation}

This residual-norm-based scheme adaptively prioritizes the interpolation path whose target velocity better matches the model's instantaneous dynamics. 
When the model-predicted velocity $v_t$ aligns more closely with the linear target, $\|v_t - u_t^{\mathrm{lin}}\|$ becomes smaller and $w_{\mathrm{lin}}$ increases, steering the flow toward the linear regime. 
Conversely, stronger agreement with the curvature-aware target increases $w_{\mathrm{bspline}}$, promoting nonlinear transport behavior.

\subsection{Unified Latent Trajectory and Adaptive Objective}

Using the adaptive weights from Eq.~\eqref{eq:w_lin_residual}, we construct a unified latent trajectory:
\begin{equation}
z_t = w_{\mathrm{lin}}\,z_t^{\mathrm{lin}} + w_{\mathrm{bspline}}\,z_t^{\mathrm{bspline}},
\label{eq:zt_residual_combined}
\end{equation}
where $z_t^{\mathrm{lin}} = (1-t)x_0 + t\varepsilon$ and 
$z_t^{\mathrm{bspline}} = \sum_i C_i B_{i,p}(t)$.

The predicted velocity $v_t = v_\Theta(z_t, t, c)$ is then reused across both conditional flow matching losses:
\begin{align}
\mathcal{L}_{\mathrm{lin}}
&= \mathbb{E}_{t,\,x_0,\,\varepsilon,\,c}
\!\left[
\|v_t - u_t^{\mathrm{lin}}\|_2^2
\right],\\[2pt]
\mathcal{L}_{\mathrm{bspline}}
&= \mathbb{E}_{t,\,x_0,\,\varepsilon,\,c}
\!\left[
\|v_t - u_t^{\mathrm{bspline}}\|_2^2
\right].
\end{align}

Finally, the overall objective adaptively merges the two losses based on the residual-norm-derived weights:
\begin{equation}
\mathcal{L}_{\mathrm{dual\text{-}CFM}}
= w_{\mathrm{lin}}\,\mathcal{L}_{\mathrm{lin}}
  + w_{\mathrm{bspline}}\,\mathcal{L}_{\mathrm{bspline}}.
\label{eq:dual_cfm_residual_final}
\end{equation}

This formulation eliminates the need for separate velocity evaluations while dynamically selecting the most consistent flow direction relative to the model’s current state, ensuring stable and geometry-aware blending between linear and B-spline regimes.

\begin{algorithm}[H]
\caption{Residual-Norm Adaptive Dual Conditional Flow Matching}
\label{alg:residual-norm-dual-cfm}
\begin{algorithmic}[1]
\State \textbf{Inputs:} dataset $\mathcal{D}=\{(x_0, c)\}$, velocity model $v_\Theta$
\State \textbf{Hyperparameters:} control points $\{C_i\}$ for B-spline basis
\vspace{3pt}

\While{not converged}
    \State Sample $(x_0,c)\!\sim\!\mathcal{D}$, $\varepsilon\!\sim\!\mathcal{N}(0,I)$, $t\!\sim\!\mathrm{Uniform}(0,1)$
    \State Construct interpolation paths:
    \[
    z_t^{\mathrm{lin}} = (1-t)x_0 + t\varepsilon, \quad
    z_t^{\mathrm{bspline}} = \sum_{i=0}^{3} C_i B_{i,3}(t)
    \]
    \State Evaluate model velocity:
    \[
    z_t = w_{\mathrm{lin}} z_t^{\mathrm{lin}} + w_{\mathrm{bspline}} z_t^{\mathrm{bspline}}, \quad
    v_t = v_\Theta(z_t, t, c)
    \]
    \State Compute target velocities:
    \[
    u_t^{\mathrm{lin}} = \varepsilon - x_0, \quad
    u_t^{\mathrm{bspline}} = \sum_{i=0}^{3} C_i B'_{i,3}(t)
    \]
    \State Compute residual-norm-based weights:
    \[
    w_{\mathrm{lin}} = \sigma(\|v_t - u_t^{\mathrm{lin}}\| - \|v_t - u_t^{\mathrm{bspline}}\|), \quad
    w_{\mathrm{bspline}} = 1 - w_{\mathrm{lin}}
    \]
    \State Reconstruct unified latent:
    \[
    z_t = w_{\mathrm{lin}} z_t^{\mathrm{lin}} + w_{\mathrm{bspline}} z_t^{\mathrm{bspline}}
    \]
    \State Compute individual losses:
    \[
    \mathcal{L}_{\mathrm{lin}} = \|v_t - u_t^{\mathrm{lin}}\|_2^2, \quad
    \mathcal{L}_{\mathrm{bspline}} = \|v_t - u_t^{\mathrm{bspline}}\|_2^2
    \]
    \State Combine adaptively:
    \[
    \mathcal{L}_{\mathrm{dual\text{-}CFM}} =
    w_{\mathrm{lin}}\mathcal{L}_{\mathrm{lin}} + 
    w_{\mathrm{bspline}}\mathcal{L}_{\mathrm{bspline}}
    \]
    \State Update $\Theta$ via gradient descent.
\EndWhile
\State \textbf{Output:} trained model $v_\Theta$
\end{algorithmic}
\end{algorithm}



% ---------------------------
% GA for flow
% \section{Problem Statement: Genetic-Algorithm Training of Discrete Flow Trajectories}

% \paragraph{Setup.}
% Let $E:\mathbb{R}^{H\times W\times 3}\!\to\!\mathbb{R}^{h\times w\times d}$ and $D:\mathbb{R}^{h\times w\times d}\!\to\!\mathbb{R}^{H\times W\times 3}$ denote the encoder and decoder of a latent autoencoder.
% We work in latent space $z\in\mathbb{R}^{h\times w\times d}$.
% Given data $x_0\sim p_{\text{data}}$ and noise $\varepsilon\sim\mathcal{N}(0,I)$, the (rectified) forward path is
% \begin{equation}
%     z_t \;=\; (1-t)\,E(x_0) + t\,\varepsilon,\qquad t\in[0,1].
% \end{equation}
% Classical rectified flows learn a velocity $v_\Theta(z,t)$ via (conditional) flow matching; here we \emph{replace} that learning target with a black-box, evolutionary optimization that searches for a sequence of \emph{discrete mutations} that transports $z_{t}$ toward $z_{t-\Delta t}$ and ultimately reconstructs $x_0$ at $t=0$.

% \paragraph{Goal.}
% For each training pair $(x_0,\varepsilon)$ and a discretization $\mathcal{T}=\{t_K{=}1>t_{K-1}>\!\cdots\!>t_0{=}0\}$, we seek a sequence of mutations
% \[
% \mathcal{M}\;=\;\big\{M_k(\cdot,t_k;\phi_k)\big\}_{k=1}^{K},
% \quad M_k:\mathbb{R}^{h\times w\times d}\!\to\!\mathbb{R}^{h\times w\times d},
% \]
% parameterized by low-dimensional \emph{genes} $\phi_k\in\mathbb{R}^m$,
% such that the iterates
% \begin{equation}
%     \tilde z_{t_{k-1}}
%     \;=\;
%     \tilde z_{t_k} \;+\; \Delta t_k\,M_k\!\big(\tilde z_{t_k},\,t_k;\,\phi_k\big),
%     \qquad \tilde z_{t_K}=z_{t_K}=(1)\cdot \varepsilon,
% \end{equation}
% satisfy $D(\tilde z_{t_0})\approx x_0$.
% Intuitively, each $M_k$ is a discrete-time, mutation-style \emph{flow step}.

% \paragraph{Fitness.}
% Define a differentiable image-domain similarity $\mathcal{S}(\hat x,x_0)$ (e.g., negative $\ell_2$, MSSSIM, LPIPS, or mixtures) and an optional latent penalty $\Omega(\{\phi_k\})$ (e.g., smoothness or energy budget). The GA fitness to \emph{maximize} is
% \begin{equation}
%     \mathcal{F}(\{\phi_k\})
%     \;=\;
%     \mathcal{S}\!\Big(D(\tilde z_{t_0}),\,x_0\Big) \;-\; \lambda\,\Omega\!\big(\{\phi_k\}\big).
% \end{equation}

% \subsection{Genetic Algorithm (GA) Formulation}

% \paragraph{Chromosome.}
% An \emph{individual} (chromosome) encodes the full control sequence
% $\Phi \!=\! (\phi_1,\ldots,\phi_K)\in\mathbb{R}^{mK}$.
% To make search tractable, parameterize the time-varying mutation field in a low-dimensional basis:
% \begin{equation}
%     M_k(\cdot,t_k;\phi_k)
%     \;\equiv\;
%     \sum_{j=1}^{m} \phi_{k,j}\,B_j(\cdot, t_k),
% \end{equation}
% where $\{B_j\}$ are fixed mutation bases (e.g., learned or random low-rank filters in latent space, multi-scale wavelets, or Fourier modes).
% This reduces GA dimensionality while retaining expressive transport.

% \paragraph{Population Dynamics.}
% Initialize a population $\{\Phi^{(i)}\}_{i=1}^P$ (e.g., near zero controls).
% For each generation $g=1,\dots,G$:
% \begin{enumerate}
%     \item \textbf{Evaluation.} For each $\Phi^{(i)}$, roll out the discrete transport from $t_K$ to $t_0$ using the recurrence above and compute $\mathcal{F}(\Phi^{(i)})$.
%     \item \textbf{Selection.} Choose parents via tournament or fitness-proportional sampling.
%     \item \textbf{Variation.} Produce offspring via
%     \begin{align}
%         \text{Crossover:}\quad &\Phi^{\text{child}} \leftarrow \alpha\,\Phi^{(p_1)} + (1{-}\alpha)\,\Phi^{(p_2)},\; \alpha\!\sim\!\text{Unif}[0,1],\\
%         \text{Mutation:}\quad &\Phi^{\text{child}} \leftarrow \Phi^{\text{child}} + \sigma\,\xi,\;\;\xi\!\sim\!\mathcal{N}(0,I).
%     \end{align}
%     \item \textbf{Elitism.} Preserve top-$e$ solutions to ensure monotone best-of-generation fitness.
% \end{enumerate}

% \subsection{Two Practical Solutions}

% \paragraph{(A) Direct GA Sampler (Training-Free).}
% Use the GA online at inference for a given $(x_0,\varepsilon)$:
% the best chromosome $\Phi^\star$ yields a transport policy $\{M_k^\star\}$ that deterministically maps $z_{t_K}=\varepsilon$ to $\tilde z_{t_0}$ with $D(\tilde z_{t_0})\!\approx\!x_0$.
% This replaces trained $v_\Theta$ with a search-based controller.
% It is compute-heavy but can be parallelized over the population and timesteps.

% \paragraph{(B) GA-to-Flow Distillation (Offline Teacher $\to$ Student).}
% Use GA \emph{offline} to produce pseudo-target \emph{velocities} for many $(x_0,\varepsilon)$ and times:
% \begin{equation}
%     u^*_{t_k}\big(\tilde z_{t_k}\big) \;\triangleq\; M_k^\star\!\big(\tilde z_{t_k}, t_k; \phi_k^\star\big).
% \end{equation}
% Then train a parametric velocity $v_\Theta$ by supervised regression on these teacher signals:
% \begin{equation}
%     \min_{\Theta}\;
%     \sum_{(x_0,\varepsilon)}\;\sum_{k=1}^{K}
%     \left\|v_\Theta\!\big(\tilde z_{t_k},t_k\big) - u^*_{t_k}\!\big(\tilde z_{t_k}\big)\right\|_2^2.
% \end{equation}
% At test time, discard GA and sample with the learned $v_\Theta$ as in rectified flows (ODE integration or few-step Euler), recovering efficient inference while retaining GA’s search benefits.

% \subsection{Design of the Fitness and Regularizers}

% \paragraph{Image-Space Targets.}
% Typical choices are
% $\mathcal{S}(\hat x,x_0) = -\| \hat x-x_0\|_2^2$,
% or multi-term scores
% $\mathcal{S}=\alpha_1\!\cdot\!\text{PSNR} + \alpha_2\!\cdot\!\text{SSIM} - \alpha_3\!\cdot\!\text{LPIPS}$.
% For conditional generation (e.g., text), include guidance in the rollout but keep fitness anchored to reconstruction of $x_0$.

% \paragraph{Stability/Complexity Control.}
% Penalize excessive transport:
% \begin{equation}
%     \Omega(\{\phi_k\})
%     =
%     \beta_1 \sum_{k}\|\phi_k\|_2^2
%     \;+\;
%     \beta_2 \sum_{k}\|\phi_k-\phi_{k-1}\|_2^2,
% \end{equation}
% encouraging small, smooth mutations (short path length), which is known to aid few-step sampling in rectified flows.

% \subsection{Computational Strategy and Hybrids}

% \paragraph{Low-Rank / Multi-Scale Bases.}
% Choose $\{B_j\}$ as low-rank latent filters (rank-$r$ factorizations), or multi-scale wavelet/Fourier atoms, drastically shrinking $m$.

% \paragraph{Curriculum over $t$.}
% Evolve controls on short horizons (e.g., $t\!\in\![\tau,1]$) and progressively extend toward $t{=}0$; reuse elites as warm starts.

% \paragraph{Memetic Refinement.}
% Although GA is gradient-free, we can apply a local, differentiable \emph{Lamarckian} step on each offspring by one or two gradient updates in latent space (via $\partial D/\partial z$) before fitness evaluation, then write back the improved chromosome. This accelerates convergence without requiring end-to-end backprop through the entire trajectory.

% \subsection{Theoretical Notes (Sketch)}
% Let $\tilde z_{t_{k-1}}=\tilde z_{t_k}+\Delta t_k\,M_k^\star(\tilde z_{t_k},t_k)$ be the best-evolved step.
% If $\max_k\|M_k^\star(\cdot,t_k)-u^\star(\cdot,t_k)\|\le \epsilon$ for a target continuous field $u^\star$, then (by standard ODE discretization stability) the terminal error satisfies
% \[
% \|\tilde z_{t_0}-z^\star_{t_0}\|\;\le\; C\big(\Delta t_{\max} + \epsilon\big),
% \]
% for some $C$ depending on a Lipschitz bound of $u^\star$.
% Hence, accurate GA approximations of stepwise velocities yield bounded terminal reconstruction error; distillation inherits these bounds up to regression error.

% \subsection{Algorithm (GA $\to$ Flow Distillation)}
% \begin{algorithm}[H]
% \caption{Evolve mutations, then distill to $v_\Theta$}
% \begin{algorithmic}[1]
% \State \textbf{Input:} dataset $\mathcal{D}=\{x_0\}$, encoder/decoder $(E,D)$, discretization $\{t_k\}_{k=0}^K$
% \For{each training example $x_0$}
%   \State Sample $\varepsilon\sim\mathcal{N}(0,I)$, set $z_{t_K}=\varepsilon$, form forward path $z_t$
%   \State Initialize population $\{\Phi^{(i)}\}_{i=1}^P$; set elites $\mathcal{E}\leftarrow\emptyset$
%   \For{generation $g=1{:}G$}
%     \For{each individual $\Phi^{(i)}$}
%       \State Roll out $\{\tilde z_{t_k}\}_{k=K}^{0}$ using $\Phi^{(i)}$; compute $\mathcal{F}(\Phi^{(i)})$
%       \State Optional: one-step memetic refinement of $\Phi^{(i)}$
%     \EndFor
%     \State $\mathcal{E}\leftarrow$ top-$e$ individuals; produce offspring via selection, crossover, mutation
%   \EndFor
%   \State Let $\Phi^\star\in\mathcal{E}$ be best; define $u^*_{t_k}(\tilde z_{t_k}) \gets M_k^\star(\tilde z_{t_k},t_k)$
%   \State Accumulate pairs $\big(\tilde z_{t_k},t_k, u^*_{t_k}(\tilde z_{t_k})\big)$ into a replay buffer
% \EndFor
% \State Train $v_\Theta$ by minimizing $\sum\|v_\Theta(\tilde z_{t_k},t_k)-u^*_{t_k}(\tilde z_{t_k})\|_2^2$
% \State \textbf{return} $v_\Theta$ (efficient sampler without GA at test time)
% \end{algorithmic}
% \end{algorithm}

% ----------------------------
% Robustness to sample scale problem
% \section{Problem Statement: Robustness of Evaluation Metrics to Testing Sample Scale}
% \label{sec:robustness_testing_scale}

% In image generation evaluation, quantitative metrics such as Fréchet Inception Distance (FID), Inception Score (IS), and CLIPScore are commonly computed between two sets of images: a generated set $\mathcal{G}$ and a real reference set $\mathcal{R}$. 
% Let $|\mathcal{R}| = N_{\text{real}}$ denote the total number of real images, and $|\mathcal{G}| = N_{\text{gen}}$ denote the number of generated images used for evaluation. 
% Ideally, $\mathcal{G}$ should approximate $\mathcal{R}$ in both diversity and fidelity, such that the estimated metric reflects the true generative quality. 

% However, in practice, evaluations are often performed with \emph{subsampled} sets of generated images, where only a proportion $p \in (0, 1]$ of $\mathcal{G}$ is compared against the full real set $\mathcal{R}$. 
% That is,
% \begin{equation}
% \mathcal{G}_p \subseteq \mathcal{G}, \quad |\mathcal{G}_p| = p \cdot N_{\text{gen}}.
% \end{equation}
% Empirically, we observe that the evaluation results vary substantially with different $p$, as shown in Table~\ref{tab:scale_variance}.

% \begin{table}[h]
% \centering
% \caption{Variance of metrics across different proportions $p$ of generated samples.}
% \begin{tabular}{c|c|c|c|c}
% \hline
% Proportion $p$ & Sample Size & FID $\downarrow$ & IS $\uparrow$ & CLIPScore $\uparrow$ \\
% \hline
% 0.1 & 100 & 189.67 & 5.70 & 34.64 \\
% 0.3 & 300 & 119.64 & 11.57 & 34.54 \\
% 0.5 & 500 & 91.14 & 14.27 & 34.62 \\
% 0.7 & 700 & 77.01 & 16.76 & 34.53 \\
% 0.9 & 900 & 69.45 & 18.21 & 34.66 \\
% 1.0 & 1000 & 65.92 & 19.02 & 34.68 \\
% \hline
% \end{tabular}
% \label{tab:scale_variance}
% \end{table}

% The significant discrepancies across scales reveal that evaluation metrics are sensitive to the number of generated samples used for testing. 
% This raises an open question of \textbf{robustness under sample scaling}:
% \begin{quote}
% \textit{To what extent do standard generative evaluation metrics (e.g., FID, IS, CLIPScore) remain consistent when the number of generated samples varies, and how can we design evaluation protocols that are robust to such scale-dependent variance?}
% \end{quote}

% Formally, let $M(\mathcal{G}_p, \mathcal{R})$ denote the metric value computed at proportion $p$. 
% We define the robustness of the metric as the stability of $M(\mathcal{G}_p, \mathcal{R})$ across $p$, quantified by its variance:
% \begin{equation}
% \mathrm{Var}_p[M(\mathcal{G}_p, \mathcal{R})] = \mathbb{E}_p\big[(M(\mathcal{G}_p, \mathcal{R}) - \mathbb{E}_p[M(\mathcal{G}_p, \mathcal{R})])^2\big].
% \end{equation}
% A metric is considered \emph{robust to sample scale} if $\mathrm{Var}_p[M(\mathcal{G}_p, \mathcal{R})]$ is small for all reasonable $p \in (0,1]$. 

% The goal of this study is to systematically quantify and mitigate this variance, thereby establishing \textbf{scale-robust evaluation metrics} for image generation tasks.


% --------------------------
% Flow-as-Optimizer
\section{Problem Statement: Training-Free Flow-as-Optimizer Sampling with Per-Trajectory Moments}

Let $p_0$ denote the data distribution and $p_1=\mathcal{N}(0,I)$ the noise prior.
Generative flow models define a probability path $(p_t)_{t\in[0,1]}$ and an ODE
\begin{equation}
\frac{d z_t}{dt} \;=\; v_\Theta(z_t, t, c),
\quad z_1 \sim p_1,\;\; z_0 \sim p_0,
\label{eq:flow_ode}
\end{equation}
where $v_\Theta$ is a learned velocity field and $c$ is (optional) conditioning.
In \emph{rectified flows} (RF), a straight-line forward path
$z_t=(1-t)x_0+t\varepsilon$ motivates efficient training via Conditional Flow Matching and
sampling via the ODE in \eqref{eq:flow_ode}. We build on this formulation and its SNR/timestep
parameterizations to design a \emph{training-free} sampler that treats $v_\Theta$ as an
\emph{optimizer direction} and augments it with \textbf{per-trajectory} first and second moments
to accelerate convergence in the \emph{sampling} phase while preserving the learned dynamics
of $v_\Theta$.\,\footnote{Background on ODE view, RF straight path $z_t=(1-t)x_0+t\varepsilon$, and SNR-weighted training/scheduling can be found in recent RF literature. We follow these definitions for notation and scheduling.} \,\textit{(cf. rectified-flow ODE and straight-path formulation)}~:contentReference[oaicite:0]{index=0}

\paragraph{Goal.}
Given a trained $v_\Theta$, design a sampler that:
(i) increases sample fidelity at a fixed (or reduced) step budget,
(ii) improves stability and \emph{effective} step size in stiff regions,
and (iii) remains \emph{training-free} and \emph{per-trajectory}, i.e., momentum statistics are maintained \emph{independently for each sample path}.

\section{Methodology: Flow-as-Optimizer (FAO) for Sampling}

\subsection{From ODE Integration to Optimizer-Guided Transport}
Classical explicit integrators (e.g., forward Euler) advance
$z_{k+1}=z_k - \eta_k \,\tilde{v}_k$ where $\tilde{v}_k=-v_\Theta(z_k,t_k,c)$ and $t_{k+1}=t_k-\Delta_k$.
We reinterpret $-\tilde{v}_k$ as a \emph{descent direction} on an implicit energy landscape whose stationary points match flow-consistent states along \eqref{eq:flow_ode}.
This view suggests reusing well-understood optimizer mechanics to (a) smooth noisy directions,
(b) adapt the per-coordinate step size, and (c) trust regions with large curvature.

\subsection{Per-Trajectory Adam-like Moments}
For each trajectory (i.e., for each generated sample), we maintain \emph{independent} first/second moments:
\begin{align}
m_{k} &= \beta_1(t_k)\, m_{k-1} + \bigl(1-\beta_1(t_k)\bigr)\,\tilde{v}_k, \\
s_{k} &= \beta_2(t_k)\, s_{k-1} + \bigl(1-\beta_2(t_k)\bigr)\,\tilde{v}_k^{\odot 2}, \\
\hat{m}_{k} &= \frac{m_k}{1-\prod_{j=1}^k \beta_1(t_j)}, \qquad
\hat{s}_{k} = \frac{s_k}{1-\prod_{j=1}^k \beta_2(t_j)},
\end{align}
where $\odot 2$ denotes elementwise square.
We then advance
\begin{equation}
z_{k+1} \;=\; z_k \;-\; \eta_k \;\frac{\hat{m}_k}{\sqrt{\hat{s}_k} + \epsilon}.
\label{eq:fao_update}
\end{equation}
All statistics are reset per trajectory at $k=0$ so that coupling does not occur across different samples.

\subsection{SNR- and Time-Aware Schedules}
Let $\lambda(t)$ denote the (log-)SNR schedule associated with the forward path used for training (e.g., for RF and cosine schedules).
We modulate the optimizer hyperparameters by time/SNR to respect the dynamics learned by $v_\Theta$:
\begin{align}
\eta_k &= \alpha \,\Delta_k \, \sigma_\eta(t_k), 
& \sigma_\eta(t) &= \frac{1}{1 + e^{-(a_0 + a_1\lambda(t))}}, \\
\beta_1(t) &= \beta_{1,\min} + (\beta_{1,\max}-\beta_{1,\min})\,\rho(t), \\
\beta_2(t) &= \beta_{2,\min} + (\beta_{2,\max}-\beta_{2,\min})\,\rho(t),
\end{align}
with a monotone schedule $\rho(t)$ increasing towards high-noise endpoints if desired.
Intuition: early steps (large noise, small signal) benefit from stronger smoothing (larger $\beta_1,\beta_2$) and conservative $\eta_k$; mid-range SNR can exploit larger \emph{effective} steps as $v_\Theta$ is informative; near $t\!\to\!0$ we reduce $\eta_k$ to prevent overshooting.

% \paragraph{Corrector step (optional).}
% To preserve faithfulness to \eqref{eq:flow_ode}, add a small explicit Euler ``corrector''
% \(
% z_{k+1}\leftarrow z_{k+1}-\gamma_k\, v_\Theta(z_{k+1},t_{k+1},c)
% \)
% with $\gamma_k \ll \eta_k$. This acts like a predictor--corrector that recenters the trajectory on the learned vector field.

\paragraph{Stability and clipping.}
We use per-trajectory norm clipping on $\hat{m}_k / (\sqrt{\hat{s}_k}+\epsilon)$:
\[
u_k = \mathrm{clip}\!\left(\frac{\hat{m}_k}{\sqrt{\hat{s}_k}+\epsilon}, \tau\right),\quad
z_{k+1}=z_k - \eta_k\,u_k,
\]
which attenuates rare spikes from $v_\Theta$ without retraining.

\subsection{Why It Works (Sampling-Time View)}
\begin{itemize}
\item \textbf{Variance reduction.} EMA ($\beta_1$) lowers stochastic directional variance from $v_\Theta$ across nearby time levels.
\item \textbf{Adaptive step sizes.} $\hat{s}_k$ rescales coordinates with high curvature or unreliable magnitude, enabling aggressive steps where safe.
\item \textbf{Time/SNR awareness.} Coupling to $\lambda(t)$ aligns step aggressiveness with regions where the ODE is stiff vs.\ smooth, reducing solver steps for the same fidelity.
\end{itemize}

\section{Pseudo-Algorithms}

\subsection{Algorithm 1: FAO Sampler (Training-Free, Per-Trajectory Adam Moments)}
\begin{algorithm}[H]
\renewcommand{\thealgorithm}{1}
\caption{FAO-RectifiedFlow Sampler (training-free)}
\begin{algorithmic}[1]
\Require Trained $v_\Theta$, conditioning $c$, step count $K$, schedule $\{t_k\}_{k=0}^K$ with $t_0=1>t_1>\dots>t_K=0$, base step sizes $\{\Delta_k\}$, hyperparams $\alpha,\epsilon,\tau$, time/SNR maps $\sigma_\eta(t),\beta_1(t),\beta_2(t)$.
\State Sample $z_0 \sim \mathcal{N}(0,I)$ \Comment{initialize trajectory at $t_0=1$}
\State $m_0 \gets 0$, $s_0 \gets 0$
\For{$k=0$ to $K-1$}
  \State $\tilde{v}_k \gets -\,v_\Theta(z_k, t_k, c)$
  \State $m_{k+1} \gets \beta_1(t_k)\, m_k + \bigl(1-\beta_1(t_k)\bigr)\,\tilde{v}_k$
  \State $s_{k+1} \gets \beta_2(t_k)\, s_k + \bigl(1-\beta_2(t_k)\bigr)\,\tilde{v}_k^{\odot 2}$
  \State $\hat{m}_{k+1} \gets m_{k+1}/\!\bigl(1-\prod_{j=0}^{k}\beta_1(t_j)\bigr)$; \quad
         $\hat{s}_{k+1} \gets s_{k+1}/\!\bigl(1-\prod_{j=0}^{k}\beta_2(t_j)\bigr)$
  \State $u \gets \hat{m}_{k+1}/\bigl(\sqrt{\hat{s}_{k+1}}+\epsilon\bigr)$; \quad
         $u \gets \mathrm{clip}(u, \tau)$
  \State $\eta_k \gets \alpha\,\Delta_k\,\sigma_\eta(t_k)$
  \State $z_{k+1} \gets z_k - \eta_k\, u$ \Comment{FAO predictor}
  % \State \textbf{(optional)} $z_{k+1} \gets z_{k+1} - \gamma_k\, v_\Theta(z_{k+1}, t_{k+1}, c)$ \Comment{ODE corrector}
\EndFor
\State \Return $z_K$ \Comment{decode if using a latent autoencoder}
\end{algorithmic}
\end{algorithm}

\subsection{Algorithm 2: SNR-/Schedule-Aware Step and Momentum Policies}
\begin{algorithm}[H]
\renewcommand{\thealgorithm}{2}
\caption{Time/SNR-aware hyperparameters}
\begin{algorithmic}[1]
\Require log-SNR $\lambda(t)$, bounds $\beta_{1,\min}\!\le\!\beta_{1,\max}$, $\beta_{2,\min}\!\le\!\beta_{2,\max}$, logistic parameters $a_0,a_1$, map $\rho(t)\!\in\![0,1]$.
\For{$k=0$ to $K-1$}
  \State $\lambda_k \gets \lambda(t_k)$
  \State $\sigma_\eta(t_k) \gets \bigl(1 + \exp(-(a_0 + a_1 \lambda_k))\bigr)^{-1}$
  \State $\beta_1(t_k) \gets \beta_{1,\min} + (\beta_{1,\max}-\beta_{1,\min})\,\rho(t_k)$
  \State $\beta_2(t_k) \gets \beta_{2,\min} + (\beta_{2,\max}-\beta_{2,\min})\,\rho(t_k)$
\EndFor
\end{algorithmic}
\end{algorithm}

\paragraph{Practical defaults.}
For $K\in\{10,\,20,\,30\}$ steps, good starting points are
$\alpha\in[0.8,1.2]$, $\epsilon=10^{-8}$, $\tau=10$--$20$ (latent units),
$\beta_{1,\min}=0.5$, $\beta_{1,\max}=0.95$,
$\beta_{2,\min}=0.9$, $\beta_{2,\max}=0.999$,
$a_0=0$, $a_1\in[0.5,1.5]$, and $\rho(t)$ increasing towards the endpoints
if the schedule concentrates mass away from the mid-range SNR.

\section{Discussion and Guarantees}

\paragraph{Consistency.}
When $\beta_1(t)\!=\!0$ and $\beta_2(t)\!=\!0$, FAO reduces to explicit Euler with
time-scaled step $\eta_k=\alpha\Delta_k$, recovering the standard ODE sampler.

\paragraph{Bias vs.\ variance.}
Bias-corrected moments $(\hat m_k,\hat s_k)$ guarantee zero-mean estimates
under stationarity of the local velocity field; in practice the local drift along $t$
is mild across adjacent $k$, so momentum reduces variance without visible bias.

\paragraph{Complexity.}
FAO introduces negligible overhead: two vector EMA buffers per trajectory and a few elementwise ops. Network calls remain the dominant cost.

\paragraph{Compatibility.}
FAO is orthogonal to guidance (e.g., CFG), second-order solvers (Heun),
and latent-space autoencoding. It can be wrapped around the predicted velocity $\tilde v_k$
after any guidance combination.

% ----------------------
% Flow-as-Optimizer, diminishing version
\section{Problem Statement: Training-Free Flow-as-Optimizer Sampling with Per-Trajectory Moments}

Let $p_0$ denote the data distribution and $p_1 = \mathcal{N}(0,I)$ the noise prior.
Rectified flow models define a continuous path of intermediate distributions $\{p_t\}_{t\in[0,1]}$
and an ODE governing the latent evolution:
\begin{equation}
\frac{dz_t}{dt} = v_\Theta(z_t, t, c),
\quad z_1 \sim p_1, \;\; z_0 \sim p_0,
\label{eq:flow_ode}
\end{equation}
where $v_\Theta$ is the learned velocity field parameterized by a neural network, and $c$ is an optional conditioning input (e.g., text embedding).

Unlike classical optimization, the velocity magnitude $\|v_\Theta(z_t,t)\|$ does not necessarily diminish near the data manifold; 
in optimization, gradients vanish near local minima, whereas in flow dynamics the vector field may remain large even at convergence.
Hence, directly applying optimizer dynamics (e.g., Adam) can distort the learned flow geometry.
We therefore introduce a \textbf{time- and SNR-aware momentum schedule} that activates per-trajectory moments in early and middle steps 
(where stochasticity and stiffness are high) and attenuates them near $t\!\to\!0$, smoothly reverting to Euler-like updates.

\paragraph{Why ODE Velocities Differ from Optimization Gradients.}
In an optimization process minimizing a scalar potential $\mathcal{L}(z)$, the dynamics follow
\begin{equation}
\frac{dz_t}{dt} = - \nabla_z \mathcal{L}(z_t),
\quad \text{so that } \| \nabla_z \mathcal{L}(z_t) \| \to 0 \text{ as } z_t \to z^*,
\end{equation}
where $z^*$ is a local minimum.
However, the flow-based dynamics in~\eqref{eq:flow_ode} do not correspond to gradient descent on an explicit scalar potential.
Instead, $v_\Theta(z_t,t)$ defines a transport field satisfying the continuity equation
\begin{equation}
\frac{\partial p_t(z)}{\partial t} + \nabla_z \!\cdot\! \big(p_t(z) \, v_\Theta(z,t)\big) = 0,
\label{eq:continuity}
\end{equation}
which enforces mass conservation but imposes no condition that $v_\Theta(z,t)$ vanishes when $p_t$ aligns with $p_0$.
Even when $p_t \approx p_0$, the divergence term $\nabla_z \!\cdot\! v_\Theta(z,t)$ may remain finite, leading to non-negligible $\|v_\Theta(z_t,t)\|$.
Consequently, the flow trajectory continues to evolve along the manifold rather than converging to a single stationary point.
If optimizer dynamics such as Adam are applied without modification, their inherent assumption of vanishing gradients near equilibrium
can introduce over-damping effects, break the geometric consistency of the transport field, and distort the probability-preserving flow path.



\section{Methodology: Time- and SNR-Aware Flow-as-Optimizer (FAO)}

We interpret the rectified flow sampling process as an optimization trajectory that seeks to minimize an implicit energy function 
whose gradients are approximated by $v_\Theta(z_t,t)$. 
At each time step $t_k$, we compute the per-trajectory adaptive moments:
\begin{align}
g_k &= v_\Theta(z_k, t_k, c), \\
m_k &= \beta_1(t_k) \, m_{k+1} + \big(1 - \beta_1(t_k)\big) \, g_k, \\
s_k &= \beta_2(t_k) \, s_{k+1} + \big(1 - \beta_2(t_k)\big) \, g_k^2.
\end{align}

The coefficients $\beta_1(t)$ and $\beta_2(t)$ control the temporal memory of the first and second moments, respectively.
To make this memory state diminish smoothly near the data manifold, we define them as bounded, monotonically increasing functions of time:
\begin{equation}
\beta_i(t) = \beta_i^{\max} \cdot \sigma\!\left(\frac{t - t_0}{\delta_i}\right),
\quad i \in \{1,2\},
\label{eq:beta_schedule}
\end{equation}
where $\sigma(x) = 1/(1+e^{-x})$ is the logistic sigmoid, $\beta_i^{\max}$ are asymptotic constants 
(e.g., $\beta_1^{\max}=0.9$, $\beta_2^{\max}=0.999$), $t_0$ sets the midpoint of activation, and $\delta_i$ controls smoothness.
For small $t$, $\sigma((t-t_0)/\delta_i)\!\approx\!0$, thus $\beta_i(t)\!\approx\!0$ and the recursions reduce to
$m_k = g_k$ and $s_k = g_k^2$, corresponding to a pure Euler update.
As $t$ increases, $\beta_i(t)$ rises toward $\beta_i^{\max}$, reintroducing exponential averaging and momentum accumulation
when the dynamics are most stochastic (mid-to-high SNR regimes).



\paragraph{Decay of Momentum Near the Data Distribution.}
To see why the momentum naturally vanishes near the data manifold ($t\!\to\!0$), 
consider the effective update direction in \eqref{eq:flow_ode}:
\begin{equation}
\tilde{v}_t = \rho(t) \, \frac{m_t}{\sqrt{s_t} + \epsilon} + \big(1 - \rho(t)\big) \, g_t.
\label{eq:vtilde}
\end{equation}
The modulation factor $\rho(t)$ is coupled to the signal-to-noise ratio (SNR):
\begin{equation}
\rho(t) = \sigma\!\big(\alpha(\mathrm{SNR}(t) - \tau)\big),
\quad \mathrm{SNR}(t) = \frac{a_t^2}{b_t^2}, \;\; \lambda_t = \log \mathrm{SNR}(t),
\label{eq:rho}
\end{equation}
where $a_t,b_t$ define the rectified flow parameterization $z_t = a_t x_0 + b_t \epsilon$.
For rectified flows, $a_t \!\to\! 1$ and $b_t \!\to\! 0$ as $t \!\to\! 0$, implying $\mathrm{SNR}(t) \!\to\! \infty$.
Because $\sigma(x)$ saturates for large positive $x$, the factor $\rho(t)$ approaches zero exponentially fast if we shift the sigmoid
so that $\tau$ corresponds to the midpoint SNR. Explicitly, choosing $\alpha<0$ yields:
\[
\lim_{t\to0} \rho(t) = \sigma\!\big(\alpha(\infty - \tau)\big) = 0,
\quad \text{and} \quad \lim_{t\to0} \beta_i(t) = 0.
\]
Thus, as $t\!\to\!0$, both $\rho(t)$ and $\beta_i(t)$ vanish, forcing the update
\begin{equation}
\tilde{v}_t \approx g_t = v_\Theta(z_t,t),
\end{equation}
which reduces to the standard Euler integration without any accumulated momentum.
Therefore, the overall momentum contribution decays continuously toward zero as the trajectory approaches $p_0$, 
guaranteeing that the flow’s terminal behavior preserves its learned geometry rather than overshooting or oscillating near the data manifold.



\section{Algorithm: Flow-as-Optimizer Sampling (Training-Free)}

\begin{algorithm}[H]
\caption{Flow-as-Optimizer (FAO) Sampling with Per-Trajectory Moments}
\label{alg:FAO}
\begin{algorithmic}[1]
\State \textbf{Input:} pretrained flow $v_\Theta$, total steps $K$, timestep schedule $\{t_k\}_{k=1}^K$, 
initial $z_K \sim \mathcal{N}(0,I)$, hyperparameters $\alpha$, $\tau$, $\beta_1(\cdot)$, $\beta_2(\cdot)$, $\rho(\cdot)$
\State Initialize $m_K = 0$, $s_K = 0$
\For{$k = K$ down to $1$}
    \State $g_k \gets v_\Theta(z_k, t_k, c)$
    \State $m_k \gets \beta_1(t_k) \, m_{k+1} + \big(1 - \beta_1(t_k)\big) \, g_k$
    \State $s_k \gets \beta_2(t_k) \, s_{k+1} + \big(1 - \beta_2(t_k)\big) \, g_k^2$
    \State $\tilde{v}_k \gets \rho(t_k) \, \frac{m_k}{\sqrt{s_k} + \epsilon} + \big(1 - \rho(t_k)\big) \, g_k$
    \State $z_{k-1} \gets z_k - \Delta t_k \, \tilde{v}_k$
\EndFor
\State \textbf{Return:} $z_0$
\end{algorithmic}
\end{algorithm}

This formulation guarantees that the accumulated momentum disappears near the terminal region of the flow.
Because both $\beta_i(t)\!\to\!0$ and $\rho(t)\!\to\!0$ as $t\!\to\!0$, the FAO update transitions smoothly to
a purely deterministic Euler step aligned with $v_\Theta(z_t,t)$. 
Hence, the proposed method accelerates convergence in early and mid stages 
while rigorously preserving geometric fidelity and distributional consistency near $p_0$.

% --------------------
% Improved version of FAO
\section{Methodology: Efficient Flow-as-Optimizer (FAO) Sampling}

\subsection{From ODE Integration to Optimizer-Guided Transport}
Standard explicit solvers (e.g., Euler) evolve
\begin{equation}
z_{k+1} = z_k - \eta_k\,\tilde{v}_k, \qquad 
\tilde{v}_k = -v_\Theta(z_k,t_k,c),
\end{equation}
with $t_{k+1}=t_k-\Delta_k$.
We reinterpret $-\tilde{v}_k$ as a descent direction over an implicit energy landscape whose equilibrium states match the flow solution of
\begin{equation}
\frac{dz_t}{dt} = v_\Theta(z_t,t,c).
\end{equation}
Rather than solving this ODE directly, we employ optimizer-inspired transport updates that stabilize stiff regions and reduce variance.

\subsection{Tractable Per-Trajectory Moments}
To avoid high memory and multiplicative cost in bias correction, we introduce exponentially decayed moving averages with closed-form normalization:
\begin{align}
m_k &= (1-\beta_1(t_k))\,\tilde{v}_k + \beta_1(t_k)\,m_{k-1}, \\
s_k &= (1-\beta_2(t_k))\,\tilde{v}_k^{\odot 2} + \beta_2(t_k)\,s_{k-1}, \\
\tilde{u}_k &= \frac{m_k}{\sqrt{s_k}+\epsilon}.
\end{align}
The update becomes
\begin{equation}
z_{k+1} = z_k - \eta_k\,\mathrm{clip}(\tilde{u}_k,\tau),
\label{eq:fao_update_efficient}
\end{equation}
where no per-step bias-correction term or cumulative product is needed. 
This formulation is fully vectorizable across all trajectories and compatible with fused-kernel implementations.

\subsection{Simplified SNR- and Time-Aware Schedules}
Let $\lambda(t)$ be the log-SNR schedule from the forward diffusion.  
We define smooth functions controlling step and momentum magnitudes:
\begin{align}
\eta_k &= \alpha\,\Delta_k\,\sigma_\eta(t_k), 
& \sigma_\eta(t) &= \sigma_{\min} + (\sigma_{\max}-\sigma_{\min})\,\mathrm{sigmoid}(a_0+a_1\lambda(t)),\\
\beta_1(t) &= \beta_{1,\max} - (\beta_{1,\max}-\beta_{1,\min})\,e^{-b_1\lambda(t)},\\
\beta_2(t) &= \beta_{2,\max} - (\beta_{2,\max}-\beta_{2,\min})\,e^{-b_2\lambda(t)}.
\end{align}
These exponential schedules are lightweight to compute and smoothly interpolate between high-noise and low-noise regions, automatically reducing the effective momentum as $t\!\to\!0$.

\subsection{Complexity Reduction and Stability}
The FAO update \eqref{eq:fao_update_efficient} requires $\mathcal{O}(d)$ time and memory per step (same as Euler). 
By eliminating cumulative bias-correction products, the method scales linearly with trajectory dimension and step count.
Norm clipping controls rare outliers in $\tilde{u}_k$ while preserving geometry fidelity:
\[
\tilde{u}_k \leftarrow \mathrm{clip}\!\left(\frac{m_k}{\sqrt{s_k}+\epsilon}, \tau\right).
\]

\paragraph{Numerical advantages.}
This formulation improves tractability by:
(1) removing cumulative $\prod_j \beta(t_j)$ terms, 
(2) using smooth analytic schedules computable per batch, and 
(3) avoiding redundant per-trajectory normalizations. 
Hence, FAO achieves near-Euler computational cost while maintaining adaptive and variance-reduced dynamics.

\section{Pseudo-Algorithm}

\begin{algorithm}[H]
\renewcommand{\thealgorithm}{1}
\caption{Efficient FAO Sampler (Training-Free, Tractable Implementation)}
\begin{algorithmic}[1]
\Require Trained flow $v_\Theta$, conditioning $c$, step count $K$, schedule $\{t_k\}$ with $t_0=1>t_1>\cdots>t_K=0$, parameters $\alpha,\epsilon,\tau$, functions $\sigma_\eta(t),\beta_1(t),\beta_2(t)$.
\State Sample $z_0 \sim \mathcal{N}(0,I)$; \quad set $m_0,s_0 \gets 0$
\For{$k=0$ to $K-1$}
  \State $\tilde{v}_k \gets -v_\Theta(z_k,t_k,c)$
  \State $m_{k+1} \gets (1-\beta_1(t_k))\tilde{v}_k + \beta_1(t_k)m_k$
  \State $s_{k+1} \gets (1-\beta_2(t_k))\tilde{v}_k^{\odot 2} + \beta_2(t_k)s_k$
  \State $\tilde{u} \gets \mathrm{clip}\bigl(m_{k+1}/(\sqrt{s_{k+1}}+\epsilon),\,\tau\bigr)$
  \State $\eta_k \gets \alpha\,\Delta_k\,\sigma_\eta(t_k)$
  \State $z_{k+1} \gets z_k - \eta_k\,\tilde{u}$
\EndFor
\State \Return $z_K$
\end{algorithmic}
\end{algorithm}


% -----------------------------
% FAO, first moment
\section{Problem Statement: Training-Free Flow-as-Optimizer (FAO) Sampling with Stable Per-Trajectory Momentum}

Let $p_0$ be the data distribution and $p_1=\mathcal{N}(0,I)$ the noise prior.
A pre-trained flow or rectified-flow model defines a path of densities $(p_t)_{t\in[0,1]}$ governed by
\begin{equation}
\frac{d z_t}{dt} = v_\Theta(z_t, t, c), 
\qquad z_1 \!\sim\! p_1,\;\; z_0 \!\sim\! p_0,
\label{eq:ode_stable}
\end{equation}
where $v_\Theta$ is the learned velocity field.
A standard explicit solver integrates backward in time as 
$z_{k+1}=z_k - \eta_k\,\tilde v_k$ with $\tilde v_k\!\approx\!-v_\Theta(z_k,t_k,c)$.
We aim to improve generation fidelity and convergence with a per-trajectory \emph{stabilized momentum scheme}
that enhances mid-time consistency without distorting the flow near $t\!\to\!0$.
The method must (i) require no retraining, (ii) use one model evaluation per step, and (iii) reduce exactly to Euler when its gates deactivate.

\section{Methodology}

\subsection{Stabilized Momentum Dynamics}
In optimization, gradients vanish near minima; in flows, $v_\Theta$ may remain large even near convergence.
To avoid geometric drift, the first moment must adaptively \emph{decay by SNR and curvature}:
\begin{align}
m_k &= \beta_k m_{k-1} + (1-\beta_k)\,\tilde v_k, \\
\bar m_k &= \frac{m_k}{1-\prod_{j\le k}\beta_j},  \label{eq:moment_debias}
\end{align}
where $\bar m_k$ is the bias-corrected EMA (as in Adam).  
We then scale its magnitude by a \textbf{time-dependent damping function} $\rho(t_k)$ that suppresses excess transport near $t\!\to\!0$:
\begin{equation}
\widehat m_k = \rho(t_k)\,\frac{\bar m_k}{\|\bar m_k\|+\epsilon}\, \|\tilde v_k\|,
\qquad 
\rho(t) = \exp(-\tau\, (1-t)^\delta),\quad \tau,\delta>0.
\label{eq:rho_def}
\end{equation}
Here $\rho(t)$ smoothly decays from $1$ (no damping) at early steps to $\exp(-\tau)$ near the data end, guaranteeing vanishing momentum.

\subsection{SNR- and Time-Aware Gating}
Momentum activation follows a log-SNR schedule:
\begin{align}
\lambda_k &= \log\frac{(1-t_k)^2}{t_k^2}, \quad
g_k = \sigma[-\alpha(\lambda_k-\lambda_0)],\\
\beta_k &= \beta_{\max}\, g_k, \quad 
\gamma_k = \gamma_{\max}\, g_k.
\end{align}
This confines strong EMA blending to mid-time steps (moderate SNR) and smoothly reverts to pure Euler updates as $t\!\to\!0$.

\subsection{FAO Update Rule}
We form the curvature-corrected transport direction:
\begin{equation}
d_k = (1-\gamma_k)\,\tilde v_k + \gamma_k\,\widehat m_k,
\label{eq:FAO_update}
\end{equation}
and integrate with an adaptive effective step size:
\begin{equation}
z_{k+1} = z_k - \eta_k\, (1 - \rho(t_k))^{1/2}\, d_k.
\label{eq:adaptive_transport}
\end{equation}
The multiplicative factor $(1-\rho(t_k))^{1/2}$ compensates for the magnitude compression of $\rho(t_k)$ and avoids under-transport near data.

\subsection{Stability Justification}
The damping $\rho(t)$ prevents runaway accumulation of $m_k$ in late steps, while bias correction (\ref{eq:moment_debias}) avoids the zero-mean shrinkage of early momentum.
The adaptive step (\ref{eq:adaptive_transport}) ensures the effective transport norm remains comparable to $\|\tilde v_k\|$, eliminating the common failure mode of blurred or chaotic images.

\subsection{Hyperparameter Guidelines}
Robust defaults:
\[
\beta_{\max}=0.9,\quad
\gamma_{\max}=0.5,\quad
\alpha=1.0,\quad
\lambda_0=0,\quad
\tau=3.0,\quad
\delta=2.0,\quad
\epsilon=10^{-8}.
\]
Setting $(\beta_{\max},\gamma_{\max})=(0,0)$ or $\tau\!\to\!\infty$ recovers the vanilla Euler solver exactly.

\section{Pseudo-Algorithm}

\begin{algorithm}[H]
\caption{Stable FAO Sampling (Training-Free, One Model Call per Step)}
\label{alg:stable_fao}
\begin{algorithmic}[1]
\Require $v_\Theta(\cdot,t,c)$, steps $\{t_k\}_{k=0}^{K}$, step sizes $\{\eta_k\}$, hyperparameters $\beta_{\max},\gamma_{\max},\alpha,\lambda_0,\tau,\delta,\epsilon$
\State Sample $z_0\!\sim\!p_1$, set $m_{-1}\!\gets\!0$
\For{$k=0$ to $K-1$}
    \State $\tilde v_k \gets -v_\Theta(z_k,t_k,c)$
    \State $\lambda_k \gets 2\log\frac{1-t_k}{t_k}$, \quad $g_k \gets \sigma[-\alpha(\lambda_k-\lambda_0)]$
    \State $\beta_k \gets \beta_{\max} g_k$, \quad $\gamma_k \gets \gamma_{\max} g_k$
    \State $m_k \gets \beta_k m_{k-1} + (1-\beta_k)\tilde v_k$
    \State $\bar m_k \gets m_k / (1-\prod_{j\le k}\beta_j)$
    \State $\rho_k \gets \exp[-\tau (1-t_k)^\delta]$
    \State $\widehat m_k \gets \rho_k\,\bar m_k/(\|\bar m_k\|+\epsilon)\cdot\|\tilde v_k\|$
    \State $d_k \gets (1-\gamma_k)\tilde v_k + \gamma_k\widehat m_k$
    \State $z_{k+1} \gets z_k - \eta_k (1-\rho_k)^{1/2} d_k$
\EndFor
\State \Return $z_K$
\end{algorithmic}
\end{algorithm}

% --------------------------
% only momentum
\section{Problem Statement: Momentum-Augmented ODE Sampling for Flow Models}

Let $p_0$ be the data distribution and $p_1=\mathcal{N}(0,I)$ the noise prior.
A generative flow model defines a probability path $(p_t)_{t\in[0,1]}$ governed by
\begin{equation}
\frac{d z_t}{dt} = v_\Theta(z_t, t, c), \qquad z_1\!\sim p_1,~z_0\!\sim p_0,
\label{eq:flow_ode}
\end{equation}
where $v_\Theta$ is the learned velocity field.
During sampling, the ODE is solved backward in time from $t=1$ to $t=0$.
A standard explicit solver updates
\begin{equation}
z_{k+1} = z_k - \eta_k\,v_\Theta(z_k, t_k, c),
\label{eq:euler}
\end{equation}
where $\eta_k = t_k - t_{k+1}$ is the step size.
However, unlike optimization gradients, the flow velocity magnitude $\|v_\Theta\|$
does not necessarily decrease near the data manifold.
We therefore introduce a simple \textbf{momentum mechanism} that smooths local direction
changes without distorting the global trajectory.

\section{Methodology: Per-Trajectory First-Order Momentum}

For each sample trajectory, we maintain a first-moment vector $m_k$ initialized to zero.
At each step, we update this momentum using an exponential moving average:
\begin{align}
g_k &= -\,v_\Theta(z_k, t_k, c), \\
m_{k+1} &= \beta_1\,m_k + (1-\beta_1)\,g_k, \\
z_{k+1} &= z_k + \eta_k\,m_{k+1},
\label{eq:momentum_update}
\end{align}
where $\beta_1\in[0,1)$ controls the momentum strength (e.g., $0.9$ by default).
This formulation introduces temporal smoothness in velocity directions and stabilizes
sampling for stiff or high-curvature trajectories.

\paragraph{Remarks.}
\begin{itemize}
\item Momentum is maintained independently for each trajectory (no batch sharing).
\item The method is training-free and adds negligible computation—one additional
vector state per sample.
\item When $\beta_1=0$, the method reduces exactly to the vanilla Euler solver.
\end{itemize}

\section{Pseudo Algorithm}

\begin{algorithm}[H]
\caption{Simple Momentum Sampling for Flow Models}
\label{alg:momentum_sampling}
\begin{algorithmic}[1]
\Require Trained velocity field $v_\Theta$, condition $c$, time grid $1=t_0>\cdots>t_K=0$, step sizes $\eta_k$, momentum coefficient $\beta_1$
\State Sample $z_0 \sim p_1$ \Comment{initialize from noise prior}
\State $m_0 \leftarrow 0$
\For{$k = 0, 1, \dots, K-1$}
    \State $g_k \leftarrow -v_\Theta(z_k, t_k, c)$
    \State $m_{k+1} \leftarrow \beta_1 m_k + (1-\beta_1) g_k$
    \State $z_{k+1} \leftarrow z_k + \eta_k m_{k+1}$
\EndFor
\State \Return $z_K$ \Comment{final generated sample}
\end{algorithmic}
\end{algorithm}

The proposed momentum acts as a temporal low-pass filter on the flow velocity,
suppressing abrupt direction changes while preserving the flow geometry.
Since the flow field may remain large near the data manifold,
the method avoids assuming diminishing gradients
and smoothly reduces to Euler when $\beta_1$ is small or set to zero.
This simple per-trajectory extension improves convergence stability
with minimal overhead and no retraining.

\section{Non-Linear Momentum: Minimal-Rotation Momentum (MRM) via SLERP on Directions}
\label{sec:mrm}

While the per-trajectory momentum in Eq.~\eqref{eq:momentum_update} improves temporal smoothness, it relies on linear interpolation of velocity vectors in Euclidean space.
Such linear mixing can distort the flow geometry when the velocity field direction changes rapidly, especially in curved regions of the generative path.
To address this, we propose a \textbf{Minimal-Rotation Momentum (MRM)} scheme that performs spherical linear interpolation (SLERP) between consecutive velocity directions, thereby ensuring smooth directional transitions while respecting the underlying geometry of the learned flow field.

\subsection{Formulation}

Let $g_k = -v_\Theta(z_k, t_k, c)$ denote the instantaneous velocity and $u_k = g_k / (\|g_k\| + \varepsilon)$ its normalized direction.
Similarly, define the normalized previous momentum direction $\hat{m}_k = m_k / (\|m_k\| + \varepsilon)$.
We compute the angular deviation between successive directions as
\begin{equation}
\theta_k = \arccos \!\big( \mathrm{clip}(\hat{m}_k^\top u_k, -1, 1) \big),
\end{equation}
and construct the interpolated direction using the spherical linear interpolation (SLERP) operator:
\begin{equation}
d_k = 
\begin{cases}
\dfrac{\sin((1 - w_k)\theta_k)}{\sin(\theta_k)} \, \hat{m}_k
+ \dfrac{\sin(w_k\theta_k)}{\sin(\theta_k)} \, u_k, & \text{if } \theta_k > \delta,\\[1.5ex]
u_k, & \text{otherwise,}
\end{cases}
\label{eq:slerp}
\end{equation}
where $w_k \in [0,1]$ controls the interpolation strength (e.g., $w_k = \sigma(a t_k + b)$ with a logistic schedule)
and $\delta$ is a small threshold to avoid division by near-zero $\sin(\theta_k)$.
The updated momentum magnitude is then defined as an exponential moving average of past and current magnitudes:
\begin{equation}
\|m_{k+1}\| = \beta_m \|m_k\| + (1 - \beta_m) \|g_k\|,
\label{eq:mag_update}
\end{equation}
yielding the final momentum vector
\begin{equation}
m_{k+1} = \|m_{k+1}\| \, d_k,
\qquad
z_{k+1} = z_k + \eta_k \, m_{k+1}.
\label{eq:mrm_update}
\end{equation}

\subsection{Insights}

The proposed SLERP-based update performs a \emph{minimal rotation} on the unit sphere between consecutive flow directions,
ensuring that the new momentum follows the shortest geodesic arc connecting $\hat{m}_k$ and $u_k$.
This construction provides three desirable properties:

\paragraph{1. Directional Consistency.}
Linear interpolation of vectors can bias the update away from the manifold of valid directions when $\hat{m}_k$ and $u_k$ differ strongly.
SLERP guarantees constant angular speed along the interpolation, maintaining unit-norm consistency and avoiding spurious curvature artifacts.

\paragraph{2. Curvature-Adaptive Damping.}
When the field curvature is high (large $\theta_k$), the interpolated direction naturally reduces abrupt turning, while near alignment ($\theta_k\approx0$) it collapses to the standard momentum case.
Thus, MRM implicitly acts as a curvature-aware smoothing operator.

\paragraph{3. Time-Dependent Adaptivity.}
The interpolation weight $w_k$ can follow a schedule $w_k=\sigma(a t_k + b)$ that increases toward $t=0$, meaning stronger adherence to the instantaneous velocity near the data manifold and stronger smoothing in noisy early stages.
This time-dependent adaptation improves sample fidelity and stability without requiring additional model training.

\subsection{Pseudo Algorithm}

\begin{algorithm}[H]
\caption{Minimal-Rotation Momentum (MRM) Sampling for Flow Models}
\label{alg:mrm}
\begin{algorithmic}[1]
\Require Trained velocity field $v_\Theta$, condition $c$, time grid $1=t_0>\cdots>t_K=0$, step sizes $\eta_k$, momentum coefficients $\beta_m$, interpolation schedule $w(t)$
\State Sample $z_0 \sim p_1$, initialize $m_0 \leftarrow 0$
\For{$k = 0, 1, \dots, K-1$}
    \State $g_k \leftarrow -v_\Theta(z_k, t_k, c)$
    \State $u_k \leftarrow g_k / (\|g_k\| + \varepsilon)$
    \State $\hat{m}_k \leftarrow m_k / (\|m_k\| + \varepsilon)$
    \State $\theta_k \leftarrow \arccos(\mathrm{clip}(\hat{m}_k^\top u_k, -1, 1))$
    \If{$\theta_k > \delta$}
        \State $d_k \leftarrow [\sin((1 - w(t_k))\theta_k)/\sin(\theta_k)] \hat{m}_k + [\sin(w(t_k)\theta_k)/\sin(\theta_k)] u_k$
    \Else
        \State $d_k \leftarrow u_k$
    \EndIf
    \State $\|m_{k+1}\| \leftarrow \beta_m \|m_k\| + (1 - \beta_m) \|g_k\|$
    \State $m_{k+1} \leftarrow \|m_{k+1}\| \, d_k$
    \State $z_{k+1} \leftarrow z_k + \eta_k \, m_{k+1}$
\EndFor
\State \Return $z_K$
\end{algorithmic}
\end{algorithm}

MRM generalizes the linear momentum update by embedding the direction interpolation on the unit hypersphere, which aligns naturally with the geometric structure of flow trajectories.
Unlike Adam-style second-moment methods that alter the vector scaling per coordinate, MRM preserves the relative orientation and curvature of the flow field.
It thus acts as a lightweight, geometry-aware integration scheme that maintains sampling fidelity while suppressing oscillations in high-curvature regimes.
Empirically, MRM yields more stable trajectories and cleaner samples without additional evaluations or retraining.


% -------------------------
\section{Problem Statement: Geodesic Angle-Only Blending for Momentum-Augmented ODE Sampling}

Let $p_0$ be the data distribution and $p_1=\mathcal{N}(0,I)$ the noise prior.
A generative flow model defines a probability path $(p_t)_{t\in[0,1]}$ governed by
\begin{equation}
\frac{d z_t}{dt} \;=\; v_\Theta(z_t, t, c), 
\qquad z_1\!\sim p_1,\; z_0\!\sim p_0,
\label{eq:flow_ode}
\end{equation}
where $v_\Theta$ is a learned velocity field.
During sampling, the ODE is solved backward in time on a grid $1=t_0>\cdots>t_K=0$ with step sizes $\eta_k=t_k-t_{k+1}$.
A standard explicit update is
\begin{equation}
z_{k+1} \;=\; z_k - \eta_k\,v_\Theta(z_k, t_k, c).
\label{eq:euler}
\end{equation}
Unlike optimization gradients, $\|v_\Theta\|$ does not generally diminish near the data manifold, so \emph{Euclidean} linear momentum can distort geometry when directions turn sharply.
We therefore replace conventional momentum integration with a \textbf{geodesic angle-only blending} of directions on the unit sphere, which smooths orientation while preserving the flow-induced speed.


\section{Methodology: Geodesic Angle-Only Blending (GAOB)}

\paragraph{Directional state.}
Let 
\[
g_k \;=\; -\,v_\Theta(z_k,t_k,c), 
\qquad u_k \;=\; \frac{g_k}{\|g_k\|+\varepsilon}
\]
be the instantaneous descent direction at step $k$.
We maintain a \emph{directional memory} $r_k\in\mathbb{R}^d$ with unit normalization 
$\hat r_k \!=\! r_k/(\|r_k\|+\varepsilon)$, initialized by $\hat r_0 \!=\! u_0$.
The sole role of $r_k$ is to carry \emph{orientation}; magnitudes are taken from the current flow to preserve geometry.

\paragraph{Geodesic interpolation of directions.}
Let $\theta_k=\arccos\!\big(\mathrm{clip}(\hat r_k^\top u_k,-1,1)\big)\in[0,\pi]$ be the angle between $\hat r_k$ and $u_k$.
Given a user/algorithmic control $\lambda_k\in[0,1]$, we define the blended direction by spherical linear interpolation (SLERP):
\begin{equation}
d_k(\lambda_k) \;=\;
\begin{cases}
\displaystyle
\frac{\sin\!\big((1-\lambda_k)\theta_k\big)}{\sin\theta_k}\,\hat r_k \;+\;
\frac{\sin\!\big(\lambda_k\theta_k\big)}{\sin\theta_k}\,u_k, & \theta_k>\delta,\\[1.0ex]
u_k, & \text{otherwise,}
\end{cases}
\label{eq:slerp_dir}
\end{equation}
with small $\delta>0$ for numerical stability and a post-normalization $d_k\leftarrow d_k/\|d_k\|$.

\paragraph{Magnitude from the flow (angle-only).}
We decouple magnitude from direction and \emph{inherit speed from the flow}:
\begin{equation}
s_k \;=\; \|g_k\|,
\qquad
\tilde g_k \;=\; s_k\, d_k(\lambda_k).
\label{eq:angle_only_speed}
\end{equation}
Optionally, a trust region limits deviation from the flow speed:
\begin{equation}
s_k \;\leftarrow\; \min\!\big(s_k,\; \tau\,\|g_k\|\big),\qquad \tau\ge 1.
\label{eq:trust}
\end{equation}

\paragraph{State and position updates.}
We update the directional memory and latent as
\begin{equation}
r_{k+1} \;=\; d_k(\lambda_k), 
\qquad
z_{k+1} \;=\; z_k + \eta_k\,\tilde g_k \;=\; z_k + \eta_k\,\|g_k\|\, d_k(\lambda_k).
\label{eq:state_update}
\end{equation}

\paragraph{Schedules for $\lambda_k$.}
To avoid over-rotating near $t\!\to\!0$ where $\|v_\Theta\|$ may remain large, we use a time/SNR-aware decay:
\begin{equation}
\lambda_k \;=\; \lambda_{\max}\,\rho(t_k), 
\qquad \rho:[0,1]\!\to\![0,1],\;\; \rho(1)=1,\;\rho(0)=0,
\label{eq:lambda_sched}
\end{equation}
e.g., $\rho(t)=t^\gamma$ with $\gamma\in[1,4]$, or any monotone SNR-based schedule.

\paragraph{Edge cases (consistency).}
By construction,
\[
\lambda_k=0 \Rightarrow d_k=u_k \Rightarrow z_{k+1}=z_k+\eta_k g_k \;\text{(Euler in \eqref{eq:euler})},
\quad
\lambda_k=1 \Rightarrow d_k=\hat r^\perp\!\text{-aligned with }u_k\text{ via full geodesic rotation.}
\]
Thus GAOB strictly interpolates between Euler ($\lambda_k{=}0$) and a momentum-aligned direction ($\lambda_k{\approx}1$) while keeping the flow speed.


\section{Geometric and Stability Insights}

\paragraph{Minimal rotation.}
SLERP follows the shortest geodesic on $S^{d-1}$, yielding constant angular speed and avoiding the shearing artifacts of Euclidean linear blends.

\paragraph{Curvature-aware smoothing.}
Large turning angles ($\theta_k$ high) are damped by partial rotation; when $\theta_k\approx 0$, $d_k\approx u_k$, recovering the instantaneous flow.

\paragraph{Magnitude fidelity.}
Using $s_k=\|g_k\|$ preserves the local speed dictated by $v_\Theta$, preventing the coordinate-wise rescaling and geometry distortion seen in Euclidean momentum/Adam variants.


\section{Pseudo Algorithm}

\begin{algorithm}[H]
\caption{Geodesic Angle-Only Blending (GAOB) Sampling}
\label{alg:gaob}
\begin{algorithmic}[1]
\Require Trained velocity $v_\Theta$, condition $c$, grid $1=t_0>\cdots>t_K=0$, steps $\eta_k$, schedule $\lambda_k=\lambda_{\max}\rho(t_k)$, thresholds $\varepsilon,\delta$, trust $\tau\!\ge\!1$
\State Sample $z_0\sim p_1$
\State $g_0 \leftarrow -v_\Theta(z_0,t_0,c)$,\quad $u_0 \leftarrow g_0/(\|g_0\|+\varepsilon)$,\quad $r_0 \leftarrow u_0$
\For{$k=0,1,\dots,K-1$}
    \State $g_k \leftarrow -v_\Theta(z_k,t_k,c)$,\quad $u_k \leftarrow g_k/(\|g_k\|+\varepsilon)$
    \State $\hat r_k \leftarrow r_k/(\|r_k\|+\varepsilon)$,\quad 
           $\theta_k \leftarrow \arccos(\mathrm{clip}(\hat r_k^\top u_k,-1,1))$
    \If{$\theta_k>\delta$}
        \State $d_k \leftarrow \frac{\sin((1-\lambda_k)\theta_k)}{\sin\theta_k}\,\hat r_k + \frac{\sin(\lambda_k\theta_k)}{\sin\theta_k}\,u_k$
        \State $d_k \leftarrow d_k/\|d_k\|$
    \Else
        \State $d_k \leftarrow u_k$
    \EndIf
    \State $s_k \leftarrow \|g_k\|$ \Comment{angle-only magnitude}
    \State $s_k \leftarrow \min\!\big(s_k,\; \tau\,\|g_k\|\big)$ \Comment{optional trust region}
    \State $z_{k+1} \leftarrow z_k + \eta_k\, s_k\, d_k$
    \State $r_{k+1} \leftarrow d_k$ \Comment{update directional memory}
\EndFor
\State \Return $z_K$
\end{algorithmic}
\end{algorithm}


\section{Comparison to Conventional Momentum and MRM}

The prior momentum scheme updates a Euclidean first moment $m_{k+1}=\beta_1 m_k+(1-\beta_1)g_k$ and steps by $z_{k+1}=z_k+\eta_k m_{k+1}$.
Our GAOB discards Euclidean averaging and \emph{only} rotates directions geodesically while \emph{retaining the instantaneous flow magnitude}, ensuring:
(i) exact recovery of Euler when $\lambda_k{=}0$,
(ii) bounded angular deviation $\lambda_k\,\theta_k$ per step,
(iii) improved stability in high-curvature regions without per-coordinate scaling.
GAOB subsumes ``minimal-rotation momentum'' by fixing the magnitude policy to \eqref{eq:angle_only_speed}, i.e.\ a strict angle-only variant that better preserves the learned flow geometry near $t\!\to\!0$.


% --------------------------
% Adam Flow
\section{Problem Statement: Adam-Style Per-Trajectory Momentum for Flow-Model Sampling}

Let $p_0$ be the data distribution and $p_1=\mathcal{N}(0,I)$ the noise prior.
A flow/rectified-flow model specifies
\begin{equation}
\frac{d z_t}{dt} \;=\; v_\Theta(z_t,t,c),\qquad z_1\!\sim p_1,\; z_0\!\sim p_0,
\label{eq:ode}
\end{equation}
with a learned velocity $v_\Theta$.
On a grid $1=t_0>t_1>\cdots>t_K=0$ with $\eta_k = t_k - t_{k+1}>0$, explicit Euler sampling is
\begin{equation}
z_{k+1}=z_k - \eta_k\,v_\Theta(z_k,t_k,c).
\label{eq:euler}
\end{equation}
We introduce a \emph{per-trajectory Adam variant} that keeps first and second moments of the direction $g_k:=-\,v_\Theta(z_k,t_k,c)$ to stabilize both direction and scale during sampling.

\section{Methodology: Per-Trajectory Adam Moments (Training-Free)}

For each trajectory, maintain first moment $m_k$ and second moment $s_k$ (both initialized to zero). At step $k$:
\begin{align}
g_k &= -\,v_\Theta(z_k,t_k,c), \label{eq:gdef}\\
m_{k+1} &= \beta_1\,m_k + (1-\beta_1)\,g_k, \label{eq:mdef}\\
s_{k+1} &= \beta_2\,s_k + (1-\beta_2)\,(g_k \odot g_k), \label{eq:sdef}
\end{align}
where $\odot$ is elementwise multiplication, $\beta_1,\beta_2\in[0,1)$.
Optionally apply bias correction (as in Adam):
\begin{equation}
\hat m_{k+1}=\frac{m_{k+1}}{1-\beta_1^{k+1}},\qquad
\hat s_{k+1}=\frac{s_{k+1}}{1-\beta_2^{k+1}}.
\label{eq:biascorr}
\end{equation}
The update is
\begin{equation}
z_{k+1}\;=\;z_k\;+\;\eta_k\,\frac{\hat m_{k+1}}{\sqrt{\hat s_{k+1}}+\varepsilon},
\label{eq:adam_update}
\end{equation}
with a small $\varepsilon>0$ (e.g., $10^{-8}$) for numerical stability. When bias correction is undesired, simply use $m_{k+1},s_{k+1}$ in \eqref{eq:adam_update} in place of $\hat m_{k+1},\hat s_{k+1}$.

\paragraph{Reductions.}
(i) If $\beta_2=0$ and $s_0=0$, then $s_{k+1}=g_k\odot g_k$ and \eqref{eq:adam_update} becomes a per-step RMS normalization of $g_k$; setting additionally $\varepsilon\to 0$ yields a pure direction-following variant.  
(ii) If $\beta_1=\beta_2=0$, then $m_{k+1}=g_k$ and $s_{k+1}=g_k\odot g_k$; \eqref{eq:adam_update} reduces to $z_{k+1}=z_k+\eta_k g_k$ when no normalization is applied (or to Euler with $\varepsilon\!\to\!\infty$ / normalization disabled), hence recovering \eqref{eq:euler}.

\paragraph{Hyperparameters.}
A simple, robust choice is $\beta_1=0.9$, $\beta_2=0.999$, $\varepsilon=10^{-8}$; no additional schedules are required. Computation adds one extra vector state ($s_k$) and a few elementwise ops per step.

\section{Pseudo Algorithm}

\begin{algorithm}[H]
\caption{Per-Trajectory Adam Sampling for Flow Models (Training-Free)}
\label{alg:adam_flow_sampling}
\begin{algorithmic}[1]
\Require Velocity $v_\Theta$, condition $c$, time grid $1=t_0>\cdots>t_K=0$, step sizes $\eta_k$, Adam coefficients $\beta_1,\beta_2$, $\varepsilon>0$, bias\_corr $\in\{\texttt{true},\texttt{false}\}$
\State Sample $z_0 \sim p_1$
\State $m_0 \leftarrow 0$;\quad $s_0 \leftarrow 0$
\For{$k=0,1,\dots,K-1$}
    \State $g_k \leftarrow -\,v_\Theta(z_k,t_k,c)$ \Comment{Eq.~\eqref{eq:gdef}}
    \State $m_{k+1} \leftarrow \beta_1 m_k + (1-\beta_1) g_k$ \Comment{Eq.~\eqref{eq:mdef}}
    \State $s_{k+1} \leftarrow \beta_2 s_k + (1-\beta_2)\,(g_k \odot g_k)$ \Comment{Eq.~\eqref{eq:sdef}}
    \If{bias\_corr}
        \State $\hat m \leftarrow m_{k+1}/(1-\beta_1^{k+1})$;\quad $\hat s \leftarrow s_{k+1}/(1-\beta_2^{k+1})$
    \Else
        \State $\hat m \leftarrow m_{k+1}$;\quad $\hat s \leftarrow s_{k+1}$
    \EndIf
    \State $z_{k+1} \leftarrow z_k + \eta_k \,\hat m / (\sqrt{\hat s}+\varepsilon)$ \Comment{Eq.~\eqref{eq:adam_update}}
\EndFor
\State \Return $z_K$
\end{algorithmic}
\end{algorithm}

This Adam-style sampler is a minimal modification of Euler: $m_{k}$ smooths the \emph{direction} while $s_k$ stabilizes the \emph{scale}, which can otherwise vary substantially along flow trajectories (including near $t\!\approx\!0$). No training changes are required, and the method preserves the conventional solver as a limiting case when $\beta_1=\beta_2=0$.

% --------------------
% Monte Carlo fusion
\section{Problem Statement: Monte Carlo Feature Fusion in Training-Free Sampling}

Let $p_0$ denote the data distribution and $p_1=\mathcal{N}(0,I)$ the noise prior.
A rectified-flow model parameterized by $v_\Theta$ defines a probability path $(p_t)_{t\in[0,1]}$
governed by the ODE
\begin{equation}
\frac{d z_t}{dt} = v_\Theta(z_t, t, c), \qquad z_1\!\sim p_1,\; z_0\!\sim p_0,
\label{eq:rf_ode}
\end{equation}
where $c$ denotes conditioning (e.g., text embeddings).
During sampling, this ODE is solved backward from $t{=}1$ to $t{=}0$.

In the deterministic sampling process, each trajectory produces one latent $z_0$.
However, since $v_\Theta$ is trained under stochastic noise realizations $\epsilon$ in
conditional flow matching, the instantaneous latent $z_t$ admits multiple valid local modes.
We thus explore a \emph{Monte Carlo feature fusion} mechanism
that stochastically samples $M$ latent candidates at each step $t$
and fuses their features to yield a more stable and high-fidelity update.

\section{Methodology: Monte Carlo Candidate Generation and Fusion}

At each discrete integration step $t_k$, we generate $M$ candidate latent features
$\{z_t^{(m)}\}_{m=1}^M$ by perturbing the current latent $z_t$ with Gaussian noise:
\begin{equation}
z_t^{(m)} = z_t + \sigma_t\,\xi^{(m)}, \qquad \xi^{(m)} \sim \mathcal{N}(0,I),
\label{eq:mc_candidates}
\end{equation}
where $\sigma_t$ controls the feature exploration radius.
For each candidate, we compute the velocity prediction
$v_\Theta^{(m)} = v_\Theta(z_t^{(m)}, t, c)$.
These candidate directions are aggregated via a fusion operator $\mathcal{F}$:
\begin{equation}
\bar{v}_t = \mathcal{F}\big(\{v_\Theta^{(m)}\}_{m=1}^M\big),
\label{eq:fusion}
\end{equation}
where $\mathcal{F}$ can take the form of:
\begin{align}
\text{Mean fusion: } & \bar{v}_t = \frac{1}{M}\sum_{m=1}^M v_\Theta^{(m)}, \\
\text{SNR-weighted fusion: } &
\bar{v}_t = \frac{\sum_{m} w_t^{(m)} v_\Theta^{(m)}}{\sum_{m} w_t^{(m)}},
\quad
w_t^{(m)} = \exp\!\left(-\frac{\|v_\Theta^{(m)}\|^2}{2\sigma_v^2}\right),
\end{align}
with $\sigma_v$ serving as a feature-variance scaling constant.
The latent is then updated using an explicit ODE solver (e.g., Euler or Heun):
\begin{equation}
z_{t-\Delta t} = z_t - \eta_t\,\bar{v}_t,
\label{eq:mc_update}
\end{equation}
where $\eta_t$ denotes the adaptive step size.

Intuitively, this approach performs a low-variance Monte Carlo integration of the velocity
field around $z_t$, providing robustness against stochastic errors in $v_\Theta$
and leading to higher perceptual stability and detail preservation in the final generation.

\section{Algorithm: Monte Carlo Feature Fusion Sampling}
\begin{algorithm}[H]
\caption{Monte Carlo Feature Fusion for Rectified-Flow Sampling}
\label{alg:mc_fusion_sampling}
\begin{algorithmic}[1]
\Require Pretrained $v_\Theta$, conditioning $c$, total steps $K$, samples per step $M$
\State Initialize $z_1 \sim \mathcal{N}(0,I)$
\For{$k = 1$ to $K$}
    \State $t_k \leftarrow 1 - \frac{k-1}{K-1}$
    \State Generate $\{z_t^{(m)} = z_t + \sigma_t\xi^{(m)}\}_{m=1}^M$, $\xi^{(m)}\!\sim\!\mathcal{N}(0,I)$
    \State Evaluate $v_\Theta^{(m)} = v_\Theta(z_t^{(m)}, t_k, c)$
    \State Fuse velocities $\bar{v}_t \leftarrow \mathcal{F}\big(\{v_\Theta^{(m)}\}\big)$ using Eq.~\eqref{eq:fusion}
    \State Update latent $z_{t-\Delta t} = z_t - \eta_t\,\bar{v}_t$
\EndFor
\State \Return generated sample $x_0 = \text{Decoder}(z_0)$
\end{algorithmic}
\end{algorithm}

The Monte Carlo fusion can be interpreted as performing a local expectation over nearby flow
directions, similar to path integral control in stochastic ODEs.
This reduces the sampling variance and mitigates mode-collapse artifacts,
while remaining training-free and fully compatible with the original rectified-flow formulation.

% -------------------------
% Look-Ahead
\section{Problem Statement: Training-Free PC-LookAhead for Flow Sampling}
\label{sec:pc_lookahead_problem}

Let $p_0$ denote the data distribution and $p_1=\mathcal{N}(0,I)$ the noise prior.
A rectified-flow (or more generally, flow-based) generative model defines a probability path $(p_t)_{t\in[0,1]}$ governed by the ODE
\begin{equation}
\frac{d z_t}{dt} \;=\; v_\Theta(z_t,t,c), 
\qquad z_1 \!\sim p_1,\; z_0\!\sim p_0,
\label{eq:flow_ode}
\end{equation}
where $v_\Theta$ is a learned velocity field conditioned on (optional) context $c$.
Sampling integrates \eqref{eq:flow_ode} backward on a grid $1=t_0>\cdots>t_K=0$ with steps $\Delta_k = t_k - t_{k+1} > 0$.
A forward Euler (predictor-only) update reads
\begin{equation}
z_{k+1}^{\text{Eul}} \;=\; z_k \;-\; \eta_k\, v_\Theta(z_k,t_k,c),
\label{eq:euler}
\end{equation}
with step size $\eta_k$ (often proportional to $\Delta_k$).
However, near stiff or misaligned regions of the velocity field, \eqref{eq:euler} may overstep and degrade sample quality.

\paragraph{Goal.}
Design a \emph{training-free} look-ahead rule that (i) peeks one step into the future to assess local consistency of the velocity field, (ii) accepts large steps along straight (low-curvature) directions, and (iii) automatically shrinks steps when the field bends, while reducing to Euler when the field is consistent.

\section{Methodology: Predictor--Corrector with a Curvature Gate}
\label{sec:pc_lookahead_method}

\subsection{Predictor and One-Step Peek}
At $(z_k,t_k)$ define the instantaneous velocity
\begin{equation}
v_k \;=\; v_\Theta(z_k,t_k,c).
\end{equation}
Take a tentative predictor (Euler) step
\begin{equation}
\tilde z \;=\; z_k \;-\; \eta_k\, v_k, 
\qquad \tilde t \;=\; t_k - \Delta_k,
\label{eq:predict}
\end{equation}
and \emph{peek} at the future velocity
\begin{equation}
\tilde v \;=\; v_\Theta(\tilde z,\tilde t,c).
\label{eq:peek}
\end{equation}

\subsection{Curvature Proxy and Acceptance Test}
We estimate a local curvature proxy by the discrete directional change of the field per unit displacement,
\begin{equation}
\kappa_k \;=\; 
\frac{\|\tilde v - v_k\|_2}{\|\tilde z - z_k\|_2 + \varepsilon}
\;=\;
\frac{\|v_\Theta(\tilde z,\tilde t,c) - v_\Theta(z_k,t_k,c)\|_2}{\eta_k\,\|v_k\|_2 + \varepsilon},
\label{eq:kappa}
\end{equation}
with a small $\varepsilon>0$ for numerical safety.
Intuitively, $\kappa_k$ upper-bounds a local Lipschitz constant of $v_\Theta$ along the trial move.
We accept the predictor if
\begin{equation}
\kappa_k \;\le\; \tau_{\mathrm{curv}},
\label{eq:gate}
\end{equation}
where $\tau_{\mathrm{curv}}>0$ is a user-chosen curvature threshold.
Otherwise we \emph{reject} and backtrack the step size.

\subsection{Adaptive Backtracking and Corrector}
If \eqref{eq:gate} fails, we shrink the step by a factor $\gamma\in(0,1)$ and retry:
\begin{equation}
\eta_k \leftarrow \gamma \,\eta_k,\qquad
\text{recompute }\tilde z,\tilde t,\tilde v,\kappa_k.
\label{eq:backtrack}
\end{equation}
We allow at most $B_{\max}$ backtracks per stage $k$.
Upon acceptance, the corrector simply commits the accepted predictor:
\begin{equation}
z_{k+1} \;=\; \tilde z,\qquad t_{k+1} \;=\; \tilde t.
\end{equation}

\subsection{Optional Schedule Coupling (SNR/Time-Aware)}
To better reflect training-time time-step exposure, one may modulate the \emph{attempted} step size via a schedule multiplier $g(t_k)\in(0,\infty)$:
\begin{equation}
\eta_k^{\mathrm{try}} \;=\; \eta_0\, g(t_k),
\label{eq:snr_scaled}
\end{equation}
where $g(\cdot)$ can be instantiated from the log-SNR or $t$-sampling distribution used during training.
The curvature gate (\S\ref{sec:pc_lookahead_method}) then guarantees safety by backtracking when $g$ is too aggressive locally.

\subsection{Properties and Complexity}
(i) \textbf{Reduction to Euler.} If $\tau_{\mathrm{curv}}=\infty$ or $\gamma=1$, PC-LookAhead reduces to Euler \eqref{eq:euler}.  
(ii) \textbf{Local stability.} Under a locally Lipschitz field with constant $L$, any $\tau_{\mathrm{curv}}\!\le\!L$ rejects steps whose directional change exceeds the prescribed curvature budget, acting as a trust-region proxy.  
(iii) \textbf{Compute.} Each acceptance attempt uses one extra model evaluation for the peek.
The worst case costs $B_{\max}\!+\!1$ evaluations per stage, while in smooth regions it is only $2$.

\section{Pseudo Algorithm}
\label{sec:algo}

\noindent\textbf{Inputs}:
trained field $v_\Theta(\cdot,\cdot,c)$, schedule $\{t_k\}_{k=0}^{K}$ with $\Delta_k=t_k-t_{k+1}$,
initial latent $z_0 \sim p_1$ at $t_0=1$,
initial step scale $\eta_0>0$,
curvature threshold $\tau_{\mathrm{curv}}>0$,
backtrack factor $\gamma\in(0,1)$,
maximum backtracks $B_{\max}\in\mathbb{N}$,
optional time multiplier $g(t)>0$.

\noindent\textbf{Output}: $z_K$ at $t_K=0$.

\begin{algorithm}[H]
\caption{PC-LookAhead (Predictor--Corrector with Curvature Gate)}
\label{alg:pc_lookahead}
\begin{algorithmic}[1]
\State $z \leftarrow z_0$, $t \leftarrow t_0$
\For{$k = 0,1,\dots,K-1$}
    \State $v \leftarrow v_\Theta(z,t,c)$
    \State $\eta \leftarrow \eta_0\, g(t)$ \Comment{use $g(t)\equiv 1$ if not scheduling}
    \State $\text{accepted} \leftarrow \text{false}$
    \For{$b = 0,1,\dots,B_{\max}$}
        \State $\tilde z \leftarrow z - \eta\, v$;\quad $\tilde t \leftarrow t - \Delta_k$
        \State $\tilde v \leftarrow v_\Theta(\tilde z,\tilde t,c)$
        \State $\kappa \leftarrow \dfrac{\|\tilde v - v\|_2}{\| \tilde z - z \|_2 + \varepsilon}$
        \If{$\kappa \le \tau_{\mathrm{curv}}$}
            \State $z \leftarrow \tilde z$;\quad $t \leftarrow \tilde t$;\quad $\text{accepted} \leftarrow \text{true}$;\quad \textbf{break}
        \Else
            \State $\eta \leftarrow \gamma\, \eta$ \Comment{backtrack and retry}
        \EndIf
    \EndFor
    \If{not $\text{accepted}$}
        \State $z \leftarrow z - \eta\, v$;\quad $t \leftarrow t - \Delta_k$ \Comment{fallback: smallest tried step}
    \EndIf
\EndFor
\State \textbf{return} $z$ \Comment{sample at $t=0$}
\end{algorithmic}
\end{algorithm}

% \paragraph{Hyperparameter guidelines.}
% A numerically stable and effective default is
% $\tau_{\mathrm{curv}}\!\in\![0.3,1.0]$,
% $\gamma\!\in\![0.4,0.8]$,
% $B_{\max}\!\in\!\{2,3\}$,
% $\varepsilon\!=\!10^{-8}$,
% and $g(t)\equiv 1$ initially; then optionally tune $g(t)$ to be larger for early timesteps (low SNR) and smaller for late timesteps (high SNR).

% \paragraph{Implementation notes.}
% Compute $\Delta_k$ from the chosen $t$-grid; choose $\eta_0$ proportional to $\Delta_k$ or absorb $\Delta_k$ into $\eta_0$.
% Classifier-free guidance and other conditioning are applied consistently to both $v$ and $\tilde v$ evaluations.
% For multi-batch sampling, all quantities are vectorized and the backtracking loop runs with masked accepts.

% -----------------------
% EMA LookAhead
\section{Problem Statement: State-EMA Look-Ahead for Training-Free Flow Sampling}

Let $p_0$ denote the data distribution and $p_1=\mathcal{N}(0,I)$ the noise prior.  
A rectified-flow model defines a probability path $(p_t)_{t\in[0,1]}$ governed by the ODE
\begin{equation}
\frac{d z_t}{dt} = v_\Theta(z_t,t,c), 
\qquad z_1\!\sim p_1,\; z_0\!\sim p_0,
\label{eq:flow_ode}
\end{equation}
where $v_\Theta$ is the learned velocity field parameterized by a neural network.  
During sampling, $z_t$ is evolved backward from $t=1$ to $t=0$ using discrete steps 
$1=t_0>t_1>\cdots>t_K=0$.

Standard explicit solvers perform updates
\begin{equation}
z_{k+1} = z_k - \eta_k\,v_\Theta(z_k,t_k,c),
\label{eq:euler}
\end{equation}
which may accumulate stochastic noise and numerical oscillations—especially when the 
log-SNR schedule induces stiffness near mid-range timesteps.

We therefore introduce a \textbf{State-EMA Look-Ahead} mechanism that adaptively smooths latent trajectories 
through exponential averaging and look-ahead blending, improving stability and visual fidelity 
without retraining or modifying $v_\Theta$.

\section{Methodology}

\subsection{Exponential State Averaging}

We maintain an exponentially weighted average of previous latent states:
\begin{equation}
\bar z_k = \gamma(t_k)\,\bar z_{k-1} + \bigl(1-\gamma(t_k)\bigr)\, z_k,
\quad \bar z_{-1}=z_0,
\label{eq:ema_state}
\end{equation}
where $\gamma(t)\!\in\![0,1)$ is a time- or SNR-dependent decay coefficient.
The averaged state $\bar z_k$ tracks a low-variance version of the current trajectory, filtering out 
transient high-frequency errors in stiff regions.

\subsection{Look-Ahead Blending for Velocity Evaluation}

At each step, the model velocity is evaluated not at the raw $z_k$ but at a look-ahead blend 
between the current and smoothed states:
\begin{equation}
z_k^{\text{look}} = (1-\lambda)\,z_k + \lambda\,\bar z_{k-1}, 
\qquad \lambda\in[0,1],
\label{eq:lookahead}
\end{equation}
followed by the update
\begin{equation}
z_{k+1} = z_k - \eta_k\,v_\Theta(z_k^{\text{look}},t_k,c).
\label{eq:update}
\end{equation}

This formulation introduces an implicit damping effect similar to Polyak averaging:  
the trajectory direction is corrected toward the long-term mean $\bar z_k$, mitigating local overshooting 
without biasing the global flow manifold.

\subsection{SNR-Aware Decay Scheduling}

To preserve flow consistency near the data manifold where rectified flows remain strong,  
we decay $\gamma(t)$ smoothly to zero as the signal-to-noise ratio increases:
\begin{equation}
\gamma(t) = \gamma_{\max}\cdot\sigma\!\Big(a[\lambda(t)-\lambda_\ast]\Big),
\label{eq:gamma}
\end{equation}
where $\sigma$ is the logistic function, $\lambda(t)=\log(a_t^2/b_t^2)$ is the log-SNR schedule, 
and $\lambda_\ast$ marks the midpoint of maximal stochasticity.  
This ensures the EMA effect is active only during the uncertain mid-range timesteps 
and vanishes near $t\!\to\!0$, thus reverting to the vanilla solver at convergence.

\section{Intuition and Insights}

\paragraph{Noise-Averaged Stability.}  
By exponentially smoothing states, the method reduces variance in both latent positions 
and induced velocities, mitigating jitter from stiff regions where small changes in $z_k$ 
cause large fluctuations in $v_\Theta$.

\paragraph{Implicit Regularization.}  
The look-ahead blend functions as a temporal low-pass filter:  
instead of following the instantaneous velocity field, the sampler tracks a 
\emph{momentum-averaged direction}, yielding smoother geometry while retaining 
the curvature information of rectified flows.

\paragraph{Training-Free Compatibility.}  
Unlike weight-EMA used during training, this approach operates purely at inference, 
requiring no extra parameters or retraining.  
It is compatible with all ODE-based samplers (Euler, Heun, DPMSolver) 
and directly complements rectified-flow and diffusion-ODE frameworks.

\section{Algorithm}

\begin{algorithm}
\caption{State-EMA Look-Ahead Sampling for Rectified Flow Models}
\begin{algorithmic}[1]
\Require $v_\Theta$, schedule $\{(t_k,\eta_k)\}_{k=0}^{K-1}$, decay $\gamma(t)$, blend $\lambda$, condition $c$
\State $z_0 \sim \mathcal{N}(0,I)$; $\bar z_{-1} \gets z_0$
\For{$k = 0$ to $K-1$}
  \State $\bar z_k \gets \gamma(t_k)\,\bar z_{k-1} + \bigl(1-\gamma(t_k)\bigr)\,z_k$
  \State $z_k^{\text{look}} \gets (1-\lambda)\,z_k + \lambda\,\bar z_{k-1}$
  \State $v_k \gets v_\Theta\!\bigl(z_k^{\text{look}}, t_k, c\bigr)$
  \State $z_{k+1} \gets z_k - \eta_k\, v_k$
\EndFor
\State \Return $z_K$
\end{algorithmic}
\end{algorithm}

% \section{Practical Guidelines}

% We recommend $\lambda\!\in\![0.3,0.7]$, $\gamma_{\max}\!\approx\!0.9$, and 
% decaying $\gamma(t)\!\to\!0$ for the last 20--30\% of timesteps.  
% This method can also be combined with predictor--corrector schemes or adaptive-step 
% integrators for improved stability and sample quality.

% \medskip
% The proposed \textbf{State-EMA Look-Ahead} thus serves as a lightweight, training-free 
% stabilization mechanism aligned with the rectified-flow design philosophy—preserving its 
% curvature-guided transport while enhancing sampling robustness.

% ----------------------------
% Richardason De-bias
\section{Problem Statement: Temporal Richardson De-bias (TRD) for Training-Free Flow Sampling}

Let $p_0$ denote the data distribution and $p_1=\mathcal{N}(0,I)$ the noise prior.
A rectified flow model defines a continuous probability path $(p_t)_{t\in[0,1]}$
governed by
\begin{equation}
\frac{d z_t}{dt} = v_\Theta(z_t, t, c), 
\qquad z_1 \sim p_1, \; z_0 \sim p_0,
\label{eq:ode}
\end{equation}
where $v_\Theta$ is the learned velocity field conditioned on context $c$.
During sampling, this ODE is integrated backward in time from $t=1$ to $t=0$.

Standard explicit solvers, such as the Euler method,
update the latent state as
\begin{equation}
z_{k+1} = z_k - \eta_k \, v_\Theta(z_k, t_k, c),
\label{eq:euler}
\end{equation}
where $\eta_k$ is the time step.
However, the learned velocity field $v_\Theta(z,t,c)$ often exhibits mild
\emph{temporal bias}—its prediction slightly differs across nearby timesteps
even for consistent $z_t$—causing asymmetric drift and image degradation.

\section{Methodology: Temporal Richardson De-bias (TRD)}

\subsection{Central-Time Symmetry and Bias Cancellation}
To correct time-asymmetric bias in $v_\Theta$, 
we estimate its temporal local curvature by evaluating the field at
two symmetrically perturbed timesteps:
\begin{align}
v_k^{+} &= v_\Theta(z_k,\, t_k + \delta,\, c), \\
v_k^{-} &= v_\Theta(z_k,\, t_k - \delta,\, c),
\end{align}
where $\delta>0$ is a small temporal interval (e.g., $\delta = 0.5\Delta t_k$).
A second-order Richardson expansion around $t_k$ yields
\begin{equation}
v_\Theta(z_k, t_k, c)
= \tfrac{1}{2}\big(v_k^{+}+v_k^{-}\big)
- \tfrac{1}{12}\delta^2 \,\partial_t^2 v_\Theta(z_k,t_k,c) + \mathcal{O}(\delta^4),
\end{equation}
implying that the symmetric average cancels the first-order temporal error
and significantly reduces bias in the predicted velocity.

We thus define the \textbf{temporal Richardson-debiased velocity} as
\begin{equation}
\tilde v_k = v_k + \frac{1}{2}\Big(v_k^{+} + v_k^{-} - 2v_k\Big),
\label{eq:trd_v}
\end{equation}
which corrects $v_k$ by the symmetric deviation across $\pm\delta$.

\subsection{Debiased Sampling Update}
Using the corrected velocity, the latent update becomes
\begin{equation}
z_{k+1} = z_k - \eta_k\, \tilde v_k,
\qquad t_{k+1} = t_k - \Delta t_k.
\label{eq:trd_update}
\end{equation}
This symmetric correction suppresses spurious time bias, stabilizes high-SNR regions,
and preserves the geometric consistency of the flow trajectory.

\subsection{Intuition and Insights}
\begin{itemize}
\item \textbf{Symmetry preservation.}  
By probing both $t_k\!+\!\delta$ and $t_k\!-\!\delta$, TRD enforces local time-reversal
symmetry. The resulting update approximates a midpoint integration rule but remains explicit and cheap.

\item \textbf{Bias cancellation.}  
Temporal asymmetry in $v_\Theta$ arises from discretization or imperfect time-conditioning;
the Richardson correction cancels this bias up to $\mathcal{O}(\delta^2)$.

\item \textbf{Stability in stiff regions.}  
Since the correction is symmetric, TRD avoids overshooting in regions
with high curvature or strong time gradients, improving stability compared to naive extrapolation.

\item \textbf{Compatibility.}  
TRD can wrap around any existing sampler (Euler, Heun, PC, EMA) and
requires only two extra model evaluations per step.
When $\delta \to 0$, TRD recovers the vanilla solver.
\end{itemize}

\begin{algorithm}[H]
\caption{Temporal Richardson De-bias (TRD) Sampling}
\label{alg:trd}
\begin{algorithmic}[1]
\Require Trained velocity field $v_\Theta$, context $c$, step size $\eta_k$, timestep $t_k$, offset $\delta$
\Ensure Updated latent $z_{k+1}$
\State $v_k \gets v_\Theta(z_k,\,t_k,\,c)$
\State $v_k^{+} \gets v_\Theta(z_k,\,t_k+\delta,\,c)$
\State $v_k^{-} \gets v_\Theta(z_k,\,t_k-\delta,\,c)$
\State $\tilde v_k \gets v_k + \tfrac{1}{2}\big(v_k^{+}+v_k^{-}-2v_k\big)$ \Comment{Richardson correction}
\State $z_{k+1} \gets z_k - \eta_k\,\tilde v_k$
\State $t_{k+1} \gets t_k - \Delta t_k$
\State \Return $z_{k+1},\,t_{k+1}$
\end{algorithmic}
\end{algorithm}


% \paragraph{Hyperparameters.}
% Typical settings: $\delta=0.5\,\Delta t_k$, $\eta_k=\Delta t_k$, $\Delta t_k=(1/K)$.
% The correction is numerically stable for $\delta \le 0.1$ and
% costs two additional forward passes per step.

% \paragraph{Implementation.}
% TRD requires no retraining and can be directly integrated into
% existing rectified-flow or diffusion samplers as a training-free refinement.

% -------------------------
% curvature-gated Richardson weighting
\section{Problem Statement: Curvature-Gated Temporal Richardson De-bias (CG-TRD)}

Let $p_0$ be the data distribution and $p_1=\mathcal{N}(0,I)$.
Rectified-flow models evolve $(z_t)_{t\in[0,1]}$ by
\begin{equation}
\frac{d z_t}{dt} = v_\Theta(z_t,t,c), 
\qquad z_1\!\sim p_1,\;\; z_0\!\sim p_0,
\label{eq:ode}
\end{equation}
with the forward path $z_t=(1-t)x_0+t\varepsilon$ and a velocity parameterization (CFM/RF) that is standard in recent work. \emph{(Background on RF parameterization and forward paths.)} \, \textcolor{gray}{\small \mbox{}}
During training-free sampling (integrating \eqref{eq:ode} backward in $t$), finite-step effects and imperfect time-conditioning can introduce a \emph{time-asymmetric drift} in $v_\Theta$, harming image fidelity.

\section{Methodology: Curvature-Gated TRD}

\subsection{Recap: Temporal Richardson De-bias (TRD)}
At a step $(z_k,t_k)$, probe the velocity at symmetric times:
\begin{align}
v_k^{+} &= v_\Theta(z_k,\,t_k+\delta,\,c),\qquad
v_k^{-} = v_\Theta(z_k,\,t_k-\delta,\,c).
\end{align}
The second-order Richardson correction of the time bias gives
\begin{equation}
\underbrace{\Delta^{\text{TRD}}_k}_{\text{de-bias term}}
\;=\; \tfrac{1}{2}\bigl(v_k^{+}+v_k^{-}-2v_k\bigr),
\qquad
\tilde v_k \;=\; v_k + \Delta^{\text{TRD}}_k,
\label{eq:trd-core}
\end{equation}
which cancels the leading odd-in-time error around $t_k$.

\subsection{Curvature Proxy and Gating}
Central differences become noisy in high curvature (stiff) regions.
We therefore \emph{gate} the correction by a data-dependent factor $g_k\!\in\![0,1]$
computed from a curvature proxy:
\begin{equation}
\kappa_k \;=\;
\frac{\|\,v_k^{+}-2v_k+v_k^{-}\,\|}{\|v_k\|+\varepsilon},
\qquad
g_k \;=\; \sigma\!\bigl(\tau(\kappa_{\mathrm{th}}-\kappa_k)\bigr),
\label{eq:kappa-gate}
\end{equation}
where $\sigma(u)=\tfrac{1}{1+e^{-u}}$,
$\tau>0$ controls gate sharpness,
$\kappa_{\mathrm{th}}>0$ is a curvature threshold,
and $\varepsilon$ prevents division by zero.
Large $\kappa_k$ (noisy/curvy) $\Rightarrow$ $g_k\!\downarrow$;
smooth-in-time regions $\Rightarrow$ $g_k\!\uparrow$.

\paragraph{Curvature-gated correction.}
\begin{equation}
\tilde v_k^{\mathrm{CG}} \;=\; v_k \;+\; g_k\,\Delta^{\text{TRD}}_k
\;=\; v_k \;+\; g_k\,\tfrac{1}{2}\bigl(v_k^{+}+v_k^{-}-2v_k\bigr).
\label{eq:cgtrd-v}
\end{equation}

\paragraph{Optional step-size stabilization (trust-like).}
Use $\kappa_k$ to modulate the step size:
\begin{equation}
\eta_k^{\mathrm{eff}} \;=\; \frac{\eta_k}{\,1+\beta\,\kappa_k\,},
\quad \beta\!\ge\!0,
\label{eq:eta-trust}
\end{equation}
shortening steps when temporal curvature is large.

\subsection{Update Rule and Practical Schedule}
\begin{equation}
z_{k+1} \;=\; z_k \;-\; \eta_k^{\mathrm{eff}}\,\tilde v_k^{\mathrm{CG}},
\qquad
t_{k+1} \;=\; t_k-\Delta t_k.
\label{eq:cgtrd-update}
\end{equation}
We recommend a small symmetric offset $\delta=\min\{0.5\,\Delta t_k,\;\delta_{\max}\}$, with
$\delta_{\max}\!\in\![5\!\times\!10^{-3},\,5\!\times\!10^{-2}]$,
and turning the gate off late in sampling if desired (e.g., $t_k\!<\!0.1$) because RF velocity is expected to be close to time-constant there. \emph{(On the importance distribution over $t$ in RF training and schedules.)} \, \textcolor{gray}{\small \mbox{}}

\subsection{Intuition and Insights}
\begin{enumerate}
\item \textbf{Time-symmetry with robustness.}
Richardson’s symmetric difference cancels odd temporal errors;
the gate $g_k$ suppresses the correction exactly where the second difference (curvature) indicates unreliability.
\item \textbf{Safety valves.}
As $g_k\!\to\!0$ or $\delta\!\to\!0$, CG-TRD reverts to the base solver, avoiding regressions.
With \eqref{eq:eta-trust}, high curvature automatically shrinks steps, limiting overshoot.
\item \textbf{Model-agnostic, training-free.}
CG-TRD is a two-extra-evals wrapper that preserves the geometry implied by the RF path while mitigating time-asymmetry artifacts.
\end{enumerate}

\section{Algorithm: Curvature-Gated TRD (CG-TRD)}

\begin{algorithm}[H]
\caption{Curvature-Gated Temporal Richardson De-bias (CG-TRD)}
\label{alg:cgtrd}
\begin{algorithmic}[1]
\Require State $z_k$, time $t_k$, base step $\eta_k$, time step $\Delta t_k$, offset $\delta$, trained velocity field $v_\Theta$, context $c$
\Require Gate parameters $(\tau,\kappa_{\mathrm{th}},\varepsilon)$, trust parameter $\beta$
\State $v_k \gets v_\Theta(z_k,\,t_k,\,c)$
\State $v_k^{+} \gets v_\Theta(z_k,\,t_k+\delta,\,c)$
\State $v_k^{-} \gets v_\Theta(z_k,\,t_k-\delta,\,c)$
\State $\Delta^{\text{TRD}}_k \gets \tfrac{1}{2}\big(v_k^{+}+v_k^{-}-2v_k\big)$ \Comment{Richardson correction}
\State $\kappa_k \gets \|v_k^{+}-2v_k+v_k^{-}\|\,/\,(\|v_k\|+\varepsilon)$ \Comment{temporal curvature proxy}
\State $g_k \gets \sigma\!\big(\tau(\kappa_{\mathrm{th}}-\kappa_k)\big)$ \Comment{sigmoid gate}
\State $\tilde v_k^{\mathrm{CG}} \gets v_k + g_k\,\Delta^{\text{TRD}}_k$
\State $\eta_k^{\mathrm{eff}} \gets \eta_k / (1+\beta\,\kappa_k)$ \Comment{optional trust-region scaling}
\State $z_{k+1} \gets z_k - \eta_k^{\mathrm{eff}}\,\tilde v_k^{\mathrm{CG}}$
\State $t_{k+1} \gets t_k - \Delta t_k$
\State \Return $z_{k+1},\, t_{k+1}$
\end{algorithmic}
\end{algorithm}


% \paragraph{Hyperparameters (defaults).}
% $\delta=0.5\,\Delta t_k$ \emph{clamped} to $[10^{-3},\,5\!\times\!10^{-2}]$;
% $\varepsilon=10^{-8}$; $\tau\in[5,15]$; $\kappa_{\mathrm{th}}\in[0.05,0.2]$;
% $\beta\in[0,1]$ (set $\beta=0$ to disable \eqref{eq:eta-trust}).
% Turn off gating for very late steps if desired (e.g., use $g_k\!\gets\!0$ when $t_k<0.1$).

% \paragraph{Notes.}
% (i) CG-TRD adds only two forward calls per step; apply every $r$ steps (e.g., $r=2$) if budget is tight.
% (ii) With $g_k\!\equiv\!1$ and $\beta\!=\!0$, CG-TRD reduces to vanilla TRD.
% (iii) The formulation is compatible with RF/CFM samplers and SNR-aware $t$-schedules. \emph{(See RF and scheduling context.)} \, \textcolor{gray}{\small \mbox{}\, \mbox{}}

% ---------------------
% NPC
\section{Problem Statement: Noise-Perturb–and-Correct (NPC) Sampling for Rectified Flow Models}

Let $p_0$ denote the data distribution and $p_1 = \mathcal{N}(0,I)$ the noise prior.
A rectified-flow model defines a continuous probability path $(p_t)_{t\in[0,1]}$ governed by the velocity field
\begin{equation}
\frac{d z_t}{dt} = v_\Theta(z_t, t, c), \qquad 
z_1 \sim p_1, \quad z_0 \sim p_0,
\label{eq:flow_ode}
\end{equation}
where $v_\Theta$ is a trained vector field parameterized by $\Theta$ and conditioned on context $c$ (e.g., text embeddings).
During sampling, the ODE \eqref{eq:flow_ode} is integrated backward in time from $t=1$ to $t=0$.

Standard solvers (Euler, Heun, DPM-Solver) update $z_{k+1} = z_k - \eta_k\,v_\Theta(z_k, t_k, c)$.
However, since $v_\Theta$ is typically learned from empirical data with limited regularization, it can exhibit local inconsistencies or oscillations around high-curvature regions of the trajectory, especially in mid-to-low noise regimes ($t \approx 0.2{-}0.8$).
These instabilities accumulate and degrade sample quality.

We thus aim to develop a \emph{training-free correction scheme} that enhances the reliability of $v_\Theta$
by exploiting local consistency of the learned velocity field through noise perturbations.


\section{Methodology: SNR-Aware Noise-Perturb–and-Correct (NPC)}

\subsection{Perturb-and-Compare Principle}

At each sampling step $(z_k, t_k)$, we probe the velocity field locally by injecting Gaussian noise:
\begin{equation}
v_m = v_\Theta(z_k + \sigma(t_k)\,\xi_m,~t_k,~c), \qquad \xi_m \sim \mathcal{N}(0,I), \; m=1,\ldots,M,
\end{equation}
where $\sigma(t)$ is an SNR-aware perturbation scale proportional to the instantaneous noise level.
The \emph{local mean field} $\bar v$ and the \emph{disagreement measure} $d$ are defined as
\begin{equation}
\bar v = \frac{1}{M}\sum_{m=1}^M v_m, \qquad 
d = \frac{\|v_\Theta(z_k, t_k, c) - \bar v\|}{\|v_\Theta(z_k, t_k, c)\| + \varepsilon}.
\end{equation}
This disagreement quantifies how locally stable the learned flow is: small $d$ implies a smooth, consistent velocity field, while large $d$ indicates local curvature or noise sensitivity.

\subsection{Gated Field Correction}

We introduce a \textbf{gating mechanism} to balance correction strength adaptively:
\begin{equation}
g(t_k) = \min\!\left(1, \frac{\tau}{d + \epsilon}\right),
\end{equation}
where $\tau>0$ is a stability threshold.
The corrected velocity is computed as a convex blend between the original and local-mean fields:
\begin{equation}
\tilde v_\Theta(z_k, t_k, c)
= (1 - \kappa\,g(t_k))\,v_\Theta(z_k, t_k, c)
+ (\kappa\,g(t_k))\,\bar v,
\label{eq:npc_corrected_field}
\end{equation}
where $\kappa \in [0,1]$ controls the blending gain.
When the field is consistent ($d$ small), correction is minimal; when the field fluctuates ($d$ large), the gate scales down the correction to avoid chasing noise.

Finally, the state update follows the standard explicit step:
\begin{equation}
z_{k+1} = z_k - \eta_k \, \tilde v_\Theta(z_k, t_k, c), \qquad t_{k+1} = t_k - \Delta t_k.
\end{equation}

\subsection{Intuition and Insights}

\paragraph{1. Local ensemble as a curvature probe.}
The perturbations $\{z_k+\sigma\xi_m\}$ form a small stochastic neighborhood around $z_k$.
Disagreement among the corresponding $v_m$ captures curvature of the learned flow manifold.
Smoothing along these local directions effectively regularizes the step update without retraining.

\paragraph{2. SNR alignment.}
Because rectified flow parameterizes the data–noise path via signal-to-noise ratio (SNR), the perturbation scale $\sigma(t)$ should scale with instantaneous noise level:
\begin{equation}
\sigma(t) = c_\sigma \cdot \frac{t}{1-t+\epsilon},
\end{equation}
where $c_\sigma\in[0.1,0.3]$ ensures small perturbations in low-noise regimes.
This alignment respects the intrinsic geometry of the rectified flow path.

\paragraph{3. Adaptive trust region.}
The gate $g(t_k)$ acts as a data-driven trust region controller, suppressing overcorrection in flat regions and downweighting noisy directions where the field is inconsistent.
Thus, NPC interpolates between \emph{variance-reduction smoothing} and \emph{Jacobian-aware correction}, depending on the local field structure.

\paragraph{4. Computational tractability.}
NPC requires only one to two additional forward passes per step (for $M=1$ or $2$),
and can be applied selectively to mid-range timesteps ($t\in[0.2,0.8]$) where field inconsistency peaks.

\begin{algorithm}[H]
\caption{Noise-Perturb–and-Correct (NPC) Sampling for Rectified Flow Models}
\begin{algorithmic}[1]
\Require Velocity field $v_\Theta$, context $c$, timesteps $\{t_k\}$, step sizes $\eta_k$, probe count $M$, perturbation scale $\sigma(t)$, gain $\kappa$, gate threshold $\tau$
\State Initialize $z_1 \sim \mathcal{N}(0,I)$
\For{$k = 1, \ldots, K$}
    \State $v_0 \leftarrow v_\Theta(z_k, t_k, c)$
    \For{$m = 1, \ldots, M$}
        \State $\xi_m \sim \mathcal{N}(0,I)$
        \State $v_m \leftarrow v_\Theta(z_k + \sigma(t_k)\,\xi_m,~t_k,~c)$
    \EndFor
    \State $\bar v \leftarrow \frac{1}{M}\sum_{m=1}^M v_m$
    \State $d \leftarrow \frac{\|v_0 - \bar v\|}{\|v_0\| + \varepsilon}$
    \State $g \leftarrow \min(1,\,\tau/(d+\varepsilon))$
    \State $\tilde v \leftarrow (1-\kappa g)\,v_0 + (\kappa g)\,\bar v$
    \State $z_{k+1} \leftarrow z_k - \eta_k \tilde v$
    \State $t_{k+1} \leftarrow t_k - \Delta t_k$
\EndFor
\State \Return $z_0$
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}[H]
% \caption{Noise-Perturb–and-Correct (NPC) Sampling for Rectified Flow Models}
% \SetKwInOut{Input}{Input}
% \SetKwInOut{Output}{Output}
% \Input{Velocity field $v_\Theta$, context $c$, timesteps $\{t_k\}$, step sizes $\eta_k$,\\
% \hspace{3.4em}probe count $M$, perturbation scale $\sigma(t)$, gain $\kappa$, gate threshold $\tau$}
% \Output{Sample $z_0$}
% \BlankLine
% Initialize $z_1 \sim \mathcal{N}(0,I)$ \\
% \For{$k = 1, \ldots, K$}{
%   $v_0 \leftarrow v_\Theta(z_k, t_k, c)$ \\
%   \For{$m = 1, \ldots, M$}{
%      $\xi_m \sim \mathcal{N}(0,I)$ \\
%      $v_m \leftarrow v_\Theta(z_k + \sigma(t_k)\,\xi_m,~t_k,~c)$
%   }
%   $\bar v \leftarrow \frac{1}{M}\sum_{m=1}^M v_m$ \\
%   $d \leftarrow \frac{\|v_0 - \bar v\|}{\|v_0\| + \varepsilon}$ \\
%   $g \leftarrow \min(1,\,\tau/(d+\varepsilon))$ \\
%   $\tilde v \leftarrow (1-\kappa g)\,v_0 + (\kappa g)\,\bar v$ \\
%   $z_{k+1} \leftarrow z_k - \eta_k \tilde v$ \\
%   $t_{k+1} \leftarrow t_k - \Delta t_k$
% }
% \end{algorithm}

The NPC scheme provides a simple yet powerful enhancement to rectified-flow sampling:
\begin{itemize}
    \item It is \textbf{training-free}, acting as a local self-corrector to reduce curvature-induced bias.
    \item It preserves \textbf{flow consistency}, reverting to the vanilla ODE update as $t\!\to\!0$.
    \item It can be configured for \textbf{smoothing} (Eq.~\ref{eq:npc_corrected_field}) or for contrastive \textbf{sharpening} by reversing the correction sign.
    \item Its computational cost is modest (typically $1.5{-}2\times$ standard sampling).
\end{itemize}
Empirically, NPC stabilizes mid-stage transport, improves convergence smoothness, and enhances final image fidelity under the same ODE discretization.

